Perfect Matchings, Rank of Connection Tensors and Graph Homomorphisms

We develop a theory of graph algebras over general fields. This is modeled after the theory developed by Freedman, Lov\'asz and Schrijver in [22] for connection matrices, in the study of graph homomorphism functions over real edge weight and positive vertex weight. We introduce connection tensors for graph properties. This notion naturally generalizes the concept of connection matrices. It is shown that counting perfect matchings, and a host of other graph properties naturally defined as Holant problems (edge models), cannot be expressed by graph homomorphism functions with both complex vertex and edge weights (or even from more general fields). Our necessary and sufficient condition in terms of connection tensors is a simple exponential rank bound. It shows that positive semidefiniteness is not needed in the more general setting.

==> applications-short.tex <==
\section{Applications}\label{sec:apps-short}

\subsection{Tensor rank lower bound of certain tensors}

%{\color{red} (cite Holant literature?)}
 
We first state
% prove 
a lemma about the
rank of the connection tensor for graph matchings.
Let $\calM_{a, b} = \calM_{n; a, b} \in \Sym^n(\bbF^2)$
denote the function $\{0, 1\}^n \rightarrow \bbF$ ($n \ge 0$),
such that on the all-$0$ input $\mathbf 0$ it takes value $a$,
on all inputs of Hamming weight one it takes value $b$,
and on all other inputs it takes value $0$.
This function is denoted by $[a, b, 0, \ldots, 0]$ in the Holant literature.
($\calM_{0; a, b}$ is just a constant $a$.)
We have the following lemma;
its proof is  an adaptation of the proof of Lemma 5.1 in~\cite{Comon-Golub-Lim-Mourrain-2008},
and  is given in subsection~\ref{subsec:tensor-rank-lower-bound}. %the  appendix  (Section~\ref{sec:Preliminary-continued}).

\begin{lemma}\label{lem:weighted-matchings-tensor-rank-lower-bound-short}
If $b \ne 0$ and $n \ge 0$, then $\symrank \calM_{n; a, b} \ge n$.
\end{lemma}

\subsection{Perfect matchings~\label{sec:Perfect-Matchings}}

Let  $\mathcal{F}$ be any set of
$\bbF$-valued constraint functions, a.k.a. signatures,
from some finite set $[q]$.
E.g., the  binary {\sc Equality} $(=_2)$ signature
on $(x, y)$ outputs value 1 if $x=y$, and 0 otherwise.
Similarly one can define {\sc All-Distinct} on $[q]$,
and {\sc Exact-One} and {\sc Exact-Two}
 on the Boolean domain $(q=2)$.
%
An input to a Holant problem $\Holant(\mathcal{F})$ is 
 $\Omega = (G, \pi)$
where  $G = (V,E)$  a graph (with possible multiple edges and loops),
and $\pi$ assigns to each $v \in V$ some $f_v \in \mathcal{F}$
of arity $\deg(v)$, and its incident edges as inputs.
 The output is $\Holant(G; \mathcal{F})
 = \sum_{\sigma} \prod_{v \in V} f_v(\sigma \mid_{E(v)})$, where the sum is  over all edge assignments $\sigma: E \to [q]$,
 $E(v)$ denotes the incident edges of $v$ and $\sigma \mid_{E(v)}$ denotes the restriction.
Bipartite $\Holant(G;  \mathcal{F} \mid \mathcal{G})$ are
defined on bipartite graphs $G = (U, V, E)$ where vertices in
$U$ and $V$ are assigned signatures from $\mathcal{F}$ and $\mathcal{G}$
respectively.

The graph parameter that counts the number of perfect matchings in a graph,
denoted by \textsc{\#Perfect-Matching} (or $\pmatch$),
is a quintessential Holant problem, corresponding to the {\sc Exact-One} function.
In this subsection we show it 
is not expressible as a GH function over any field.
%This was proved in~\cite{Freedman-Lovasz-Schrijver-2007} for real-valued GH with positive vertex weights.
This was proved in~\cite{Freedman-Lovasz-Schrijver-2007} for GH functions with real edge and positive vertex weights.
 However
that proof does not work for arbitrary fields, 
e.g., for the field of complex numbers $\bbC$,
 or even for real numbers with arbitrary (not necessarily positive) vertex weights. A crucial condition in~\cite{Freedman-Lovasz-Schrijver-2007} is positive semidefiniteness. 
%A succinct reason that the proof fails for $\bbC$
%is that for  complex matrices, $M^{\tt T}M$ is in general
%not positive semidefinite. 
%{\color{red} (Is this the reason, I asked the same in the introduction.)} 
%In fact, one of the most important
%%% I know. i decided as thus.
%holographic transformations~\cite{CLX11a, Cai-Fu-Guo-W}
%\cite{citesome-holographic-alg-dichotomypapers}
%{\color{red} (citesome-holographic-alg-dichotomypapers, hence I cite two papers here, make sure they fit in this context)}
%is $Z = \frac{1}{\sqrt{2}} \left[\begin{smallmatrix} 1 & 1\\
%\mathfrak{i} & -\mathfrak{i} \end{smallmatrix}\right]$,
%satisfying $Z^{\tt T} Z = \left[\begin{smallmatrix} 0 & 1\\ 
%1 & 0 \end{smallmatrix}\right]$. 
%\footnote{This transformation transforms
%binary equality functions to binary disequality functions,
%thus is crucial in dealing with orientation problems in the
%complexity classification of counting problems.}
\sout{ Our main result (Theorems~\ref{thm:uniform-exponential-rank-boundedness}, \ref{thm:uniform-exponential-rank-boundedness-converse} and~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened})
indicates that, to be expressible as GH,
   this condition of positive semidefiniteness is actually incidental
if we state it for connection tensors; 
indeed the property of being a GH function is
completely characterized by tensor rank.}
{\color{red} Our main result (Theorems~\ref{thm:uniform-exponential-rank-boundedness}, \ref{thm:uniform-exponential-rank-boundedness-converse} and~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened})
indicates that the property of being expressible as a GH function
is completely characterized by (the?) tensor rank. (JYC, replaced)}

Let $\pmatch(G) = m \cdot 1 \in \bbF$ (the sum of $m$ copies of $1 \in \bbF$) where 
 $m$ is the  number of perfect matchings in $G$.
Obviously, $\pmatch$ is a multiplicative graph parameter with $\pmatch(K_0) = 1$. Next, let $G$ be a $k$-labeled graph, let $X \subseteq [k]$, and let $\pmatch(G, X)$ denote the number of matchings in $G$ (expressed in $\bbF$)
%or this number mod $p$
%if $\Char \bbF = p$) 
that match all the unlabeled nodes and, for labeled nodes,
% within $[k]$
exactly the nodes in $X$. 
Then 
%we have 
for any $k$-labeled graphs $G_1, \ldots, G_n$,
\[
\pmatch(G_1 \cdots G_n) = \sum_{X_1 \sqcup \ldots \sqcup X_n = [k]} \pmatch(G_1, X_1) \cdots \pmatch(G_n, X_n).
\]

%This can be read as follows: the tensor
This means that $T(\pmatch, k, n)$ is 
the product $N_k^{\otimes n} W_{k, n}$ where $N_k$ has 
infinitely many rows indexed by all $k$-labeled graphs $G$, but only $2^k$ columns indexed by the subsets $X$ of $[k]$, with the entry at $(G, X)$
\[
N_{k; G, X} = \pmatch(G, X),
\]
and $W_{k, n}$ is a symmetric $\underbrace{2^k \times \ldots \times 2^k}_{n \text{ times}}$ tensor (from $\Sym^n(\bbF^{2^k})$), where
\[
W_{k, n; X_1, \ldots, X_n} =
\begin{lcases}
& 1 \quad \text{if } X_1 \sqcup \ldots \sqcup X_n = [k], \\
& 0 \quad \text{otherwise.}
\end{lcases}
\]
For any $k$,  if  $W_{k, n} = \sum_{i=1}^r a_i v_i^{\otimes n}$, then
$T(\pmatch, k, n) = \sum_{i=1}^r a_i (N_{k} v_i)^{\otimes n}$.
Hence 
%the symmetric rank of $T(\pmatch, k, n)$ is at most that of $W_{k, n}$, i.e.,
 $\symrank T(\pmatch, k, n) \le \symrank W_{k, n}$. 
We show that in fact equality holds. Consider the family of $k$-labeled graphs $\{ P_X \}_{X \subseteq [k]}$ of cardinality $2^k$ indexed by the subsets of $[k]$ and defined as follows: each $P_X$ has $|X|$ unlabeled vertices $\{ x_i \}_{i \in X}$ and $k$ labeled vertices $\{ y_i \}_{i = 1}^k$ labeled $1$ to $k$,
 with an edge between $x_i$ and $y_j$ iff $i = j$. It is easy so see that for $X, Y \subseteq [k]$, $N_{k; P_X, Y} = 1$ if $X = Y$ and $0$ otherwise. Then if we consider the subset of rows in $N_k$ corresponding to $\{ P_X \}_{X \subseteq [k]}$ we see that they form the identity matrix $I_{2^k}$ with a suitable
order of rows. Therefore $\symrank W_{k, n} = \symrank \left( I_{2^k}^{\otimes n} W_{k, n} \right) \le \symrank T(\pmatch, k, n)$ and so $\symrank T(\pmatch, k, n) = \symrank W_{k, n}$.

Note that for $k = 1$, $W_{1, n}$ is just the perfect matching
tensor (or the {\sc Exact-One} function on $n$ inputs) $\calM_{0, 1}
%%% didn't dsfine this symmetric signature notation. no need.
% = [0, 1, 0, \ldots 0]
 \in \Sym^n(\bbF^2)$ where $n \ge 1$. Applying Lemma \ref{lem:weighted-matchings-tensor-rank-lower-bound-short} with $a = 0, b = 1$, we get $\symrank W_{1, n} \ge n$ and therefore $\symrank T(\pmatch, 1, n) \ge n$ for $n \ge 1$. Now if $\pmatch$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness}, $\symrank T(\pmatch, k, n) \le q^k$ for $k, n \ge 0$ so that $\symrank T(\pmatch, 1, n) \le q$ for $n \ge 0$. However, as we have just shown $\symrank T(\pmatch, 1, n) \ge n$ for $n \ge 1$ which contradicts the upper bound when $n > q$. Hence $\pmatch$ is not expressible as a graph homomorphism function over any field. We state it as a theorem:
\begin{theorem}\label{thm:Perfect-Matching-not-expressible}
The graph parameter \textsc{\#Perfect-Matching} \emph{($\pmatch$)} is not expressible as a graph homomorphism function over any field.
\end{theorem}

%\begin{remark}
In this proof we have only used simple $k$-labeled graphs that  do
not have edges between the $k$ labeled vertices. The graphs $\{ P_X \}_{X \subseteq [k]}$ clearly have this property, and this property is
preserved under product of 
$k$-labeled graphs. 
It follows that Theorem~\ref{thm:Perfect-Matching-not-expressible}
holds even when $\pmatch$ is restricted to simple graphs. 
%for simple graphs.

We can prove the same inexpressibility results for
weighted matchings, 
proper edge colorings, and
vertex disjoint cycle covers (see Section~\ref{sec:apps}).
%In the appendix (Section~\ref{sec:apps}) we give the details.
For bounded degree graphs
% (see also Section~\ref{sec:apps}), 
we can also prove
% (see Section~\ref{sec:bonded-deg-graphs})
\begin{theorem}\label{thm:pm-as-GH-for-deg-bounded-graphs-short}
Let $\bbF$ be a field and $d \ge 2$. Then for the graph parameter \textsc{\#Perfect-Matching} \emph{($\pmatch$)}
as a function defined on degree-$d$ bounded graphs the following hold:
\begin{enumerate}
\item $\pmatch$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$ even on degree-$d$ bounded \emph{simple} graphs.
\item If $\bbF$ is infinite, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$ unless $\Char \bbF = 2$ and $d = 2$
(and in which case the minimum value is $|V(H)| = d + 1 = 3$).
%{\color{red} and the inexpressibility with $|V(H)| = d \le 2$ holds even degree-$d$ bounded \emph{simple} graphs. (add) }
%in which case $\pmatch$ is not expressible $\hom(\cdot, H)$ with $|V(H)| = d$ even on degree-$d$ bounded \emph{simple} graphs
%but is expressible as $\hom(\cdot, H)$ with $|V(H)| = d + 1 = 3$.
\end{enumerate}
\end{theorem}

%{\color{red} (old statement, can be commented out)}
%
%{\color{blue}
%\begin{theorem}\label{thm:pm-as-GH-for-deg-bounded-graphs-short-old}
%Let $\bbF$ be a field and $d \ge 2$. Then for the graph parameter
 %\textsc{\#Perfect-Matching} \emph{($\pmatch$)}  as a function 
%defined on $d$-degree bounded graphs the following hold:
%\begin{enumerate}
%\item $\pmatch$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$  even on $d$-degree bounded \emph{simple} graphs.
%\item If $\bbF$ is infinite, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d \text{ or } d + 1$.
%\item If $\Char \bbF = 0$, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$.
%\end{enumerate}
%\end{theorem}
%}



==> applications.tex <==
%\section{Applications Continued~\label{sec:apps}}
\section{More Applications~\label{sec:apps}}
%%%
\subsection{Tensor rank lower bound of certain tensors}\label{subsec:tensor-rank-lower-bound}

%{\color{red} some stuff repeats}

We first prove a lemma about  $\calM_{n; a, b}
\in \Sym^n(\bbF^2)$, which was defined in
Section~\ref{sec:apps-short}.
%rank of the connection tensor for graph matching.
%Let $\calM_{a, b} = \calM_{n; a, b} \in \Sym^n(\bbF^2)$
%denote the function $\{0, 1\}^n \rightarrow \bbF$ ($n \ge 1$),
%such that on the all-0 input {\bf 0} it takes value $a$,
%on all inputs of Hamming weight one it takes value $b$,
%and on all other inputs it takes value 0.
%This function is denoted by $[a, b, 0, \ldots, 0]$ in the Holant literature.
Below is a restatement of Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound-short};
the proof
%The following proof
is adapted from the proof of Lemma 5.1 in~\cite{Comon-Golub-Lim-Mourrain-2008}.

\begin{lemma}\label{lem:weighted-matchings-tensor-rank-lower-bound}
If $b \ne 0$ and $n \ge 0$, then $\symrank \calM_{n; a, b} \ge n$.
\end{lemma}
%%% this is lm 4.1
\begin{proof}
% of Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound-short}.
For $n = 0$ the lemma is trivial. Let $n \ge 1$.
Clearly $\calM_{n; a, b} \not = 0$, and so  $r = \symrank \calM_{n; a, b} \ge 1$.
Suppose  $r < n$ for a contradiction. 
Then we can write $\calM_{n; a, b} = \sum_{i = 1}^r \lambda_i v_i^{\otimes n}$ 
where  $\lambda_i \in \bbF$, and $v_i = (\alpha_i, \beta_i) \in \bbF^2$
are nonzero and 
pairwise linearly independent.
The decomposition implies that
the linear system $A x = \vec b$ with the extended matrix
\begin{equation}\label{eqn:wm-vand-sys}
\widehat A = [A \mid \vec b] =
\left[
\begin{array}{cccc|c}
\alpha_1^n & \alpha_2^n & \ldots & \alpha_r^n & a \\
\alpha_1^{n - 1} \beta_1 & \alpha_2^{n - 1} \beta_2 & \ldots & \alpha_r^{n - 1} \beta_r & b \\
\alpha_1^{n - 2} \beta_1^2 & \alpha_2^{n - 2} \beta_2^2 & \ldots & \alpha_r^{n - 2} \beta_r^2 & 0 \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
\beta_1^n & \beta_2^n & \ldots & \beta_r^n & 0
\end{array}
\right]
\end{equation}
has a solution $x_i = \lambda_i,\, 1 \le i \le r$.
Note that $\widehat A$ is $(n+1) \times (r+1)$ and
$A$ has only $r$ columns.
We show that $\matrank \,\widehat A = r+1 > \matrank \, A$.
This is a contradiction.

\begin{enumerate}
\item All $\beta_i \ne 0$.
\sout{Then} {\color{red} Then, by the pairwise linear independence of $v_i$, (JYC: added maybe add "the numbers" after $v_i$ to separate the symbols)} $\alpha_i / \beta_i$ are pairwise distinct.
Then the last $r$ rows of $A$, i.e., rows $n - r + 2$ to $n + 1$
form an $r \times r$ Vandermonde matrix of rank $r$.
Note that $n+1 \ge n - r + 2 > 2$.
By $b \ne 0$, we get an $(r + 1) \times (r + 1)$ submatrix
of  $\widehat A$  of rank $r+1$ by taking row $2$ and the last $r$ rows.

\item Some  $\beta_i = 0$. Without loss of generality we can assume it is $\beta_1$.
\sout{Then} {\color{red} Then, by the pairwise linear independence of $v_i$, (JYC: added maybe add "the numbers" after $v_i$ to separate the symbols)} all  other $\beta_i \not = 0$,
and all $\alpha_i / \beta_i$ are pairwise distinct for $2 \le i \le r$.
Then since $b \ne 0$, the submatrix  of $\widehat A$
formed by taking rows $1, 2$ and the last $r - 1 \ge 0$
rows have rank $r+1$.
%More precisely, when $r \ge 2$, we take rows $1, 2, n - r + 3, \ldots, n + 1$,
%and when $r = 1$, we only take rows $1, 2$.
%When $r \ge 2$, note that $3 < n - r + 3 \le n + 1$ because also $r < n$.
%Thus $\matrank \widehat A = r + 1$.
\end{enumerate}
\end{proof}


%%%---------

We now show that for an infinite field $\bbF$, 
%{\color{red} (only say $\bbF$ is infinite, and then split)}
we can give a tight
 upper bound for $\symrank \calM_{n; a, b}$ where $b \ne 0$  and $n \ge 1$.
The existence of
a decomposition $\calM_{n; a, b} = \sum_{i = 1}^r \lambda_i v_i^{\otimes n}$
where $r \ge 1$, $\lambda_i \in \bbF$ and $v_i = (\alpha_i, \beta_i) \in \bbF^2$
($1 \le i \le r$)
is equivalent to the statement that system~(\ref{eqn:wm-vand-sys})
has a solution $x_i = \lambda_i\, (1 \le i \le r)$.
Note that by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound},
we must have $r \ge n$.

Assume $\bbF$ is infinite. 
We show how to achieve $r = n$ with one exceptional case.
First, we set all $\beta_i = 1$.
By comparing with the Vandermonde determinant
$\det  [A \mid \vec t\,]$ as a polynomial in $t$, where the last column is
 $\vec t = (t^n, t^{n - 1}, \ldots, t, 1)^T$,
we see that 
\[
\det \widehat A  = \det([A \mid \vec b]) = (-1)^{n} \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \cdot \Big(a - b \sum_{i = 1}^n \alpha_i\Big).
\]
{\color{red} More precisely, we derive this equation as follows. Note that as a polynomial in $t$ the Vandermonde determinant $\det[A \mid \vec t\,] = \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \prod_{i = 1}^n (\alpha_i - t)= \sum_{i = 0}^n c_i t^i$ for some $c_i \in \bbF$ ($0 \le i \le n$) so they can be easily computed. Then $\det \widehat A = a c_n + b c_{n - 1}$ and the equation follows. (JYC: added, start the next sentence from a new paragraph?)}
If we set $\alpha_1, \ldots, \alpha_n  \in \bbF$ 
to be pairwise distinct, and $\sum_{i = 1}^n \alpha_i = a/b$,
then $\matrank A = \matrank \hat A = n$.
The (affine) hyperplane ${\mathbf \Pi}: \sum_{i = 1}^n \alpha_i = a/b$
has points away from its intersections with finitely many
hyperplanes $x_i = x_j$ ($i \ne j$), as long as
each of these hyperplanes is distinct from ${\mathbf \Pi}$.
This is trivially true if $n=1$. Let $n \ge 2$.
Under an affine linear transformation 
we may assume ${\mathbf \Pi}$ is the hyperplane $x_n =0$ in $\bbF^n$
and we only need to show $\bbF^{n-1}$ is not the union of finitely many,
say $k$, affine hyperplanes.
Consider the cube $S^{n-1}$ for a large subset $S \subseteq \bbF$.
The union of these  $k$ affine hyperplanes intersecting $S^{n-1}$
 has cardinality at 
most $k|S|^{n-2} < |S|^{n-1}$, for a large $S$.

Each hyperplane  $x_i = x_j$ ($i \ne j$) is distinct from ${\mathbf \Pi}$,
except in one case
\begin{equation}\label{case:exception}
a=0, ~n=2, ~\mbox{and}~ \Char \bbF = 2.
\end{equation}
In this exceptional case, we can easily prove that indeed 
 $\symrank \calM_{2; 0, b} =3$.



%Next, we show how to get $\matrank A = \matrank \hat A = n$ in (\ref{eqn:wm-vand-sys})
%with $r=n$.
%Suppose $\alpha_i \in \bbF$ are pairwise distinct.
%Then we get an $n \times n$ Vandermonde matrix of rank $n$ from row $2$ to row $n + 1$ of $A$.
%Clearly $\matrank \widehat A \ge \matrank A = n$,
%so for the $(n + 1) \times (n + 1)$ matrix $\widehat A$
%we only additionally need to have  $\det \widehat A = 0$.
%We can compute $\det \widehat A$ by expanding it along the last column.
%To compute the minors in the expansion,
%replace the last column $\vec b$
%by the column $\vec t = (t^n, t^{n - 1}, \ldots, t, 1)^T$ where $t$ is an indeterminate,
%then we get a Vandermonde $(n + 1) \times (n + 1)$ matrix $[A \mid \vec t]$ with the determinant
%\[
%\det [A \mid \vec t] = \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \prod_{1 \le i \le n} ( \alpha_i - t).
%\]
%Now comparing coefficients of $t^n$ and $t^{n-1}$ we get
%\[
%\det \widehat A  = \det([A \mid \vec b]) = (-1)^{n} \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \cdot \Big(a - b \sum_{i = 1}^n \alpha_i\Big).
%\]
%Thus for pairwise distinct $\alpha_i  \in \bbF$,
 %$\det \widehat A = 0$ is equivalent to $\sum_{i = 1}^n \alpha_i = a / b$.
%If $n = 1$, then let $\alpha_1 = a / b$ and we are done.
%Assume $n \ge 2$.
%% Then $n - 1 \ge 1$.
%%We let $\alpha_n = a / b - \sum_{i = 1}^{n - 1} \alpha_i$.
%Consider the polynomial
%\[
%p(x_1, \ldots, x_{n - 1}) =  \Big( \prod_{1 \le i < j \le n - 1} (x_i - x_j) \Big) \prod_{1 \le i \le n - 1} \Big(\frac{a}{b} - \sum_{j = 1}^{n - 1} x_j - x_i \Big).
%\]
%Note that $p(x_1, \ldots, x_{n - 1})$ is the zero polynomial iff 
%$a = 0$, $n = 2$ and $\Char \bbF = 2$.
%
%%\begin{enumerate}
%%\item \label{item:bbF-inf-generic-case} 
%
%
%Suppose it is not the case that $a = 0$, $n = 2$ and $\Char \bbF = 2$.
%Since $\bbF$ is infinite,
%then we can pick $\alpha_i \in \bbF$ such that
%$p(\alpha_1, \ldots, \alpha_{n - 1}) \ne 0$,
%and  $\alpha_n = a / b - \sum_{i = 1}^{n - 1} \alpha_i$.
%Hence  all $\alpha_i$ are pairwise distinct
%and $\sum_{i = 1}^n \alpha_i = a / b$.
%It follows that $\matrank A = \matrank \widehat A = n$.
%
%In the exceptional case $\Char \bbF = 2$,
%we can show indeed $\symrank \calM_{2; 0, b} = 3 > 2$, for $b \not =0$.
%
%%and therefore system~(\ref{eqn:wm-vand-sys}) (with $r = n$)
%%has a solution $x_i = \lambda_i, \, 1 \le i \le n$.
%%Then $\calM_{a, b} = \sum_{i = 1}^n \lambda_i (\alpha_i, 1)^{\otimes n}$.
%We conclude that $\symrank \calM_{a, b} = n$.
%
%\item \label{item:bbF-inf-exceptional-case} Now let $\Char \bbF = 2$, $n = 2$ and $a = 0$.
%We show first how to achieve $r = 3$
%and then that achieving $r = 2$ is impossible.
%Put all $\alpha_i = 1$ ($\alpha_1 = \alpha_2 = \alpha_3 = 1$).
%Next, choose $\beta_i \in \bbF$ ($\beta_1, \beta_2, \beta_3$)
%to be pairwise distinct which can be done as $\bbF$ is infinite.
%Then $A$ is a nondegenerate $3 \times 3$ Vandermonde matrix.
%It follows that system~(\ref{eqn:wm-vand-sys}) (with $r = 3$)
%has a (unique) solution $x_i = \lambda_i, \, 1 \le i \le 3$ ($x_1 = \lambda_1,\, x_2 = \lambda_2, x_3 = \lambda_3$).
%Then $\calM_{a, b} = \sum_{i = 1}^3 \lambda_i (1, \beta_i)^{\otimes 2}$ ($\calM_{a, b} = \lambda_1 (1, \beta_1)^{\otimes 2} + \lambda_2 (1, \beta_2)^{\otimes 2} + \lambda_3 (1, \beta_3)^{\otimes 2}$). In particular, $\symrank \calM_{a, b} \le 3$.
%
%{\color{red} must include it, but look at the variable names}
%
%Now we show that $\symrank \calM_{a, b} > 2$.
%Suppose otherwise. Then it can only be $\symrank \calM_{a, b} = 2$
%so we can write $\calM_{a, b} = \alpha (x, y)^{\otimes 2} + \beta (z, t)^{\otimes 2}$ where $\alpha, \beta \ne 0$.
%Then $\alpha x^2 + \beta z^2 = \alpha y^2 + \beta t^2 = 0$ ($= a$) and $\alpha x y + \beta z t = b$.
%In particular, $\alpha x^2 = -\beta z^2 = \beta z^2$ and $\alpha y^2 = -\beta t^2 = \beta t^2$
%and so $(\alpha x y)^2 = (\beta z t)^2$.
%Next, we have $(\alpha x y - \beta z t)^2 = (\alpha x y)^2 + (\beta z t)^2 = 0$
%so $\alpha x y = \beta z t$.
%Therefore $b = \alpha x y + \beta z t = 0$ which is a contraction with $b \ne 0$.
%Hence $\symrank \calM_{a, b} > 2$
%which implies $\symrank \calM_{a, b} = 3$.
%%\end{enumerate}

We have proved
\begin{lemma}\label{lem:weighted-matchings-tensor-rank-upper-bound}
If $\bbF$ is infinite, $b \ne 0$ and $n \ge 1$, then $\symrank \calM_{n; a, b} = n$
with one exception (\ref{case:exception}).
In that exceptional case, $\symrank \calM_{2;0, b} = 3$.
%unless $a = 0$, $n = 2$ and $\Char \bbF = 2$,
%in which case $\symrank \calM_{n;a, b} = 3$.
\end{lemma}
We remark that for any infinite $\bbF$
not in case (\ref{case:exception}), for $n \ge 2$
we can achieve $\matrank A = \matrank \widehat A = n$ in (\ref{eqn:wm-vand-sys})
by further requiring that all $\alpha_i \not =0$ (in addition to
being pairwise distinct, and all $\beta_i=1$.)
This is simply to avoid the  intersections of ${\mathbf \Pi}$
 with  another finitely many  hyperplanes distinct from ${\mathbf \Pi}$.
Setting $a_i = 1/\alpha_i$, we can set $a_i\in \bbF$ such that
 $\matrank A = \matrank \widehat A = n$ for the following $\widehat A$.
\begin{equation}\label{eqn:wm-vand-sys-for-d-deg-bounded-graphs}
\widehat A = [A \mid \vec b] =
\left[
\begin{array}{cccc|c}
1 & 1  & \ldots  & 1 & a\\
a_1 & a_2 & \ldots & a_n & 1 \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
a_1^{n-1} & a_2^{n-1} & \ldots & a_n^{n-1} & 0\\
a_1^n & a_2^n & \ldots & a_n^n & 0 
\end{array}
\right].
\end{equation}
The linear system $A x = \vec b$ has a solution $(\lambda_1, 
\ldots, \lambda_n)$ implies that
 $\calM_{m; a, b} = \sum_{i = 1}^n \lambda_i v_i^{\otimes m}$,
where $v_i = (1, a_i)$,
for  all $0 \le m \le n$.
(For $m=0$, $\calM_{0; a, 1} = a$ is a constant, and $v_i^{\otimes 0} = 1$.)
%%%---------


In Section~\ref{sec:apps-short}
we discussed \textsc{\#Perfect-Matching} ($\pmatch$).
Here we continue the discussion on  \textsc{\#Weighted-Matching$_a$}
and other $\Holant$ problems,
including proper edge colorings and vertex-disjoint cycle covers.

\subsection{Weighted matchings~\label{sec:Weighted-Matchings}}

%We now generalize the result to weighted matchings.
We prove that the problem \textsc{\#Weighted-Matching$_a$} defined by
$\wmatch_a(G) = \Holant(G; \{ \calM_{n; a, 1} \}_{n \ge 0})$ 
is not expressible as a GH function over any field,
for any $a$.
%(For $n=0$, $\calM_{0; a, 1} = a \in \mathbb F$.)
%$ is the scalar $a \in \mathbb F$.)
%The  Holant problem defining the graph parameter $\wmatch_a$
 %is the following: It takes input a  graph $G$, where every
%vertex of degree $d$ is attached a function $\calM_{d; a, 1}
%\in \Sym^d(\bbF^2)$ with the incident edges as input variables.
%The value $\wmatch_a(G)$ is the sum over all $\{0,1\}$-edge assignments
%of the product over $v \in V(G)$
%of evaluations of $\calM_{{\deg}(v); a, 1}$.
%% {\color{red} [What about $n = 0$]}

Clearly, $\wmatch_a$ is a multiplicative graph parameter with $\wmatch_a(K_0) = 1$. If  $a = 0$ then  $\wmatch_a$ is just \textsc{\#Perfect-Matching} ($\pmatch$). Counting all  matchings
is  $\wmatch_a$ for $a=1$.

Let $G$ be a $k$-labeled graph,  $X \subseteq [k]$,
and let $\wmatch_a(G, X)$ denote the partial $\Holant$ 
sum in $\wmatch_a(G)$
over all $\{ 0, 1 \}$-edge assignments of $G$ such that
within $[k]$, those in $X$ have  exactly one
 incident edge assigned $1$ and all nodes in $[k] \setminus X$ have no
incident edges assigned $1$.  
Then we have for any $k$-labeled graphs $G_1, \ldots, G_n$,
\[
\wmatch_a(G_1 \cdots G_n) = \sum_{X_1 \sqcup \ldots \sqcup X_n \subseteq [k]} a^{k - |X_1 \sqcup \ldots \sqcup X_n|} \wmatch_a(G_1, X_1) \cdots \wmatch_a(G_n, X_n).
\]
This means that $T(\wmatch_a, k, n)$ is
the product  $N_{k; a}^{\otimes n} W_{k, n; a}$,  where $N_{k; a}$ has
infinitely many rows indexed by all $k$-labeled graphs $G$, 
and $2^k$ columns indexed by $X \subseteq [k]$, with the entry at $(G, X)$
\[
N_{k; a; G, X} = \wmatch_a(G, X),
\]
and $W_{k, n; a}$ is a symmetric $\underbrace{2^k \times \ldots \times 2^k}_{n \text{ times}}$ tensor (from $\Sym^n(\bbF^{2^k})$), where
\[
W_{k, n; a; X_1, \ldots, X_n} =
\begin{lcases}
& a^{k - |X_1 \sqcup \ldots \sqcup X_n|} \quad \text{if } X_1 \sqcup \ldots \sqcup X_n \subseteq [k], \\
& 0 \quad \text{otherwise.}
\end{lcases}
\]
Hence 
 $\symrank T(\wmatch_a, k, n) \le \symrank W_{k, n; a}$. We show that in fact equality holds. Consider the same family of $k$-labeled graphs
 $\{ P_X \}_{X \subseteq [k]}$ defined in Section~\ref{sec:apps-short}.
It is easy to see that for $X, Y \subseteq [k]$, $N_{k; a; P_X, Y} = a^{|X| - |Y|}$ if $Y \subseteq X$ and $0$ otherwise. Here by convention, $a^0 = 1$ even if $a = 0$. Consider the rows in $N_{k; a}$ corresponding to $\{ P_X \}_{X \subseteq [k]}$. 
They form the nonsingular matrix $\trans{1}{0}{a}{1}^{\otimes n}$ 
if the rows and columns are ordered lexicographically for $X, Y \subseteq[k]$.
Therefore $\symrank W_{k, n; a} = \symrank 
\left(\trans{1}{0}{a}{1}^{\otimes n} W_{k, n; a} \right) \le \symrank T(\wmatch_a, k, n)$ and so $\symrank T(\wmatch_a, k, n) = \symrank W_{k, n; a}$.

Note that for $k = 1$, $W_{1, n; a} = \calM_{n;a, 1} = [a, 1, 0, \ldots 0] \in \Sym^n(\bbF^2)$ where $n \ge 1$. Applying Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound} with $b = 1$, we get $\symrank W_{1, n; a} \ge n$ and therefore $\symrank T(\wmatch_a, 1, n) \ge n$ for $n \ge 1$. Now if $\wmatch_a$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness}, $\symrank T(\wmatch_a, k, n) \le q^k$ for $k, n \ge 0$ so that $\symrank T(\wmatch_a, 1, n) \le q$ for $n \ge 0$. 
This contradicts  $\symrank T(\wmatch_a, 1, n) \ge n$ when $n > q$.
Hence $\wmatch_a$ is not expressible as a graph homomorphism function over any field. 

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible}, the proof for
 Theorem~\ref{thm:weighted-Matching-not-expressible-simple}
 carries over to simple graphs.


\begin{theorem}\label{thm:weighted-Matching-not-expressible-simple}
The graph parameter \textsc{\#Weighted-Matching} \emph{($\wmatch_a$)} where $a \in \bbF$ as a function defined on simple graphs is not expressible as a graph homomorphism function over any field $\bbF$.
\end{theorem}

\input{bounded-degree-graphs}

\subsection{Proper edge \texorpdfstring{$d$}{d}-colorings}

Next we show that the graph parameter  \#$d$-\textsc{Edge-Coloring}
($\edgecol_d$) is not expressible as
a GH function over any field of characteristic $0$. Given a graph $G$,
$\edgecol_d(G)$ counts the number of proper edge $d$-colorings in a graph,
 where $d \ge 1$ is the number of colors available.

Clearly, $\edgecol_d$ is a multiplicative graph parameter with $\edgecol(K_0) = 1$. Since $\Char \bbF = 0$, $\bbF$ is infinite. 
Consider $K_1$ as a $1$-labeled graph and the star graph $S_d$
with one internal node labeled by $1$ and $d$ unlabeled external nodes
all connected to node 1, where $d \ge 1$. 
Consider the  connection tensor $T(\edgecol_d, k, n)$ 
restricted to $\{ K_1, S_d \}^n$. For $(G_1, \ldots, G_n) \in \{ K_1, S_d \}^n$,
 if more than one $G_i = S_d$ then the product $G_1 \cdots G_n$ has no
proper edge $d$-coloring because the labeled vertex
has degree $\ge 2d > d$. Then
 it is easy to see that the connection tensor $T(\edgecol_d, k, n)$ restricted to $\{ K_1, S_d \}^n$ has the
 form $\calM_{1, d!} = [1, d!, 0, \ldots, 0] \in \Sym^n(\bbF^2)$,
and $d! \ne 0$ in $\bbF$ as $\Char \bbF = 0$.
Therefore by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound}, $\symrank \calM_{1, d!} \ge n$ for $n \ge 1$. Hence $\symrank T(\edgecol_d, 1, n) \ge n$ for $n \ge 1$.

Now if $\edgecol_d$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness},
% $\symrank T(\edgecol_d, k, n) \le q^k$ for $k, n \ge 0$ so that
 $\symrank T(\edgecol_d, 1, n) \le q$ for $n \ge 0$. This contradicts the upper bound when $n > q$. Hence $\edgecol_d$ is not expressible as a graph homomorphism function over any field $\bbF$ of $\Char \bbF = 0$.

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible},
the proof for
 Theorem~\ref{thm:Edge-Coloring-not-expressible-simple}
 carries over to  simple graphs.
%%%

\begin{theorem}\label{thm:Edge-Coloring-not-expressible-simple}
The graph parameter \#$d$-\textsc{Edge-Coloring} \emph{($\edgecol_d$)} with $d \ge 1$ as a function defined on simple graphs is not expressible as a graph homomorphism function over any field of characteristic $0$.
\end{theorem}


\subsection{Vertex-disjoint cycle covers}

We show that the graph parameter $\vdccover$
(\#\textsc{Vertex-Disjoint-Cycle-Cover})
 which counts the number of vertex disjoint cycle covers in a graph
is not expressible as a GH function over an arbitrary field.
%Here we follow the convention that 
In a multigraph without loop a cycle is
 a vertex disjoint closed path of length at least $2$.
The graph parameter $\vdccover(G) = m \cdot 1 \in {\mathbb F}$, where $m$ is
the number of edge subsets $E'$ that 
form  a vertex disjoint set of cycles that cover all vertices.

%%% not omitted
Clearly, $\vdccover$ is a multiplicative graph parameter with $\vdccover(K_0) = 1$. Next, consider $K_1$ and $K_3$ as $1$-labeled graphs.
Note that $K_3$ is a cycle of 3 vertices.
 It is easy to see that the connection tensor $T(\vdccover, k, n)$ restricted to $\{ K_1, K_3 \}^n$ has the form $\calM_{0, 1} = [0, 1, 0, \ldots, 0] \in \Sym^n(\bbF^2)$ and therefore by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound}, $\symrank \calM_{0, 1} \ge n$ for $n \ge 1$. Hence $\symrank T(\vdccover, 1, n) \ge n$ for $n \ge 1$.

Now if $\vdccover$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness},  $\symrank T(\vdccover, 1, n) \le q$ for $n \ge 0$. This contradicts the upper bound when $n > q$. Hence $\vdccover$ is not expressible as a 
GH function over any field. 

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible},
the proof for
 Theorem~\ref{thm:Vertex-Disjoint-Cycle-Cover-not-expressible-simple}
 carries over to  simple graphs.
%%%

\begin{theorem}\label{thm:Vertex-Disjoint-Cycle-Cover-not-expressible-simple}
The graph parameter \#\textsc{Vertex-Disjoint-Cycle-Cover} \emph{($\vdccover$)} as a function defined on simple graphs is not expressible as a graph homomorphism function over any field.
\end{theorem}




==> bibliography.tex <==
\begin{thebibliography}{50}
\bibitem{baxter-6-8}
R. J. Baxter: The Six and Eight-Vertex Models Revisited, Journal of Statistical Physics 116 (2004), 43-66.

\bibitem{Bulatov}
A. A. Bulatov:
The complexity of the counting constraint satisfaction problem. J. ACM 60(5): 34:1-34:41 (2013).

\bibitem{bulatov-dalmu}
A. Bulatov and V. Dalmau:
Towards a dichotomy theorem for the counting constraint satisfaction problem. Inf. Comput. 205(5): 651-678 (2007).

%\bibitem{Bulatov-etal}
%A. Bulatov, M. E. Dyer, L. Ann Goldberg and M. Jalsenius, D. Richerby: The complexity of weighted Boolean \#CSP with mixed signs.
%Theor. Comput. Sci. 410(38-40): 3949-3961 (2009).

\bibitem{Bulatov-Grohe-2005}
A. Bulatov and M. Grohe: The complexity of partition functions. Theor. Comput.
Sci., 348(2): 148-186, 2005.

\bibitem{Cai-Chen-2017}
J.-Y. Cai and X. Chen:
Complexity of Counting CSP with Complex Weights. J. ACM 64(3): 19:1-19:39 (2017).
A preliminary version appeared in Proceedings of the 44th Symposium on Theory of Computing (STOC), 2012, pp. 909-920.

\bibitem{cai-chen-book}
J.-Y. Cai and X. Chen: {\it Complexity Dichotomies for Counting Problems}, Volume 1: Boolean Domain,
 Cambridge University Press, 2017.
\url{https://doi.org/10.1017/9781107477063}
%\href{https://doi.org/10.1017/9781107477063}{https://doi.org/10.1017/9781107477063}

\bibitem{Cai-Chen-Lu-2013}
J.-Y. Cai, X. Chen and P. Lu:
Graph Homomorphisms with Complex Values: A Dichotomy Theorem. SIAM J. Comput. 42(3): 924-1029 (2013).

\bibitem{Cai-Zhiguo-2017}
J.-Y. Cai and Z. Fu: Holographic Algorithm with Matchgates Is Universal for
Planar \#CSP Over Boolean Domain. In Proc. of the 49th Annual ACM SIGACT
Symposium on Theory of Computing (STOC) 2017: 842-855. 
To appear in SIAM Journal on Computing.
Full version available at
\url{https://arxiv.org/abs/1603.07046}
%\href{https://arxiv.org/abs/1603.07046}{https://arxiv.org/abs/1603.07046}

\bibitem{Cai-Fu-Guo-W}
J.-Y. Cai, Z. Fu, H. Guo and T. Williams:
A Holant Dichotomy: Is the FKT Algorithm Universal? FOCS 2015: 1259-1276.

\bibitem{Cai-Govorov-2019}
%J.-Y. Cai, A. G.: Perfect matchings, rank of connection tensors and graph homomorphisms. SODA 2019: 476-495.
J.-Y. Cai and A. Govorov: Perfect matchings, rank of connection tensors and graph homomorphisms, In Proc. of ACM-SIAM Symposium on Discrete Algorithms (SODA) 2019, pp. 476-495.

\bibitem{caiguowilliams13}
J.-Y. Cai, H. Guo and T. Williams: A Complete Dichotomy Rises from the Capture of Vanishing Signatures.
SIAM J. Comput. 45(5): 1671-1728 (2016).
A preliminary version in STOC, pages 635-644. ACM, 2013.

%\bibitem{cgw-focs-2014}
%J.-Y. Cai, H. Guo and T. Williams:
%The Complexity of Counting Edge Colorings and a Dichotomy for Some Higher Domain Holant Problems.
%Research in the Mathematical Sciences,
%(2016) 3:18.
%A preliminary version in FOCS 2014: 601-610.

\bibitem{Cai-Lu-2007}
J.-Y. Cai and P. Lu:
Holographic algorithms: From art to science. J. Comput. Syst. Sci. 77(1): 41-61 (2011).
%Jin-Yi Cai, Pinyan Lu: Holographic algorithms: from art to science. STOC 2007: 401-410

%\bibitem{clx-focs-2008}
%J.-Y. Cai, P. Lu and M. Xia:
%Holographic Algorithms by Fibonacci Gates and Holographic Reductions for Hardness. FOCS 2008: 644-653.

\bibitem{clx-holant}
J.-Y. Cai, P. Lu and M. Xia:
Holant problems and counting CSP. STOC 2009: 715-724.

%\bibitem{CLX11a}
%J.-Y. Cai, P. Lu and M. Xia:
%Dichotomy for Holant* Problems of Boolean Domain. SODA 2011: 1714-1728.

\bibitem{Cohn-book}
P. M. Cohn, {\it Algebra}, Volume 3, John Wiley \& Sons, 2nd Edition, 1991. %Wiley

\bibitem{Comon-Golub-Lim-Mourrain-2008}
P. Comon, G. Golub, L.-H. Lim and B. Mourrain: Symmetric tensors and symmetric tensor rank, SIAM J. Matrix Anal. Appl., Vol. 30, No 3. (2008), pp. 1254-1279.

%\bibitem{Dyer-Goldberg-Jerrum}
%M. E. Dyer, L. A. Goldberg and M. Jerrum:
%The Complexity of Weighted Boolean \#CSP. SIAM J. Comput. 38(5): 1970-1986 (2009).

\bibitem{Dyer-Greenhill-2000}
M. E. Dyer and C. S. Greenhill:
The complexity of counting graph homomorphisms. Random Struct. Algorithms 17(3-4): 260-289 (2000).

\bibitem{Dyer-Greenhill-corrig-2004}
M. E. Dyer and C. S. Greenhill:
Corrigendum: The complexity of counting graph homomorphisms. Random Struct. Algorithms 25(3): 346-352 (2004).

\bibitem{Dyer-Richerby}
M. E. Dyer and D. Richerby:
An Effective Dichotomy for the Counting Constraint Satisfaction Problem. SIAM J. Comput. 42(3): 1245-1274 (2013).

\bibitem{Freedman-Lovasz-Schrijver-2007}
M. Freedman,  L. Lov\'asz, and A. Schrijver: Reflection positivity, rank connectivity, and homomorphism of graphs, Journal of AMS 20 (2007) 37-51. %M. H. Freedman

\bibitem{Goldberg-et-al-2010}
L. A. Goldberg, M. Grohe, M. Jerrum and M. Thurley: A complexity dichotomy for
partition functions with mixed signs, SIAM J. Comput., 39 (2010), pp. 3336-3402.

\bibitem{GRS}
 C. G\'{o}mez, M. Ruiz-Altaba and G. Sierra: Quantum Groups in Two-Dimensional Physics. Cambridge University
Press, Cambridge (1996).

\bibitem{Grohe-Thurley-2011}
M. Grohe and M. Thurley: Counting homomorphisms and partition functions. In Grohe, M. and Makowsky, J., editors,
Model Theoretic Methods in Finite Combinatorics, Contemporary Mathematics, Vol. 558, pages 243-292. American Mathematical Society (2011).

\bibitem{glva-2013}
H. Guo, P. Lu and L. G. Valiant:
The Complexity of Symmetric Boolean Parity Holant Problems. SIAM J. Comput. 42(1): 324-356 (2013).

\bibitem{GH-book}
P. Hell and J. Ne\v{s}et\v{r}il:
{\it Graphs and Homomorphisms},
(Oxford Lecture Series in Mathematics and Its Applications)
Oxford University Press; 1 edition (September 30, 2004).
% ISBN-13: 978-0198528173.

%\bibitem{HL12}
%S. Huang and P. Lu:
%A Dichotomy for Real Weighted Holant Problems. Computational Complexity 25(1): 255-304 (2016).

%\bibitem{Jacobson-book}
%N. Jacobson: {\it Basic Algebra II}, Dover Publications, 2nd Edition, 2012.

\bibitem{Kasteleyn-1961}
P. W. Kasteleyn: The Statistics of Dimers on a Lattice, Physica 27 (1961) 1209-1225.

\bibitem{Kasteleyn-1967}
P. W. Kasteleyn: Graph Theory and Crystal Physics. In Graph Theory and Theoretical
Physics, (F. Harary, ed.), Academic Press, London, 43-110 (1967).

\bibitem{Lovasz-1967}
L. Lov\'asz: Operations with structures, Acta Math. Hungar., 18 (1967), pp. 321-328.

\bibitem{Lovasz-Schrijver-2008}
L. Lov\'asz and A. Schriver: Graph parameters and semigroup functions, European Journal of Combinatorics 29 (2008) 987-1002.

\bibitem{B-Szegedy}
B. Szegedy: Edge  coloring  models  and  reflection  positivity,
J. Amer. Math. Soc., 20 (2007), no. 4, 969-988.

\bibitem{Tempereley-Fisher-1961}
H. N. V. Temperley and M. E. Fisher: Dimer Problem in Statistical Mechanics - an Exact
Result. Philosophical Magazine 6: 1061-1063 (1961).

\bibitem{Thurley-2009}
M. Thurley: The complexity of partition functions. PhD Thesis,
Humboldt Universitat zu Berlin, 2009.

\bibitem{Valiant-2004}
L. G. Valiant: Holographic Algorithms, SIAM J. Comput., 37(5) (2008) 1565-1594.
A preliminary version appeared in FOCS 2004: 306-315.

\bibitem{Val06}
L. G. Valiant: Accidental algorithms, FOCS 2006: 509-517.
%%%
\end{thebibliography}


==> his-preamble.tex <==
%\documentclass[11pt,twoside]{article}
\usepackage{amsmath, amsfonts, amssymb, amsthm, amscd, graphicx, 
%hyperref, 
enumerate, footmisc, mathtools, xcolor}
\setcounter{MaxMatrixCols}{30}
\setcounter{tocdepth}{10}
\providecommand{\U}[1]{\protect\rule{.1in}{.1in}}
\setlength{\topmargin}{-1.0in}
\setlength{\textheight}{9.25in}
\setlength{\oddsidemargin}{0.0in}
\setlength{\evensidemargin}{0.0in}
\setlength{\textwidth}{6.5in}
\def\labelenumi{\arabic{enumi}.}
\def\theenumi{\arabic{enumi}}
\def\labelenumii{(\alph{enumii})}
\def\theenumii{\alph{enumii}}
\def\p@enumii{\theenumi.}
\def\labelenumiii{\arabic{enumiii}.}
\def\theenumiii{\arabic{enumiii}}
\def\p@enumiii{(\theenumi)(\theenumii)}
\def\labelenumiv{\arabic{enumiv}.}
\def\theenumiv{\arabic{enumiv}}
\def\p@enumiv{\p@enumiii.\theenumiii}
\pagestyle{plain}
%\parindent=0pt
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}{Remark}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{axiom}{Axiom}

\newenvironment{lcases}
  {\left\lbrace\begin{aligned}}
  {\end{aligned}\right.}
\newcommand{\bbF}{\mathbb F}
\newcommand{\bbN}{\mathbb N}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbC}{\mathbb C}
\newcommand{\bbH}{\mathbb H}
\newcommand{\pmatch}{\operatorname{pm}}
\newcommand{\edgecol}{\operatorname{ec}}
\newcommand{\vdccover}{\operatorname{vdcc}}
\newcommand{\wmatch}{\operatorname{wm}}
\newcommand{\Char}{\operatorname{char}}
\newcommand{\Mod}{\operatorname{mod}}
%\newcommand{\rank}{\operatorname{rk}}
\newcommand{\symrank}{\operatorname{rk_\mathsf S}}
\newcommand{\matrank}{\operatorname{rank}}
\newcommand{\im}{\operatorname{im}}
%\newcommand{\Holant}{\operatorname{Holant}}
%\newcommand{\trans}[4]{\ensuremath{\left[ \begin{smallmatrix} #1 & #2 \\ #3 & #4 \end{smallmatrix} \right]}}
\newcommand{\Span}{\operatorname{span}}
%\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\id}{\operatorname{id}}
%\newcommand{\diag}{\operatorname{diag}}
%\newcommand{\dom}{\operatorname{dom}}

\newcommand{\calPLG}{\mathcal{PLG}}
\newcommand{\calG}{\mathcal G}
\newcommand{\calK}{\mathcal K}
\newcommand{\calP}{\mathcal P}
\newcommand{\bfx}{\mathbf x}
\newcommand{\bfy}{\mathbf y}
\newcommand{\bfz}{\mathbf z}
\newcommand{\sfS}{\mathsf S}
\newcommand{\sfT}{\mathsf T}
\newcommand{\calM}{\mathcal M}
\newcommand{\bfu}{\mathbf u}
\newcommand{\bfv}{\mathbf v}
\newcommand{\bff}{\mathbf f}
\newcommand{\textbfit}[1]{\textbf{\textit{#1}}}
\newcommand{\calI}{\mathcal I}
\newcommand{\calJ}{\mathcal J}
\newcommand{\calA}{\mathcal A}
\newcommand{\calT}{\mathcal T}

%%%\newcommand*{\mainflag}{}



==> line-numbers-patch.tex <==
%https://tex.stackexchange.com/questions/461186/how-to-use-lineno-with-amsmath-align
\usepackage[displaymath,mathlines]{lineno}
\linenumbers

%\makeatletter
%% Make a copy of macros responsible for entering display math mode
%\let\start@align@nopar\start@align
%\let\start@gather@nopar\start@gather
%\let\start@multline@nopar\start@multline
%% Add the "empty line" command to the macros
%\long\def\start@align{\par\start@align@nopar}
%\long\def\start@gather{\par\start@gather@nopar}
%\long\def\start@multline{\par\start@multline@nopar}
%\makeatother
\usepackage{etoolbox} %% <- for \pretocmd, \apptocmd and \patchcmd

%% Patch 'normal' math environment: (currently unused, but good to have)
% \newcommand*\linenomathpatch[1]{%
%   \expandafter\pretocmd\csname #1\endcsname {\linenomath}{}{}%
%   \expandafter\pretocmd\csname #1*\endcsname{\linenomath}{}{}%
%   \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}%
%   \expandafter\apptocmd\csname end#1*\endcsname{\endlinenomath}{}{}%
% }
%% Patch AMS math environment:
\newcommand*\linenomathpatchAMS[1]{%
  \expandafter\pretocmd\csname #1\endcsname {\linenomathAMS}{}{}%
  \expandafter\pretocmd\csname #1*\endcsname{\linenomathAMS}{}{}%
  \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}%
  \expandafter\apptocmd\csname end#1*\endcsname{\endlinenomath}{}{}%
}

%% Definition of \linenomathAMS depends on whether the mathlines option is provided
\expandafter\ifx\linenomath\linenomathWithnumbers
  \let\linenomathAMS\linenomathWithnumbers
  %% The following line gets rid of an extra line numbers at the bottom:
  \patchcmd\linenomathAMS{\advance\postdisplaypenalty\linenopenalty}{}{}{}
\else
  \let\linenomathAMS\linenomathNonumbers
\fi

% \linenomathpatch{equation} %% <- unnecessary, equation is already patched
\linenomathpatchAMS{gather}
\linenomathpatchAMS{multline}
\linenomathpatchAMS{align}
\linenomathpatchAMS{alignat}
\linenomathpatchAMS{flalign}



==> pm-rk-con-ten-GH-article-(cpc-submission)/applications-merged.tex <==
\section{Applications}\label{sec:apps} %\label{sec:apps-short}

%\subsection{Tensor rank lower bound of certain tensors}

%{\color{red} (cite Holant literature?)}
 
%We first state
%% prove 
%a lemma about the
%rank of the connection tensor for graph matchings.
%Let $\calM_{a, b} = \calM_{n; a, b} \in \Sym^n(\bbF^2)$
%denote the function $\{0, 1\}^n \rightarrow \bbF$ ($n \ge 0$),
%such that on the all-$0$ input $\mathbf 0$ it takes value $a$,
%on all inputs of Hamming weight one it takes value $b$,
%and on all other inputs it takes value $0$.
%This function is denoted by $[a, b, 0, \ldots, 0]$ in the Holant literature.
%($\calM_{0; a, b}$ is just a constant $a$.)
%We have the following lemma;
%its proof is  an adaptation of the proof of Lemma 5.1 in~\cite{Comon-Golub-Lim-Mourrain-2008},
%and  is given in subsection~\ref{subsec:tensor-rank-lower-bound}. %the  appendix  (Section~\ref{sec:Preliminary-continued}).
%
%\begin{lemma}\label{lem:weighted-matchings-tensor-rank-lower-bound-short}
%If $b \ne 0$ and $n \ge 0$, then $\symrank \calM_{n; a, b} \ge n$.
%\end{lemma}

%\section{Applications Continued~\label{sec:apps}}
%\section{More Applications~\label{sec:apps}}
%%%
\subsection{Tensor rank lower bound of certain tensors}\label{subsec:tensor-rank-lower-bound}

%{\color{red} some stuff repeats}

%We first prove a lemma about  $\calM_{n; a, b}
%\in \Sym^n(\bbF^2)$, which was defined in
%Section~\ref{sec:apps-short}.
%%rank of the connection tensor for graph matching.
%%Let $\calM_{a, b} = \calM_{n; a, b} \in \Sym^n(\bbF^2)$
%%denote the function $\{0, 1\}^n \rightarrow \bbF$ ($n \ge 1$),
%%such that on the all-0 input {\bf 0} it takes value $a$,
%%on all inputs of Hamming weight one it takes value $b$,
%%and on all other inputs it takes value 0.
%%This function is denoted by $[a, b, 0, \ldots, 0]$ in the Holant literature.
%Below is a restatement of Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound-short};
%the proof
%%The following proof
%is adapted from the proof of Lemma 5.1 in~\cite{Comon-Golub-Lim-Mourrain-2008}.

We first %state
prove 
a lemma about the
rank of the connection tensor for graph matchings.
Let $\calM_{a, b} = \calM_{n; a, b} \in \Sym^n(\bbF^2)$
denote the function $\{0, 1\}^n \rightarrow \bbF$ ($n \ge 0$),
such that on the all-$0$ input $\mathbf 0$ it takes value $a$,
on all inputs of Hamming weight one it takes value $b$,
and on all other inputs it takes value $0$.
This function is denoted by $[a, b, 0, \ldots, 0]$ in the Holant literature.
($\calM_{0; a, b}$ is just a constant $a$.)
We have the following lemma;
the proof
%The following proof
is adapted from the proof of Lemma 5.1 in~\cite{Comon-Golub-Lim-Mourrain-2008}.

\begin{lemma}\label{lem:weighted-matchings-tensor-rank-lower-bound}
If $b \ne 0$ and $n \ge 0$, then $\symrank \calM_{n; a, b} \ge n$.
\end{lemma}
%%% this is lm 4.1
\begin{proof}
% of Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound-short}.
For $n = 0$ the lemma is trivial. Let $n \ge 1$.
Clearly $\calM_{n; a, b} \not = 0$, and so  $r = \symrank \calM_{n; a, b} \ge 1$.
Suppose  $r < n$ for a contradiction. 
Then we can write $\calM_{n; a, b} = \sum_{i = 1}^r \lambda_i v_i^{\otimes n}$ 
where  $\lambda_i \in \bbF$, and $v_i = (\alpha_i, \beta_i) \in \bbF^2$
are nonzero and 
pairwise linearly independent.
The decomposition implies that
the linear system $A x = \vec b$ with the extended matrix
\begin{equation}\label{eqn:wm-vand-sys}
\widehat A = [A \mid \vec b] =
\left[
\begin{array}{cccc|c}
\alpha_1^n & \alpha_2^n & \ldots & \alpha_r^n & a \\
\alpha_1^{n - 1} \beta_1 & \alpha_2^{n - 1} \beta_2 & \ldots & \alpha_r^{n - 1} \beta_r & b \\
\alpha_1^{n - 2} \beta_1^2 & \alpha_2^{n - 2} \beta_2^2 & \ldots & \alpha_r^{n - 2} \beta_r^2 & 0 \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
\beta_1^n & \beta_2^n & \ldots & \beta_r^n & 0
\end{array}
\right]
\end{equation}
has a solution $x_i = \lambda_i,\, 1 \le i \le r$.
Note that $\widehat A$ is $(n+1) \times (r+1)$ and
$A$ has only $r$ columns.
We show that $\matrank \,\widehat A = r+1 > \matrank \, A$.
This is a contradiction. We consider the following two cases.

\begin{enumerate}
\item All $\beta_i \ne 0$.
Then, by the pairwise linear independence of $v_i$, the ratios 
 $\alpha_i / \beta_i$ are pairwise distinct.
Then the last $r$ rows of $A$, i.e., rows $n - r + 2$ to $n + 1$
form an $r \times r$ Vandermonde matrix of rank $r$.
Note that $n+1 \ge n - r + 2 > 2$.
By $b \ne 0$, we get an $(r + 1) \times (r + 1)$ submatrix
of  $\widehat A$  of rank $r+1$ by taking row $2$ and the last $r$ rows.

\item Some  $\beta_i = 0$. Without loss of generality we can assume it is $\beta_1$.
Again by the pairwise linear independence of $v_i$, 
 all  other $\beta_i \not = 0$,
and all $\alpha_i / \beta_i$ are pairwise distinct for $2 \le i \le r$
(vacuously true if $r=1$).
Then since $b \ne 0$, the submatrix  of $\widehat A$
formed by taking rows $1, 2$ and the last $r - 1 \ge 0$
rows have rank $r+1$.
%More precisely, when $r \ge 2$, we take rows $1, 2, n - r + 3, \ldots, n + 1$,
%and when $r = 1$, we only take rows $1, 2$.
%When $r \ge 2$, note that $3 < n - r + 3 \le n + 1$ because also $r < n$.
%Thus $\matrank \widehat A = r + 1$.
\end{enumerate}
\end{proof}


%%%---------

We now show that for an infinite field $\bbF$, 
%{\color{red} (only say $\bbF$ is infinite, and then split)}
we can give a tight
 upper bound for $\symrank \calM_{n; a, b}$ where $b \ne 0$  and $n \ge 1$.
The existence of
a decomposition $\calM_{n; a, b} = \sum_{i = 1}^r \lambda_i v_i^{\otimes n}$
where $r \ge 1$, $\lambda_i \in \bbF$ and $v_i = (\alpha_i, \beta_i) \in \bbF^2$
($1 \le i \le r$)
is equivalent to the statement that system~(\ref{eqn:wm-vand-sys})
has a solution $x_i = \lambda_i\, (1 \le i \le r)$.
Note that by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound},
we must have $r \ge n$.

Assume $\bbF$ is infinite. 
We show how to achieve $r = n$ with one exceptional case.
First, we set all $\beta_i = 1$.
By comparing with the Vandermonde determinant
$\det([A \mid \vec t\,])$ as a polynomial in $t$, where the last column is
 $\vec t = (t^n, t^{n - 1}, \ldots, t, 1)^T$,
we have 
\[
\det \widehat A  = \det([A \mid \vec b]) = (-1)^{n} \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \cdot \Big(a - b \sum_{i = 1}^n \alpha_i\Big).
\]
To see this equation, note that as a polynomial in $t$ the Vandermonde determinant $\det([A \mid \vec t\,]) = \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \prod_{i = 1}^n (\alpha_i - t)= \sum_{i = 0}^n c_i t^i$ for 
some $c_i \in \bbF$ ($0 \le i \le n$).
% so they can be easily computed. 
Then $\det \widehat A = a c_n + b c_{n - 1}$. 

If we set $\alpha_1, \ldots, \alpha_n  \in \bbF$ 
to be pairwise distinct, and $\sum_{i = 1}^n \alpha_i = a/b$,
then $\matrank A = \matrank \hat A = n$.
The (affine) hyperplane ${\mathbf \Pi}: \sum_{i = 1}^n \alpha_i = a/b$
has points away from its intersections with finitely many
hyperplanes $x_i = x_j$ ($i \ne j$), as long as
each of these hyperplanes is distinct from ${\mathbf \Pi}$.
This is trivially true if $n=1$. Let $n \ge 2$.
Under an affine linear transformation 
we may assume ${\mathbf \Pi}$ is the hyperplane $x_n =0$ in $\bbF^n$
and we only need to show $\bbF^{n-1}$ is not the union of finitely many,
say $k$, affine hyperplanes.
Consider the cube $S^{n-1}$ for a large subset $S \subseteq \bbF$.
The union of these  $k$ affine hyperplanes intersecting $S^{n-1}$
 has cardinality at 
most $k|S|^{n-2} < |S|^{n-1}$, for a large $S$.

Each hyperplane  $x_i = x_j$ ($i \ne j$) is distinct from ${\mathbf \Pi}$,
except in one case
\begin{equation}\label{case:exception}
a=0, ~n=2, ~\mbox{and}~ \Char \bbF = 2.
\end{equation}
In this exceptional case, we can easily prove that indeed 
 $\symrank \calM_{2; 0, b} =3$.



%Next, we show how to get $\matrank A = \matrank \hat A = n$ in (\ref{eqn:wm-vand-sys})
%with $r=n$.
%Suppose $\alpha_i \in \bbF$ are pairwise distinct.
%Then we get an $n \times n$ Vandermonde matrix of rank $n$ from row $2$ to row $n + 1$ of $A$.
%Clearly $\matrank \widehat A \ge \matrank A = n$,
%so for the $(n + 1) \times (n + 1)$ matrix $\widehat A$
%we only additionally need to have  $\det \widehat A = 0$.
%We can compute $\det \widehat A$ by expanding it along the last column.
%To compute the minors in the expansion,
%replace the last column $\vec b$
%by the column $\vec t = (t^n, t^{n - 1}, \ldots, t, 1)^T$ where $t$ is an indeterminate,
%then we get a Vandermonde $(n + 1) \times (n + 1)$ matrix $[A \mid \vec t]$ with the determinant
%\[
%\det [A \mid \vec t] = \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \prod_{1 \le i \le n} ( \alpha_i - t).
%\]
%Now comparing coefficients of $t^n$ and $t^{n-1}$ we get
%\[
%\det \widehat A  = \det([A \mid \vec b]) = (-1)^{n} \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \cdot \Big(a - b \sum_{i = 1}^n \alpha_i\Big).
%\]
%Thus for pairwise distinct $\alpha_i  \in \bbF$,
 %$\det \widehat A = 0$ is equivalent to $\sum_{i = 1}^n \alpha_i = a / b$.
%If $n = 1$, then let $\alpha_1 = a / b$ and we are done.
%Assume $n \ge 2$.
%% Then $n - 1 \ge 1$.
%%We let $\alpha_n = a / b - \sum_{i = 1}^{n - 1} \alpha_i$.
%Consider the polynomial
%\[
%p(x_1, \ldots, x_{n - 1}) =  \Big( \prod_{1 \le i < j \le n - 1} (x_i - x_j) \Big) \prod_{1 \le i \le n - 1} \Big(\frac{a}{b} - \sum_{j = 1}^{n - 1} x_j - x_i \Big).
%\]
%Note that $p(x_1, \ldots, x_{n - 1})$ is the zero polynomial iff 
%$a = 0$, $n = 2$ and $\Char \bbF = 2$.
%
%%\begin{enumerate}
%%\item \label{item:bbF-inf-generic-case} 
%
%
%Suppose it is not the case that $a = 0$, $n = 2$ and $\Char \bbF = 2$.
%Since $\bbF$ is infinite,
%then we can pick $\alpha_i \in \bbF$ such that
%$p(\alpha_1, \ldots, \alpha_{n - 1}) \ne 0$,
%and  $\alpha_n = a / b - \sum_{i = 1}^{n - 1} \alpha_i$.
%Hence  all $\alpha_i$ are pairwise distinct
%and $\sum_{i = 1}^n \alpha_i = a / b$.
%It follows that $\matrank A = \matrank \widehat A = n$.
%
%In the exceptional case $\Char \bbF = 2$,
%we can show indeed $\symrank \calM_{2; 0, b} = 3 > 2$, for $b \not =0$.
%
%%and therefore system~(\ref{eqn:wm-vand-sys}) (with $r = n$)
%%has a solution $x_i = \lambda_i, \, 1 \le i \le n$.
%%Then $\calM_{a, b} = \sum_{i = 1}^n \lambda_i (\alpha_i, 1)^{\otimes n}$.
%We conclude that $\symrank \calM_{a, b} = n$.
%
%\item \label{item:bbF-inf-exceptional-case} Now let $\Char \bbF = 2$, $n = 2$ and $a = 0$.
%We show first how to achieve $r = 3$
%and then that achieving $r = 2$ is impossible.
%Put all $\alpha_i = 1$ ($\alpha_1 = \alpha_2 = \alpha_3 = 1$).
%Next, choose $\beta_i \in \bbF$ ($\beta_1, \beta_2, \beta_3$)
%to be pairwise distinct which can be done as $\bbF$ is infinite.
%Then $A$ is a nondegenerate $3 \times 3$ Vandermonde matrix.
%It follows that system~(\ref{eqn:wm-vand-sys}) (with $r = 3$)
%has a (unique) solution $x_i = \lambda_i, \, 1 \le i \le 3$ ($x_1 = \lambda_1,\, x_2 = \lambda_2, x_3 = \lambda_3$).
%Then $\calM_{a, b} = \sum_{i = 1}^3 \lambda_i (1, \beta_i)^{\otimes 2}$ ($\calM_{a, b} = \lambda_1 (1, \beta_1)^{\otimes 2} + \lambda_2 (1, \beta_2)^{\otimes 2} + \lambda_3 (1, \beta_3)^{\otimes 2}$). In particular, $\symrank \calM_{a, b} \le 3$.
%
%{\color{red} must include it, but look at the variable names}
%
%Now we show that $\symrank \calM_{a, b} > 2$.
%Suppose otherwise. Then it can only be $\symrank \calM_{a, b} = 2$
%so we can write $\calM_{a, b} = \alpha (x, y)^{\otimes 2} + \beta (z, t)^{\otimes 2}$ where $\alpha, \beta \ne 0$.
%Then $\alpha x^2 + \beta z^2 = \alpha y^2 + \beta t^2 = 0$ ($= a$) and $\alpha x y + \beta z t = b$.
%In particular, $\alpha x^2 = -\beta z^2 = \beta z^2$ and $\alpha y^2 = -\beta t^2 = \beta t^2$
%and so $(\alpha x y)^2 = (\beta z t)^2$.
%Next, we have $(\alpha x y - \beta z t)^2 = (\alpha x y)^2 + (\beta z t)^2 = 0$
%so $\alpha x y = \beta z t$.
%Therefore $b = \alpha x y + \beta z t = 0$ which is a contraction with $b \ne 0$.
%Hence $\symrank \calM_{a, b} > 2$
%which implies $\symrank \calM_{a, b} = 3$.
%%\end{enumerate}

We have proved the following. 
\begin{lemma}\label{lem:weighted-matchings-tensor-rank-upper-bound}
If $\bbF$ is infinite, $b \ne 0$ and $n \ge 1$, then $\symrank \calM_{n; a, b} = n$
with one exception (\ref{case:exception}).
In that exceptional case, $\symrank \calM_{2;0, b} = 3$.
%unless $a = 0$, $n = 2$ and $\Char \bbF = 2$,
%in which case $\symrank \calM_{n;a, b} = 3$.
\end{lemma}
We remark that for any infinite $\bbF$
not in case (\ref{case:exception}), for $n \ge 2$
we can achieve $\matrank A = \matrank \widehat A = n$ in (\ref{eqn:wm-vand-sys})
by further requiring that all $\alpha_i \not =0$ (in addition to
being pairwise distinct, and all $\beta_i=1$.)
This is simply to avoid the  intersections of ${\mathbf \Pi}$
 with  another finitely many  hyperplanes distinct from ${\mathbf \Pi}$.
Setting $a_i = 1/\alpha_i$, we can set $a_i\in \bbF$ such that
 $\matrank A = \matrank \widehat A = n$ for the following $\widehat A$.
\begin{equation}\label{eqn:wm-vand-sys-for-d-deg-bounded-graphs}
\widehat A = [A \mid \vec b] =
\left[
\begin{array}{cccc|c}
1 & 1  & \ldots  & 1 & a\\
a_1 & a_2 & \ldots & a_n & 1 \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
a_1^{n-1} & a_2^{n-1} & \ldots & a_n^{n-1} & 0\\
a_1^n & a_2^n & \ldots & a_n^n & 0 
\end{array}
\right].
\end{equation}
The linear system $A x = \vec b$ has a solution $(\lambda_1, 
\ldots, \lambda_n)$ implies that
 $\calM_{m; a, b} = \sum_{i = 1}^n \lambda_i v_i^{\otimes m}$,
where $v_i = (1, a_i)$,
for  all $0 \le m \le n$.
(For $m=0$, $\calM_{0; a, 1} = a$ is a constant, and $v_i^{\otimes 0} = 1$.)
%%%---------


%In Section~\ref{sec:apps-short}
%we discussed \textsc{\#Perfect-Matching} ($\pmatch$).
%Here we continue the discussion on  \textsc{\#Weighted-Matching$_a$}
%and other $\Holant$ problems,
%including proper edge colorings and vertex-disjoint cycle covers.

\subsection{Perfect matchings~\label{sec:Perfect-Matchings}}

Let  $\mathcal{F}$ be any set of
$\bbF$-valued constraint functions, a.k.a. signatures,
from some finite set $[q]$.
E.g., the  binary {\sc Equality} $(=_2)$ signature
on $(x, y)$ outputs value 1 if $x=y$, and 0 otherwise.
Similarly one can define {\sc All-Distinct} on $[q]$,
and {\sc Exact-One} and {\sc Exact-Two}
 on the Boolean domain $(q=2)$.
%
An input to a Holant problem $\Holant(\mathcal{F})$ is 
 $\Omega = (G, \pi)$
where  $G = (V,E)$ is  a graph (with possible multiple edges and loops),
and $\pi$ assigns to each $v \in V$ some $f_v \in \mathcal{F}$
of arity $\deg(v)$, and associate its incident edges as input variables
 to $f_v$.
 The output is $\Holant(G; \mathcal{F})
 = \sum_{\sigma} \prod_{v \in V} f_v(\sigma \mid_{E(v)})$, where the sum is  over all edge assignments $\sigma: E \to [q]$,
 $E(v)$ denotes the incident edges of $v$ and $\sigma \mid_{E(v)}$ denotes the restriction of $\sigma$.
Bipartite $\Holant(G;  \mathcal{F} \mid \mathcal{G})$ are
defined on bipartite graphs $G = (U, V, E)$ where vertices in
$U$ and $V$ are assigned signatures from $\mathcal{F}$ and $\mathcal{G}$
respectively.

The graph parameter that counts the number of perfect matchings in a graph,
denoted by \textsc{\#Perfect-Matching} (or $\pmatch$),
is a quintessential Holant problem, corresponding to the {\sc Exact-One} function.
In this subsection we show it 
is not expressible as a GH function over any field.
%This was proved in~\cite{Freedman-Lovasz-Schrijver-2007} for real-valued GH with positive vertex weights.
This was proved in~\cite{Freedman-Lovasz-Schrijver-2007} for GH functions with real edge and positive vertex weights.
 However
that proof does not work for arbitrary fields, 
e.g., for the field of complex numbers $\bbC$,
 or even for real numbers with arbitrary (not necessarily positive) vertex weights. A crucial condition in~\cite{Freedman-Lovasz-Schrijver-2007} is positive semidefiniteness. 
%A succinct reason that the proof fails for $\bbC$
%is that for  complex matrices, $M^{\tt T}M$ is in general
%not positive semidefinite. 
%{\color{red} (Is this the reason, I asked the same in the introduction.)} 
%In fact, one of the most important
%%% I know. i decided as thus.
%holographic transformations~\cite{CLX11a, Cai-Fu-Guo-W}
%\cite{citesome-holographic-alg-dichotomypapers}
%{\color{red} (citesome-holographic-alg-dichotomypapers, hence I cite two papers here, make sure they fit in this context)}
%is $Z = \frac{1}{\sqrt{2}} \left[\begin{smallmatrix} 1 & 1\\
%\mathfrak{i} & -\mathfrak{i} \end{smallmatrix}\right]$,
%satisfying $Z^{\tt T} Z = \left[\begin{smallmatrix} 0 & 1\\ 
%1 & 0 \end{smallmatrix}\right]$. 
%\footnote{This transformation transforms
%binary equality functions to binary disequality functions,
%thus is crucial in dealing with orientation problems in the
%complexity classification of counting problems.}
%\sout{ Our main result (Theorems~\ref{thm:uniform-exponential-rank-boundedness}, \ref{thm:uniform-exponential-rank-boundedness-converse} and~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened})
%indicates that, to be expressible as GH,
%   this condition of positive semidefiniteness is actually incidental
%if we state it for connection tensors; 
%indeed the property of being a GH function is
%completely characterized by tensor rank.}
Our main result (Theorems~\ref{thm:uniform-exponential-rank-boundedness}, \ref{thm:uniform-exponential-rank-boundedness-converse} and~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened})
indicates that the property of being expressible as a GH function
is completely characterized by tensor rank. 

Let $\pmatch(G) = m \cdot 1 \in \bbF$ (the sum of $m$ copies of $1 \in \bbF$) where 
 $m$ is the  number of perfect matchings in $G$.
Obviously, $\pmatch$ is a multiplicative graph parameter with $\pmatch(K_0) = 1$. Next, let $G$ be a $k$-labeled graph, let $X \subseteq [k]$, and let $\pmatch(G, X)$ denote the number of matchings in $G$ (expressed in $\bbF$)
%or this number mod $p$
%if $\Char \bbF = p$) 
that match all the unlabeled nodes and, for labeled nodes,
% within $[k]$
exactly the nodes in $X$. 
Then 
%we have 
for any $k$-labeled graphs $G_1, \ldots, G_n$,
\[
\pmatch(G_1 \cdots G_n) = \sum_{X_1 \sqcup \ldots \sqcup X_n = [k]} \pmatch(G_1, X_1) \cdots \pmatch(G_n, X_n).
\]

%This can be read as follows: the tensor
This means that $T(\pmatch, k, n)$ is 
the product $N_k^{\otimes n} W_{k, n}$ where $N_k$ has 
infinitely many rows indexed by all $k$-labeled graphs $G$, but only $2^k$ columns indexed by the subsets $X$ of $[k]$, with the entry at $(G, X)$
\[
N_{k; G, X} = \pmatch(G, X),
\]
and $W_{k, n}$ is a symmetric $\underbrace{2^k \times \ldots \times 2^k}_{n \text{ times}}$ tensor (from $\Sym^n(\bbF^{2^k})$), where
\[
W_{k, n; X_1, \ldots, X_n} =
\begin{lcases}
& 1 \quad \text{if } X_1 \sqcup \ldots \sqcup X_n = [k], \\
& 0 \quad \text{otherwise.}
\end{lcases}
\]
For any $k$,  if  $W_{k, n} = \sum_{i=1}^r a_i v_i^{\otimes n}$, then
$T(\pmatch, k, n) = \sum_{i=1}^r a_i (N_{k} v_i)^{\otimes n}$.
Hence 
%the symmetric rank of $T(\pmatch, k, n)$ is at most that of $W_{k, n}$, i.e.,
 $\symrank T(\pmatch, k, n) \le \symrank W_{k, n}$. 
We show that in fact equality holds. Consider the family of $k$-labeled graphs $\{ P_X \}_{X \subseteq [k]}$ of cardinality $2^k$ indexed by the subsets of $[k]$ and defined as follows: each $P_X$ has $|X|$ unlabeled vertices $\{ x_i \}_{i \in X}$ and $k$ labeled vertices $\{ y_i \}_{i = 1}^k$ labeled $1$ to $k$,
 with an edge between $x_i$ and $y_j$ iff $i = j$. It is easy so see that for $X, Y \subseteq [k]$, $N_{k; P_X, Y} = 1$ if $X = Y$ and $0$ otherwise. Then if we consider the subset of rows in $N_k$ corresponding to $\{ P_X \}_{X \subseteq [k]}$ we see that they form the identity matrix $I_{2^k}$ with a suitable
order of rows. Therefore $\symrank W_{k, n} = \symrank \left( I_{2^k}^{\otimes n} W_{k, n} \right) \le \symrank T(\pmatch, k, n)$ and so $\symrank T(\pmatch, k, n) = \symrank W_{k, n}$.

Note that for $k = 1$, $W_{1, n}$ is just the perfect matching
tensor (or the {\sc Exact-One} function on $n$ inputs) $\calM_{0, 1}
%%% didn't dsfine this symmetric signature notation. no need.
% = [0, 1, 0, \ldots 0]
 \in \Sym^n(\bbF^2)$ where $n \ge 1$. Applying Lemma \ref{lem:weighted-matchings-tensor-rank-lower-bound} with $a = 0, b = 1$, we get $\symrank W_{1, n} \ge n$ and therefore $\symrank T(\pmatch, 1, n) \ge n$ for $n \ge 1$. Now if $\pmatch$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness}, $\symrank T(\pmatch, k, n) \le q^k$ for $k, n \ge 0$ so that $\symrank T(\pmatch, 1, n) \le q$ for $n \ge 0$. However, as we have just shown $\symrank T(\pmatch, 1, n) \ge n$ for $n \ge 1$ which contradicts the upper bound when $n > q$. Hence $\pmatch$ is not expressible as a graph homomorphism function over any field. We state it as a theorem:
\begin{theorem}\label{thm:Perfect-Matching-not-expressible}
The graph parameter \textsc{\#Perfect-Matching} \emph{($\pmatch$)} is not expressible as a graph homomorphism function over any field.
\end{theorem}

%\begin{remark}
In this proof we have only used simple $k$-labeled graphs that  do
not have edges between the $k$ labeled vertices. The graphs $\{ P_X \}_{X \subseteq [k]}$ clearly have this property, and this property is
preserved under product of 
$k$-labeled graphs. 
It follows that Theorem~\ref{thm:Perfect-Matching-not-expressible}
holds even when $\pmatch$ is restricted to simple graphs. 
%for simple graphs.

We can prove the same inexpressibility results for
other Holant problems, such as weighted matchings,
proper edge colorings, and
vertex disjoint cycle covers.
We will also discuss bounded degree cases of weighted matchings.

\begin{comment}
We can prove the same inexpressibility results for
weighted matchings, 
proper edge colorings, and
vertex disjoint cycle covers (see Section~\ref{sec:apps}).
%In the appendix (Section~\ref{sec:apps}) we give the details.
For bounded degree graphs
% (see also Section~\ref{sec:apps}), 
we can also prove {\color{red} the following (see Section~\ref{sec:bonded-deg-graphs}). (JYC, added)}
% (see Section~\ref{sec:bonded-deg-graphs})
\begin{theorem}\label{thm:pm-as-GH-for-deg-bounded-graphs-short}
Let $\bbF$ be a field and $d \ge 2$. Then for the graph parameter \textsc{\#Perfect-Matching} \emph{($\pmatch$)}
as a function defined on degree-$d$ bounded graphs the following hold:
\begin{enumerate}
\item $\pmatch$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$ even on degree-$d$ bounded \emph{simple} graphs.
\item If $\bbF$ is infinite, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$ unless $\Char \bbF = 2$ and $d = 2$
(and in which case the minimum value is $|V(H)| = d + 1 = 3$).
%{\color{red} and the inexpressibility with $|V(H)| = d \le 2$ holds even degree-$d$ bounded \emph{simple} graphs. (add) }
%in which case $\pmatch$ is not expressible $\hom(\cdot, H)$ with $|V(H)| = d$ even on degree-$d$ bounded \emph{simple} graphs
%but is expressible as $\hom(\cdot, H)$ with $|V(H)| = d + 1 = 3$.
\end{enumerate}
\end{theorem}

%{\color{red} (old statement, can be commented out)}
%
%{\color{blue}
%\begin{theorem}\label{thm:pm-as-GH-for-deg-bounded-graphs-short-old}
%Let $\bbF$ be a field and $d \ge 2$. Then for the graph parameter
 %\textsc{\#Perfect-Matching} \emph{($\pmatch$)}  as a function 
%defined on $d$-degree bounded graphs the following hold:
%\begin{enumerate}
%\item $\pmatch$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$  even on $d$-degree bounded \emph{simple} graphs.
%\item If $\bbF$ is infinite, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d \text{ or } d + 1$.
%\item If $\Char \bbF = 0$, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$.
%\end{enumerate}
%\end{theorem}
%}

%In Section~\ref{sec:apps-short}
%we discussed \textsc{\#Perfect-Matching} ($\pmatch$).
%Here we continue the discussion on  \textsc{\#Weighted-Matching$_a$}
%and other $\Holant$ problems,
%including proper edge colorings and vertex-disjoint cycle covers.

{\color{red}
We have discussed \textsc{\#Perfect-Matching} ($\pmatch$).
Here we continue the discussion on more general \textsc{\#Weighted-Matching$_a$}
and other $\Holant$ problems,
including proper edge colorings and vertex-disjoint cycle covers.
(JYC: adapted from the previous text, see the hidden comment in tex above)}

{\color{red} (JYC: Note that we need weighted matchings including the definition.
We can say that the proof for weighted matchings is more technical but is included for completeness.
For perfect matching, we also need to have a proof, because it's the first simplistic argument. Basically keep both.)}

\end{comment}

%%%%%%%%%%%%%%

\subsection{Weighted matchings~\label{sec:Weighted-Matchings}}

%We now generalize the result to weighted matchings.
We prove that the problem \textsc{\#Weighted-Matching$_a$} defined by
$\wmatch_a(G) = \Holant(G; \{ \calM_{n; a, 1} \}_{n \ge 0})$ 
is not expressible as a GH function over any field,
for any $a$.
%(For $n=0$, $\calM_{0; a, 1} = a \in \mathbb F$.)
%$ is the scalar $a \in \mathbb F$.)
%The  Holant problem defining the graph parameter $\wmatch_a$
 %is the following: It takes input a  graph $G$, where every
%vertex of degree $d$ is attached a function $\calM_{d; a, 1}
%\in \Sym^d(\bbF^2)$ with the incident edges as input variables.
%The value $\wmatch_a(G)$ is the sum over all $\{0,1\}$-edge assignments
%of the product over $v \in V(G)$
%of evaluations of $\calM_{{\deg}(v); a, 1}$.
%% {\color{red} [What about $n = 0$]}

Clearly, $\wmatch_a$ is a multiplicative graph parameter with $\wmatch_a(K_0) = 1$. If  $a = 0$ then  $\wmatch_a$ is just \textsc{\#Perfect-Matching} ($\pmatch$). Counting all  matchings
is  $\wmatch_a$ for $a=1$.

Let $G$ be a $k$-labeled graph,  $X \subseteq [k]$,
and let $\wmatch_a(G, X)$ denote the partial $\Holant$ 
sum in $\wmatch_a(G)$
over all $\{ 0, 1 \}$-edge assignments of $G$ such that
within $[k]$, those in $X$ have  exactly one
 incident edge assigned $1$ and all nodes in $[k] \setminus X$ have no
incident edges assigned $1$.  
Then we have for any $k$-labeled graphs $G_1, \ldots, G_n$,
\[
\wmatch_a(G_1 \cdots G_n) = \sum_{X_1 \sqcup \ldots \sqcup X_n \subseteq [k]} a^{k - |X_1 \sqcup \ldots \sqcup X_n|} \wmatch_a(G_1, X_1) \cdots \wmatch_a(G_n, X_n).
\]
This means that $T(\wmatch_a, k, n)$ is
the product  $N_{k; a}^{\otimes n} W_{k, n; a}$,  where $N_{k; a}$ has
infinitely many rows indexed by all $k$-labeled graphs $G$, 
and $2^k$ columns indexed by $X \subseteq [k]$, with the entry at $(G, X)$
\[
N_{k; a; G, X} = \wmatch_a(G, X),
\]
and $W_{k, n; a}$ is a symmetric $\underbrace{2^k \times \ldots \times 2^k}_{n \text{ times}}$ tensor (from $\Sym^n(\bbF^{2^k})$), where
\[
W_{k, n; a; X_1, \ldots, X_n} =
\begin{lcases}
& a^{k - |X_1 \sqcup \ldots \sqcup X_n|} \quad \text{if } X_1 \sqcup \ldots \sqcup X_n \subseteq [k], \\
& 0 \quad \text{otherwise.}
\end{lcases}
\]
Hence 
 $\symrank T(\wmatch_a, k, n) \le \symrank W_{k, n; a}$. We show that in fact equality holds. Consider the same family of $k$-labeled graphs
 $\{ P_X \}_{X \subseteq [k]}$ defined in the previous subsection.
% (JYC: changed)} %Section~\ref{sec:apps-short}.
It is easy to see that for $X, Y \subseteq [k]$, $N_{k; a; P_X, Y} = a^{|X| - |Y|}$ if $Y \subseteq X$ and $0$ otherwise. Here by convention, $a^0 = 1$ even if $a = 0$. Consider the rows in $N_{k; a}$ corresponding to $\{ P_X \}_{X \subseteq [k]}$. 
They form the nonsingular matrix $\trans{1}{0}{a}{1}^{\otimes n}$ 
if the rows and columns are ordered lexicographically for $X, Y \subseteq[k]$.
Therefore $\symrank W_{k, n; a} = \symrank 
\left(\trans{1}{0}{a}{1}^{\otimes n} W_{k, n; a} \right) \le \symrank T(\wmatch_a, k, n)$ and so $\symrank T(\wmatch_a, k, n) = \symrank W_{k, n; a}$.

Note that for $k = 1$, $W_{1, n; a} = \calM_{n;a, 1} = [a, 1, 0, \ldots 0] \in \Sym^n(\bbF^2)$ where $n \ge 1$. Applying Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound} with $b = 1$, we get $\symrank W_{1, n; a} \ge n$ and therefore $\symrank T(\wmatch_a, 1, n) \ge n$ for $n \ge 1$. Now if $\wmatch_a$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem~\ref{thm:uniform-exponential-rank-boundedness}, $\symrank T(\wmatch_a, k, n) \le q^k$ for $k, n \ge 0$ so that $\symrank T(\wmatch_a, 1, n) \le q$ for $n \ge 0$. 
This contradicts  $\symrank T(\wmatch_a, 1, n) \ge n$ when $n > q$.
Hence $\wmatch_a$ is not expressible as a graph homomorphism function over any field. 

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible}, the proof for
 Theorem~\ref{thm:weighted-Matching-not-expressible-simple}
 carries over to simple graphs.


\begin{theorem}\label{thm:weighted-Matching-not-expressible-simple}
The graph parameter \textsc{\#Weighted-Matching} \emph{($\wmatch_a$)} where $a \in \bbF$ as a function defined on simple graphs is not expressible as a graph homomorphism function over any field $\bbF$.
\end{theorem}

\input{bounded-degree-graphs}

\subsection{Proper edge \texorpdfstring{$d$}{d}-colorings}

Next we show that the graph parameter  \#$d$-\textsc{Edge-Coloring}
($\edgecol_d$) is not expressible as
a GH function over any field of characteristic $0$. Given a graph $G$,
$\edgecol_d(G)$ counts the number of proper edge $d$-colorings in a graph,
 where $d \ge 1$ is the number of colors available.

Clearly, $\edgecol_d$ is a multiplicative graph parameter with $\edgecol(K_0) = 1$. Since $\Char \bbF = 0$, $\bbF$ is infinite. 
Consider $K_1$ as a $1$-labeled graph and the star graph $S_d$
with one internal node labeled by $1$ and $d$ unlabeled external nodes
all connected to node 1, where $d \ge 1$. 
Consider the  connection tensor $T(\edgecol_d, k, n)$ 
restricted to $\{ K_1, S_d \}^n$. For $(G_1, \ldots, G_n) \in \{ K_1, S_d \}^n$,
 if more than one $G_i = S_d$ then the product $G_1 \cdots G_n$ has no
proper edge $d$-coloring because the labeled vertex
has degree $\ge 2d > d$. Then
 it is easy to see that the connection tensor $T(\edgecol_d, k, n)$ restricted to $\{ K_1, S_d \}^n$ has the
 form $\calM_{1, d!} = [1, d!, 0, \ldots, 0] \in \Sym^n(\bbF^2)$,
and $d! \ne 0$ in $\bbF$ as $\Char \bbF = 0$.
Therefore by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound}, $\symrank \calM_{1, d!} \ge n$ for $n \ge 1$. Hence $\symrank T(\edgecol_d, 1, n) \ge n$ for $n \ge 1$.

Now if $\edgecol_d$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness},
% $\symrank T(\edgecol_d, k, n) \le q^k$ for $k, n \ge 0$ so that
 $\symrank T(\edgecol_d, 1, n) \le q$ for $n \ge 0$. This contradicts the upper bound when $n > q$. Hence $\edgecol_d$ is not expressible as a graph homomorphism function over any field $\bbF$ of $\Char \bbF = 0$.

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible},
the proof for
 Theorem~\ref{thm:Edge-Coloring-not-expressible-simple}
 carries over to  simple graphs.
%%%

\begin{theorem}\label{thm:Edge-Coloring-not-expressible-simple}
The graph parameter \#$d$-\textsc{Edge-Coloring} \emph{($\edgecol_d$)} with $d \ge 1$ as a function defined on simple graphs is not expressible as a graph homomorphism function over any field of characteristic $0$.
\end{theorem}


\subsection{Vertex-disjoint cycle covers}

We show that the graph parameter $\vdccover$
(\#\textsc{Vertex-Disjoint-Cycle-Cover})
 which counts the number of vertex disjoint cycle covers in a graph
is not expressible as a GH function over an arbitrary field.
%Here we follow the convention that 
In a multigraph without loop a cycle is
 a vertex disjoint closed path of length at least $2$.
The graph parameter $\vdccover(G) = m \cdot 1 \in {\mathbb F}$, where $m$ is
the number of edge subsets $E'$ that 
form  a vertex disjoint set of cycles that cover all vertices.

%%% not omitted
Clearly, $\vdccover$ is a multiplicative graph parameter with $\vdccover(K_0) = 1$. Next, consider $K_1$ and $K_3$ as $1$-labeled graphs.
Note that $K_3$ is a cycle of 3 vertices.
 It is easy to see that the connection tensor $T(\vdccover, k, n)$ restricted to $\{ K_1, K_3 \}^n$ has the form $\calM_{0, 1} = [0, 1, 0, \ldots, 0] \in \Sym^n(\bbF^2)$ and therefore by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound}, $\symrank \calM_{0, 1} \ge n$ for $n \ge 1$. Hence $\symrank T(\vdccover, 1, n) \ge n$ for $n \ge 1$.

Now if $\vdccover$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness},  $\symrank T(\vdccover, 1, n) \le q$ for $n \ge 0$. This contradicts the upper bound when $n > q$. Hence $\vdccover$ is not expressible as a 
GH function over any field. 

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible},
the proof for
 Theorem~\ref{thm:Vertex-Disjoint-Cycle-Cover-not-expressible-simple}
 carries over to  simple graphs.
%%%

\begin{theorem}\label{thm:Vertex-Disjoint-Cycle-Cover-not-expressible-simple}
The graph parameter \#\textsc{Vertex-Disjoint-Cycle-Cover} \emph{($\vdccover$)} as a function defined on simple graphs is not expressible as a graph homomorphism function over any field.
\end{theorem}




==> pm-rk-con-ten-GH-article-(cpc-submission)/applications-short.tex <==
\section{Applications}\label{sec:apps-short}

\subsection{Tensor rank lower bound of certain tensors}

%{\color{red} (cite Holant literature?)}
 
We first state
% prove 
a lemma about the
rank of the connection tensor for graph matchings.
Let $\calM_{a, b} = \calM_{n; a, b} \in \Sym^n(\bbF^2)$
denote the function $\{0, 1\}^n \rightarrow \bbF$ ($n \ge 0$),
such that on the all-$0$ input $\mathbf 0$ it takes value $a$,
on all inputs of Hamming weight one it takes value $b$,
and on all other inputs it takes value $0$.
This function is denoted by $[a, b, 0, \ldots, 0]$ in the Holant literature.
($\calM_{0; a, b}$ is just a constant $a$.)
We have the following lemma;
its proof is  an adaptation of the proof of Lemma 5.1 in~\cite{Comon-Golub-Lim-Mourrain-2008},
and  is given in subsection~\ref{subsec:tensor-rank-lower-bound}. %the  appendix  (Section~\ref{sec:Preliminary-continued}).

\begin{lemma}\label{lem:weighted-matchings-tensor-rank-lower-bound-short}
If $b \ne 0$ and $n \ge 0$, then $\symrank \calM_{n; a, b} \ge n$.
\end{lemma}

\subsection{Perfect matchings~\label{sec:Perfect-Matchings}}

Let  $\mathcal{F}$ be any set of
$\bbF$-valued constraint functions, a.k.a. signatures,
from some finite set $[q]$.
E.g., the  binary {\sc Equality} $(=_2)$ signature
on $(x, y)$ outputs value 1 if $x=y$, and 0 otherwise.
Similarly one can define {\sc All-Distinct} on $[q]$,
and {\sc Exact-One} and {\sc Exact-Two}
 on the Boolean domain $(q=2)$.
%
An input to a Holant problem $\Holant(\mathcal{F})$ is 
 $\Omega = (G, \pi)$
where  $G = (V,E)$  a graph (with possible multiple edges and loops),
and $\pi$ assigns to each $v \in V$ some $f_v \in \mathcal{F}$
of arity $\deg(v)$, and its incident edges as inputs.
 The output is $\Holant(G; \mathcal{F})
 = \sum_{\sigma} \prod_{v \in V} f_v(\sigma \mid_{E(v)})$, where the sum is  over all edge assignments $\sigma: E \to [q]$,
 $E(v)$ denotes the incident edges of $v$ and $\sigma \mid_{E(v)}$ denotes the restriction.
Bipartite $\Holant(G;  \mathcal{F} \mid \mathcal{G})$ are
defined on bipartite graphs $G = (U, V, E)$ where vertices in
$U$ and $V$ are assigned signatures from $\mathcal{F}$ and $\mathcal{G}$
respectively.

The graph parameter that counts the number of perfect matchings in a graph,
denoted by \textsc{\#Perfect-Matching} (or $\pmatch$),
is a quintessential Holant problem, corresponding to the {\sc Exact-One} function.
In this subsection we show it 
is not expressible as a GH function over any field.
%This was proved in~\cite{Freedman-Lovasz-Schrijver-2007} for real-valued GH with positive vertex weights.
This was proved in~\cite{Freedman-Lovasz-Schrijver-2007} for GH functions with real edge and positive vertex weights.
 However
that proof does not work for arbitrary fields, 
e.g., for the field of complex numbers $\bbC$,
 or even for real numbers with arbitrary (not necessarily positive) vertex weights. A crucial condition in~\cite{Freedman-Lovasz-Schrijver-2007} is positive semidefiniteness. 
%A succinct reason that the proof fails for $\bbC$
%is that for  complex matrices, $M^{\tt T}M$ is in general
%not positive semidefinite. 
%{\color{red} (Is this the reason, I asked the same in the introduction.)} 
%In fact, one of the most important
%%% I know. i decided as thus.
%holographic transformations~\cite{CLX11a, Cai-Fu-Guo-W}
%\cite{citesome-holographic-alg-dichotomypapers}
%{\color{red} (citesome-holographic-alg-dichotomypapers, hence I cite two papers here, make sure they fit in this context)}
%is $Z = \frac{1}{\sqrt{2}} \left[\begin{smallmatrix} 1 & 1\\
%\mathfrak{i} & -\mathfrak{i} \end{smallmatrix}\right]$,
%satisfying $Z^{\tt T} Z = \left[\begin{smallmatrix} 0 & 1\\ 
%1 & 0 \end{smallmatrix}\right]$. 
%\footnote{This transformation transforms
%binary equality functions to binary disequality functions,
%thus is crucial in dealing with orientation problems in the
%complexity classification of counting problems.}
\sout{ Our main result (Theorems~\ref{thm:uniform-exponential-rank-boundedness}, \ref{thm:uniform-exponential-rank-boundedness-converse} and~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened})
indicates that, to be expressible as GH,
   this condition of positive semidefiniteness is actually incidental
if we state it for connection tensors; 
indeed the property of being a GH function is
completely characterized by tensor rank.}
{\color{red} Our main result (Theorems~\ref{thm:uniform-exponential-rank-boundedness}, \ref{thm:uniform-exponential-rank-boundedness-converse} and~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened})
indicates that the property of being expressible as a GH function
is completely characterized by (the?) tensor rank. (JYC, replaced)}

Let $\pmatch(G) = m \cdot 1 \in \bbF$ (the sum of $m$ copies of $1 \in \bbF$) where 
 $m$ is the  number of perfect matchings in $G$.
Obviously, $\pmatch$ is a multiplicative graph parameter with $\pmatch(K_0) = 1$. Next, let $G$ be a $k$-labeled graph, let $X \subseteq [k]$, and let $\pmatch(G, X)$ denote the number of matchings in $G$ (expressed in $\bbF$)
%or this number mod $p$
%if $\Char \bbF = p$) 
that match all the unlabeled nodes and, for labeled nodes,
% within $[k]$
exactly the nodes in $X$. 
Then 
%we have 
for any $k$-labeled graphs $G_1, \ldots, G_n$,
\[
\pmatch(G_1 \cdots G_n) = \sum_{X_1 \sqcup \ldots \sqcup X_n = [k]} \pmatch(G_1, X_1) \cdots \pmatch(G_n, X_n).
\]

%This can be read as follows: the tensor
This means that $T(\pmatch, k, n)$ is 
the product $N_k^{\otimes n} W_{k, n}$ where $N_k$ has 
infinitely many rows indexed by all $k$-labeled graphs $G$, but only $2^k$ columns indexed by the subsets $X$ of $[k]$, with the entry at $(G, X)$
\[
N_{k; G, X} = \pmatch(G, X),
\]
and $W_{k, n}$ is a symmetric $\underbrace{2^k \times \ldots \times 2^k}_{n \text{ times}}$ tensor (from $\Sym^n(\bbF^{2^k})$), where
\[
W_{k, n; X_1, \ldots, X_n} =
\begin{lcases}
& 1 \quad \text{if } X_1 \sqcup \ldots \sqcup X_n = [k], \\
& 0 \quad \text{otherwise.}
\end{lcases}
\]
For any $k$,  if  $W_{k, n} = \sum_{i=1}^r a_i v_i^{\otimes n}$, then
$T(\pmatch, k, n) = \sum_{i=1}^r a_i (N_{k} v_i)^{\otimes n}$.
Hence 
%the symmetric rank of $T(\pmatch, k, n)$ is at most that of $W_{k, n}$, i.e.,
 $\symrank T(\pmatch, k, n) \le \symrank W_{k, n}$. 
We show that in fact equality holds. Consider the family of $k$-labeled graphs $\{ P_X \}_{X \subseteq [k]}$ of cardinality $2^k$ indexed by the subsets of $[k]$ and defined as follows: each $P_X$ has $|X|$ unlabeled vertices $\{ x_i \}_{i \in X}$ and $k$ labeled vertices $\{ y_i \}_{i = 1}^k$ labeled $1$ to $k$,
 with an edge between $x_i$ and $y_j$ iff $i = j$. It is easy so see that for $X, Y \subseteq [k]$, $N_{k; P_X, Y} = 1$ if $X = Y$ and $0$ otherwise. Then if we consider the subset of rows in $N_k$ corresponding to $\{ P_X \}_{X \subseteq [k]}$ we see that they form the identity matrix $I_{2^k}$ with a suitable
order of rows. Therefore $\symrank W_{k, n} = \symrank \left( I_{2^k}^{\otimes n} W_{k, n} \right) \le \symrank T(\pmatch, k, n)$ and so $\symrank T(\pmatch, k, n) = \symrank W_{k, n}$.

Note that for $k = 1$, $W_{1, n}$ is just the perfect matching
tensor (or the {\sc Exact-One} function on $n$ inputs) $\calM_{0, 1}
%%% didn't dsfine this symmetric signature notation. no need.
% = [0, 1, 0, \ldots 0]
 \in \Sym^n(\bbF^2)$ where $n \ge 1$. Applying Lemma \ref{lem:weighted-matchings-tensor-rank-lower-bound-short} with $a = 0, b = 1$, we get $\symrank W_{1, n} \ge n$ and therefore $\symrank T(\pmatch, 1, n) \ge n$ for $n \ge 1$. Now if $\pmatch$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness}, $\symrank T(\pmatch, k, n) \le q^k$ for $k, n \ge 0$ so that $\symrank T(\pmatch, 1, n) \le q$ for $n \ge 0$. However, as we have just shown $\symrank T(\pmatch, 1, n) \ge n$ for $n \ge 1$ which contradicts the upper bound when $n > q$. Hence $\pmatch$ is not expressible as a graph homomorphism function over any field. We state it as a theorem:
\begin{theorem}\label{thm:Perfect-Matching-not-expressible}
The graph parameter \textsc{\#Perfect-Matching} \emph{($\pmatch$)} is not expressible as a graph homomorphism function over any field.
\end{theorem}

%\begin{remark}
In this proof we have only used simple $k$-labeled graphs that  do
not have edges between the $k$ labeled vertices. The graphs $\{ P_X \}_{X \subseteq [k]}$ clearly have this property, and this property is
preserved under product of 
$k$-labeled graphs. 
It follows that Theorem~\ref{thm:Perfect-Matching-not-expressible}
holds even when $\pmatch$ is restricted to simple graphs. 
%for simple graphs.

We can prove the same inexpressibility results for
weighted matchings, 
proper edge colorings, and
vertex disjoint cycle covers (see Section~\ref{sec:apps}).
%In the appendix (Section~\ref{sec:apps}) we give the details.
For bounded degree graphs
% (see also Section~\ref{sec:apps}), 
we can also prove
% (see Section~\ref{sec:bonded-deg-graphs})
\begin{theorem}\label{thm:pm-as-GH-for-deg-bounded-graphs-short}
Let $\bbF$ be a field and $d \ge 2$. Then for the graph parameter \textsc{\#Perfect-Matching} \emph{($\pmatch$)}
as a function defined on degree-$d$ bounded graphs the following hold:
\begin{enumerate}
\item $\pmatch$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$ even on degree-$d$ bounded \emph{simple} graphs.
\item If $\bbF$ is infinite, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$ unless $\Char \bbF = 2$ and $d = 2$
(and in which case the minimum value is $|V(H)| = d + 1 = 3$).
%{\color{red} and the inexpressibility with $|V(H)| = d \le 2$ holds even degree-$d$ bounded \emph{simple} graphs. (add) }
%in which case $\pmatch$ is not expressible $\hom(\cdot, H)$ with $|V(H)| = d$ even on degree-$d$ bounded \emph{simple} graphs
%but is expressible as $\hom(\cdot, H)$ with $|V(H)| = d + 1 = 3$.
\end{enumerate}
\end{theorem}

%{\color{red} (old statement, can be commented out)}
%
%{\color{blue}
%\begin{theorem}\label{thm:pm-as-GH-for-deg-bounded-graphs-short-old}
%Let $\bbF$ be a field and $d \ge 2$. Then for the graph parameter
 %\textsc{\#Perfect-Matching} \emph{($\pmatch$)}  as a function 
%defined on $d$-degree bounded graphs the following hold:
%\begin{enumerate}
%\item $\pmatch$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$  even on $d$-degree bounded \emph{simple} graphs.
%\item If $\bbF$ is infinite, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d \text{ or } d + 1$.
%\item If $\Char \bbF = 0$, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$.
%\end{enumerate}
%\end{theorem}
%}



==> pm-rk-con-ten-GH-article-(cpc-submission)/applications.tex <==
%\section{Applications Continued~\label{sec:apps}}
\section{More Applications~\label{sec:apps}}
%%%
\subsection{Tensor rank lower bound of certain tensors}\label{subsec:tensor-rank-lower-bound}

%{\color{red} some stuff repeats}

We first prove a lemma about  $\calM_{n; a, b}
\in \Sym^n(\bbF^2)$, which was defined in
Section~\ref{sec:apps-short}.
%rank of the connection tensor for graph matching.
%Let $\calM_{a, b} = \calM_{n; a, b} \in \Sym^n(\bbF^2)$
%denote the function $\{0, 1\}^n \rightarrow \bbF$ ($n \ge 1$),
%such that on the all-0 input {\bf 0} it takes value $a$,
%on all inputs of Hamming weight one it takes value $b$,
%and on all other inputs it takes value 0.
%This function is denoted by $[a, b, 0, \ldots, 0]$ in the Holant literature.
Below is a restatement of Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound-short};
the proof
%The following proof
is adapted from the proof of Lemma 5.1 in~\cite{Comon-Golub-Lim-Mourrain-2008}.

\begin{lemma}\label{lem:weighted-matchings-tensor-rank-lower-bound}
If $b \ne 0$ and $n \ge 0$, then $\symrank \calM_{n; a, b} \ge n$.
\end{lemma}
%%% this is lm 4.1
\begin{proof}
% of Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound-short}.
For $n = 0$ the lemma is trivial. Let $n \ge 1$.
Clearly $\calM_{n; a, b} \not = 0$, and so  $r = \symrank \calM_{n; a, b} \ge 1$.
Suppose  $r < n$ for a contradiction. 
Then we can write $\calM_{n; a, b} = \sum_{i = 1}^r \lambda_i v_i^{\otimes n}$ 
where  $\lambda_i \in \bbF$, and $v_i = (\alpha_i, \beta_i) \in \bbF^2$
are nonzero and 
pairwise linearly independent.
The decomposition implies that
the linear system $A x = \vec b$ with the extended matrix
\begin{equation}\label{eqn:wm-vand-sys}
\widehat A = [A \mid \vec b] =
\left[
\begin{array}{cccc|c}
\alpha_1^n & \alpha_2^n & \ldots & \alpha_r^n & a \\
\alpha_1^{n - 1} \beta_1 & \alpha_2^{n - 1} \beta_2 & \ldots & \alpha_r^{n - 1} \beta_r & b \\
\alpha_1^{n - 2} \beta_1^2 & \alpha_2^{n - 2} \beta_2^2 & \ldots & \alpha_r^{n - 2} \beta_r^2 & 0 \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
\beta_1^n & \beta_2^n & \ldots & \beta_r^n & 0
\end{array}
\right]
\end{equation}
has a solution $x_i = \lambda_i,\, 1 \le i \le r$.
Note that $\widehat A$ is $(n+1) \times (r+1)$ and
$A$ has only $r$ columns.
We show that $\matrank \,\widehat A = r+1 > \matrank \, A$.
This is a contradiction.

\begin{enumerate}
\item All $\beta_i \ne 0$.
\sout{Then} {\color{red} Then, by the pairwise linear independence of $v_i$, (JYC: added maybe add "the numbers" after $v_i$ to separate the symbols)} $\alpha_i / \beta_i$ are pairwise distinct.
Then the last $r$ rows of $A$, i.e., rows $n - r + 2$ to $n + 1$
form an $r \times r$ Vandermonde matrix of rank $r$.
Note that $n+1 \ge n - r + 2 > 2$.
By $b \ne 0$, we get an $(r + 1) \times (r + 1)$ submatrix
of  $\widehat A$  of rank $r+1$ by taking row $2$ and the last $r$ rows.

\item Some  $\beta_i = 0$. Without loss of generality we can assume it is $\beta_1$.
\sout{Then} {\color{red} Then, by the pairwise linear independence of $v_i$, (JYC: added maybe add "the numbers" after $v_i$ to separate the symbols)} all  other $\beta_i \not = 0$,
and all $\alpha_i / \beta_i$ are pairwise distinct for $2 \le i \le r$.
Then since $b \ne 0$, the submatrix  of $\widehat A$
formed by taking rows $1, 2$ and the last $r - 1 \ge 0$
rows have rank $r+1$.
%More precisely, when $r \ge 2$, we take rows $1, 2, n - r + 3, \ldots, n + 1$,
%and when $r = 1$, we only take rows $1, 2$.
%When $r \ge 2$, note that $3 < n - r + 3 \le n + 1$ because also $r < n$.
%Thus $\matrank \widehat A = r + 1$.
\end{enumerate}
\end{proof}


%%%---------

We now show that for an infinite field $\bbF$, 
%{\color{red} (only say $\bbF$ is infinite, and then split)}
we can give a tight
 upper bound for $\symrank \calM_{n; a, b}$ where $b \ne 0$  and $n \ge 1$.
The existence of
a decomposition $\calM_{n; a, b} = \sum_{i = 1}^r \lambda_i v_i^{\otimes n}$
where $r \ge 1$, $\lambda_i \in \bbF$ and $v_i = (\alpha_i, \beta_i) \in \bbF^2$
($1 \le i \le r$)
is equivalent to the statement that system~(\ref{eqn:wm-vand-sys})
has a solution $x_i = \lambda_i\, (1 \le i \le r)$.
Note that by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound},
we must have $r \ge n$.

Assume $\bbF$ is infinite. 
We show how to achieve $r = n$ with one exceptional case.
First, we set all $\beta_i = 1$.
By comparing with the Vandermonde determinant
$\det  [A \mid \vec t\,]$ as a polynomial in $t$, where the last column is
 $\vec t = (t^n, t^{n - 1}, \ldots, t, 1)^T$,
we see that 
\[
\det \widehat A  = \det([A \mid \vec b]) = (-1)^{n} \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \cdot \Big(a - b \sum_{i = 1}^n \alpha_i\Big).
\]
{\color{red} More precisely, we derive this equation as follows. Note that as a polynomial in $t$ the Vandermonde determinant $\det[A \mid \vec t\,] = \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \prod_{i = 1}^n (\alpha_i - t)= \sum_{i = 0}^n c_i t^i$ for some $c_i \in \bbF$ ($0 \le i \le n$) so they can be easily computed. Then $\det \widehat A = a c_n + b c_{n - 1}$ and the equation follows. (JYC: added, start the next sentence from a new paragraph?)}
If we set $\alpha_1, \ldots, \alpha_n  \in \bbF$ 
to be pairwise distinct, and $\sum_{i = 1}^n \alpha_i = a/b$,
then $\matrank A = \matrank \hat A = n$.
The (affine) hyperplane ${\mathbf \Pi}: \sum_{i = 1}^n \alpha_i = a/b$
has points away from its intersections with finitely many
hyperplanes $x_i = x_j$ ($i \ne j$), as long as
each of these hyperplanes is distinct from ${\mathbf \Pi}$.
This is trivially true if $n=1$. Let $n \ge 2$.
Under an affine linear transformation 
we may assume ${\mathbf \Pi}$ is the hyperplane $x_n =0$ in $\bbF^n$
and we only need to show $\bbF^{n-1}$ is not the union of finitely many,
say $k$, affine hyperplanes.
Consider the cube $S^{n-1}$ for a large subset $S \subseteq \bbF$.
The union of these  $k$ affine hyperplanes intersecting $S^{n-1}$
 has cardinality at 
most $k|S|^{n-2} < |S|^{n-1}$, for a large $S$.

Each hyperplane  $x_i = x_j$ ($i \ne j$) is distinct from ${\mathbf \Pi}$,
except in one case
\begin{equation}\label{case:exception}
a=0, ~n=2, ~\mbox{and}~ \Char \bbF = 2.
\end{equation}
In this exceptional case, we can easily prove that indeed 
 $\symrank \calM_{2; 0, b} =3$.



%Next, we show how to get $\matrank A = \matrank \hat A = n$ in (\ref{eqn:wm-vand-sys})
%with $r=n$.
%Suppose $\alpha_i \in \bbF$ are pairwise distinct.
%Then we get an $n \times n$ Vandermonde matrix of rank $n$ from row $2$ to row $n + 1$ of $A$.
%Clearly $\matrank \widehat A \ge \matrank A = n$,
%so for the $(n + 1) \times (n + 1)$ matrix $\widehat A$
%we only additionally need to have  $\det \widehat A = 0$.
%We can compute $\det \widehat A$ by expanding it along the last column.
%To compute the minors in the expansion,
%replace the last column $\vec b$
%by the column $\vec t = (t^n, t^{n - 1}, \ldots, t, 1)^T$ where $t$ is an indeterminate,
%then we get a Vandermonde $(n + 1) \times (n + 1)$ matrix $[A \mid \vec t]$ with the determinant
%\[
%\det [A \mid \vec t] = \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \prod_{1 \le i \le n} ( \alpha_i - t).
%\]
%Now comparing coefficients of $t^n$ and $t^{n-1}$ we get
%\[
%\det \widehat A  = \det([A \mid \vec b]) = (-1)^{n} \prod_{1 \le i < j \le n} (\alpha_i - \alpha_j) \cdot \Big(a - b \sum_{i = 1}^n \alpha_i\Big).
%\]
%Thus for pairwise distinct $\alpha_i  \in \bbF$,
 %$\det \widehat A = 0$ is equivalent to $\sum_{i = 1}^n \alpha_i = a / b$.
%If $n = 1$, then let $\alpha_1 = a / b$ and we are done.
%Assume $n \ge 2$.
%% Then $n - 1 \ge 1$.
%%We let $\alpha_n = a / b - \sum_{i = 1}^{n - 1} \alpha_i$.
%Consider the polynomial
%\[
%p(x_1, \ldots, x_{n - 1}) =  \Big( \prod_{1 \le i < j \le n - 1} (x_i - x_j) \Big) \prod_{1 \le i \le n - 1} \Big(\frac{a}{b} - \sum_{j = 1}^{n - 1} x_j - x_i \Big).
%\]
%Note that $p(x_1, \ldots, x_{n - 1})$ is the zero polynomial iff 
%$a = 0$, $n = 2$ and $\Char \bbF = 2$.
%
%%\begin{enumerate}
%%\item \label{item:bbF-inf-generic-case} 
%
%
%Suppose it is not the case that $a = 0$, $n = 2$ and $\Char \bbF = 2$.
%Since $\bbF$ is infinite,
%then we can pick $\alpha_i \in \bbF$ such that
%$p(\alpha_1, \ldots, \alpha_{n - 1}) \ne 0$,
%and  $\alpha_n = a / b - \sum_{i = 1}^{n - 1} \alpha_i$.
%Hence  all $\alpha_i$ are pairwise distinct
%and $\sum_{i = 1}^n \alpha_i = a / b$.
%It follows that $\matrank A = \matrank \widehat A = n$.
%
%In the exceptional case $\Char \bbF = 2$,
%we can show indeed $\symrank \calM_{2; 0, b} = 3 > 2$, for $b \not =0$.
%
%%and therefore system~(\ref{eqn:wm-vand-sys}) (with $r = n$)
%%has a solution $x_i = \lambda_i, \, 1 \le i \le n$.
%%Then $\calM_{a, b} = \sum_{i = 1}^n \lambda_i (\alpha_i, 1)^{\otimes n}$.
%We conclude that $\symrank \calM_{a, b} = n$.
%
%\item \label{item:bbF-inf-exceptional-case} Now let $\Char \bbF = 2$, $n = 2$ and $a = 0$.
%We show first how to achieve $r = 3$
%and then that achieving $r = 2$ is impossible.
%Put all $\alpha_i = 1$ ($\alpha_1 = \alpha_2 = \alpha_3 = 1$).
%Next, choose $\beta_i \in \bbF$ ($\beta_1, \beta_2, \beta_3$)
%to be pairwise distinct which can be done as $\bbF$ is infinite.
%Then $A$ is a nondegenerate $3 \times 3$ Vandermonde matrix.
%It follows that system~(\ref{eqn:wm-vand-sys}) (with $r = 3$)
%has a (unique) solution $x_i = \lambda_i, \, 1 \le i \le 3$ ($x_1 = \lambda_1,\, x_2 = \lambda_2, x_3 = \lambda_3$).
%Then $\calM_{a, b} = \sum_{i = 1}^3 \lambda_i (1, \beta_i)^{\otimes 2}$ ($\calM_{a, b} = \lambda_1 (1, \beta_1)^{\otimes 2} + \lambda_2 (1, \beta_2)^{\otimes 2} + \lambda_3 (1, \beta_3)^{\otimes 2}$). In particular, $\symrank \calM_{a, b} \le 3$.
%
%{\color{red} must include it, but look at the variable names}
%
%Now we show that $\symrank \calM_{a, b} > 2$.
%Suppose otherwise. Then it can only be $\symrank \calM_{a, b} = 2$
%so we can write $\calM_{a, b} = \alpha (x, y)^{\otimes 2} + \beta (z, t)^{\otimes 2}$ where $\alpha, \beta \ne 0$.
%Then $\alpha x^2 + \beta z^2 = \alpha y^2 + \beta t^2 = 0$ ($= a$) and $\alpha x y + \beta z t = b$.
%In particular, $\alpha x^2 = -\beta z^2 = \beta z^2$ and $\alpha y^2 = -\beta t^2 = \beta t^2$
%and so $(\alpha x y)^2 = (\beta z t)^2$.
%Next, we have $(\alpha x y - \beta z t)^2 = (\alpha x y)^2 + (\beta z t)^2 = 0$
%so $\alpha x y = \beta z t$.
%Therefore $b = \alpha x y + \beta z t = 0$ which is a contraction with $b \ne 0$.
%Hence $\symrank \calM_{a, b} > 2$
%which implies $\symrank \calM_{a, b} = 3$.
%%\end{enumerate}

We have proved
\begin{lemma}\label{lem:weighted-matchings-tensor-rank-upper-bound}
If $\bbF$ is infinite, $b \ne 0$ and $n \ge 1$, then $\symrank \calM_{n; a, b} = n$
with one exception (\ref{case:exception}).
In that exceptional case, $\symrank \calM_{2;0, b} = 3$.
%unless $a = 0$, $n = 2$ and $\Char \bbF = 2$,
%in which case $\symrank \calM_{n;a, b} = 3$.
\end{lemma}
We remark that for any infinite $\bbF$
not in case (\ref{case:exception}), for $n \ge 2$
we can achieve $\matrank A = \matrank \widehat A = n$ in (\ref{eqn:wm-vand-sys})
by further requiring that all $\alpha_i \not =0$ (in addition to
being pairwise distinct, and all $\beta_i=1$.)
This is simply to avoid the  intersections of ${\mathbf \Pi}$
 with  another finitely many  hyperplanes distinct from ${\mathbf \Pi}$.
Setting $a_i = 1/\alpha_i$, we can set $a_i\in \bbF$ such that
 $\matrank A = \matrank \widehat A = n$ for the following $\widehat A$.
\begin{equation}\label{eqn:wm-vand-sys-for-d-deg-bounded-graphs}
\widehat A = [A \mid \vec b] =
\left[
\begin{array}{cccc|c}
1 & 1  & \ldots  & 1 & a\\
a_1 & a_2 & \ldots & a_n & 1 \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
a_1^{n-1} & a_2^{n-1} & \ldots & a_n^{n-1} & 0\\
a_1^n & a_2^n & \ldots & a_n^n & 0 
\end{array}
\right].
\end{equation}
The linear system $A x = \vec b$ has a solution $(\lambda_1, 
\ldots, \lambda_n)$ implies that
 $\calM_{m; a, b} = \sum_{i = 1}^n \lambda_i v_i^{\otimes m}$,
where $v_i = (1, a_i)$,
for  all $0 \le m \le n$.
(For $m=0$, $\calM_{0; a, 1} = a$ is a constant, and $v_i^{\otimes 0} = 1$.)
%%%---------


In Section~\ref{sec:apps-short}
we discussed \textsc{\#Perfect-Matching} ($\pmatch$).
Here we continue the discussion on  \textsc{\#Weighted-Matching$_a$}
and other $\Holant$ problems,
including proper edge colorings and vertex-disjoint cycle covers.

\subsection{Weighted matchings~\label{sec:Weighted-Matchings}}

%We now generalize the result to weighted matchings.
We prove that the problem \textsc{\#Weighted-Matching$_a$} defined by
$\wmatch_a(G) = \Holant(G; \{ \calM_{n; a, 1} \}_{n \ge 0})$ 
is not expressible as a GH function over any field,
for any $a$.
%(For $n=0$, $\calM_{0; a, 1} = a \in \mathbb F$.)
%$ is the scalar $a \in \mathbb F$.)
%The  Holant problem defining the graph parameter $\wmatch_a$
 %is the following: It takes input a  graph $G$, where every
%vertex of degree $d$ is attached a function $\calM_{d; a, 1}
%\in \Sym^d(\bbF^2)$ with the incident edges as input variables.
%The value $\wmatch_a(G)$ is the sum over all $\{0,1\}$-edge assignments
%of the product over $v \in V(G)$
%of evaluations of $\calM_{{\deg}(v); a, 1}$.
%% {\color{red} [What about $n = 0$]}

Clearly, $\wmatch_a$ is a multiplicative graph parameter with $\wmatch_a(K_0) = 1$. If  $a = 0$ then  $\wmatch_a$ is just \textsc{\#Perfect-Matching} ($\pmatch$). Counting all  matchings
is  $\wmatch_a$ for $a=1$.

Let $G$ be a $k$-labeled graph,  $X \subseteq [k]$,
and let $\wmatch_a(G, X)$ denote the partial $\Holant$ 
sum in $\wmatch_a(G)$
over all $\{ 0, 1 \}$-edge assignments of $G$ such that
within $[k]$, those in $X$ have  exactly one
 incident edge assigned $1$ and all nodes in $[k] \setminus X$ have no
incident edges assigned $1$.  
Then we have for any $k$-labeled graphs $G_1, \ldots, G_n$,
\[
\wmatch_a(G_1 \cdots G_n) = \sum_{X_1 \sqcup \ldots \sqcup X_n \subseteq [k]} a^{k - |X_1 \sqcup \ldots \sqcup X_n|} \wmatch_a(G_1, X_1) \cdots \wmatch_a(G_n, X_n).
\]
This means that $T(\wmatch_a, k, n)$ is
the product  $N_{k; a}^{\otimes n} W_{k, n; a}$,  where $N_{k; a}$ has
infinitely many rows indexed by all $k$-labeled graphs $G$, 
and $2^k$ columns indexed by $X \subseteq [k]$, with the entry at $(G, X)$
\[
N_{k; a; G, X} = \wmatch_a(G, X),
\]
and $W_{k, n; a}$ is a symmetric $\underbrace{2^k \times \ldots \times 2^k}_{n \text{ times}}$ tensor (from $\Sym^n(\bbF^{2^k})$), where
\[
W_{k, n; a; X_1, \ldots, X_n} =
\begin{lcases}
& a^{k - |X_1 \sqcup \ldots \sqcup X_n|} \quad \text{if } X_1 \sqcup \ldots \sqcup X_n \subseteq [k], \\
& 0 \quad \text{otherwise.}
\end{lcases}
\]
Hence 
 $\symrank T(\wmatch_a, k, n) \le \symrank W_{k, n; a}$. We show that in fact equality holds. Consider the same family of $k$-labeled graphs
 $\{ P_X \}_{X \subseteq [k]}$ defined in Section~\ref{sec:apps-short}.
It is easy to see that for $X, Y \subseteq [k]$, $N_{k; a; P_X, Y} = a^{|X| - |Y|}$ if $Y \subseteq X$ and $0$ otherwise. Here by convention, $a^0 = 1$ even if $a = 0$. Consider the rows in $N_{k; a}$ corresponding to $\{ P_X \}_{X \subseteq [k]}$. 
They form the nonsingular matrix $\trans{1}{0}{a}{1}^{\otimes n}$ 
if the rows and columns are ordered lexicographically for $X, Y \subseteq[k]$.
Therefore $\symrank W_{k, n; a} = \symrank 
\left(\trans{1}{0}{a}{1}^{\otimes n} W_{k, n; a} \right) \le \symrank T(\wmatch_a, k, n)$ and so $\symrank T(\wmatch_a, k, n) = \symrank W_{k, n; a}$.

Note that for $k = 1$, $W_{1, n; a} = \calM_{n;a, 1} = [a, 1, 0, \ldots 0] \in \Sym^n(\bbF^2)$ where $n \ge 1$. Applying Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound} with $b = 1$, we get $\symrank W_{1, n; a} \ge n$ and therefore $\symrank T(\wmatch_a, 1, n) \ge n$ for $n \ge 1$. Now if $\wmatch_a$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness}, $\symrank T(\wmatch_a, k, n) \le q^k$ for $k, n \ge 0$ so that $\symrank T(\wmatch_a, 1, n) \le q$ for $n \ge 0$. 
This contradicts  $\symrank T(\wmatch_a, 1, n) \ge n$ when $n > q$.
Hence $\wmatch_a$ is not expressible as a graph homomorphism function over any field. 

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible}, the proof for
 Theorem~\ref{thm:weighted-Matching-not-expressible-simple}
 carries over to simple graphs.


\begin{theorem}\label{thm:weighted-Matching-not-expressible-simple}
The graph parameter \textsc{\#Weighted-Matching} \emph{($\wmatch_a$)} where $a \in \bbF$ as a function defined on simple graphs is not expressible as a graph homomorphism function over any field $\bbF$.
\end{theorem}

\input{bounded-degree-graphs}

\subsection{Proper edge \texorpdfstring{$d$}{d}-colorings}

Next we show that the graph parameter  \#$d$-\textsc{Edge-Coloring}
($\edgecol_d$) is not expressible as
a GH function over any field of characteristic $0$. Given a graph $G$,
$\edgecol_d(G)$ counts the number of proper edge $d$-colorings in a graph,
 where $d \ge 1$ is the number of colors available.

Clearly, $\edgecol_d$ is a multiplicative graph parameter with $\edgecol(K_0) = 1$. Since $\Char \bbF = 0$, $\bbF$ is infinite. 
Consider $K_1$ as a $1$-labeled graph and the star graph $S_d$
with one internal node labeled by $1$ and $d$ unlabeled external nodes
all connected to node 1, where $d \ge 1$. 
Consider the  connection tensor $T(\edgecol_d, k, n)$ 
restricted to $\{ K_1, S_d \}^n$. For $(G_1, \ldots, G_n) \in \{ K_1, S_d \}^n$,
 if more than one $G_i = S_d$ then the product $G_1 \cdots G_n$ has no
proper edge $d$-coloring because the labeled vertex
has degree $\ge 2d > d$. Then
 it is easy to see that the connection tensor $T(\edgecol_d, k, n)$ restricted to $\{ K_1, S_d \}^n$ has the
 form $\calM_{1, d!} = [1, d!, 0, \ldots, 0] \in \Sym^n(\bbF^2)$,
and $d! \ne 0$ in $\bbF$ as $\Char \bbF = 0$.
Therefore by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound}, $\symrank \calM_{1, d!} \ge n$ for $n \ge 1$. Hence $\symrank T(\edgecol_d, 1, n) \ge n$ for $n \ge 1$.

Now if $\edgecol_d$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness},
% $\symrank T(\edgecol_d, k, n) \le q^k$ for $k, n \ge 0$ so that
 $\symrank T(\edgecol_d, 1, n) \le q$ for $n \ge 0$. This contradicts the upper bound when $n > q$. Hence $\edgecol_d$ is not expressible as a graph homomorphism function over any field $\bbF$ of $\Char \bbF = 0$.

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible},
the proof for
 Theorem~\ref{thm:Edge-Coloring-not-expressible-simple}
 carries over to  simple graphs.
%%%

\begin{theorem}\label{thm:Edge-Coloring-not-expressible-simple}
The graph parameter \#$d$-\textsc{Edge-Coloring} \emph{($\edgecol_d$)} with $d \ge 1$ as a function defined on simple graphs is not expressible as a graph homomorphism function over any field of characteristic $0$.
\end{theorem}


\subsection{Vertex-disjoint cycle covers}

We show that the graph parameter $\vdccover$
(\#\textsc{Vertex-Disjoint-Cycle-Cover})
 which counts the number of vertex disjoint cycle covers in a graph
is not expressible as a GH function over an arbitrary field.
%Here we follow the convention that 
In a multigraph without loop a cycle is
 a vertex disjoint closed path of length at least $2$.
The graph parameter $\vdccover(G) = m \cdot 1 \in {\mathbb F}$, where $m$ is
the number of edge subsets $E'$ that 
form  a vertex disjoint set of cycles that cover all vertices.

%%% not omitted
Clearly, $\vdccover$ is a multiplicative graph parameter with $\vdccover(K_0) = 1$. Next, consider $K_1$ and $K_3$ as $1$-labeled graphs.
Note that $K_3$ is a cycle of 3 vertices.
 It is easy to see that the connection tensor $T(\vdccover, k, n)$ restricted to $\{ K_1, K_3 \}^n$ has the form $\calM_{0, 1} = [0, 1, 0, \ldots, 0] \in \Sym^n(\bbF^2)$ and therefore by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound}, $\symrank \calM_{0, 1} \ge n$ for $n \ge 1$. Hence $\symrank T(\vdccover, 1, n) \ge n$ for $n \ge 1$.

Now if $\vdccover$ were expressible as $\hom(\cdot, H)$ for some weighted graph $H$ with $q = |V(H)|$, then by Theorem \ref{thm:uniform-exponential-rank-boundedness},  $\symrank T(\vdccover, 1, n) \le q$ for $n \ge 0$. This contradicts the upper bound when $n > q$. Hence $\vdccover$ is not expressible as a 
GH function over any field. 

By the same remark for
Theorem~\ref{thm:Perfect-Matching-not-expressible},
the proof for
 Theorem~\ref{thm:Vertex-Disjoint-Cycle-Cover-not-expressible-simple}
 carries over to  simple graphs.
%%%

\begin{theorem}\label{thm:Vertex-Disjoint-Cycle-Cover-not-expressible-simple}
The graph parameter \#\textsc{Vertex-Disjoint-Cycle-Cover} \emph{($\vdccover$)} as a function defined on simple graphs is not expressible as a graph homomorphism function over any field.
\end{theorem}




==> pm-rk-con-ten-GH-article-(cpc-submission)/bibliography.tex <==
\begin{thebibliography}{50}
\bibitem{baxter-6-8}
R. J. Baxter: The Six and Eight-Vertex Models Revisited, Journal of Statistical Physics 116 (2004), 43-66.

\bibitem{Bulatov}
A. A. Bulatov:
The complexity of the counting constraint satisfaction problem. J. ACM 60(5): 34:1-34:41 (2013).

\bibitem{bulatov-dalmu}
A. Bulatov and V. Dalmau:
Towards a dichotomy theorem for the counting constraint satisfaction problem. Inf. Comput. 205(5): 651-678 (2007).

%\bibitem{Bulatov-etal}
%A. Bulatov, M. E. Dyer, L. Ann Goldberg and M. Jalsenius, D. Richerby: The complexity of weighted Boolean \#CSP with mixed signs.
%Theor. Comput. Sci. 410(38-40): 3949-3961 (2009).

\bibitem{Bulatov-Grohe-2005}
A. Bulatov and M. Grohe: The complexity of partition functions. Theor. Comput.
Sci., 348(2): 148-186, 2005.

\bibitem{Cai-Chen-2017}
J.-Y. Cai and X. Chen:
Complexity of Counting CSP with Complex Weights. J. ACM 64(3): 19:1-19:39 (2017).
A preliminary version appeared in Proceedings of the 44th Symposium on Theory of Computing (STOC), 2012, pp. 909-920.

\bibitem{cai-chen-book}
J.-Y. Cai and X. Chen: {\it Complexity Dichotomies for Counting Problems}, Volume 1: Boolean Domain,
 Cambridge University Press, 2017.
\url{https://doi.org/10.1017/9781107477063}
%\href{https://doi.org/10.1017/9781107477063}{https://doi.org/10.1017/9781107477063}

\bibitem{Cai-Chen-Lu-2013}
J.-Y. Cai, X. Chen and P. Lu:
Graph Homomorphisms with Complex Values: A Dichotomy Theorem. SIAM J. Comput. 42(3): 924-1029 (2013).

\bibitem{Cai-Zhiguo-2017}
J.-Y. Cai and Z. Fu: Holographic Algorithm with Matchgates Is Universal for
Planar \#CSP Over Boolean Domain. In Proc. of the 49th Annual ACM SIGACT
Symposium on Theory of Computing (STOC) 2017: 842-855. 
To appear in SIAM Journal on Computing.
Full version available at
\url{https://arxiv.org/abs/1603.07046}
%\href{https://arxiv.org/abs/1603.07046}{https://arxiv.org/abs/1603.07046}

\bibitem{Cai-Fu-Guo-W}
J.-Y. Cai, Z. Fu, H. Guo and T. Williams:
A Holant Dichotomy: Is the FKT Algorithm Universal? FOCS 2015: 1259-1276.

\bibitem{Cai-Govorov-2019}
%J.-Y. Cai, A. G.: Perfect matchings, rank of connection tensors and graph homomorphisms. SODA 2019: 476-495.
J.-Y. Cai and A. Govorov: Perfect matchings, rank of connection tensors and graph homomorphisms, In Proc. of ACM-SIAM Symposium on Discrete Algorithms (SODA) 2019, pp. 476-495.

\bibitem{caiguowilliams13}
J.-Y. Cai, H. Guo and T. Williams: A Complete Dichotomy Rises from the Capture of Vanishing Signatures.
SIAM J. Comput. 45(5): 1671-1728 (2016).
A preliminary version in STOC, pages 635-644. ACM, 2013.

%\bibitem{cgw-focs-2014}
%J.-Y. Cai, H. Guo and T. Williams:
%The Complexity of Counting Edge Colorings and a Dichotomy for Some Higher Domain Holant Problems.
%Research in the Mathematical Sciences,
%(2016) 3:18.
%A preliminary version in FOCS 2014: 601-610.

\bibitem{Cai-Lu-2007}
J.-Y. Cai and P. Lu:
Holographic algorithms: From art to science. J. Comput. Syst. Sci. 77(1): 41-61 (2011).
%Jin-Yi Cai, Pinyan Lu: Holographic algorithms: from art to science. STOC 2007: 401-410

%\bibitem{clx-focs-2008}
%J.-Y. Cai, P. Lu and M. Xia:
%Holographic Algorithms by Fibonacci Gates and Holographic Reductions for Hardness. FOCS 2008: 644-653.

\bibitem{clx-holant}
J.-Y. Cai, P. Lu and M. Xia:
Holant problems and counting CSP. STOC 2009: 715-724.

%\bibitem{CLX11a}
%J.-Y. Cai, P. Lu and M. Xia:
%Dichotomy for Holant* Problems of Boolean Domain. SODA 2011: 1714-1728.

\bibitem{Cohn-book}
P. M. Cohn, {\it Algebra}, Volume 3, John Wiley \& Sons, 2nd Edition, 1991. %Wiley

\bibitem{Comon-Golub-Lim-Mourrain-2008}
P. Comon, G. Golub, L.-H. Lim and B. Mourrain: Symmetric tensors and symmetric tensor rank, SIAM J. Matrix Anal. Appl., Vol. 30, No 3. (2008), pp. 1254-1279.

%\bibitem{Dyer-Goldberg-Jerrum}
%M. E. Dyer, L. A. Goldberg and M. Jerrum:
%The Complexity of Weighted Boolean \#CSP. SIAM J. Comput. 38(5): 1970-1986 (2009).

\bibitem{Dyer-Greenhill-2000}
M. E. Dyer and C. S. Greenhill:
The complexity of counting graph homomorphisms. Random Struct. Algorithms 17(3-4): 260-289 (2000).

\bibitem{Dyer-Greenhill-corrig-2004}
M. E. Dyer and C. S. Greenhill:
Corrigendum: The complexity of counting graph homomorphisms. Random Struct. Algorithms 25(3): 346-352 (2004).

\bibitem{Dyer-Richerby}
M. E. Dyer and D. Richerby:
An Effective Dichotomy for the Counting Constraint Satisfaction Problem. SIAM J. Comput. 42(3): 1245-1274 (2013).

\bibitem{Freedman-Lovasz-Schrijver-2007}
M. Freedman,  L. Lov\'asz, and A. Schrijver: Reflection positivity, rank connectivity, and homomorphism of graphs, Journal of AMS 20 (2007) 37-51. %M. H. Freedman

\bibitem{Goldberg-et-al-2010}
L. A. Goldberg, M. Grohe, M. Jerrum and M. Thurley: A complexity dichotomy for
partition functions with mixed signs, SIAM J. Comput., 39 (2010), pp. 3336-3402.

\bibitem{GRS}
 C. G\'{o}mez, M. Ruiz-Altaba and G. Sierra: Quantum Groups in Two-Dimensional Physics. Cambridge University
Press, Cambridge (1996).

\bibitem{Grohe-Thurley-2011}
M. Grohe and M. Thurley: Counting homomorphisms and partition functions. In Grohe, M. and Makowsky, J., editors,
Model Theoretic Methods in Finite Combinatorics, Contemporary Mathematics, Vol. 558, pages 243-292. American Mathematical Society (2011).

\bibitem{glva-2013}
H. Guo, P. Lu and L. G. Valiant:
The Complexity of Symmetric Boolean Parity Holant Problems. SIAM J. Comput. 42(1): 324-356 (2013).

\bibitem{GH-book}
P. Hell and J. Ne\v{s}et\v{r}il:
{\it Graphs and Homomorphisms},
(Oxford Lecture Series in Mathematics and Its Applications)
Oxford University Press; 1 edition (September 30, 2004).
% ISBN-13: 978-0198528173.

%\bibitem{HL12}
%S. Huang and P. Lu:
%A Dichotomy for Real Weighted Holant Problems. Computational Complexity 25(1): 255-304 (2016).

%\bibitem{Jacobson-book}
%N. Jacobson: {\it Basic Algebra II}, Dover Publications, 2nd Edition, 2012.

\bibitem{Kasteleyn-1961}
P. W. Kasteleyn: The Statistics of Dimers on a Lattice, Physica 27 (1961) 1209-1225.

\bibitem{Kasteleyn-1967}
P. W. Kasteleyn: Graph Theory and Crystal Physics. In Graph Theory and Theoretical
Physics, (F. Harary, ed.), Academic Press, London, 43-110 (1967).

\bibitem{Lovasz-1967}
L. Lov\'asz: Operations with structures, Acta Math. Hungar., 18 (1967), pp. 321-328.

\bibitem{Lovasz-Schrijver-2008}
L. Lov\'asz and A. Schriver: Graph parameters and semigroup functions, European Journal of Combinatorics 29 (2008) 987-1002.

\bibitem{B-Szegedy}
B. Szegedy: Edge  coloring  models  and  reflection  positivity,
J. Amer. Math. Soc., 20 (2007), no. 4, 969-988.

\bibitem{Tempereley-Fisher-1961}
H. N. V. Temperley and M. E. Fisher: Dimer Problem in Statistical Mechanics - an Exact
Result. Philosophical Magazine 6: 1061-1063 (1961).

\bibitem{Thurley-2009}
M. Thurley: The complexity of partition functions. PhD Thesis,
Humboldt Universitat zu Berlin, 2009.

\bibitem{Valiant-2004}
L. G. Valiant: Holographic Algorithms, SIAM J. Comput., 37(5) (2008) 1565-1594.
A preliminary version appeared in FOCS 2004: 306-315.

\bibitem{Val06}
L. G. Valiant: Accidental algorithms, FOCS 2006: 509-517.
%%%
\end{thebibliography}


==> pm-rk-con-ten-GH-article-(cpc-submission)/bounded-degree-graphs.tex <==
\subsection{Bounded degree graphs}\label{sec:bonded-deg-graphs}

Fix any $d \ge 2$.
A degree-$d$ bounded graph is a graph with maximum degree at most $d$.
%A graph whose vertex degrees are bounded by $d$ is called a $d$-degree (or degree-$d$) bounded graph. 
In this subsection, we investigate the expressibility of the graph parameter \textsc{\#Weighted-Matching$_a$} ($\wmatch_a$) 
%defined in Section~\ref{sec:Weighted-Matchings} 
as a GH function on bounded degree graphs.  More precisely, we are interested when $\wmatch_a$ is expressible as a $\hom(\cdot, H)$ with $|V(H)| = q$ on degree-$d$ bounded graphs. 
For convenience, we temporarily allow vertex weights to be $0$,
and it will be addressed later.

%{\color{red} \sout{For convenience, we temporarily allow vertex weights to be $0$,
%(in the graphs $H$ of the GH function $f_H = \hom(\cdot, H)$):
%(they can be freely removed resulting in a graph $H'$ that has no more vertices that the original graph $H$
%so under this relaxation the inexpressibility statements transfer to the original model with no $0$-weighted vertex,
%and we will also deal with $0$-weighted vertices in the expressibility statements)}}
%{\color{red} REMOVE: For convenience, in this section, we also allow the vertex weights $\alpha_H(i)$ to be $0$ in the target graph $H$ of a GH function $f_H = \hom(\cdot, H)$ (see Remark~\ref{rem:GH-0-weights}), we can always remove them (with the incident edges) from $H$ with no impact on it.} {\color{red} However, I bring this issue back later on, red comments clarify it, they are optional.}

Given a graph $G$ (possibly with multiple edges but no loops), 
let $G'$ be the vertex-edge incidence graph of $G$.
%the bipartite graph obtained by placing a vertex in the middle of each edge of $G$. This is the vertex-edge incidence graph of $G$.
The vertex set $V(G')$
consists of the original vertices from $V(G)$ on the LHS 
and the edges $E(G)$
on the RHS. 
Let $H$ be the weighted graph specified by 
vertex weights $(\alpha_1, \ldots, \alpha_q) \in \bbF^q$ and a 
symmetric matrix $B = (\beta_{i j}) \in \bbF^{q \times q}$ for edge
weights, then for any $G$
\begin{equation}\label{eqn:hom-to-bip-holant}
\hom(G, H) = \Holant(G'; \{ \sum_{i = 1}^q \alpha_i e_{q, i}^{\otimes n} \}_{n \ge 0} \mid B),
\end{equation}
where $\{ e_{q, i} \}_{i = 1}^q \in \bbF^q$ 
has a single 1 at the $i$th position and 0 elsewhere.
%is the canonical (row) basis  of $\bbF^q$
%($e_{q, i}$ has a single 1 at the $i$-th position and 0 elsewhere). 
Here $\hom(G, H)$ is expressed in (\ref{eqn:hom-to-bip-holant})
 as a domain-$q$ Holant sum on $G'$: any LHS vertex of $G'$ of degree $n$ is assigned the signature $\sum_{i = 1}^q \alpha_i e_{q, i}^{\otimes n}$ (which takes value $\alpha_i$ if all
incident edges have value $i \in [q]$, and 0 otherwise),
and any RHS vertex of $G'$ (an edge of $G$)
is assigned the symmetric binary signature specified by $B$. %(When $q = 0$, we define a Holant sum (not necessarily bipartite) as $1$ if the input graph is the empty graph and $0$ otherwise.)

First, we show that for any $a \in \bbF$, if
 $\wmatch_a$ is 
expressible as $\hom(\cdot, H)$ with $|V(H)| = q$ on degree-$d$ 
bounded \emph{simple} graphs over any field $\bbF$, then $q \ge d$.
 Recall the proof
% of the inexpressiblity $\wmatch_a$ as a GH function 
from Section~\ref{sec:Weighted-Matchings}. This time we restrict the connection tensor $T(\wmatch_a, 1, d)$ (for $k = 1$) to the $1$-labeled graphs
$P_\emptyset$ and $P_{[1]}$, which are just $K_1$ and $K_2$ without
the label. 
%consider $T(\wmatch_a, 1, d)_{|\{ K_1, K_2 \}^d}$. 
The product of $d$ labeled graphs from $\{P_\emptyset, P_{[1]}\}$
having $\ell$ copies of $P_{[1]}$
is the star graph $S_\ell$ with  one internal node labeled by $1$ and 
$\ell$ external unlabeled nodes. 
%In this way, in the construction $T(\wmatch_a, 1, d)_{|\{ K_1, K_2 \}^d}$ 
%only the graphs $S_\ell, \, 0 \le \ell \le d$ are used as arguments. 
All these are degree-$d$ bounded simple graphs. 
Note that $T(\wmatch_a, 1, d)_{|\{ P_\emptyset, P_{[1]} \}^d} 
= \trans{1}{0}{a}{1}^{\otimes d} W_{1, d; a}$. Therefore $\symrank \left( T(\wmatch_a, 1, d)_{|\{ P_\emptyset, P_{[1]} \}^d} \right) = \symrank \left(\trans{1}{0}{a}{1}^{\otimes d} W_{1, d; a}\right) = \symrank W_{1, d; a} \ge d$, the last step is by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound}. On the other hand, if $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = q$ on degree-$d$ bounded \emph{simple} graphs, then arguing similarly to the proof of Theorem~\ref{thm:uniform-exponential-rank-boundedness} but restricting the domain of the arguments $G_i, \, 1 \le i \le d$ in (\ref{eqn:partial-hom-mult})
% (replace $n \to d$) 
to $\{P_\emptyset, P_{[1]} \}$, we have 
$\symrank \left( T(\wmatch_a, 1, d)_{|\{ P_\emptyset, P_{[1]} \}^d} \right) \le q$ so $d \le q$.
Then clearly this bound also holds if we do not allow $0$-weighted vertices.
%Thus in order for $\wmatch_a$ to be expressible as $\hom(\cdot, H)$ with $|V(H)| = q$ on degree-$d$ bounded graphs, we must have $q \ge d$, so we will assume it.


%Now we assume $q = d$.
%
%Let $d = 0$. Note that degree-$0$ bounded graphs are precisely the graphs consisting of isolated points (also they are all simple). For any such graph $G$, $\wmatch_a(G) = a^{|V(G)|}$. Then $\wmatch_a(\cdot) = \hom(\cdot, H)$ on degree-$0$ bounded graphs, where $H$ is a weighted graph on one vertex specified by $\alpha_1 = a$ and $\beta_{1 1} = 1$. Moreover, if $a = 0$, then we can instead take $H = \emptyset$ so $q = 0$ is sufficient. If $a \ne 0$, then $H = \emptyset$ does not work, so $q = 1$ is the least such possible number.
%
%Henceforth, let $d \ge 1$. 
%
%{\color{red} (Assume $d \ge 2$ here, cases $d = 0, 1$ are not interesting.)}
%
%{\color{red} 

%To express  $\wmatch_a(\cdot) = \hom(\cdot, H)$ for a weighted graph $H$
%with $|V(H)| = d$ we temporarily allow the graphs $H$ to have 
%vertices with weight $0$.
%We will deal with them at some point. (need to say this)}

%Let $d \ge 2$.
%Consider the linear system $A x = \vec b$ with the extended matrix
%\begin{equation}\label{eqn:wm-vand-sys-for-d-deg-bounded-graphs}
%\widehat A = [A \mid \vec b] =
%\left[
%\begin{array}{cccc|c}
%a_1^d & a_2^d & \ldots & a_d^d & a \\
%a_1^{d-1} & a_2^{d-1} & \ldots & a_d^{d-1} & 1\\
%\vdots & \vdots & \ddots & \vdots & \vdots \\
%a_1 & a_2 & \ldots & a_d & 0 \\
%1 & 1  & \ldots  & 1 & 0
%\end{array}
%\right].
%\end{equation}
%Suppose it has a solution $x_i = \alpha_i \in \bbF, \, 1 \le i \le d$. Then $\calM_{d; a, 1} = \sum_{i = 1}^d \alpha_i (a_i, 1)^{\otimes d}$.
%(By Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound},
%all $\alpha_i \not = 0$.)
% (so $q \ge d$ by Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound-short};
%we have shown this is a necessary condition for expressibility,
%and we have assumed $q \ge d$.)

Now let $\bbF$ be infinite.
By the remark after 
Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound},
 if we are not
in the exceptional case (\ref{case:exception}) (we put $n = d$), then
for some
$a_i, \alpha_i \in \bbF$  we have
 $\calM_{m; a, 1} = \sum_{i = 1}^d \alpha_i (1, a_i)^{\otimes m}$,
for every $0 \le m \le d$.
% the equations of this system corresponding to 
%rows $d-n$ to $d$ of matrix~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}) are equivalent to $\calM_{n; a, 1} = \sum_{i = 1}^d \alpha_i (a_i, 1)^{\otimes n}$.
 Let $T \in \bbF^{d \times 2}$ be the matrix 
whose $1$st and $2$nd columns 
are $(1, 1, \ldots, 1)^{\tt T}$ and $(a_1, a_2, \ldots, a_d)^{\tt T}$
respectively. Then $e_{d, i} T = (1, a_i)$.
Define the symmetric matrix $B = (\beta_{i j}) =
 T  T^{\tt T} \in \bbF^{d \times d}$. Now let $H$ be a weighted graph on $d$ vertices specified by $(\alpha_1, \ldots, \alpha_d) \in \bbF^d$ and $B = (\beta_{i j}) \in \bbF^{d \times d}$. Then for any degree-$d$ bounded graph $G$ we have the following equality chain:
\begingroup
\allowdisplaybreaks
\begin{align*}
\wmatch_a(G) &= \Holant(G; \{ \calM_{m; a, 1} \}_{0 \le m \le d}) = \Holant(G'; \{ \calM_{m; a, 1} \}_{0 \le m \le d} \mid (=_2) ) \\
&= \Holant(G'; \{ \sum_{i = 1}^d \alpha_i (1, a_i)^{\otimes m} \}_{0 \le m \le d} \mid (=_2) ) = \Holant(G'; \{  \sum_{i = 1}^d \alpha_i (e_{d, i} T )^{\otimes m} \}_{0 \le m \le d} \mid (=_2) ) \\
&= \Holant(G'; \{ \sum_{i = 1}^d \alpha_i e_{d, i}^{\otimes m} T^{\otimes m} \}_{0 \le m \le d} \mid (=_2) ) = \Holant(G'; \{ \sum_{i = 1}^d \alpha_i e_{d, i}^{\otimes m} \}_{0 \le m \le d} \mid T^{\otimes 2} (=_2) ).
% \\
%&= \Holant(G'; \{ \sum_{i = 1}^d \alpha_i e_{d, i}^{\otimes n} \}_{0 \le n \le d} \mid T I_{d, 2} T^{\tt T}) = \Holant(G'; \{ \sum_{i = 1}^d \alpha_i e_{d, i}^{\otimes n} \}_{0 \le n \le d} \mid B) = \hom(G, H).
\end{align*}
\endgroup
where the last equation moving $T^{\otimes n}$ from the left-hand side of
the Holant problem to $T^{\otimes 2}$ in the right-hand side,
is called a holographic transformation~\cite{Valiant-2004, cai-chen-book} (the argument works for arbitrary fields).
This follows from the associativity of the operation of tensor 
contraction. 
%(\sout{in a tensor network} is an ambiguous notion, better not to use it) (over commutative rings).) (must mention this)}
%Here all equalities follow from  Holant theory.
% but they can be shown 
%by the reader. 
The {\sc Equality} function  $(=_2)$ is transformed
% the binary equality function,
to $T^{\otimes 2} (=_2)$, which has the matrix form $T T^{\tt T}
= B$. Hence this is precisely the function $\hom(G, H)$.
%(We temporarily allowed $0$ vertex weights;
%but in fact by the lower bound $q \ge d$ no  $0$ weighted
%vertex exists, since otherwise by removing   $0$ weighted vertices we would 
%have $\wmatch_a(\cdot) = \hom(\cdot, H')$ with fewer vetices.
We have temporarily allowed $0$-weighted vertices;
but in fact by the lower bound $q \ge d$ no $0$-weighted
vertex exists, since otherwise by removing  $0$-weighted vertices we would 
have $\wmatch_a(\cdot) = \hom(\cdot, H')$ with fewer vertices.

The inexpressibility with $|V(H)| = 2$ for the exceptional case
(\ref{case:exception}) holds even for simple graphs, by considering
paths of $0$, $1$ or $2$ edges.
Also, in this case it can be easily shown that
$\wmatch_a = \pmatch$ is expressible as $\hom(\cdot, H)$ where $|V(H)| = 3$:
this can be done similarly to the expressibility proof above via a holographic transformation
(then $H$ cannot have $0$-weighted vertices).

%{\color{red} \sout{Also, in this exceptional case (\ref{case:exception}) 
%it can be easily shown that $\wmatch_a$ is expressible
%as $\hom(\cdot, H)$ where $|V(H)| = 3$
%(then $H$ cannot have $0$-weighted vertices);
%this can be done similarly to the expressibilty proof above via a holagraphic transformation
%but with $d + 1 = 3$ in place of $d = 2$,
%in particular, we show that by choosing $\alpha_1, \alpha_2, \alpha_3 \in \bbF$ to be pairwise different
%($\bbF$ is infinite),
%for some $\alpha_i \in \bbF$ we have $\calM_{m; 0, 1} = \sum_{i = 1}^3 \alpha_i (1, a_i)^{\otimes m}$,
%for $0 \le m \le 3$.}}

%{\color{red} (need to say this, we disallow $0$ vertex weights)
%
%However, $H$ might contain vertices the with weight $0$.
%After we remove all such vertices with the incident edges (and loops) from $H$, get a graph $H'$ with $|V(H')| \le |V(H)| = q$.
%Note that $|V(H')| \ge d$ by the inexpressibility argument (as $|(V(H')| < d$ leads to a contradiction).
%}

%As shown in Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound},
%the system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}) has a solution
%for infinite fields (with one exception, which is easily handled separately).
This proves Theorem~\ref{thm:wm-as-GH-for-deg-bounded-graphs}.

\begin{theorem}\label{thm:wm-as-GH-for-deg-bounded-graphs}
Let $\bbF$ be a field and $d \ge 2$.
Then for the graph parameter \textsc{\#Weighted-Matching$_a$} \emph{($\wmatch_a$)} where $a \in \bbF$
as a function defined on degree-$d$ bounded graphs the following hold:
\begin{enumerate}
\item $\wmatch_a$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$ even on degree-$d$ bounded \emph{simple} graphs.
\item If $\bbF$ is infinite, then $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$, 
with one exception
(\ref{case:exception})
%unless $a = 0$, $d = 2$ and  $\Char \bbF = 2$
in which case the minimal value for $|V(H)|$ is $3$.
%{\color{red} and the inexpressibility with $|V(H)| = d \le 2$ holds even degree-$d$ bounded \emph{simple} graphs. (add)}
% $q$ that $\wmatch_a = \pmatch$ is not expressible as
%$\hom(\cdot, H)$ with $|V(H)| = 2$ by is expressible with $|V(H)| = 3$.
%on degree-$d$ bounded \emph{simple} graphs
%but is expressible as $\hom(\cdot, H)$ with $|V(H)| = d + 1 = 3$.
\end{enumerate}
\end{theorem}
%The inexpressibility with $|V(H)| = 2$ for the exceptional case
%(\ref{case:exception}) holds even for simple graphs, by considering
%paths of $0$, $1$ or $2$ edges. 
%(moved this sentence before the theorem)
Note that  \textsc{\#Perfect-Matching} \emph{($\pmatch$)} is just
the special case  $a = 0$. Hence Theorem~\ref{thm:wm-as-GH-for-deg-bounded-graphs} also holds for \emph{$\pmatch$}.
%which proves Theorem~\ref{thm:pm-as-GH-for-deg-bounded-graphs-short}.



%It follows that for a weighted graph $H$ with $|V(H)|=d$,
%we have  $\wmatch_a(\cdot) = \hom(\cdot, H)$ 
%on degree-$d$ bounded graphs.
%%{\color{red} with ($|V(H')| \le q$)},
%% {\color{red} (with all entries nonzero)}. We can show that
%%with all entries nonzero. {\color{red} \sout{We can show that} (to be gone because we prove it now)}
%

% note that in the $3$nd line we change the domain from $2$ to $q$, we can freely do it because of the associativity of tensor product; the last equality is by~(\ref{eqn:hom-to-bip-holant}). 

%%%---
%{\color{red} (need to edit what's below, note that we consider cases 1, 2 before we formulate Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound})}
%{\color{red} (Case $d = 1$, not needed, REMOVE)
%
%Assume $d = 1$. Note that $q = 2$ is sufficient for any $a \in \bbF$, which can be seen by taking $b_1 = 0, \, b_2 = 1$ in~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}). Then $A$ is nondegenegate so the system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}) has a solution. Now let $q = 1$. In this case the system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}) has a solution iff $a \ne 0$, in which case $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = 1$ on degree-$1$ bounded graphs. More precisely, we take $\alpha_1 = a$ and $\beta_{1 1} = 1 / a^2$ in this case. Note that degree-$1$ bounded graphs are precisely the graphs that are disjoint unions of edges and isolated points (also they are all simple). Let $a = 0$. Suppose $\wmatch_0(\cdot) = \hom(\cdot, H)$ where $|V(H)| = 1$ on degree-$1$ bounded graphs. Computing both sides at the $1$ degree-bounded graphs $K_1, K_2$, we get $\alpha_1 = 0,\, \alpha_1^2 \beta_{1 1} = 1$ correspondingly, which is impossible. Thus $q = 1$ is sufficient iff $a = 0$.
%
%}
%
%{\color{red} (Case $d \ge 2$)}
%{\color{red} (old degree upper bound argment, can be commented out)}
%
%{\color{blue}
%From now on, let $d \ge 2$. We show how to derive an GH expressiblity of $\wmatch_a$ under additional assumptions on $\bbF$. (In fact, our arguments below work for the first case also works for $d = 1$.)
%\begin{enumerate}
%\item Assume $\bbF$ is infinite. We show how to achieve $q = d + 1$. Arguing exactly as in the proof of Case~\ref{item:bbF-inf} of Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound-old}, we can choose $b_i \in \bbF$ to be pairwise distinct to guarantee the existence (and uniqueness) of a solution to the system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}). This results in the desired graph $H$ on $d + 1$ vertices. 
%%{\color{red}REMOVE: [From Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound} we infer that at most one $\alpha_i$ can be zero. Removing the $0$ weight vertices with all the incident edges we may assume that $H$ is a graph on either $d$ or $d + 1$ vertices (with nonzero vertex weights). 
%%We show that in the first case we can make all $d + 1$ nonzero vertex weights as follows.}
%%
%%{\color{red} REMOVE: [New argument: If $H$ has $d$ vertices, then choose a vertex $u \in V(H)$ such that $t_0 = \alpha_H(u) \ne 0$. Note that we can find $t_1, t_2 \in \bbF \setminus \{ 0 \}$ such that $t_1 + t_2 = t_0$: if $t_0 \ne 1$, take $t_1 = 1, \, t_2 = t_0 - 1$; else $t_0 = 1$, take $t_1 \in \bbF$ such that $t_1 \ne 0, 1$ ($\bbF$ is infinite) and $t_2 = 1 - t_1$. Now replace the vertex $u$ by two copies retaining all the incident edges to the other vertices from each copy to the other vertices with the original edge weights, assign these two vertices weights $t_1, t_2$. It is easy to see that $\hom(\cdot, H)$ does not change by moving to the new graph. Finally, the new graph contains $d + 1$ vertices of nonzero weight.]}
%%
%%{\color{red} REMOVE: [Old argument: To guarantee that all the $d + 1$ weights of $H$ are nonzero, note that by Cramer's rule we can compute the solution $\alpha_i, 1 \le i \le d + 1$. Using the substitution trick from Remark~\ref{rem:wm-sym-rk-upper-bound}, we conclude that in addition to the pairwise distinctness of $b_i$ we only need to have $\sum_{1 \le j \le d + 1, j \ne i} b_i \ne a$ for $1 \le i \le d + 1$. Clearly, the polynomial $\prod_{1 \le i < j \le d + 1} (x_i - x_j) \prod_{1 \le i \le d + 1} (\sum_{1 \le j \le d + 1, j \ne i} x_i - a)$ is nonzero and therefore there is a point $(x_1^*, \ldots, x_{d + 1}^*)$ at which it does not vanish. It suffices to take $b_i = x_i^*, \, 1 \le i \le d + 1$, then all desired conditions are satisfied which implies that all $\alpha_i \ne 0$.]}
%
%\item Assume $\Char \bbF = 0$. We show how to achieve $q = d$. Arguing exactly as in the proof of Case~\ref{item:bbF-char=0} of Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound-old}, we have a decomposition $\calM_{d; a, 1} = \sum_{i = 1}^d \lambda_i [c_i, 1]^{\otimes d}$ for some $\lambda_i \in \bbF$, as long as $c_i \in \bbF$ are pairwise distinct and $a \sum_{i = 1}^d c_i = 1$. Let us show how to make all $c_i \ne 0$ as well. We modify the argument from the proof of Case~\ref{item:bbF-char=0} of Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound}. Note that $d = q \ge 2$. Since $\Char \bbF = 0$, we have $d \ne 0$ in $\bbF$. Let $c_i = a / d + s i$ for $1 \le i \le d - 1$ and $c_d = a / d - s d (d - 1) / 2$ where $s \in \bbF \setminus \{ 0 \}$ is yet to be chosen. Then $\sum_{i = 1}^d c_i = a$. Also $\Char \bbF = 0$ and $s \ne 0$ guarantees that $c_i$ are pairwise distinct. Consider the polynomial
%\[
%p(t) = \left( \prod_{i = 1}^{d - 1} (a / d + t i) \right) (a / d - t d (d - 1)) \, t,
%\]
%where $t$ is an indeterminate. By $\Char \bbF = 0$ and $d \ge 2$, all of its $d + 1$ factors are of degree exactly $1$. Then $\deg p(t) = d + 1 \ge 3$. In particular, $p(t)$ is a nonzero polynomial. Since $\bbF$ is clearly infinite, there exists $t^* \in \bbF$ such that $p(t^*) \ne 0$. Take $s = t^*$. Then $s \in \bbF \setminus \{ 0 \}$ and all $c_i \neq 0$. Now we can write $\calM_{d; a, 1} = \sum_{i = 1}^d \lambda_i [c_i, 1]^{\otimes d} = \sum_{i = 1}^d \lambda_i c_i^d [1, 1 / c_i]^{\otimes d}$, so by taking $b_i = 1 / c_i$ we guarantee the existence of a solution to the system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}). Namely, we can put $x_i = \alpha_i = \lambda_i c_i^d, \, 1 \le i \le d$. This results in the desired graph $H$ on $d$ vertices. From Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound} we infer that $\lambda_i \ne 0$ but $c_i \ne 0$ so $\alpha_i \ne 0$. Then all vertices of $H$ have nonzero weight. (Alternatively we can say that $H$ cannot have $< q$ nonzero vertex weights.)
%\end{enumerate}
%
%Summing up, we have the following result.
%\begin{theorem}\label{thm:wm-as-GH-for-deg-bounded-graphs-old}
%Let $\bbF$ be a field and $d \ge 2$. Then for the graph parameter \textsc{\#Weighted-Matching$_a$} \emph{($\wmatch_a$)} where $a \in \bbF$ as a function defined on degree-$d$ bounded graphs the following hold:
%\begin{enumerate}
%\item $\wmatch_a$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$  even on degree-$d$ bounded \emph{simple} graphs.
%\item If $\bbF$ is infinite, then $\wmatch_a$ is 
%expressible as $\hom(\cdot, H)$ with $|V(H)| = d \text{ or } d + 1$.
%\item If $\Char \bbF = 0$, then $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$.
%\end{enumerate}
%\end{theorem}
%}
%
%%%%--------
%{\color{red} (better argument, need to revise the text)}
%
%Assume $\bbF$ is infinite.
%We show how to achieve $q = d$ with one exceptional case.
%Arguing exactly as in the proof of (but preceeding) Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound},
%we have a decomposition $\calM_{d; a, 1} = \sum_{i = 1}^d \lambda_i [c_i, 1]^{\otimes d}$
%for some $\lambda_i \in \bbF$,
%as long as $c_i \in \bbF$ are pairwise distinct
%and $\sum_{i = 1}^d c_i = a$.
%Let us show how to additionally make all $c_i \ne 0$.
%We modify the argument from the proof of Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound}.
%Recall that we assume $d \ge 2$. 
%%We let $c_n = a / b - \sum_{i = 1}^{n - 1} c_i$.
%Consider the polynomial
%\[
%p(x_1, \ldots, x_{d - 1}) = \Big( \prod_{1 \le i < j \le d - 1} (x_j - x_i) \Big) \Big( \prod_{1 \le i \le d - 1} (a - \sum_{j = 1}^{d - 1} x_j - x_i) \Big) \Big( \prod_{1 \le i \le d - 1} x_i \Big) \Big(a - \sum_{i = 1}^{n - 1} x_i \Big).
%\]
%Note that $p(x_1, \ldots, x_{d - 1}) \ne 0$ (is a non-zero polynomial) unless $\Char \bbF = 2$, $d = 2$ and $a = 0$
%in which case indeed $p(x_1, \ldots, x_{d - 1}) = 0$.
%
%\begin{enumerate}
%\item Suppose the latter is not the case.
%Since $\bbF$ is infinite and $p(x_1, \ldots, x_{d - 1}) \ne 0$, for some $c_1^*, \ldots, c_{d - 1}^* \in \bbF$,
%we have $p(c_1^*, \ldots, c_{d - 1}^*) \ne 0$.
%Setting $c_i = c_i^*$ for $1 \le i \le d - 1$,
%and $c_d = a - \sum_{i = 1}^{d - 1} c_i^*$,
%we infer that all $c_i \ne 0$ and are pairwise distinct,
%and $\sum_{i = 1}^n c_i = a / b$.
%Now we can write $\calM_{d; a, 1} = \sum_{i = 1}^d \lambda_i [c_i, 1]^{\otimes d} = \sum_{i = 1}^d \lambda_i c_i^d [1, 1 / c_i]^{\otimes d}$,
%so by taking $b_i = 1 / c_i$
%we guarantee the existence of a solution to the system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs})
%Namely, we can put $x_i = \alpha_i = \lambda_i c_i^d, \, 1 \le i \le d$.
%This results in the desired graph $H$ on $d$ vertices.
%From Lemma~\ref{lem:weighted-matchings-tensor-rank-lower-bound}
%we infer that all $\lambda_i \ne 0$ but $c_i \ne 0$ so $\alpha_i \ne 0$.
%Then all vertices of $H$ have nonzero weights.
%(Alternatively we can say that $H$ cannot have zero vertex weights.)
%
%\item Now let $\Char \bbF = 2$, $n = 2$ and $a = 0$.
%We show first how to achieve $q = 3$
%and then that achieving $q = 2$ is impossible.
%Again, we argue exactly as in the proof of (but preceeding) Lemma~\ref{lem:weighted-matchings-tensor-rank-upper-bound}
%for the corresponding case.
%%we have a decomposition $\calM_{d; a, 1} = \sum_{i = 1}^d \lambda_i [c_i, 1]^{\otimes d}$
%Because $\bbF$ is infinite we can choose $b_i \in \bbF$ ($b_1, b_2, b_3$) to be pairwise distinct.
%%to guarantee the existence (and uniqueness) of a solution to system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}).
%Then the matrix $A$ from system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}) is a nondegenerate $3 \times 3$ Vandermonde matrix.
%It follows that system~(\ref{eqn:wm-vand-sys-for-d-deg-bounded-graphs}) (with $q = 3$)
%has a (unique) solution $x_i = \alpha_i, \, 1 \le i \le 3$ ($x_1 = \alpha_1,\, x_2 = \alpha_2, x_3 = \alpha_3$).
%This results in a graph $H$ on $q = 3$ vertices.
%We still may have some vertices with weight $0$.
%Notice that $q' = |V(H')| \ge 2$ as $d = 2$
%so there can be at most one vertex with weight $0$.
%The argument below guarantees that
%all these vertices have a nonzero weights so $H = H'$.
%Thus all vertices of $H$ have nonzero weights.
%
%{\color{red} must include it too, not that hard, certainly can be compressed. use $B_2$ instead of $B$?}
%
%Now we show that it is not possible to achieve $q = 2$.
%Suppose otherwise.
%Let $H$ be the graph on $2$ vertices with a vertex weight
%nowhere zero tuple $(\alpha_1, \alpha_2) \in \bbF^2$
%and an edge weight matrix $B = \twobytwopmatrix{\beta_{1 1}}{\beta_{1 2}}{\beta_{2 1}}{\beta_{2 2}} \in \bbF^{2 \times 2}$ ($\beta_{1 2} = \beta_{2 1}$)
%that expresses $\wmatch_a = \pmatch$ on degree-$2$ bounded graphs.
%In other words, $\hom(G, H) = \pmatch(G)$ for any degree $2$-bounded graphs $G$.
%Let $D = \diag(\alpha_1, \alpha_2)$ and let $\lambda_1, \lambda_2 \in \overline \bbF$ (algebraic closure of $\bbF$)
%be the eigenvalues of $D B$.
%Then $D B = S J S^{-1}$ for some nondegenerate $S \in \overline \bbF^{2 \times 2}$,
%and its JNF $J = \twobytwopmatrix{\lambda_1}{s}{0}{\lambda_2}$ where $s \in \{0, 1\}$.
%Consider the cycle $C_t$ of $t$ vertices where $t \ge 1$.
%Besides, $\hom(C_t, H) = \tr (D B)^t = \lambda_1^t + \lambda_2^t$ for $t \ge 1$.
%Note that each $C_t$ is a degree-$2$ bounded graph for $t \ge 3$.
%Substituting $t = 3, 4$ and using the fact that
%$\pmatch(C_3) = 0$, $\pmatch(C_4) = 2 = 0$ (by $\Char \bbF = 2$)
%we get $\lambda_1^t + \lambda_2^t = 0$
%so $\lambda_1^t = -\lambda_2^t = \lambda_2^t$ (by $\Char \bbF = 2$) for $t = 3, 4$.
%Multiplying the previous equalities for $t = 3, 4$ and then moving RHS to LHS,
%we get $\lambda_1^3 \lambda_2^3 (\lambda_1 - \lambda_2) = 0$.
%Then if $\lambda_1 = 0$ iff $\lambda_2 = 0$ so in any case $\lambda_1 = \lambda_2$.
%It follows that $(D B)^2 = S J^2 S^{-1} = S I_2 S^{-1} = I_2$ (recall that $\Char \bbF = 2$).
%(So $(D B)^{2 r} = I_2$ for $r \ge 1$).
%Next, we consider the graph path $P_t$ where $t \ge 1$.
%Note that $\hom(P_t, H) = (1, 1) (D B)^t (1, 1)^T$.
%It easy to see that $\hom(P_t, H) = (1, 1) (D B)^t D (1, 1)^T$ for $t \ge 1$.
%Since $\pmatch(P_2) = 0$, we have $0 = \hom(P_2, H) = (1, 1) (D B)^2 D (1, 1)^T = (1, 1) I_2 D (1, 1)^T = \alpha_1 + \alpha_2$,
%so $\alpha_2 = -\alpha_1 = \alpha_1$ and therefore $D = \alpha_1 I_2$
%Next, since $\pmatch(P_1) = 1$,
%we have $1 = \hom(P_1, H) = (1, 1) D B D (1, 1)^T = \alpha_1^2 (1, 1) B (1, 1)^T = \alpha_1^2 (\beta_{1 1} + \beta_{1 2} + \beta_{2 1} + \beta_{2 2}) = \alpha_1^2 (\tr B + \beta_{1 2} + \beta_{1 2}) = \alpha_1^2 (\lambda_1 + \lambda_2) = \alpha_1^2 (\lambda_1 + \lambda_1) = 0$
%which is a contradiction.
%Hence in this case the expressibility with $q = 2$ is not possible.
%Since we have only used simple degree-$2$ bounded graphs $C_3, C_4, P_1, P_2$,
%this particular inexpressibility statement holds even for degree-$2$ simple graphs.
%\end{enumerate}
%
%\begin{theorem}\label{thm:wm-as-GH-for-deg-bounded-graphs}
%Let $\bbF$ be a field and $d \ge 2$.
%Then for the graph parameter \textsc{\#Weighted-Matching$_a$} \emph{($\wmatch_a$)} where $a \in \bbF$
%as a function defined on degree-$d$ bounded graphs the following hold:
%\begin{enumerate}
%\item $\wmatch_a$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$ even on degree-$d$ bounded \emph{simple} graphs.
%\item If $\bbF$ is infinite, then $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$ unless $\Char \bbF = 2$, $d = 2$ and $a = 0$
%in which case $\wmatch_a = \pmatch$ is not expressible $\hom(\cdot, H)$ with $|V(H)| = d$ even on degree-$d$ bounded \emph{simple} graphs
%but is expressible as $\hom(\cdot, H)$ with $|V(H)| = d + 1 = 3$.
%\end{enumerate}
%\end{theorem}
%

%%%-------
%Note that  \textsc{\#Perfect-Matching} \emph{($\pmatch$)} is just
%the special case  $a = 0$. Hence Theorem~\ref{thm:wm-as-GH-for-deg-bounded-graphs} also holds for \emph{($\pmatch$)}
%which proves Theorem~\ref{thm:pm-as-GH-for-deg-bounded-graphs-short}.
%

%\begin{theorem}\label{thm:wm-as-GH-for-deg-bounded-graphs}
%Let $\bbF$ be a field and $d \ge 2$. Then for the graph parameter \textsc{\#Weighted-Matching$_a$} \emph{($\wmatch_a$)} where $a \in \bbF$ as a function defined on degree-$d$ bounded graphs the following hold:
%\begin{enumerate}
%\item $\wmatch_a$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$  even on degree-$d$ bounded \emph{simple} graphs.
%%{\color{red}
%%\item If $d = 0$, then $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = 0$ (i.e., $H = K_0$) iff $a = 0$. When $a \ne 0$, $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = 1$.
%%\item If $d = 1$, then $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = 1$ iff $a \ne 0$. When $a = 0$, $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = 2$.
%%\item If $d \ge 2$ and
%\item If $\bbF$ is infinite, then $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d \text{ or } d + 1$.
%%}
%%\item If $d \ge 2$ and 
%\item If $\Char \bbF = 0$, then $\wmatch_a$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$.
%\end{enumerate}
%\end{theorem}

%Note that  \textsc{\#Perfect-Matching} \emph{($\pmatch$)} is just
%the special case  $a = 0$. Hence Theorem~\ref{thm:wm-as-GH-for-deg-bounded-graphs} also holds for \emph{($\pmatch$)}.

%  we get a result for the graph parameter \textsc{\#Perfect-Matching} \emph{($\pmatch$)}.
%\begin{corollary}\label{cor:pm-as-GH-for-deg-bounded-graphs}
%Let $\bbF$ be a field and $d \ge 0$. Then for the graph parameter \textsc{\#Perfect-Matching$_a$} \emph{($\pmatch$)} where $a \in \bbF$ as a function defined on degree-$d$ bounded graphs the following hold:
%\begin{enumerate}
%\item $\pmatch$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| < d$ even on degree-$d$ bounded \emph{simple} graphs.
%{\color{red}
%\item If $d = 0$, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = 0$ (i.e., $H = K_0$).
%\item If $d = 1$, then $\pmatch$ is not expressible as $\hom(\cdot, H)$ with $|V(H)| = 1$ but is expressible with $|V(H)| = 2$.
%\item If $d \ge 2$ and $\bbF$ is infinite, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d + 1$.
%}
%\item If $d \ge 2$ and $\Char \bbF = 0$, then $\pmatch$ is expressible as $\hom(\cdot, H)$ with $|V(H)| = d$.
%\end{enumerate}
%{\color{red} REMOVE: Here we can assume that all vertices of $H$ have nonzero weight everywhere.}
%\end{corollary}




==> pm-rk-con-ten-GH-article-(cpc-submission)/extensions.tex <==
\section{Extensions}
%: Graphs with loops, directed graphs and hypergraphs}
%{\color{red} (Title is the same as that of the FLS paper. I think it's perfectly fine, however, a few sentences in the text coincide with th.)}.

So far we have allowed $G$ to have multiple edges but no loops
as is the standard definition. 
We can extend the results in this paper to more general graphs.
If we allow (multiple) loops in $G$,
we can show that 
the (multiplicative) graph parameter $f(G) = a^{\operatorname{\#loops}(G)}$
where $1 \ne a \in \bbF$ ($a$ can be $0$) cannot be expressed as a GH function,
even though its connection tensors $T(f, k, n)$ all have symmetric rank $1$ and $f(K_0) = 1$.
To get the corresponding representation theorem for graphs with (multiple) loops,
in the target graph $H$ each loop $e$ attached to a vertex $i$
must have two weights:
$\beta_{i i}$ which is used when a nonloop edge of $G$ is 
mapped onto $e$,  
and the other, say $\gamma_i$,
 when a loop of $G$ is mapped onto $e$.
%It is not hard to see that 
In this extended model we have the following:
\begin{itemize}
\item The main expressibility results 
%(GH expressibility criterion) 
Theorems~\ref{thm:uniform-exponential-rank-boundedness}, \ref{thm:uniform-exponential-rank-boundedness-converse} and~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened}
remain true with the proof from Section~\ref{sec:proof-of-main-results}
carrying over to this model with slight adjustments.

\item The GH inexpressibility results from
Section~\ref{sec:apps}
%Sections~\ref{sec:apps} and~\ref{sec:apps} 
%(and a fortiori Section~\ref{sec:apps-short})
remain true as the provided proofs involve only simple loopless graphs.
%{\color{red}
%Note that 
(For \#\textsc{Vertex-Disjoint-Cycle-Cover} ($\vdccover$),
a loop at a vertex is considered a cycle cover of that vertex;
this is consistent with the definition in Holant problems.)
%
%%it does not matter whether or not we consider loops as cycles covering a vertex.
%But the natural extension in agreement with Holant is to consider a loop as a cycle covering a vertex.
%}
%
%{\color{red} JYC: we can say that it doesn't matter how to extend any of these,
%but $\Holant$ gives natural extensions / defintions on looped graphs,
%in particular for $\vdccover$). The thing I want to be clear is that the reader won't ask
%a questions how they are defined on looped graphs.)}
%
%{\color{red} JYC: inexpressibility results are $\wmatch_a$ (so $\pmatch$), $\vdccover$, $\edgecol_d$
%and also the inexpressibility part for bounded degree graphs.}

\item The results from subsection~\ref{sec:bonded-deg-graphs} %Section
on bounded degree graphs remain true in the sense that
the inexpressibility results hold if we allow $\gamma_i$ to be arbitrary
(again, since only simple loopless graphs were used in the proof),
while the expressibility holds even with the stronger requirement $\gamma_i = \beta_{i i}$.
\end{itemize}

%{\color{red} (mentioned that we can do it for directed graphs in addition to looped graphs (can do their combo also), because it is obvious.
%However, the general model~\cite{Lovasz-Schrijver-2008} captures directed graphs and hypergraphs)}

Analogously, a GH expressibility criterion can be stated
and proved within the framework of directed GH with minor adjustments, too.
%It is important to mention that a generalization of the results
We note that  generalizations of 
results in~\cite{Freedman-Lovasz-Schrijver-2007}
were given in~\cite{Lovasz-Schrijver-2008}
to a more general model which captures directed graphs, hypergraphs, etc.
We expect that it is possible to generalize
the GH expressibility criterion in this paper
for arbitrary fields
to this more general model
in a similar way as done in~\cite{Lovasz-Schrijver-2008}.

%{\color{red} (old text minus garbage, just for your reference.)
%
%The constructions and results given in are in fact more general; analogously to~\cite{Freedman-Lovasz-Schrijver-2007} they extend to directed graphs and hypergraphs. The generalization of the results in~\cite{Freedman-Lovasz-Schrijver-2007} was given in~\cite{Lovasz-Schrijver-2008}, where the so-called \emph{semigroups with carriers} were introduced. It is also possible to extend the definitions and the results from~\cite{Lovasz-Schrijver-2008} in terms of these objects over an arbitrary field.
%}
%
%{\color{red} (hint for JYC):
%
%Suppose the contrary.
%Let $H$ be an $\bbF$-weighted graph
%with no loop weights such that $a^{\operatorname{\#loops}(G)} = \hom(G, H)$.
%Then consider all possible graphs $G$ with fixed $|V(G)| > |V(H)| = q$, say $q + 1$.
%That is, we take a complete graph with loops on $q + 1$,
%and then thicken its loops and edges independently, $0$-thickenings are valid.
%After that, use the Vandermonde argument
%and notice that on LHS there is nothing
%that gives you the same tuple as $a^{\operatorname{\#loops}(G)}$ does.
%Note that in this argument use graphs $G$ with multiloops.
%}

%{\color{red}
%The constructions and results given in are in fact more general; analogously to \cite{Freedman-Lovasz-Schrijver-2007} they extend to directed graphs and hypergraphs. The generalization of the results in \cite{Freedman-Lovasz-Schrijver-2007} was given in \cite{Lovasz-Schrijver-2008}, where the so-called \emph{semigroups with carriers} were introduced. It is also possible to extend the definitions and the results from \cite{Lovasz-Schrijver-2008} in terms of these objects over an arbitrary field. Besides, refining the ideas from our main proof from Section~\ref{sec:proof-of-main-results} (mostly Subsections~\ref{sec:build-alg-isom}, \ref{sec:one-implies-all}), it is possible to immediately derive an expressibility result for functions on (commutative) monoids ($=$ semigroups with identity) as a finite linear combination of characters. In this model, the labels are not needed and the exponential rank boundedness is of no importance, however, the constant or $n - 1$ bound from Theorems~\ref{thm:uniform-exponential-rank-boundedness-converse}, \ref{thm:uniform-exponential-rank-boundedness-converse-strengthened} respectively is present. We will precisely state and prove everything in a separate paper(s). {\color{red} [But not so soon...]}
%}


==> pm-rk-con-ten-GH-article-(cpc-submission)/finite-symmetric-tensor-rank.tex <==
\subsection{Finite symmetric tensor rank}\label{sec:fin-sym-ten-rank}
% over large infinite fields}\label{sec:fin-sym-ten-rank}
The proof of the following lemma is essentially the same as Lemma 4.2
in~\cite{Comon-Golub-Lim-Mourrain-2008};
the only modification needed is to avoid a
symmetrization step, which could result in a division by $0$
in a field of finite characteristic.

%{\color{red} take a look at Lemma 4.2 of Comon's paper, but its proof also uses Lemma 3.6 (see page 7)}
%
%{\color{red} title says over infinite, better say large fields???. also say $n \ge 0$.
%$n = 0$ is trivial (but when $n \ge 0$, coefficients can't be absorbed into vectors), $N = 0$ is also trivial as $A = 0$. So then let $n \ge 1$ and $N \ge 1$}
%
%{\color{red} Should say that $e_1, \ldots, e_N$ is the canonical basis of $\bbF^N$ otherwise we only have duals.}
%
%{\color{red} $(e^*_{k_1} \otimes \cdots  \otimes e^*_{k_n}) (A) = (e^*_{k_{\pi(1)}} \otimes \cdots  \otimes e^*_{k_{\pi(n)}}) (A)$,
%basically it just says that $A$ as an array is permutation symmetric (true in any basis of $V$).
%We will need to define this notion beforehand.
%In fact we can identify $\Sym^n(V)$ with symmetric arrays, and for $A$, you might use subscripts.}
%
%{\color{red} also we say that $\Sym^n(V')$ injectively embeds into $\Sym^n(V)$. Also when we go to an inner/outer space, rank doesn't change.}
%
%{\color{red} Nice explanation, but the compression operator is actually applicable on the entire $\Sym^n(V)$ and then on $T$ as a result.
%No need to define it on $T$ and then extends to $\Sym^n(V)$. It would make the explanation shorter? The compression operator is basis dependent btw.}
%
%{\color{red} add the proof of what happens when $\dim V < \infty$.}
%
%{\color{red} Note that I wrote $\dim V - 1$ below in the binomial coefficient unlike Comon (page 10). Maybe $n$ is better.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lm:finite-symmetric-tensor-rank}
If $\bbF$ is a field of cardinality $|\bbF| > n$, a fortiori if 
$\bbF$ is infinite, and
$V$ is a vector space over  $\bbF$, then every symmetric
tensor $A \in  \Sym^n(V)$ has a  finite symmetric tensor rank
$\symrank(A) < \infty$.
Moreover, when $\dim V < \infty$,
we have $\symrank(A) \le \binom{\dim V + n - 1}{n}$.
\end{lemma}
\begin{proof}
By definition, every $A \in  \Sym^n(V) \subseteq V^{\otimes n}$ 
is a finite sum $A = \sum_{i=1}^m v_{i1} \otimes \cdots  \otimes
v_{in}$. Let $V' = {\rm span}\{v_{ij} \mid i \in [m], j \in [n]\}$
 be  a finite dimensional subspace of $V$.
As  $A \in  \Sym^n(V')$, we can assume
$V$ is finite dimensional, with no change in $\symrank(A)$; so we let $V = \bbF^N$, for some $N$.

Let $T =  {\rm span}\{ x^{\otimes n}  \mid x \in V\}
 \subseteq \Sym^n(V)$.  Our claim is that equality holds.
% and
%the lemma follows.
For every entry of $x^{\otimes n}$, which is  a product of
coordinate entries of $x$, we can classify it by how many factors are
the $j$-th coordinate of $x$, for $j \in [N]$. 
%We can remove repeated entries as follows.
There are  $\binom{n + N - 1}{N - 1} = \binom{N + n - 1}{n}$ coordinates
 which can be indexed by tuples $(i_1, \ldots, i_N)$
where $i_1, \ldots, i_N \ge 0$ and $i_1 + \cdots + i_N = n$,
such that every entry of
every  $t \in T$ is equal to its entry at one of these coordinates.
We define a compression operator $C$ which selects only those
 $\binom{N + n - 1}{n}$ coordinates, and define
\[S =  {\rm span}\{ C(x^{\otimes n})  \mid x \in V\}
= \{ C(t)  \mid t \in T\}.\]

The compression operator $C$ is also applicable to $\Sym^n(V)$.
Indeed, by definition  as a symmetric array in $\bbF^{V^n}$,
 any $A \in \Sym^n(V)$ is invariant under any permutation of 
$n$. This means that
 for any $(k_1, \ldots, k_n)$, where $k_1, \ldots, k_n \in [N]$,
and any permutation $\pi \in S_n$,
if $(e^*_1, \ldots, e^*_{N})$ is the dual basis
to the canonical basis of $V$, then
$(e^*_{k_1} \otimes \cdots  \otimes e^*_{k_n}) (A)
= (e^*_{k_{\pi(1)}} \otimes \cdots  \otimes e^*_{k_{\pi(n)}}) (A)$.
This invariance can be characterized by the tuple
$(i_1,  \ldots,  i_N)$, where
$i_j = $ the number $j \in [N]$ among $(k_1, \ldots, k_n)$.
Thus  $C$ is applicable to $\Sym^n(V)$, and we denote
the result $C(\Sym^n(V)) = \{ C(v)  \mid v \in \Sym^n(V)\} \subseteq 
\bbF^{\binom{N + n - 1}{n}}$.
As $T \subseteq \Sym^n(V)$, we have $S \subseteq C(\Sym^n(V))$.

Next we prove that
$S = \bbF^{\binom{N + n - 1}{n}}$.
Then it follows that $S = C(\Sym^n(V))$, from which
it clearly follows that $T = \Sym^n(V)$ since $C$ simply
removes repeated entries.


Suppose otherwise, then $\dim S < \binom{N + n - 1}{n}$.
There exists a nonzero vector in $\bbF^{\binom{N + n - 1}{n}}$
such that it has a zero dot product with all $S$.
This means there exists a nonzero tuple
$(a_{(i_1,  \ldots,  i_N)}) \in \bbF^{\binom{N + n - 1}{n}}$
indexed by $N$-tuples of  nonnegative
integers that sum to $n$,
such that
$\sum_{(i_1,  \ldots,  i_N)} a_{(i_1,  \ldots,  i_N)} 
x_1^{i_1} \cdots x_N^{i_N} = 0$, for all $x_1, \ldots, x_N \in \bbF$.

As a polynomial in $x_N$ it has degree at most $n$, and yet it vanishes
at $|\bbF| > n$ points. So for any fixed $0 \le i_N \le n$,
$\sum_{(i_1,  \ldots,  i_{N-1})} a_{(i_1,  \ldots, i_{N-1},  i_N)}
x_1^{i_1} \cdots x_{N-1}^{i_{N-1}} = 0$, for all  $x_1, \ldots, x_{N-1}
 \in \bbF$, which can be viewed as a  polynomial in $x_{N-1}$ of
degree at most $n - i_N \le n$. 
Iterating $N$ steps, we reach a contradiction that
the tuple $(a_{(i_1,  \ldots,  i_N)})$ is entirely zero.

\end{proof}


==> pm-rk-con-ten-GH-article-(cpc-submission)/graph-algebras.tex <==
\section{Graph algebras\label{section:graph-algebras}}

%When the field  $\bbF$ is clear from its context we omit
%mentioning it explicitly.
%We also implicitly identify a (labeled) graph with its (labeled) graph isomorphism class.

\subsection{Basic definitions}

An $\bbF$-valued \textit{graph parameter} is a function from
finite graph isomorphism classes to $\bbF$~\footnote{The concept can be defined over commutative rings but our treatment uses properties of a field.}.
 For convenience, we think of a graph parameter as a function defined on finite graphs and invariant under graph isomorphism. We 
allow multiple edges in our graphs, but no loops, as input to a graph parameter.
 A graph parameter $f$ is called \textit{multiplicative}, if for any disjoint union $G_1 \sqcup G_2$ of graphs $G_1$ and $G_2$ we have $f(G_1 \sqcup G_2) = f(G_1) f(G_2)$.

%For every nonnegative integer $k$, let $[k] = \{ 1, \ldots, k \}$. In particular, $[0] = \emptyset$.

A $k$-labeled graph ($k \ge 0$) is a finite graph in which $k$ nodes are labeled by $1, 2, \ldots, k$ (the graph can have any number of unlabeled nodes). Two $k$-labeled graphs are isomorphic if there is a label-preserving isomorphism between them. 
We identify a ($k$-labeled) graph with its ($k$-labeled) graph isomorphism class.
We denote by $K_k$ the $k$-labeled complete graph on $k$ nodes, and by $U_k$, the $k$-labeled graph on $k$ nodes with no edges. In particular, $K_0 = U_0$ is the empty graph with no nodes and no edges.
%
A graph parameter on a labeled graph ignores its labels.

It is easy to see that for a multiplicative graph parameter $f$, either $f$ is identically $0$ or $f(K_0) = 1$. Every weighted graph homomorphism $f_H = \hom(\cdot, H)$ is a multiplicative graph parameter. 
%{\color{red} [Added here the last sentence]}

%The  \textit{product} of  two $k$-labeled graphs $G_1$ and $G_2$
% is defined as follows: we take their disjoint union, and then identify nodes with the same label. Hence for two $0$-labeled graphs, $G_1 G_2 = G_1 \sqcup G_2$ (disjoint union). Clearly, the graph product is associative and commutative with the unit $U_k$, so the set of all isomorphism classes of finite $k$-labeled graphs togegher with the product operation forms a commutative monoid which we denote by $\calPLG[k]$. Later, in Section~\ref{sec:proof-of-main-results} we will expand this definition to finite labeled graphs whose label sets are 
%arbitrary 
%(finite) subsets of $\bbZ_+$.

The  \textit{product} of  two $k$-labeled graphs $G_1$ and $G_2$
 is defined as follows: we take their disjoint union, and then identify nodes with the same label. Hence for two $0$-labeled graphs, $G_1 G_2 = G_1 \sqcup G_2$ (disjoint union). Clearly, the graph product is associative and commutative with the identity $U_k$, so the set of all isomorphism classes of finite $k$-labeled graphs together with the product operation forms a commutative monoid which we denote by $\calPLG[k]$.

%\sout{A ($k$-labeled, $\bbF$-)\textit{quantum graph}  is a finite formal $\bbF$-linear
%combination of finite $k$-labeled graphs.
%Let $\calG[k]$ denote the algebra of $k$-labeled $\bbF$-quantum graphs.}

Let $\calG[k]$ denote the monoid algebra $\bbF \calPLG[k]$ consisting of all
finite formal linear combinations in $\calPLG[k]$ with coefficients from $\bbF$;
they are called ($k$-labeled, $\bbF$-)\textit{quantum graphs}.
This is a commutative algebra with $U_k$ being the multiplicative identity,
and the empty sum as the additive identity.
Later, in Section~\ref{sec:proof-of-main-results} we 
will expand these definitions to allow label sets
to be arbitrary finite subsets of $\posints$.
%finite labeled graphs whose label sets are 
%arbitrary 
%finite subsets of $\bbZ_+$.

%{\color{red} (or just like in section 5)}
%{\color{red} (more correct definitions, to replace the previous defs)
%
%%A ($k$-labeled, $\bbF$-)\textit{quantum graph} is a finite formal $\bbF$-linear
%%combination of finite $k$-labeled graphs.
%%Let $\calG[k]$ denote the monoid algebra $\calPLG[k]$ consisting of all
%%finite formal linear combinations (of the elements in) $\calPLG[k]$ with coefficients from $\bbF$, i.e.,
%%$k$-labeled $\bbF$-quantum graphs.
%}

%
%{\color{red}(rephrase, say ($k$-labeled) ($\bbF$-)\textit{quantum graph} (put in $\bbF$ in () so it can be omitted) but $\bbF$-linear, don't put in (), same in Section 5)
%
%A ($k$-labeled) \textit{quantum graph} is a finite formal linear 
%combination of finite ($k$-labeled) graphs. 
%If the coefficients come from $\bbF$ we call these objects
%($k$-labeled) $\bbF$-quantum graphs.
%
%Let $\calG[k]$ denote the monoid algebra $\bbF \calPLG[k]$,
%i.e., the (infinite dimensional) vector space of finite formal $\bbF$-linear combinations of elements of $\calPLG[k]$, or, $k$-labeled $\bbF$-quantum graphs.
%Clearly, $U_k$ is the identity in $\calG[k]$.
%}
%
%Let $\mathcal G[k]$ denote the monoid algebra $\bbF \calPLG[k]$,
%i.e., the (infinite dimensional) vector space of finite formal $\bbF$-linear combinations of elements of $\calPLG[k]$, or, ($k$-labeled) $\bbF$-quantum graphs. 
%This is a commutative algebra with $U_k$ being the identity. 
%
%Let $\mathcal G$ denote the monoid algebra $\bbF \calPLG$,
%i.e., the (infinite dimensional) vector space of finite formal $\bbF$-linear combinations of elements of $\calPLG$, or, $\bbF$-quantum graphs.
% 
%Later, in Section~\ref{sec:proof-of-main-results} we will expand these definitions to finite labeled graphs whose label sets are arbitrary (finite) subsets of $\bbZ_+$.
% 


\subsection{Connection tensors}

Now we come to the central concept for our treatment. Let $f$ be any graph parameter. For all integers $k, n \ge 0$, we define the following $n$-dimensional array $T(f, k, n) \in \bbF^{(\calPLG[k])^n}$,
%which can be identified with 
%$\left( (\bigoplus_{\calPLG[k]} \bbF)^{\otimes n} \right)^*$.
which can be identified with $(V^{\otimes n})^*$,
where $V$ is the infinite dimensional vector space with
coordinates indexed by ${\calPLG[k]}$, i.e., $V = \bigoplus_{\calPLG[k]} \bbF$.
 %Each coordinate is indexed by $\calPLG[k]$. 
The entry of $T(f, k, n)$ at coordinate $(G_1, \ldots, G_n)$ is $f(G_1 \cdots G_n)$; when $n = 0$, 
we define $T(f, k, n)$ to be the scalar $f(U_k)$. Furthermore, by the commutativity of the product the arrays $T(f, k, n)$ are symmetric with respect to its coordinates,
i.e., $T(f, k, n) \in \Sym(\bbF^{(\calPLG[k])^n})$.
Fix $f, k$ and $n$, we call the $n$-dimensional
 array $T(f, k, n)$ the ($k$th, $n$-dimensional)
 \textit{connection tensor} of the graph parameter $f$. When $n = 2$, 
a connection tensor 
is exactly
a \textit{connection matrix} of the graph parameter $f$ 
studied in \cite{Freedman-Lovasz-Schrijver-2007}, i.e., $T(f, k, 2) = M(f, k)$.

In contrast to~\cite{Freedman-Lovasz-Schrijver-2007}, we will be concerned with only one property of connection tensors, namely their symmetric rank.
%\sout{Positive semidefiniteness that was central to the theory in~\cite{Freedman-Lovasz-Schrijver-2007} will not be required.} 
%{\color{red} (JYC, just remove)}
The symmetric rank $\symrank(f, k, n) = \symrank(T(f, k, n))$, as a function of $k, n$, will be called the \textit{symmetric rank connectivity function} of the parameter $f$. This may be infinite, but for many interesting parameters it is finite, and its growth rate will be important for us.

%A ($k$-labeled) \textit{quantum graph} is a finite formal linear 
%combination of finite ($k$-labeled) graphs. 
%If the coefficients come from $\bbF$ we call these objects
%($k$-labeled) $\bbF$-quantum graphs.

\begin{remark}
In~\cite{Freedman-Lovasz-Schrijver-2007}, the matrix rank  of  $M(f, k)$
was used for the connection matrices. 
The results of the present paper use the symmetric tensor rank of the connection tensors $T(f, k, n)$ and hold for arbitrary fields. 
For $n = 2$, tensor rank coincides with
matrix rank, i.e.,  $\rank(T(f, k, 2)) =  \rank(M(f, k))$,
and furthermore if $\Char \bbF \ne 2$,
then the symmetric tensor rank also coincides, %,
%{\color{red} with the previous two notions so}
$\symrank(T(f, k, 2)) = \rank(T(f, k, 2)) = \rank(M(f, k))$.
Since the field in~\cite{Freedman-Lovasz-Schrijver-2007}
is  $\bbR$, the notions are consistent.
\end{remark}

\begin{proposition}\label{prop:graph-paramater-multiplicativity-criterion}
Let $f$ be a graph parameter that is not identically $0$. 
The following are equivalent:
\begin{enumerate}
\item\label{item-multiplicative-1}
$f$ is multiplicative.
\item\label{item-all-ge0-2}
%For all $n \ge 0$,  $f(K_0) = 1$ and $\symrank T(f, 0, n) = 1$.
$f(K_0) = 1$ and for all $n \ge 0$, $\symrank T(f, 0, n) = 1$.
\item\label{item-some-ge2-3}
$f(K_0) = 1$ and 
there exists some $n \ge 2$,  $\symrank T(f, 0, n) = 1$.
\end{enumerate}
%
%Fix any $n \ge 2$. Then $f$ is multiplicative if and only if $f(K_0) = 1$ and $\symrank T(f, 0, n) = 1$.
\end{proposition}
\begin{proof}
Suppose $f \not = 0$ is multiplicative. 
Then $f(K_0)^2 = f(K_0)$, showing that $f(K_0) \in \{ 0, 1 \}$. If $f(K_0) = 0$, then the relation $f(G) = f(G) f(K_0)$ implies that $f(G) = 0$ for every $G$, which is excluded. So $f(K_0) = 1$.
Trivially $\symrank T(f, 0, n) = 1$ for $n = 0, 1$.
Fix any $n \ge 2$.
Then $f(G_1 \cdots G_n) = f(G_1) \cdots f(G_n)$ for any $0$-labeled graphs $G_1, \ldots, G_n$, which implies that $\symrank T(f, 0, n) = 1$.


Now suppose $f(K_0) = 1$ and  for some $n \ge 2$,  $\symrank(f, 0, n) = 1$.
This implies that there is a graph parameter $\phi$ and a constant $c_n$
 such that $f(G_1 \cdots G_n) = c_n \phi(G_1) \cdots \phi(G_n)$. 
Putting all $G_i = K_0$, we get $c_n \phi(K_0)^n = f(K_0) = 1$ 
so $\phi(K_0) \not =0$
and $c_n = 1 / \phi(K_0)^n$. 
Dividing $\phi$ by $\phi(K_0)$ we can assume that $\phi$ is normalized
 so that $f(G_1 \cdots G_n) = \phi(G_1) \cdots \phi(G_n)$ and $\phi(K_0) = 1$. Next, taking $G_1 = G$ and $G_i = K_0$ for $2 \le i \le n$ we see that $f(G) = \phi(G)$ for every $G$ and therefore $f(G_1 \cdots G_n) = f(G_1) \cdots f(G_n)$. Finally, substituting $G_i = K_0$ for $2 < i \le n$,  
we get $f(G_1 G_2) = f(G_1) f(G_2)$ so $f$ is multiplicative.
\end{proof}


\subsection{Connection tensors of homomorphisms}

Fix a weighted graph $H = (\alpha, B)$. 
Recall that 
in the definition of $\hom(\cdot, H)$ 
we assume
 $H$ to be a complete graph with possible
$0$ weighted edges and loops, but no $0$ weighted vertices.
For any $k$-labeled graph $G$ and mapping $\phi \colon [k] \to V(H)$, let
\begin{equation}\label{eqn:partial-hom-dec}
\hom_\phi(G, H) = \sum_{\text{\small $\substack{\psi \colon V(G) \to V(H) \\ \psi \text{ extends } \phi}$}} \frac{\alpha_\psi}{\alpha_\phi} \hom_\psi(G, H), %\tiny 
\end{equation}
where $\alpha_\phi = \prod_{i \in [k]} \alpha_H(\phi(i))$,
and $\alpha_\psi$ and $\hom_\psi$ are defined by (\ref{eqn:hom-phi-def}).
%%%
Here $\psi  \text{ extends } \phi$ means that
 if $u_i \in V(G)$ is labeled by $i \in [k]$
then $\psi(u_i) = \phi(i)$,
%and $\alpha_\phi= \prod_{i=1}^k \alpha(\phi(i))$, $\alpha_\psi
%= \prod_{v \in V(G)} \alpha(\psi(v))$,
so $\frac{\alpha_\psi}{\alpha_\phi}$
is the product of vertex weights of $\alpha_\psi$ \emph{not} in $\alpha_\phi$.
%%%
Then %So
\begin{equation}\label{eqn:full-hom-dec}
\hom(G, H) = \sum_{\phi \colon [k] \to V(H)} \alpha_\phi \hom_\phi(G, H).
\end{equation}

Our main contribution in this paper is that a simple exponential bound in $k$ on the symmetric rank of the connection tensor of a graph parameter characterizes it being expressible as $\hom(\cdot, H)$.  This holds over all fields $\bbF$.
%\sout{In contrast to the main 
%theorem in~\cite{Freedman-Lovasz-Schrijver-2007}, 
%where the theory is restricted to
%weighted graphs $H = (\alpha, B)$ where  $\alpha$ is 
%positive  and $B$ is real,
 %the requirement of positive semidefiniteness is not
%needed here (and would not be meaningful for arbitrary fields).}
In the following theorems, the rank function $\symrank(f_H, k, n)$ is defined over the field $\bbF$.

\begin{theorem}\label{thm:uniform-exponential-rank-boundedness}
For any graph parameter defined by the graph homomorphism $f_H = \hom(\cdot, H)$,
 we have $f_H(K_0) = 1$ and $\symrank (f_H, k, n) \leqslant |V(H)|^k$ for all $k, n \ge 0$. 
\end{theorem}
\begin{proof}
The first claim is obvious, as an empty product is $1$,
and the sum in~(\ref{eqn:hom-def})
 is over the unique empty map $\emptyset$ which is the only possible map
from  the empty set $V(K_0)$.
 For the second claim
  notice that for any $k$-labeled graphs $G_1, \ldots, G_n$ and $\phi \colon [k] \to V(H)$,
\begin{equation}\label{eqn:partial-hom-mult}
\hom_\phi(G_1 \cdots G_n, H) = \hom_\phi(G_1, H) \cdots \hom_\phi(G_n, H).
\end{equation}
When $n = 0$, this equality is $\hom_\phi(U_k, H) = 1$
according to~(\ref{eqn:hom-phi-def}), as an empty product is $1$.

%By (\ref{eqn:partial-hom-dec}),
%By (\ref{eqn:full-hom-dec}),
 %the connection tensor $T(f_H, k, n)$ is 
%a sum of $|V(H)|^k$ order-$n$ tensors, one for each mapping $\phi \colon [k] \to V(H)$; (\ref{eqn:partial-hom-mult}) shows that these tensors are symmetric and have symmetric rank $1$.
%

By~(\ref{eqn:full-hom-dec}) and~(\ref{eqn:partial-hom-mult}),
for the connection tensor $T(f_H, k, n)$ we have the following decomposition:
\[
T(f_H, k, n) = \sum_{\phi \colon [k] \to V(H)} \alpha_\phi (\hom_\phi(\cdot, H))^{\otimes n}
\]
where each $\hom_\phi(\cdot, H) \in \bbF^{\calPLG[k]}$ and $k, n \ge 0$. 
Let $q = |V(H)|$.
Then each $T(f_H, k, n)$ is a linear combination of $q^k$ tensor $n$-powers
and therefore $\symrank  T(f_H, k, n) \le q^k$ for $k, n \ge 0$.
\end{proof}


The main results of this paper are Theorems~\ref{thm:uniform-exponential-rank-boundedness-converse}
and~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened}, a converse
to Theorem~\ref{thm:uniform-exponential-rank-boundedness}.
% and a generalized converse to Theorem~\ref{thm:uniform-exponential-rank-boundedness} respectively. Recall that by convention, $0^0 = 1$.
\begin{theorem}\label{thm:uniform-exponential-rank-boundedness-converse}
Let $f$ be a graph parameter for which $f(K_0) = 1$ and there exists a nonnegative integer $q$ such that $\symrank(f, k, n) \le q^k$ for every $k, n \ge 0$. Then there exists a weighted graph $H$ with $|V(H)| \le q$ such that $f = f_H$.
\end{theorem}
More generally,  we have the following stronger theorem.
%. (JYC, added, could you complete the sentence)}
\begin{theorem}\label{thm:uniform-exponential-rank-boundedness-converse-strengthened}
Let $f$ be a graph parameter for which $f(K_0) = 1$ and there exists a nonnegative integer $q$ such that for every $k \ge 0$ there exists $n \ge 2$ such that $\symrank(f, k, n) \le \min(n - 1, q^k)$. Then there exists a weighted graph $H$ with $|V(H)| \le q$ such that $f = f_H$.
\end{theorem}

Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened} implies Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse} 
by choosing a large $n$. Indeed if $\symrank(f, k, n) \le q^k$,
we may choose any $n \ge \max(q^k + 1, 2)$, which is 
$q^k + 1$ unless $q=0$ and $k>0$.

In Section~\ref{sec:proof-of-main-results} we will prove Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened}, then Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse} also follows.
%is just a simple consequence of it.



==> pm-rk-con-ten-GH-article-(cpc-submission)/his-preamble.tex <==
%\documentclass[11pt,twoside]{article}
\usepackage{amsmath, amsfonts, amssymb, amsthm, amscd, graphicx, 
%hyperref, 
enumerate, footmisc, mathtools, xcolor}
\setcounter{MaxMatrixCols}{30}
\setcounter{tocdepth}{10}
\providecommand{\U}[1]{\protect\rule{.1in}{.1in}}
\setlength{\topmargin}{-1.0in}
\setlength{\textheight}{9.25in}
\setlength{\oddsidemargin}{0.0in}
\setlength{\evensidemargin}{0.0in}
\setlength{\textwidth}{6.5in}
\def\labelenumi{\arabic{enumi}.}
\def\theenumi{\arabic{enumi}}
\def\labelenumii{(\alph{enumii})}
\def\theenumii{\alph{enumii}}
\def\p@enumii{\theenumi.}
\def\labelenumiii{\arabic{enumiii}.}
\def\theenumiii{\arabic{enumiii}}
\def\p@enumiii{(\theenumi)(\theenumii)}
\def\labelenumiv{\arabic{enumiv}.}
\def\theenumiv{\arabic{enumiv}}
\def\p@enumiv{\p@enumiii.\theenumiii}
\pagestyle{plain}
%\parindent=0pt
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}{Remark}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{axiom}{Axiom}

\newenvironment{lcases}
  {\left\lbrace\begin{aligned}}
  {\end{aligned}\right.}
\newcommand{\bbF}{\mathbb F}
\newcommand{\bbN}{\mathbb N}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbC}{\mathbb C}
\newcommand{\bbH}{\mathbb H}
\newcommand{\pmatch}{\operatorname{pm}}
\newcommand{\edgecol}{\operatorname{ec}}
\newcommand{\vdccover}{\operatorname{vdcc}}
\newcommand{\wmatch}{\operatorname{wm}}
\newcommand{\Char}{\operatorname{char}}
\newcommand{\Mod}{\operatorname{mod}}
%\newcommand{\rank}{\operatorname{rk}}
\newcommand{\symrank}{\operatorname{rk_\mathsf S}}
\newcommand{\matrank}{\operatorname{rank}}
\newcommand{\im}{\operatorname{im}}
%\newcommand{\Holant}{\operatorname{Holant}}
%\newcommand{\trans}[4]{\ensuremath{\left[ \begin{smallmatrix} #1 & #2 \\ #3 & #4 \end{smallmatrix} \right]}}
\newcommand{\Span}{\operatorname{span}}
%\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\id}{\operatorname{id}}
%\newcommand{\diag}{\operatorname{diag}}
%\newcommand{\dom}{\operatorname{dom}}

\newcommand{\calPLG}{\mathcal{PLG}}
\newcommand{\calG}{\mathcal G}
\newcommand{\calK}{\mathcal K}
\newcommand{\calP}{\mathcal P}
\newcommand{\bfx}{\mathbf x}
\newcommand{\bfy}{\mathbf y}
\newcommand{\bfz}{\mathbf z}
\newcommand{\sfS}{\mathsf S}
\newcommand{\sfT}{\mathsf T}
\newcommand{\calM}{\mathcal M}
\newcommand{\bfu}{\mathbf u}
\newcommand{\bfv}{\mathbf v}
\newcommand{\bff}{\mathbf f}
\newcommand{\textbfit}[1]{\textbf{\textit{#1}}}
\newcommand{\calI}{\mathcal I}
\newcommand{\calJ}{\mathcal J}
\newcommand{\calA}{\mathcal A}
\newcommand{\calT}{\mathcal T}

%%%\newcommand*{\mainflag}{}



==> pm-rk-con-ten-GH-article-(cpc-submission)/introduction.tex <==
\section{Introduction}

Many graph properties can be described in the general
framework called \emph{graph homomorphisms}. Suppose $G$ and $H$
are two graphs.  A mapping from
the vertex set $V(G)$  to the  vertex set $V(H)$
is a graph homomorphism if every edge $\{u, v\}$ of $G$
is mapped to an edge (or a loop) of $H$.
For example, if $H$ consists of two vertices $\{0, 1\}$
with one edge  between them and a loop at $0$,
then a vertex map $\phi: V(G) \rightarrow \{0, 1\}$
is a graph homomorphism iff $\phi^{-1}(1)$ is an independent
set of $G$. As another example, if $H = K_q$ is  a clique
on $q$ vertices (no loops),
then a vertex map $\phi: V(G) \rightarrow \{1, \ldots, q\}$
is a graph homomorphism iff $\phi$ is a proper vertex coloring of
$G$ using at most $q$ colors.


A more quantitative notion is the so-called partition
function associated with graph homomorphisms.
 The idea is that
we can consider a fixed $H$ with vertex weights and edge weights,
 and aggregate  all graph homomorphisms from $G$ to $H$,
 in a sum-of-product expression called the
partition function. This expression is invariant under graph isomorphisms,
thus expressing a graph property of $G$. This is  a weighted
counting version of the underlying concept~\cite{Lovasz-1967,GH-book, Borgs-et-al-counting-GH}.

More concretely, if each vertex $i \in V(H)$ has weight $\alpha_i$
and each edge $\{i, j\}$ of $H$ has weight $\beta_{i,j}$ (non-edge has weight $0$),
then the partition function $Z_H(\cdot)$ determined by $H$ is
\begin{equation}\label{eqn:def-graph-homomorphismshomomorphisms-pa-fn}
%\[
Z_H(G) = \hom(G, H) = \sum_{\phi: V(G) \rightarrow V(H)} 
\prod_{u \in V(G)} \alpha_{\phi(u)} 
\prod_{\{v, w\} \in E(G)} \beta_{\phi(v), \phi(w)}.
%\]
\end{equation}
The partition functions of graph homomorphisms
can express a broad class of weighted
counting problems.
%
Historically these  partition functions also arise in statistical
physics, where they play a fundamental role~\cite{baxter-6-8}. In classical physics
the  vertex and edge weights are typically (nonnegative) real numbers,
but in quantum theory they are complex numbers.
But even in classical physics, sometimes a generalization to
complex numbers allows a theoretically pleasing treatment.
E.g., Baxter generalized the parameters to complex values to 
 develop the ``commuting transfer matrix'' 
for the six-vertex model~\cite{baxter-6-8}. 
The book~\cite{GRS} (section 2.5.2)  treats the Hamiltonian of a 
one-dimensional 
spin chain as  an extension of the Hamiltonian of a 
six-vertex model with complex Boltzmann
weights.
 
Another source of fascination with these objects
comes from the classification program for counting problems
in complexity theory. In recent years many far-reaching classification
theorems have been proved classifying \emph{every} problem in a broad
class of counting problems as being either computable in polynomial time, or
being \#P-hard. This has been proved for 
graph homomorphisms (GH)~\cite{Dyer-Greenhill-2000, Dyer-Greenhill-corrig-2004,
Bulatov-Grohe-2005, Thurley-2009, Grohe-Thurley-2011, Goldberg-et-al-2010, Cai-Chen-Lu-2013},
for counting
constraint satisfaction problems (\#CSP)~\cite{bulatov-dalmu,
Bulatov, Dyer-Richerby, Cai-Chen-2017},
and for Holant problems~\cite{clx-holant,Backens-2017,Backens-2018,
%Miriam Backens:
%A Complete Dichotomy for Complex-Valued Holant^c. ICALP 2018: 12:1-12:14
%CLX11a,
glva-2013,Cai-Fu-Guo-W}. %,caiguowilliams13
These
theorems are called complexity dichotomies. If we consider problem instances 
restricted to planar graphs and variables to take
Boolean values, there is usually a trichotomy,
where every problem is either (1) computable in polynomial time, or (2)
\#P-hard on general graphs but computable in polynomial time for 
planar graphs, or (3) \#P-hard on planar graphs.  Counting perfect
matchings, including weighted versions, is one such problem
that belongs to type (2). The planar tractability of
counting perfect
matchings is by Kasteleyn's algorithm (a.k.a.~FKT-algorithm)~\cite{Kasteleyn-1961, Kasteleyn-1967, Tempereley-Fisher-1961}.
Valiant introduced holographic algorithms to significantly extend
the reach of this methodology~\cite{Valiant-2004,Val06,cai-chen-book}. %,Cai-Lu-2007
It is proved  that for
\emph{all}
 \#CSP where variables are Boolean
(but constraint functions can take complex values),
the methodology of 
holographic algorithms is \emph{universal}~\cite{Cai-Zhiguo-2017}. 
More precisely,
we can prove that
(A) the three-way classification above holds, 
and (B) the problems that belong to type (2) are precisely
those that can be captured by this single algorithmic approach,
namely a holographic reduction to Kasteleyn's algorithm.

\#CSP are
 ``vertex models'' where vertices are variables,
% and 
%are to be mapped to some values, 
and constraints are placed on 
subsets of these variables. The partition function of GH
can be viewed as a special case of \#CSP  where each constraint is
a binary function as an edge weight
 (and for undirected graphs, a symmetric binary function).
When vertex weights are present they are unary functions.

In contrast to vertex models, one can consider ``edge models''
where each edge is a variable, and constraint functions are
placed at each vertex.  This is called a Holant problem~\footnote{Bal\'azs
Szegedy~\cite{B-Szegedy} 
 studied ``edge coloring models'' which are
equivalent to a special case of Holant problems where
for each arity $d$ a  symmetric vertex functions  $f_d$ 
is given and  placed at vertices of degree $d$.
%for some sequence $\{a_{i}\}_{i \ge 0}$
%a uniform family of symmetric vertex functions $\{f_d\}_{d \ge 0}$ is given,
%where $f_d$ has arity $d$ and is placed at vertices of degree $d$, 
%and  $f_d$  takes value $a_i$ on all inputs of Hamming
%weight $0 \le i \le d$.
%where at each vertex of degree $d$
%a single symmetric function of arity $d$ is provided.
In general, Holant problems allow different (possibly
non-symmetric) constraint functions from a  set  assigned at vertices; see~\cite{cai-chen-book}. 
%{\color{red} (JYC: add stuff with more citations: Lovasz's book, Szegedy's paper af an ec is almost always expressible as GH \cite{Lovasz-limits-book, Szegedy-2010})}
}.
Counting perfect matchings is a Holant problem where the
constraint function at each vertex is the {\sc Exact-One} function.
Counting all matchings is a Holant problem with the
{\sc At-Most-One} constraint.
Other Holant problems include counting edge colorings, or vertex disjoint
cycle covers. Many problems in statistical physics, such as
(weighted) orientation problems, ice models,  six-vertex models etc.
are all naturally expressible as Holant problems.

%Perhaps ironically, it has been proved~\cite{Cai-Fu-Guo-Williams}
It has been proved~\cite{Cai-Fu-Guo-W} %caiguowilliams13,
that for Holant problems defined by an arbitrary
set of complex-valued
symmetric constraint functions on Boolean variables,
 (A) the three-way classification above holds,
but (B) holographic reductions to Kasteleyn's algorithm is
\emph{not} universal for type (2); there is an additional class of
planar P-time computable problems; these, together with 
holographic reductions to Kasteleyn's algorithm,
constitute a complete algorithmic repertoire for this class.
(It is open whether this also holds for 
%not necessarily 
non-symmetric constraint functions.)

But this should strike the readers as somewhat ironic.
Counting perfect matchings \emph{is} the problem that Kasteleyn's algorithm
solves for planar graphs. However this algorithmic
approach  is  proved universal for type (2)
only for vertex models but \emph{not} for edge models, and yet  
counting perfect matchings
is a \emph{quintessential} Holant problem.
It is most naturally expressed in the edge model.
It is \emph{not} naturally expressed  as a vertex model.

Or can it? 

Freedman, Lov\'asz and Schrijver~\cite{Freedman-Lovasz-Schrijver-2007} proved that
counting perfect matchings cannot be expressed as
the partition function of GH;
%graph homomorphisms;
however their proof restricts to a definition of partition functions
with positive vertex weights and real valued edge weights.
%\footnote{For 
%this restricted version we will give a surprisingly simple proof; see
%Appendix~\ref{appendix-simple-proof-GH-cant-do-PM}}.
More importantly they give a characterization for 
a graph property
%parameter  
to be  \emph{expressible} as such a partition function
of GH.
%graph homomorphisms.

%They define a \emph{connection matrix}, and
Their characterization consists of two conditions on
a \emph{connection matrix}:
 a rank condition
and a positive semidefiniteness condition.
But when we move from ${\bbR}$ to the complex field ${\bbC}$, this 
positive semidefiniteness condition breaks down.
At a high level, a succinct reason is  that  for complex matrices
$M$, it is \emph{not} true that $M^{\tt T} M$ is positive semidefinite. 
However, partition functions of GH
% graph homomorphisms
with complex weights are interesting~\cite{Lee-Yang-1952, Asano-1970, Newman-1974, Lieb-1981, GRS, baxter-6-8}, and natural
in the quantum setting.
%~\cite{cite-physics-complex-partition-functions}.
More intrinsically (but less obviously), even if one is dealing with counting problems 
defined by real weights, 
complex matrices are essential as holographic transformations.
For example, the matrix
 $Z = \frac{1}{\sqrt{2}} \left[\begin{smallmatrix} 1 & 1\\
\mathfrak{i} & -\mathfrak{i} \end{smallmatrix}\right]$
%satisfying $Z^{\tt T} Z = \left[\begin{smallmatrix} 0 & 1\\
%1 & 0 \end{smallmatrix}\right]$, is 
is  one of the most important 
holographic transformations~\cite{cai-chen-book,
%CLX11a, 
Cai-Fu-Guo-W} in dealing with orientation problems 
such as the six-vertex model, even when all given weights are real.
Note that $Z$ transforms  the binary {\sc Equality}
function to {\sc Disequality},
which is expressible in the form of signature matrices
as: $Z^{\tt T} I Z = \left[\begin{smallmatrix} 0 & 1\\
1 & 0 \end{smallmatrix}\right]$.
Thus the results in~\cite{Freedman-Lovasz-Schrijver-2007} do not answer whether counting perfect matchings,
and other similar problems
naturally expressible as Holant problems (edge models), can be expressed
as partition functions of GH
when
complex vertex and edge weights are allowed.
We note that Schrijver~\cite{Schrijver-2009,Schrijver-2013} gave
beautiful characterizations of  graph properties  expressible 
 as partition functions of GH
with complex edge weights but no vertex weights. Thus effectively
the vertex weights are all 1  (and there are also subtle differences in the 
model which we will discuss in subsection~\ref{appendix-previous-work}
in the  Appendix).
%at the end of this section). 
So the expressibility of these Holant problems as 
(\ref{eqn:def-graph-homomorphismshomomorphisms-pa-fn})
with complex $\alpha_i$ and $\beta_{i,j}$ remained an open problem.

In this paper we resolve this question.
We define the notion of a \emph{connection tensor}.
Then we give a 
%alternative, 
tensor theoretic characterization of
when a graph parameter {can} be expressed as GH over \emph{any} field.
% as a partition function
%of graph homomorphisms, over \emph{any} field.
We show that there is \emph{only one} condition, which is both necessary and
sufficient for a graph parameter to be expressible by GH
with arbitrary vertex and edge weights,
%graph homomorphisms,
and that is a simple exponential bound on the rank of the connection tensor.
Positive semidefiniteness is not required (and would not be
meaningful in a general field). 

This characterization is purely algebraic. 
As a consequence we show that
counting perfect matchings is not expressible as partition
functions of GH over an arbitrary field  (over a field of characteristic $p > 0$ we count perfect matchings modulo $p$).
We also prove the same inexpressibility for several other
naturally defined  Holant problems. Over  bounded degree graphs,
we prove a sharp threshold  for the domain size  ($|V(H)|$)
for expressibility, using holographic transformations.
While we dispense with
their positive semidefiniteness condition, the paper~\cite{Freedman-Lovasz-Schrijver-2007}
 is an inspiration for this work from which we borrow many
definitions and ideas.

%While we borrow many
%definitions and ideas from~\cite{Freedman-Lovasz-Schrijver-2007}, 
%the possibility that vertex weights can cancel, in particular
%the sum of all vertex weights can be $0$, does create a significant
%technical obstacle, and we have to introduce some significant changes
%to their proof.
To handle general vertex weights
a significant technical difficulty we have to overcome following
the approach of~\cite{Freedman-Lovasz-Schrijver-2007} is
 the possibility that vertex weights can cancel. In particular,
the possibility that the sum of all vertex weights can be $0$
creates a nontrivial
technical obstacle, and we have to introduce some consequential changes
to their proof.
To do that, in addition to the algebras of quantum graphs $\calG(S)$, 
we define a second type of algebras of quantum graphs $\calG_\subseteq(S)$,
where $S \subseteq \bbZ_+$ is a finite set of labels. 
In  $\calG(S)$ 
the generators are precisely $S$-labeled graphs, whereas in
 $\calG_\subseteq(S)$  
their label sets can be arbitrary subsets of $S$. We need to do this because 
the normalization argument from \cite{Freedman-Lovasz-Schrijver-2007} fails
in our setting
(precisely because the sum of all vertex weights can be $0$).
One technical  step 
involves correctly defining the notion of a projection 
from one quotient algebra to another,
$\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$. 
%the objects are quotient algebras.
% yet to be defined.
It must be onto $\hat \calG_\subseteq(S)$ which is not in general the 
same as $\hat \calG(S)$, the corresponding quotient algebra
without the normalization. (In~\cite{Freedman-Lovasz-Schrijver-2007} 
this  $\calG_\subseteq(S)$ was not needed.)
After the appropriate algebraic structures are all in place,
now somewhat more elaborate than that of~\cite{Freedman-Lovasz-Schrijver-2007},
we are able to establish our algebraic
characterization of expressibility of a graph property as GH.
%%% omitted
%~\footnote{The 
%results from \cite{Freedman-Lovasz-Schrijver-2007} were extended in \cite{Lovasz-Schrijver-2008} to a more general model. It is also possible to extend the 
%results in this paper in a similar fashion.}.

An outline  of this paper
is as follows.
  Our main theorems are
Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse} 
and 
Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened}.
To prove these theorems
we need a proper algebraic setting, and these are certain
infinite-dimensional \emph{algebras}, which are
vector spaces endowed with a multiplication.
These algebras are infinite-dimensional because
we wish to account for all finite labeled graphs in one structure.
Being infinite-dimensional introduces some technical complications.
In  Section~\ref{sec:Preliminary-short} we include
some basic notions, mainly regarding tensor spaces.
%some basic notions, with some essential proofs provided
%in Section~\ref{sec:Preliminary-continued}.
In the context of this paper the coordinates of these infinite-dimensional 
vector spaces represent partially labeled graphs 
in the algebra $\calG(S)$ or $\calG_\subseteq(S)$ (to be defined in Section~\ref{sec:proof-of-main-results}). 
%and we can apply  
%the facts from Section~\ref{sec:Preliminary-short}
 %in the graph algebra framework.
% yet to be 
%introduced. 
In Section~\ref{section:graph-algebras}, 
we introduce the basic definitions of graph algebras 
and connection tensors of a graph parameter. 
%In Section~\ref{sec:apps-short}, we show how the tensor theoretic
In Section~\ref{sec:apps}, we show how the tensor theoretic
characterization can be used to prove that some graph properties cannot be 
expressed as GH over any field.
The main proof starts in Section~\ref{sec:proof-of-main-results}.
In subsection~\ref{subsec:monoid-and-algebra-of-graphs},
%Subsection~\ref{sec:proof-of-main-results} 
we define the monoid of partially labeled graphs and 
the algebra of quantum graphs in more detail.
%we give all the definitions concerning 
%quantum graph algebras in the expanded form. In particular, 
We define the algebras of quantum graphs $\calG(S)$
and $\calG_\subseteq(S)$,
the ideals $\calK_S$ and $\calK_{\subseteq S}$,
and the respective quotients $\hat \calG(S)$ and $\hat \calG_\subseteq(S)$. 
We also introduce and prove the correctness of the definition 
of the aforementioned projection $\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$, 
which arises from the linear map $\pi_S \colon \calG \to \calG_\subseteq (S)$. 
As said before, the possibility that 
the vertex weights sum to $0$ does not allow us 
to perform the corresponding normalization step, and we cannot just simply 
repeat the proofs
from~\cite{Freedman-Lovasz-Schrijver-2007} without extending all the definitions systematically. 
With all the groundwork set, we may finally proceed to the main proof.   
We show the existence of the basis of idempotents in the quotient algebras $\hat \calG(S)$ 
for finite $S \subseteq \bbZ_+$ by constructing an isomorphism 
%onto $\bbF^{r_k}$ 
onto $\bbF^{r}$ for some $r$
%(defined in Lemma~\label{lem:F^m-subalgebras})  where $k = |S|$, 
(a composition of two isomorphisms,
see Lemma~\ref{lem:Phi(k)-tilde-calG[k]-isomorphism} %defined in 
and Corollary~\ref{cor:Phi(k)-hat-calG[k]-isomorphism}) %(resulting in Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)})
thereby bounding their dimensions as well. After that we are able to proceed similarly to Section 4 
from \cite{Freedman-Lovasz-Schrijver-2007}, 
modifying the original proofs as needed.

Table~\ref{table:freq-used-notation} lists the main concepts and sets used in the paper.

\begin{table}[ht]
\centering
\begingroup
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{tabular}{|c|}
\hline
$\bigoplus_\calI \bbF, \bbF^\calI, \Sym^n(\bbF^\calI), \symrank, T(f, k, n)$ \\
\hline
$\calPLG, \calPLG_\subseteq(S), \calPLG(S), \calPLG[k](= \calPLG([k]))$ \\
\hline
$\calG, \calG_\subseteq(S), \calG(S), \calG[k](= \calG([k]))$ \\
\hline
$\calK, \calK_{\subseteq S}, \calK_S, \calK_{[k]}$ \\
\hline
$\hat \calG, \hat \calG_\subseteq(S), \hat \calG(S), \hat \calG[k]( = \hat \calG([k]))$ \\
\hline
$\tilde \calG_\subseteq(S), \tilde \calG(S), \tilde \calG[k](= \tilde \calG([k]))$ \\
\hline
$U_S, U_\emptyset, U_k( = U_{[k]}), u_S = U_S + \calK, u_\emptyset = U_\emptyset + \calK$ \\
\hline
$\pi_S \colon \calG \to \calG_\subseteq(S), \hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$ \\
\hline
\end{tabular}
\endgroup
\caption{\label{table:freq-used-notation}Main concepts and sets used in the paper.}
\end{table}



==> pm-rk-con-ten-GH-article-(cpc-submission)/line-numbers-patch.tex <==
%https://tex.stackexchange.com/questions/461186/how-to-use-lineno-with-amsmath-align
\usepackage[displaymath,mathlines]{lineno}
\linenumbers

%\makeatletter
%% Make a copy of macros responsible for entering display math mode
%\let\start@align@nopar\start@align
%\let\start@gather@nopar\start@gather
%\let\start@multline@nopar\start@multline
%% Add the "empty line" command to the macros
%\long\def\start@align{\par\start@align@nopar}
%\long\def\start@gather{\par\start@gather@nopar}
%\long\def\start@multline{\par\start@multline@nopar}
%\makeatother
\usepackage{etoolbox} %% <- for \pretocmd, \apptocmd and \patchcmd

%% Patch 'normal' math environment: (currently unused, but good to have)
% \newcommand*\linenomathpatch[1]{%
%   \expandafter\pretocmd\csname #1\endcsname {\linenomath}{}{}%
%   \expandafter\pretocmd\csname #1*\endcsname{\linenomath}{}{}%
%   \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}%
%   \expandafter\apptocmd\csname end#1*\endcsname{\endlinenomath}{}{}%
% }
%% Patch AMS math environment:
\newcommand*\linenomathpatchAMS[1]{%
  \expandafter\pretocmd\csname #1\endcsname {\linenomathAMS}{}{}%
  \expandafter\pretocmd\csname #1*\endcsname{\linenomathAMS}{}{}%
  \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}%
  \expandafter\apptocmd\csname end#1*\endcsname{\endlinenomath}{}{}%
}

%% Definition of \linenomathAMS depends on whether the mathlines option is provided
\expandafter\ifx\linenomath\linenomathWithnumbers
  \let\linenomathAMS\linenomathWithnumbers
  %% The following line gets rid of an extra line numbers at the bottom:
  \patchcmd\linenomathAMS{\advance\postdisplaypenalty\linenopenalty}{}{}{}
\else
  \let\linenomathAMS\linenomathNonumbers
\fi

% \linenomathpatch{equation} %% <- unnecessary, equation is already patched
\linenomathpatchAMS{gather}
\linenomathpatchAMS{multline}
\linenomathpatchAMS{align}
\linenomathpatchAMS{alignat}
\linenomathpatchAMS{flalign}



==> pm-rk-con-ten-GH-article-(cpc-submission)/main-theorem-proof.tex <==
\section{Proof of Main Theorem}\label{sec:proof-of-main-results}

For now, we do not make any assumptions on the graph parameter $f$;
we will introduce more assumptions as needed to prove the desired statements.
When we speak of submonoids, subrings and subalgebras we require
that the multiplicative identity coincide with that of the larger structure.
When a subset with the induced operations forms a monoid, ring or algebra
we will simply say that it is respectively
a monoid, ring or algebra in the larger structure. 
We \emph{allow} zero algebras and rings, in which $0 = 1$. 
Statements about such structures can be easily checked. 
%For convenience, we will assume that the product of "zero" elements in a multiplicative structure,
%be it a monoid, ring or algebra is its (multiplicative) identity.
A function of arity zero is a scalar.
We identify a (labeled) graph with its (labeled) graph isomorphism class.

\subsection{The monoid and algebra of graphs}\label{subsec:monoid-and-algebra-of-graphs}

For every finite set $S \subseteq \posints$, we denote
by $U_S$ the graph with $|S|$ nodes labeled by $S$ and no edges. 
Note that $U_\emptyset = K_0$ is the empty graph.

We put all $k$-labeled graphs into a single structure as follows.
By a \textit{partially labeled graph} we mean a finite graph
in which some of the nodes are labeled by distinct positive integers.
(All label sets are finite.)
Two partially labeled graphs are \textit{isomorphic}
if there is an isomorphism between them preserving all labels.
For two partially labeled graphs $G_1$ and $G_2$,
let $G_1 G_2$ denote the partially labeled graph
obtained by taking the disjoint union of $G_1$ and $G_2$,
and identifying the nodes with the same label;
the union of the label sets becomes the labels of $G_1 G_2$.
This way we obtain a commutative monoid $\calPLG$
consisting of all isomorphism classes of finite partially labeled graphs
with the empty graph $U_\emptyset$ being the identity~\footnote{In \cite{Freedman-Lovasz-Schrijver-2007},
the word semigroup instead of monoid is used.
A monoid is a semigroup with identity,
and all semigroups in~\cite{Freedman-Lovasz-Schrijver-2007}
have or assume to have identity.
Thus, our use of the term monoid is consistent with that of~\cite{Freedman-Lovasz-Schrijver-2007}.}.
For every finite set $S \subseteq \posints$,
we call a partially labeled graph $S$\textit{-labeled},
if its labels form the set $S$.
We call a partially labeled graph ${\subseteq} S$\textit{-labeled},
if its labels form a subset of $S$.
%So every $S$-labeled graph is automatically an ${\subseteq} S$-labeled graph.
We define $\calPLG(S)$ and $\calPLG_\subseteq(S)$
  to be the subsets of $\calPLG$
consisting of all isomorphism classes of $S$-labeled
and ${\subseteq} S$-labeled graphs, respectively.
Clearly $\calPLG(S) \subseteq \calPLG_\subseteq(S)$.
%Next, we define $\calPLG_\subseteq(S)$ to be the subset of $\calPLG$
%consisting of all isomorphism classes of ${\subseteq} S$-labeled graphs.
Then both $\calPLG(S)$ and $\calPLG_\subseteq(S)$ are commutative monoids in $\calPLG$.
$\calPLG_\subseteq(S)$ is a submonoid of $\calPLG$
with the same identity $U_\emptyset$,
while  $\calPLG(S)$ is a submonoid of $\calPLG$ iff $S = \emptyset$,
as the identity in $\calPLG(S)$ is $U_S$.

%Given a monoid $M$, we call a map $g \colon M \to \bbF$ a \textit{(monoid) character}
%if $g$ is a monoid homomorphism, where $\bbF$ is viewed as a monoid under multiplication.
%That is, $g$ is a character iff $g(e) = 1$ where $e$ is the identity in $M$
%and $g(a b) = g(a) g(b)$ for all $a, b \in M$.
%Note that we allow $g$ to take zero values.
%Let $\bbF M$ be the monoid algebra of $M$ over $\bbF$,
%which consists of formal finite linear combinations of $M$.
%Extending $g$ by linearity we can assume that
%$g \colon \bbF M \to \bbF$ is an algebra homomorphism.
%Clearly, this correspondence is a bijection between the characters from $M$ to $\bbF$
%and the algebra homomorphisms from $\bbF M$ to $\bbF$,
%so we can implicitly identify one with another.

%%{\color{red} (added the definitions of quantum graphs)
%

Let $\mathcal G$ denote the
 monoid algebra $\bbF \calPLG$ consisting of all finite formal
linear combinations in $\calPLG$ with coefficients from $\bbF$;
they are called (partially labeled, $\bbF$-)\textit{quantum graphs}.
Restricting the labels to precisely $S$ or to subsets of $S$, 
we have $\bbF \calPLG(S)$ or $\bbF \calPLG_\subseteq(S)$,
 the algebras of  $S$-labeled or  $\subseteq S$-labeled 
\textit{quantum graphs},
denoted  by  $\calG(S)$ or $\calG_\subseteq(S)$, respectively.
$\calG(S)$ is  
an algebra inside $\calG$ with $U_S$ being the multiplicative identity,
and $\calG_\subseteq(S)$ is a subalgebra of $\calG$.
%with $U_\emptyset$ being the identity in both.
The empty sum is the additive identity in all.

%
%A (partially labeled, $\bbF$-)\textit{quantum graph} is a finite formal 
%linear combination of finite   with coefficients from $\bbF$.
%linear combination)
%An $S$-labeled  ($\bbF$-)\textit{quantum graph} is a finite formal 
%linear combination (with coefficients from $\bbF$)
%of finite  $S$-labeled graphs. 
%The notion of a $\subseteq S$-labeled ($\bbF$-)\textit{quantum graph} is 
%defined analogously.
%%When the label sets of the constituent graphs 
%%(with nonzero coefficients) are precisely
%%$S$ ($\subseteq S$)-labeled graphs,
%%we call such a quantum graph an $S$ ($\subseteq S$)-labeled \textit{quantum graph}.
%%%((alternative phrasing) An $S$ ($\subseteq S$)-labeled \textit{quantum graph} is a finite formal linear 
%%%combination of finite  $S$ ($\subseteq S$)-labeled) graphs.)
%%%If the coefficients come from $\bbF$ we call these objects
%%%(partially, $S$ or $\subseteq S$-labeled) $\bbF$-quantum graphs, respectively.
%%%}
%
%Let $\mathcal G$ denote the monoid algebra $\bbF \calPLG$,
%i.e., the (infinite dimensional) vector space of
%finite formal $\bbF$-linear combinations of elements of $\calPLG$,
%or, {\color{red}(need to have a specifier) partially labeled} $\bbF$-quantum graphs. 
%Restricting the label set,
%for every finite set $S \subseteq \posints$,
%we have the monoid algebra $\calG(S) = \bbF \calPLG(S)$.
%This is an algebra inside $\calG$ with $U_S$ being the identity. 
%We also have the monoid algebra $\calG_\subseteq(S) = \bbF \calPLG_\subseteq(S)$.
%This $\calG_\subseteq(S)$ is a subalgebra of $\calG$,
%%with $U_\emptyset$ being the identity in both. 

%Let us consider the case
%when $f = \hom(\cdot, H)$ for some weighted graph $H$.
%For every map $\Phi \colon \posints \to V(H)$,
%and every partially labeled graph $G$ with the label set $S$,
%we define $\hom_\Phi(G, H) = \hom_{\Phi|_S}(G, H)$,
%(see Equation (\ref{eqn:partial-hom-dec})).
%Equation (\ref{eqn:partial-hom-mult}) implies that the function $\hom_\Phi(\cdot, H)$ is a 
%character of the monoid $\calPLG(S)$ and formula (\ref{eqn:full-hom-dec}) gives 
%an expression of $f$ as a linear combination of these 
%characters (from $\calPLG(S)$ to $\bbF$).
%{\color{red} (the actual labels make no difference, that's why the transition $[k] \to S$ is fine)}

Because many definitions, notations and statements
for $\calPLG(S), \calG(S)$ and $\calPLG_\subseteq(S), \calG_\subseteq(S)$ appear similar, 
we will often commingle them to minimize repetitions,
e.g., we use $\calG_{(\subseteq)}(S)$ to denote
either $\calG(S)$ or $\calG_\subseteq(S)$ (and the statements are asserted for both).

We can extend $f$ to a linear map on $\calG$, and
define an $n$-fold multilinear form,  where $n \ge 1$,
\[
\langle x_1, \ldots, x_n \rangle_{(n)} = f(x_1 \cdots x_n),~~~~~~\mbox{for}~~
x_1, \ldots, x_n \in  \calG.
\]
%for every $n \ge 1$ and $x_1, \ldots, x_n \in \calG$.
%for $x_1, \ldots, x_n \in \calG$.  
It is symmetric because $\calG$ is commutative.
Note that if we restrict each argument to $\calG[k]$
and then write it with respect to the basis $\calPLG[k]$ of $\calG[k]$,
we get precisely the connection tensor (array) $T(f, k, n)$.

Let
%\[
%\calK = \{ x \in \calG \colon f(x y) = \langle x, y \rangle = 0 \ \forall y \in \calG \}
%\]
\[
\calK = \{ x \in \calG \mid \forall y \in \calG, \, f(x y) = \langle x, y \rangle = 0 \}
\]
be the annihilator of $\calG$.
Clearly, $\calK$ is an ideal in $\calG$,
so we can form the quotient algebra $\hat \calG = \calG / \calK$
which is commutative as well.
We denote its identity by $u_\emptyset = U_\emptyset + \calK$.
More generally, we denote $u_S = U_S + \calK$
 for any finite subset $S \subseteq \posints$.
%Furthermore, 
If $x \in \calK$, then $f(x) = f(x U_\emptyset) = 0$
and so $f$ can also be considered as a linear map on $\hat \calG$
by $f(x + \calK) = f(x) + \calK$ for $x \in \calG$.
For a partially labeled graph $G$ we 
denote by $\hat G = G + \calK$ the corresponding element of $\hat \calG$.
More generally, we write $\hat x = x + \calK$ for any $x \in \calG$. 
Since $\calK$ is an ideal in $\calG$, the form
$\langle \cdot, \ldots, \cdot \rangle_{(n)}$ on $\calG$ induces
an $n$-fold multilinear symmetric form on $\hat \calG$,  where $n \ge 1$, 
%\[
\begin{equation}\label{eqn:f-on-hat-calG}
\langle x_1, \ldots, x_n \rangle_{(n)} = f(x_1 \cdots x_n),~~~~~~\mbox{for}~~
x_1, \ldots, x_n \in \hat \calG.
\end{equation}
%\]
%for every $n \ge 1$ and $x_1, \ldots, x_n \in \hat \calG$.
%for $x_1, \ldots, x_n \in \hat \calG$.

%{\color{red} (remove)
%
%If $S, T \subseteq \posints$ are finite subsets,
%then $\calPLG_{(\subseteq)}(S) \, \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$
%so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$. 
%%Going to the quotients, we conclude that $\hat \calG_{(\subseteq)}(S) \, \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cap T)$.
%}

We can also define
\[
\hat \calG_{(\subseteq)}(S) = (\calG_{(\subseteq)}(S) + \calK) / \calK = \{ x + \calK \mid x \in \calG_{(\subseteq)}(S) + \calK \}
= \{ x + \calK \mid x \in \calG_{(\subseteq)}(S)\}.
\]
%Then
%\[
%\hat \calG_{(\subseteq)}(S) = \{ x + \calK \mid x \in \calG_{(\subseteq)}(S)\}.
%\]
It is easy to see that $\hat \calG_\subseteq(S)$ is a subalgebra of $\hat \calG$
with the same identity $u_\emptyset = U_\emptyset + \calK$,
and $\hat \calG(S)$ is an algebra inside $\hat \calG$
with the identity $u_S = U_S + \calK$.~\footnote{In contrast to \cite{Freedman-Lovasz-Schrijver-2007}
we cannot in general normalize $f$ to make all elements $u_S$
the same in the quotient algebra $\hat \calG$,
 for various finite $S \subseteq \posints$.
This is because in our more general setting, it is possible $f(K_1) = 0$,
in which case the normalization step from \cite{Freedman-Lovasz-Schrijver-2007} fails.
For graph parameters expressible as a graph homomorphism function, this corresponds to the case when all vertex weights sum to $0$.}
% which is possible for any $\bbF$ since we do not place any restrictions on the vertex weights other than them being nonzero. (JYC: Steffen's comment asked to elaborate, I believe it makes sense, may compress the sentence)}}.
%\sout{$\calK$ is also an ideal in $\calG_{(\subseteq)}(S) + \calK$ and therefore $(\calG_{(\subseteq)}(S) + \calK) / \calK$ is an algebra (a subalgebra, resp.) in $\calG / \calK$.}

%{\color{red} (added here)

If $S, T \subseteq \posints$ are finite subsets,
then $\calPLG_{(\subseteq)}(S) \cdot \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$
so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$
and so, going to the quotients, we have $\hat \calG_{(\subseteq)}(S) \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cup T)$.
Also note that for a finite $S \subseteq \posints$,
we have $\calPLG(S) \subseteq \calPLG_\subseteq(S)$
so by linearity $\calG(S) \subseteq \calG_\subseteq(S)$
and then by going to the quotients we obtain $\hat \calG(S) \subseteq \hat \calG_\subseteq(S)$.
%}

Since
% $\calK$ is an ideal in $\calG$,
%we also have that 
$\calG_{(\subseteq)}(S) \cap \calK$ is an ideal in $\calG_{(\subseteq)}(S)$,
 we can also form 
another quotient algebra 
\[
\tilde \calG_{(\subseteq)}(S) = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK).
\] 
%%%
%
%{\color{red} (say it here instead)
%If $S, T \subseteq \posints$ are finite subsets, then $\calPLG_{(\subseteq)}(S) \, \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$ so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$
%and so, going to the quotitents, we have $\hat \calG_{(\subseteq)}(S) \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cup T)$.
%Also note that for a finite $S \subseteq \posints$, we have $\calPLG(S) \subseteq \calPLG_\subseteq(S)$ so by linearity $\calG(S) \subseteq \calG_\subseteq(S)$
%and then by going to the quotients we obtain $\hat \calG(S) \subseteq \hat \calG_\subseteq(S)$.}
%
%%%
%The following lemma provides us with canonical isomorphisms. {\color{red} (change the sentence)}
We have the following
 canonical isomorphisms between $\tilde \calG_{(\subseteq)}(S)$
 and $\hat \calG_{(\subseteq)}(S)$.
\begin{claim}\label{lem:calG(subseteq)(S)/calK(subseteq)S-canonical-isomorphism} %lemma
Let $S \subseteq \posints$ be finite. Then $\tilde \calG_{(\subseteq)}(S) \cong \hat \calG_{(\subseteq)}(S)$ as algebras via $x + \calG_{(\subseteq)}(S) \cap \calK \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$.
\end{claim}
\begin{proof}
It follows from
the 
%standard 
Second Isomorphism Theorem for algebraic structures
(see~\cite{Cohn-book} p.~8).
%(e.g., see page 8 of~\cite{Cohn-book}).
%, or \cite{Jacobson-book}). 
%
%We repeat the standard proof of the Second Isomorphism Theorem for algebraic structures.
%
%Obviously, the map $\calG_{(\subseteq)}(S) \mapsto (\calG_{(\subseteq)}(S) + \calK) / \calK,\, x \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$ is a surjective algrebra homormophism with the kernel equal to $\calG_{(\subseteq)}(S) \cap \calK$ which is an ideal in $\calG_{(\subseteq)}(S)$. Then this map factors through $\calG_{(\subseteq)}(S) / \calK_S$ resulting in an algebra isomorphism between $\tilde \calG_{\subseteq}(S) = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK)$ and $\hat \calG_{(\subseteq)}(S) = \calG_{(\subseteq)}(S) / \calK$ given by $x + \calK_S \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$.
\end{proof}

For finite $S \subseteq \posints$,
it is convenient to treat the algebras $\tilde \calG_{(\subseteq)}(S)$ and $\hat \calG_{(\subseteq)}(S)$ as separate objects
despite this isomorphism in Claim~\ref{lem:calG(subseteq)(S)/calK(subseteq)S-canonical-isomorphism}.
As it will be seen later, the algebras $\tilde \calG(S)$ with $S = [k]$, where $k \ge 0$, are naturally associated with the $k$th connection tensors $T(f, k, n), n \ge 0$. %($|S| = k$)
Later we will need to work with various finite $S \subseteq \posints$ simultaneously and need an ambient algebra in which dependencies between elements can be established.
The algebras $\tilde \calG(S)$ do not naturally possess this property as they are the quotients of the algebras $\calG(S)$ which have no common element except $0$.
However, the fact that $\hat \calG(S) \subseteq \hat \calG$ for any finite $S \subseteq \posints$
will allow us to establish dependencies between their elements.
In other words, $\hat \calG$ will serve as the ambient algebra in which further derivations will take place.
Next, the $\subseteq$-definitions will be needed to define a projection $\hat \pi_S \colon \calG \to \calG_\subseteq(S)$ (see Claims~\ref{lem:projection-and-preimage-of-calK-ideals} and~\ref{lem:quotion-decomposition-through-projeciton}). This projection will be used later in the proof. 
%(JYC: can say in subsection ``Putting things together''; not sure if we need to refer to Claims~\ref{lem:projection-and-preimage-of-calK-ideals} and~\ref{lem:quotion-decomposition-through-projeciton})
%
%(JYC, added that justification to explain the difference between $\tilde \calG_{(\subseteq)}(S)$ and $\hat \calG_{(\subseteq)}(S)$
%why it's not desirable to use only one version; we already talk about projections, I suppose this is the right place for this paragraph.)}

We say that elements $x, y \in \calG \,(\text{or } \hat \calG)$
are orthogonal (with respect to $f$),
if $f(x y) = 0$ and denote it by $x \perp y$.
For a subset $A \subseteq \calG \,(\text{or } \hat \calG)$, 
%denote by $A^\perp = \{ x \in \calG \,(\text{or } \hat \calG) \mid x \perp y, \, \forall y \in A \}$
denote by $A^\perp = \{ x \in \calG \,(\text{or } \hat \calG) \mid \forall y \in A, \, x \perp y\}$
 the set of those elements  in $\calG \,(\text{or } \hat \calG)$ orthogonal to all elements in $A$.
Next, we say that subsets $A, B \subseteq \calG \,(\text{or } \hat \calG)$
are orthogonal (with respect to $f$),
if $x \perp y$ for all $x \in A$ and $y \in B$.
Similarly, we can talk about an element of $\calG \,(\text{or } \hat \calG)$
being orthogonal to a subset of $\calG \,(\text{or } \hat \calG)$ and vice versa.
Note that the notion of orthogonality is symmetric
since all the multiplication operations considered are commutative.
From the definition, we have $\calK = \calG^\perp$.
Next, denote (commingling the notations $\calK_S$ and $\calK_{\subseteq S}$)
%\[
%\calK_{(\subseteq) S} = \{ x \in \calG_{(\subseteq)} (S) \mid x \perp y, \ \forall y \in \calG_{(\subseteq)}(S) \} = \calG_{(\subseteq)}(S) \cap (\calG_{(\subseteq)}(S))^\perp.
%\]
\[
\calK_{(\subseteq) S} = \{ x \in \calG_{(\subseteq)} (S) \mid \forall y \in \calG_{(\subseteq)}(S), \, x \perp y \} = \calG_{(\subseteq)}(S) \cap (\calG_{(\subseteq)}(S))^\perp.
\]
Clearly, $\calK_{(\subseteq) S}$ is an ideal in $\calG_{(\subseteq)}(S)$,
so we can form yet another quotient algebra $\calG_{(\subseteq)}(S) / \calK_{(\subseteq) S}$. 

Next, we define an orthogonal projection
from $\hat \calG$ to the subalgebra $\hat \calG_\subseteq(S)$.
We will show how to do it in a series of lemmas.
Let $S \subseteq \posints$ be finite.
For every partial labeled graph $G$,
let $G_S$ denote the ${\subseteq} S$-labeled graph obtained by deleting
the labels not in $S$ from the vertices of $G$ (unlabeling such vertices).
Extending this map by linearity,
we get a linear map $\pi_S \colon \calG \to \calG_\subseteq(S)$.
Note that $(\pi_S)_{| \calG_\subseteq(S)} = \id_{|\calG_\subseteq(S)}$.
In particular, $\pi_S \colon \calG \to \calG_\subseteq(S)$ is surjective.

\begin{claim}\label{lem:projection} %lemma
Let $S \subseteq \posints$ be finite.
If $x \in \calG$ and $y \in \calG_\subseteq(S)$, then
\[
f(x y) = f(\pi_S(x) y).
\]
\end{claim}
\begin{proof}
For every $G_1 \in \calPLG$ and $G_2 \in \calPLG_\subseteq(S)$,
the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic as unlabeled graphs.
Hence $f(G_1 G_2) = f(\pi_S(G_1) G_2)$ as $f$ ignores labels.
The claim follows by linearity.
%{\color{red}, because only the labeled vertices that belong to the intersection of the label sets of $G_1$ and $G_2$, which is a subset of $S$, are identified in $G_1 G_2$, as well as in $\pi_S(G_1) G_2$.}
\end{proof}

\begin{claim}\label{cor:projection-part-orthogonality} %corollary
Let $S \subseteq \posints$ be finite.
If $x \in \calG$, then $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
\end{claim}
\begin{proof}
Fix any $y \in \calG_\subseteq(S)$. By Claim~\ref{lem:projection},
$f(x y) = f(\pi_S(x) y)$ so $f((x - \pi_S(x)) y) = 0$.
Thus $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
\end{proof}

So for any $x \in \calG$, we can write $x = \pi_S(x) + (x - \pi_S(x))$
where $\pi_S(x) \in \calG_\subseteq(S)$, and $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
%by Corollary~\ref{cor:projection-part-orthogonality}.
This gives a decomposition $\calG = \calG_\subseteq(S) + (\calG_\subseteq(S))^\perp$.
%To get a similar decomposition into a direct sum,
To get a direct sum decomposition,
% make such a decomposition into a direct sum,
we need to pass to the quotient algebra.
But to do so properly we need some more properties.
%first  it correctly we first need to prove some statements.

\begin{claim}\label{lem:calKS} %lemma
Let $S \subseteq \posints$ be finite.
Then $\calK_S = \calG(S) \cap \calK$.
\end{claim}
\begin{proof}
Clearly,
$\calG(S) \cap \calK = \calG(S) \cap \calG^\perp \subseteq
 \calG(S) \cap (\calG(S))^\perp = \calK_S$,
% $\calK_S = \calG(S) \cap (\calG(S))^\perp \supseteq \calG(S) \cap \calG^\perp = \calG(S) \cap \calK$,
so we only need to prove the reverse inclusion. 
Let $x \in \calK_S = \calG(S) \cap (\calG(S))^\perp$.
Take any $y \in \calG$. Then
\[
f(x y) \stackrel{(1)}{=} f(x \pi_S(y)) \stackrel{(2)}{=} f(x U_S \pi_S(y)) \stackrel{(3)}{=} 0.
\]
Here step $(1)$ uses Claim~\ref{lem:projection} 
as $x \in \calG(S) \subseteq \calG_{\subseteq}(S)$;
$(2)$ is true because $x = x U_S$ for $x \in \calG(S)$;
$(3)$ is true as $\pi_S(y) \in \calG_\subseteq(S)$
so $U_S \pi_S(y) \in \calG(S)$, and as $x \in (\calG(S))^\perp$.
Then $x \in \calK$ so $x \in \calG(S) \cap \calK$,
implying $\calK_S \subseteq \calG(S) \cap \calK$.
\end{proof}

\begin{claim}\label{lem:calKsubseteqS}
Let $S \subseteq \posints$ be finite.
Then $\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap \calK$.
\end{claim}
\begin{proof}
Clearly,
$\calG_\subseteq(S) \cap \calK = \calG_\subseteq(S) \cap \calG^\perp
\subseteq  \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp = 
\calK_{{\subseteq}S}$,
% $\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp \supseteq \calG_\subseteq(S) \cap \calG^\perp = \calG_\subseteq(S) \cap \calK$,
so we only need to prove the reverse inclusion. 
Let $x \in \calK_{{\subseteq}S} = \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp$.
Take any $y \in \calG$. Then
\[
f(x y) \stackrel{(1)}{=} f(x \pi_S(y)) \stackrel{(2)}{=} 0.
\]
Here step $(1)$ uses Claim~\ref{lem:projection};
$(2)$ is true as $\pi_S(y) \in \calG_\subseteq(S)$
and $x \in (\calG_\subseteq(S))^\perp$.
Then $x \in \calK$ so $x \in \calG_\subseteq(S) \cap \calK$,
implying $\calK_{\subseteq S} \subseteq \calG_\subseteq(S) \cap \cal K$.
\end{proof}

It follows from Claims~\ref{lem:calKS}~and~\ref{lem:calKsubseteqS} that
$\calG_{(\subseteq)}(S) / \calK_{(\subseteq) S} = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK) = \tilde \calG_{(\subseteq)}(S)$
so the (canonical) isomorphism of algebras from
Claim~\ref{lem:calG(subseteq)(S)/calK(subseteq)S-canonical-isomorphism} takes the following form:
\begin{equation}\label{eqn:calG(subseteq)(S)-canonical-isomorphisms-new}
\tilde \calG_{(\subseteq)}(S) \cong \hat \calG_{(\subseteq)}(S),\quad x + \calK_{(\subseteq) S} \mapsto x + \calK,\quad x \in \calG_{(\subseteq)}(S).
\end{equation}

\begin{claim}\label{lem:projection-and-preimage-of-calK-ideals}
Let $S \subseteq \posints$ be finite.
For the linear map $\pi_S \colon \calG \to \calG_\subseteq(S)$
we have $\pi_S(\calK) = \calK_{{\subseteq}S}$.
\end{claim}
\begin{proof}
Because $(\pi_S)_{| \calG_\subseteq(S)} = \id_{|\calG_\subseteq(S)}$ and by Lemma~\ref{lem:calKsubseteqS}
$\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap \calK$,
we infer that $\pi_S(\calK) \supseteq \calK_{{\subseteq}S}$.
For the reverse inclusion, let $x \in \calK$.
Fix any $y \in \calG_\subseteq(S)$.
Then by Claim~\ref{lem:projection}, $f(\pi_S(x) y) = f(x y) = 0$,
the last equality is true because $x \in \calK$.
Hence $\pi_S(x) \in \calK_{{\subseteq}S}$
so that $\pi_S(\calK) \subseteq \calK_{{\subseteq}S}$.
\end{proof}

For the linear map $\pi_S \colon \calG \to \calG_\subseteq(S) \subseteq \calG$
by Lemmas~\ref{lem:projection-and-preimage-of-calK-ideals} and~\ref{lem:calKsubseteqS},
$\pi_S(\calK) = \calK_{{\subseteq}S} = \calG_{\subseteq}(S) \cap \calK$,
so that we have the well-defined linear map (which we denote by $\hat \pi_S$)
\begin{equation}\label{eqn:quotient-projection}
\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S),\quad \hat \pi_S(x + \calK) = \pi_S(x) + \calK,\quad x \in \calG.
\end{equation}
 
It is easy to see that $(\hat \pi_S)_{| \hat \calG_\subseteq(S)} = \id_{|\hat \calG_\subseteq(S)}$.
In particular, $\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$ is surjective.
 
\begin{claim}\label{lem:quotion-decomposition-through-projeciton}
Let $S \subseteq \posints$ be finite. Then $\hat \calG = \hat \calG_\subseteq(S) \oplus (\hat \calG_\subseteq(S))^\perp$ via $x = \hat \pi_S(x) + (x - \hat \pi_S(x)),\, x \in \hat \calG$.
\end{claim}
\begin{proof}
%First, let $x \in \hat \calG$. Write $x = y + \calK$ where $y \in \calG$. Then $\hat \pi_S(x) = \pi_S(y) + \calK$ and $\pi_S(y) \in \calG_\subseteq(S)$ so $\hat \pi_S(x) \in \hat \calG_\subseteq(S)$.
%Also $x - \hat \pi_S(x) = y - \pi_S(y) + \calK$. By Claim~\ref{cor:projection-part-orthogonality}, $y - \pi_S(y) \in (\calG_\subseteq(S))^\perp$ so that $x - \hat \pi_S(x) \in (\hat \calG_\subseteq(S))^\perp$.
%
%So we only need to show that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0 (= \calK)$. Let $z$ belong to this intersection.
%Write $z = t + \calK = t' + \calK$ where $t \in \calG_\subseteq(S)$
%and $t' \in (\calG_\subseteq(S))^\perp$. Then $t-t' \in  \calK$,
%and so $t \in (\calG_\subseteq(S))^\perp$.
%Thus $t \in \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp
%= \calK_{{\subseteq}S} \subseteq \calK$, the last inclusion holds by Lemma~\ref{lem:calKsubseteqS}. 
%Therefore $z = t + \calK = \calK$, implying that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0$.

%%%corrected proof
First, let $x \in \hat \calG$. Write $x = y + \calK$ where $y \in \calG$.
Then $\hat \pi_S(x) = \pi_S(y) + \calK$ and $\pi_S(y) \in \calG_\subseteq(S)$.
We have $x - \hat \pi_S(x) = y - \pi_S(y) + \calK$.
By Claim~\ref{cor:projection-part-orthogonality}, $y - \pi_S(y) \in (\calG_\subseteq(S))^\perp$
so that $x - \hat \pi_S(x) \in (\hat \calG_\subseteq(S))^\perp$,
since the bilinear form on $\calG$ extends to $\hat \calG$ in~(\ref{eqn:f-on-hat-calG}).

So we only need to show that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0 (= \{\calK\})$.
Let $z$ belong to this intersection.
Write $z = t + \calK = t' + \calK$ where $t \in \calG_\subseteq(S)$
and $t' \in (\calG_\subseteq(S))^\perp$.
Then clearly $t - t' \in  \calK \subseteq (\calG_{\subseteq}(S))^\perp$,
%%% i removed ( and ) in \calG_{(\subseteq)}(S)
and so $t = (t - t') + t' \in (\calG_\subseteq(S))^\perp$.
Thus $t \in \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp = \calK_{{\subseteq}S} \subseteq \calK$,
the last inclusion holds by Claim~\ref{lem:calKsubseteqS}. 
Therefore $z = t + \calK = \calK$,
implying that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0$.
\end{proof}

Thus Claim~\ref{lem:quotion-decomposition-through-projeciton} allows us
to rightfully call $\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$
an orthogonal projection of $\hat \calG$ to $\hat \calG_\subseteq(S)$.

If $S, T \subseteq \posints$ are finite subsets,
then $\pi_S(\calPLG_{(\subseteq)}(T)) = \calPLG_{(\subseteq)}(S \cap T)$,
where the projection is surjective because
the restriction $(\pi_S)_{| \calPLG_{(\subseteq)}(S \cap T)} = \id_{|\calPLG_{(\subseteq)}(S \cap T)}$.
So by linearity we get $\pi_S(\calG_{(\subseteq)}(T)) = \calG_{(\subseteq)}(S \cap T)$.
Going to the quotients, we conclude that $\hat \pi_S(\hat \calG_{(\subseteq)}(T)) = \hat \calG_{(\subseteq)}(S \cap T)$.

\begin{claim}\label{lem:orthogonal-complement-equivalence-for-calG(subseteq)(S)}
Let $n \ge 2$ and $S \subseteq \posints$ be finite.
Then for any $x \in \calG_{(\subseteq)}(S)$, we have $x \in \calK_{(\subseteq) S}$
iff $f(x x_1 \cdots x_{n - 1}) = 0$ for all $x_1, \ldots, x_{n - 1} \in \calG_{(\subseteq)}(S)$.
\end{claim}
\begin{proof}
%For $\Rightarrow$, it suffices to note that $\calG_{(\subseteq)}(S)$ is 
%closed under multiplication (in $\calG$). To prove $\Leftarrow$, note that $n - 2 \ge 0$ and for any $y \in \calG_{(\subseteq)}(S)$, we have $f(x y) = f(x y U_0^{n - 2}) = 0$ so $x \in \calK_{(\subseteq) S}$.

%%%corrected proof
For $\Rightarrow$, it suffices to note that $\calG_{(\subseteq)}(S)$
is closed under multiplication (in $\calG$).
To prove $\Leftarrow$, note that $n - 2 \ge 0$ and for any $y \in \calG_{(\subseteq)}(S)$,
we have $f(x y) = f(x y U^{n - 2}) = 0$,
where $U = U_\emptyset$ in the $\calG_\subseteq(S)$ case and
$U = U_S$ in the $\calG(S)$ case,
so $x \in \calK_{(\subseteq) S}$.
\end{proof}

The primary goal of the various Claims above is to define the projection $\hat \pi_S \colon \calG \to \calG_\subseteq(S)$ to be used later and to prove Lemmas~\ref{lem:empty-annihilator-for-hat-calG(subseteq)(S)} and~\ref{lem:calK[k]-T(f,k,n)-xi(h)-criterion}.
% (JYC, added because the referee couldn't understand ther purpose of these lemmas)

\begin{lemma}\label{lem:empty-annihilator-for-hat-calG(subseteq)(S)}
Let $S \subseteq \posints$ be finite.
Then the annihilator of $\hat \calG_{(\subseteq)}(S)$ in $\hat \calG_{(\subseteq)}(S)$ is zero, i.e.,
if $x \in \hat \calG_{(\subseteq)}(S)$ and $f(x y) = 0$
for every $y \in \hat \calG_{(\subseteq)}(S)$, then $x$
is
the zero element of $\hat \calG_{(\subseteq)}(S)$, namely $\calK$.
%for every $y \in \hat \calG_{(\subseteq)}(S)$, then $x = \calK$.
\end{lemma}
\begin{proof}
%%% corrected proof
Let $x \in \hat \calG_{(\subseteq)}(S)$ be
an element satisfying the hypothesis of the lemma.
Write $x = h_1 + \calK$ where $h_1 \in \calG_{(\subseteq)}(S)$.
By hypothesis, for every 
$y \in \hat \calG_{(\subseteq)}(S)$ we have $f(x y) = 0$.
Let $h_2 \in \calG_{(\subseteq)}(S)$
and put $y = h_2 + \calK \in \hat \calG_{(\subseteq)}(S)$.
Then $x y = h_1 h_2 + \calK$.
By the definition of $f$ on $\hat \calG$, $f(h_1 h_2) = f(x y) = 0$. 
Hence $h_1 \in \calK_{(\subseteq) S} \subseteq \calK$
where the last inclusion is true by Claims~\ref{lem:calKS} and~\ref{lem:calKsubseteqS}.
This implies that $x$ is the  zero element of $\hat \calG_{(\subseteq)}(S)$,
which is $\calK$.
\end{proof}

\begin{lemma}\label{lem:calK[k]-T(f,k,n)-xi(h)-criterion}
Let $k, r \ge 0$ and $n \ge \max(2, r)$.
Suppose the connection tensor $T(f, k, n)$ can be expressed as
\[
T(f, k, n) = \sum_{i = 1}^r a_i \bfx_i^{\otimes n},
\]
where $a_i \ne 0$ and $\bfx_i
\in \bbF^{\calPLG[k]}$ are nonzero and \emph{pairwise} linearly independent for $1 \le i \le r$.
Then for any $h \in \calG[k]$, we have $h \in \calK_{[k]}$ iff $\bfx_i(h) = 0, \, 1 \le i \le r$.
\end{lemma}
\begin{proof}
The lemma is clearly true for $r=0$. Let $r \ge 1$.
By Claim~\ref{lem:orthogonal-complement-equivalence-for-calG(subseteq)(S)},
$h \in \calK_{[k]}$ iff $f(h h_1 \cdots h_{n - 1}) = 0$ for all $h_1, \ldots, h_{n - 1} \in \calG[k]$.
In terms of $T(f, k, n)$, this is equivalent to $(T(f, k, n))(h, \cdot, \ldots, \cdot) = 0$
which is the same as
\[
\sum_{i = 1}^r a_i \, \bfx_i(h) \, \bfx_i^{\otimes (n - 1)} = 0.
\]
Now if $\bfx_i(h) = 0, \, 1 \le i \le r$, then this equality clearly holds.
Conversely, if this equality holds, then by Lemma~\ref{lem:tensor-powers-pairwise-implies-linear-independence-long},
$a_i \bfx_i(h) = 0$ but $a_i \ne 0$ so $\bfx_i(h) = 0, \,  1 \le i \le r$.
\end{proof}

We will also need the following lemma 
that classifies all subalgebras of $\bbF^m$ for $m \ge 0$.
A proof is given in
 subsection~\ref{subsec:bbF^m-subalgebras} of the Appendix. 
%(or the Appendix (Section~\ref{sec:Preliminary-continued}).)
Recall that we allow zero algebras %(i.e., $\bbF^0 = \{ \emptyset \}$, where $0 = 1 = \emptyset$)
and require any subalgebra of an algebra to share the multiplicative identity.
%{\color{red} with the larger algebra (added)}.

\begin{lemma}\label{lem:F^m-subalgebras}
All subalgebras of $\bbF^m$, where $m \ge 0$, are of the following form:
For some partition $[m] = \bigsqcup_{i = 1}^s \calI_i$,
where $s \ge 0$, and $\calI_i \ne \emptyset$ for $i \in [s]$, 
the subalgebra has equal values on each $I_i$,
\[
\bbF^{(\calI_1, \ldots, \calI_s)} = \{ (c_1, \ldots, c_m) \in \bbF^m \mid \forall i \in [s], \ \forall j, j' \in \calI_i, \ c_j = c_{j'} \}.
\]
\end{lemma}

\subsection{Building an algebra isomorphism~\label{sec:build-alg-isom}}

%In this part of the proof regarding $f$ we assume that for every $k \ge 0$
%there exists $n = n_k \ge 2$ such that $\symrank T(f, k, n) \le n - 1$.
%We will pick an arbitrary such $n$ and call it $n_k$,
%and then write $r_k = \symrank T(f, k, n_k)$. 
In this part of the proof regarding $f$,
for an arbitrary fixed $k \ge 0$,
we assume that
there exists $n = n_k \ge 2$ such that $\symrank T(f, k, n) \le n - 1$.
We will pick an arbitrary such $n$ and call it $n_k$,
and then write $r_k = \symrank T(f, k, n_k)$.
%% 
(Note that this is weaker than the
uniform exponential boundedness in $k$ for $\symrank T(f, k, n)$
in Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse},
nor do we require $f(K_0) = 1$ here.)
% to be (uniformly) exponentially bounded in $k$ or $f(K_0) = 1$,
%as the conditions in Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse} would require.)
% {\color{red} (require / do / just remove)}.)
%The results of this part will be valid without these assumptions.

Then, for $n = n_k$, we can write %, {(JYC, get rid of the comma)}
\begin{equation}\label{eqn:T(f,k,n)-gen-dec}
T(f, k, n) = \sum_{i = 1}^{r_{k}} a_{k, n, i} \bfx_{k, n, i}^{\otimes n}.
\end{equation}
Then $a_{k, n, i} \ne 0$ and $0 \ne\bfx_{k, n, i} \in \bbF^{\calPLG[k]}$ 
are pairwise linearly independent for $1 \le i \le r_{k}$.

Define the linear map
\begin{equation}\label{eqn:Phi-map}
\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}},\quad \Phi_{k, n}(h) = ( \bfx_{k, n, i}(h) )_{i= 1, \ldots, r_{k}}, \quad h \in \calG[k].
\end{equation}
We show that $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$
is a surjective algebra homomorphism,  
after a normalization step (to be carried out later).
% (algebra epimorphism).
Clearly, as $n \ge 2$, 
%{\color{red} (check the commas)}
\[
h_1 \cdot h_2 \cdot h_3 \cdots h_n = (h_1 h_2) \cdot U_k \cdot h_3 \cdots h_n
\]
so
\[
f(h_1 \cdot h_2 \cdot h_3 \cdots h_n) = f((h_1 h_2) \cdot U_k \cdot h_3 \cdots h_n)
\]
for all $h_1, \ldots, h_n \in \calG[k]$.
(When $n = 2$ this is $f(h_1 h_2) = f((h_1 h_2) U_k)$.)
Therefore
\[
(T(f, k, n))(h_1, h_2, \cdot, \ldots, \cdot) =  (T(f, k, n))(h_1 h_2, U_k, \cdot, \ldots, \cdot)
\]
for all $h_1, h_2 \in \calG[k]$.
In terms of the decomposition in (\ref{eqn:T(f,k,n)-gen-dec}),
this is equivalent to 
\[
\sum_{i = 1}^{r_{k}} \, a_{k, n, i} \, \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) \, \bfx_{k, n, i}^{\otimes (n - 2)} = \sum_{i = 1}^{r_{k}} a_{k, n, i} \, \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k) \, \bfx_{k, n, i}^{\otimes (n - 2)}.
\]
It follows that
\[
\sum_{i = 1}^{r_{k}} a_{k, n, i} \, \left( \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) - \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k) \right) \, \bfx_{k, i}^{\otimes (n - 2)} = 0
\]
for any $h_1, h_2 \in \calG[k]$.
The condition $r_{k} \le n - 1$ allows
us to apply Lemma~\ref{lem:tensor-powers-pairwise-implies-linear-independence-long}.
Since $a_{k, n, i} \ne 0$ for $1 \le i \le r_{k}$,
we obtain that
\begin{equation}\label{eqn:char-prop-unsimp}
\bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) = \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k), \quad h_1, h_2 \in \calG[k], \quad 1 \le i \le r_{k}.
\end{equation}
Let $1 \le i \le r_{k}$.
Since $\bfx_{k, n, i} \ne 0$, there exists $h \in \calG[k]$ such that $\bfx_{k, n, i}(h) \ne 0$.
Substituting $h_1 = h_2 = h$ into (\ref{eqn:char-prop-unsimp}),
we infer that $\bfx_{k, n, i}(U_k) \ne 0, \, 1 \le i \le r_{k}$.

Therefore we can assume
in (\ref{eqn:T(f,k,n)-gen-dec})
 that each $\bfx_{k, n, i}$ is normalized so that $\bfx_{k, n, i}(U_k) = 1$ ($1 \le i \le r_{k}$).
Combined with this, condition (\ref{eqn:char-prop-unsimp}) becomes for $1 \le i \le r_{k}$,
\begin{equation}\label{eqn:char-prop-simp-full}
\begin{lcases}
\bfx_{k, n, i}(h_1 h_2) &= \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2), \quad h_1, h_2 \in \calG[k]; \\
\bfx_{k, n, i}(U_k) &= 1;
\end{lcases}
\end{equation}
so the linear functions $\bfx_{k, n, i} \colon \calG[k] \to \bbF, \, 1 \le i \le r_{k}$
are algebra homomorphisms. %(equivalently, characters from $\calPLG[k]$ to $\bbF$).
Then we have
\begin{gather*}
\Phi_{k, n}(g h) = ( \bfx_{k, n, 1}(g h), \ldots, \bfx_{k, n, r_k}(g h) ) = ( \bfx_{k, n, 1}(g) \, \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(g) \, \bfx_{k, n, r_k}(h)) \\
= ( \bfx_{k, n, 1}(g), \ldots, \bfx_{k, n, r_k}(g) ) \cdot ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ) = \Phi_{k, n}(g) \Phi_{k, n}(h). 
\end{gather*}
So we have
\begin{gather*}
\Phi_{k, n}(g h) = \Phi_{k, n}(g) \Phi_{k, n}(h), \quad g, h \in \calG[k], \\
\Phi_{k, n}(U_k) = ( \bfx_{k, n, 1}(U_k) \ldots, \bfx_{k, n, r_k}(U_k) ) = \underbrace{(1, \ldots, 1)}_{r_{k} \text{ times}} \in \bbF^{r_{k}},
\end{gather*}
and therefore $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$ is an algebra homomorphism.
We now prove its surjectivity.
Clearly, $\im(\Phi_{k, n})$ is a subalgebra of $\bbF^{r_{k}}$.
By Lemma~\ref{lem:F^m-subalgebras},
we may assume that $\im(\Phi_{k, n})$
has the form $\bbF^{(\calI_1, \ldots, \calI_s)}$ for some partition
$\{\calI_1, \ldots, \calI_s\}$ of $[r_{k}]$.
The pairwise linear independence of $\bfx_{k, n, i}$
for $1 \le i \le r_{k}$ implies that for any $1 \le i_1 < i_2 \le r_{k}$,
we have $\bfx_{k, n, i_1} \ne \bfx_{k, n, i_2}$,
so there exists $h \in \calG[k]$ such that $\bfx_{k, n, i_1}(h) \ne \bfx_{k, n, i_2}(h)$.
Since each $\calI_i \ne \emptyset$,
it follows that $|\calI_i| = 1$ for $1 \le i \le s$.
Hence $\im(\Phi_{k, n}) = \bbF^{(\{ 1 \}, \ldots, \{ r_k \})} = \bbF^{r_{k}}$.
We have shown that $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$ is surjective.

This results in the following lemma.
\begin{lemma}\label{lem:Phi-surjective-homomorphism}
Let $k \ge 0$. The constructed map $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$ defined in~(\ref{eqn:Phi-map}) is a surjective algebra homomorphism,
after the  normalization to set $\bfx_{k, n, i}(U_k) = 1$ for $1 \le i \le r_k$.
%
%Here the statement is assumed after the normalization step to make $\bfx_{k, n, i}(U_k) = 1$ for $1 \le i \le r_k$ takes place.
\end{lemma}
%(JYC: actually, this lemma doesn't make any sense, very stupid, we must remove it, it's just only to showcase its uselessness for you, we must not address this comment, so no need for the red text)}

Next, by $r_{k} \le n - 1$ and $n \ge 2$, 
clearly $n \ge \max(2, r_{k})$, 
so Lemma~\ref{lem:calK[k]-T(f,k,n)-xi(h)-criterion} applies. So we have
\[
\ker \Phi_{k, n} = \{ h \in \calG[k] \mid \bfx_{k, n, i}(h) = 0,\,
1 \le i \le r_{k}  \} = \calK_{[k]},
\]
where the first equality is by the definition of $\Phi_{k, n}$,
and the second equality is by Lemma~\ref{lem:calK[k]-T(f,k,n)-xi(h)-criterion}.
Note that by Claim~\ref{lem:calKS}, we have $\calK_{[k]} =
\calG[k] \cap \calK$.
%
%Therefore
Then $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_k}$
factors through $\calG[k] / \ker \Phi_{k, n} = \calG[k] / \calK_{[k]} = \tilde \calG[k]$,
inducing an algebra isomorphism
\[
\tilde \Phi_{k, n} \colon \tilde \calG[k] \to \bbF^{r_{k}}, \quad \tilde \Phi_{k, n}(h + \calK_{[k]}) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \calG[k].
\]
It follows that $\dim \tilde \calG[k] = \dim \bbF^{r_{k}} = r_{k}$.
In particular, $\tilde \calG[k]$ is a finite dimensional algebra.
Applying Lemma~\ref{lem:quotient-space-dimension-long},
we get $\dim \tilde \calG[k] = \dim \Span \{ \bfx_{k, n, i} \}_{i = 1}^{r_{k}}$.
Then $\dim \Span \{ \bfx_{k, n, i} \}_{i = 1}^{r_{k}} = r_{k}$
implying that $\bfx_{k, n, i}$,  $1 \le i \le r_{k}$, are linearly independent.
(Note that we started off only assuming they are nonzero and pairwise linearly independent.)
%
We formalize some of the results obtained above.
\begin{lemma}\label{lem:Phi(k)-tilde-calG[k]-isomorphism}
%Assume for every $k \ge 0$ there exists $n = n_k \ge 2$ 
Let $k \ge 0$. Assume there exists $n = n_k \ge 2$
such that $r_{k} = \symrank T(f, k, n_k) \le n_k - 1$.
Then the constructed map
\[
\tilde \Phi_{k, n} \colon \tilde \calG[k] \to \bbF^{r_{k}}, \quad \tilde \Phi_k(h + \calK_{[k]}) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \tilde \calG[k].
\]
is an algebra isomorphism and $\dim \tilde \calG[k] = r_{k}$.
\end{lemma}

Composing $\tilde \Phi_k \colon \tilde \calG[k] \to \bbF^{r_{k}}$
with the canonical algebra isomorphism between $\tilde \calG[k]$ and $\hat \calG[k]$
given in (\ref{eqn:calG(subseteq)(S)-canonical-isomorphisms-new}),
we have an algebra isomorphism $\hat \Phi_k \colon \hat \calG[k] \to \bbF^{r_{k}}$.
In particular, $\dim \hat \calG[k] = \dim \tilde \calG[k] = r_{k}$.
\begin{corollary}\label{cor:Phi(k)-hat-calG[k]-isomorphism}
With the same assumption as in Lemma~\ref{lem:Phi(k)-tilde-calG[k]-isomorphism},
%for any $k \ge 0$,
the  map
%constructed map
\[
\hat \Phi_{k, n} \colon \hat \calG[k] \to \bbF^{r_{k}}, \quad \hat \Phi_{k, n}(h + \calK) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \hat \calG[k].
\]
is an algebra isomorphism and  $\dim \hat \calG[k] = r_{k}$.
\end{corollary}

Note that if $S \subseteq \posints$ is finite and $|S| = k$,
there are natural isomorphisms between $\tilde \calG(S)$ and $\tilde \calG[k]$
and also between $\hat \calG(S)$ and $\hat \calG[k]$,
both resulting from any bijective map between $S$ and $[k]$.
As a result, we conclude the following.
\begin{corollary}\label{cor:dimension-of-tilde-hat-calG(S)}
%Let $S \subseteq \posints$ be finite, $k = |S|$ and suppose there exists
%some $n \ge 2$ so that $\symrank(T(f, k, n))  \le n - 1$. 
%Let $n = n_k$ be any such choice, and let
%$r_k = \symrank(T(f, k, n_k))$.
%Then  $\tilde \calG(S) \cong \hat \calG(S) \cong \bbF^{r_{k}}$ and $\dim \tilde \calG(S) = \dim \hat \calG(S) = r_{k}$. In particular,
%the value $r_k$ is independent of any particular choice of $n_k$.
%
%%corrected
%{\color{red} corrected statement}
%For any $k \ge 0$ and finite $S \subseteq \posints$ with $|S| = k$,
%suppose there exists some $n \ge 2$ so that $\symrank T(f, k, n) \le n - 1$. 
%Let $n = n_k$ be any such choice where $k \ge 0$, and let $r_k = \symrank T(f, k, n_k)$.
%Then $\tilde \calG(S) \cong \hat \calG(S) \cong \bbF^{r_{k}}$
%and $\dim \tilde \calG(S) = \dim \hat \calG(S) = r_{k}$.
%In particular, the value $r_k$ is independent of any particular choice of $n_k$.
%{\color{red} corrected statement once more}
Let $k \ge 0$ and $S \subseteq \posints$ with $|S| = k$.
Suppose there exists some $n = n_k \ge 2$ so that $\symrank T(f, k, n) \le n - 1$. 
Let $r_k = \symrank T(f, k, n)$.
Then $\tilde \calG(S) \cong \hat \calG(S) \cong \bbF^{r_{k}}$
and $\dim \tilde \calG(S) = \dim \hat \calG(S) = r_{k}$.
In particular, the value $r_k$ is independent of the choice of $n$.
\end{corollary}

\subsection{One \texorpdfstring{$n$}{n} implies for all \texorpdfstring{$n$}{n}~\label{sec:one-implies-all}}

Let $n_k$ retain the same meaning
as in Lemma~\ref{lem:Phi(k)-tilde-calG[k]-isomorphism},
and let $r = r_k =  \symrank(T(f, k, n_k))$.
For any $h \in \calG[k]$, clearly
$h = h U_k^{n_k - 1}$ so $f(h) = f(h U_k^{n_k - 1})$.
As $\bfx_{k, n_k, i}(U_k) = 1, \, 1 \le i \le r$,
%Therefore
\[
\begin{split}
f(h) &= f(h U_k^{n_k - 1}) = (T(f, k, n_k))(h, U_k, \ldots, U_k) = \sum_{i = 1}^r a_{k, n_k, i} (\bfx_{k, n_k, i}(U_k))^{n_k - 1} \bfx_{k, n_k, i}(h) \\
&= \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h)
\end{split}
\]
for any $h \in \calG[k]$.
Hence $f_{|\calG[k]} = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}$, i.e.,
$f_{|\calG[k]}$ is a linear combination of $r$ algebra 
homomorphisms $\bfx_{k, n_k, i} \colon \calG[k] \to \bbF$, for $1 \le i \le r$.
In particular, applying to the product $h_1 \cdots h_n$,
for any $n \ge 0$ and  any  $h_1, \ldots, h_n \in \calG[k]$,
(note that this $n$ is arbitrary, not only for  those $n$ satisfying
the requirements for the choice of $n_k$)
\[
f(h_1 \cdots h_n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h_1 \cdots h_n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h_1) \cdots  \bfx_{k, n_k, i}(h_n).
\]
(When $n = 0$, we view it as $f(U_k) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(U_k) = \sum_{i = 1}^r a_{k, n_k, i}$.)
Hence
\begin{equation}\label{eqn:T(f,k,n)-char-dec}
T(f, k, n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}^{\otimes n}
\end{equation}
for all $n \ge 0$.
(When $n = 0$, 
%we continue the previous consideration for this case,
%so 
(\ref{eqn:T(f,k,n)-char-dec}) is still valid as
$T(f, k, 0) = f(U_k) = \sum_{i = 1}^r a_{k, n_k, i} = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}^{\otimes 0}$
where the last equality is true as $\bfx_{k, n_k, i}^{\otimes 0} = 1$.)
% by convention,
%and therefore in this case (\ref{eqn:T(f,k,n)-char-dec}) is still correct.)}

As shown before, $\bfx_{k, n_k, i}$ where $1 \le i \le r$ are linearly independent.
Then by Lemma~\ref{lem:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-long} 
applied to (\ref{eqn:T(f,k,n)-char-dec}),
we get $\symrank(T(f, k, n)) = r$ for all $n \ge 2$;
and the decomposition (\ref{eqn:T(f,k,n)-char-dec})
is actually unique up to a permutation for $n \ge 3$.

To summarize, this leads to the following. 

\begin{theorem}\label{thm:T(f,k,n)-rk-unif-dec-uniq}
Let $k \ge 0$.
Assume that for some $n = n_k \ge 2$, $\symrank T(f, k, n) = r \le n - 1$.
Then the following hold:
\begin{enumerate}
\item $\symrank T(f, k, n) = r$ for every $n \ge 2$.
\item There exist $r$ linearly independent algebra homomorphisms $\bfx_i \colon \calG[k] \to \bbF$,
and $a_1, \ldots, a_r \in \bbF \setminus \{ 0 \}$ such that $f_{|\calG[k]} = \sum_{i = 1}^r a_i \bfx_i$;
also for every $n \ge 0$,
\begin{equation}\label{eqn:T(f,k,n)-unif-dec}
T(f, k, n) = \sum_{i = 1}^r a_i \bfx_i^{\otimes n}.
\end{equation}
Moreover, for any $n \ge 3$, any expression of $T(f, k, n)$ as $\sum_{i = 1}^r b_i \bfy_i^{\otimes n}$,
where $\bfy_i \colon \calG[k] \to \bbF$ are linear maps,
is a permutation of the sum in (\ref{eqn:T(f,k,n)-unif-dec}).
\end{enumerate}
\end{theorem}

%The reader may agree that
%something very nontrivial has happened.
We remark that this  is  a nontrivial statement:
The existence of some $n_k$ has produced
a uniform expression for the tensors $T(f, k, n)$
all the way down to $n = 0$.

\subsection{Putting things together}

From now on, we assume that for every $k \ge 0$,
there exist some $n = n_k \ge 2$ such that $\symrank T(f, k, n) \le n - 1$.
For every $k \ge 0$, we pick an arbitrary such $n$, call it $n_k$,
and let $r_k = \symrank T(f, k, n_k)$.
%As before, we pick an arbitrary such $n$, call it $n_k$,
%and let $r_k = \symrank T(f, k, n_k)$ but we do it for every $k \ge 0$.
%We will pick an arbitrary such $n$ and call it $n_k$,
%and then write $r_k = \symrank T(f, k, n_k)$.

Having developed the theory in a more general setting,
we can now follow the proof in~\cite{Freedman-Lovasz-Schrijver-2007} closely.
As mentioned before, developing this theory in a more general setting
is necessary because $f(K_1) = 0$  is possible which makes
 the normalization step from~\cite{Freedman-Lovasz-Schrijver-2007} infeasible. Now the main difference from~\cite{Freedman-Lovasz-Schrijver-2007} starting from this point is that many of our derivations will additionally contain units of the form $u_S$ for various finite $S \subseteq \posints$ because we cannot ensure that $u_S = u_\emptyset$. 
%(JYC: my insertion, maybe elaborate as the referee asked, but again the stuff about normalization was already mentioned in the intro and $f(K_1) = 0$ was mentioned in the footnote so there may be complaints about the 1st sentence, and note that we actually use $u_{T / S}, u_T$ and $u_S$, but I say here $u_S$ because $S$ is arbitrary, not sure if it's fine. Or we can say ``we modify the statements to work in the extended framework'', simple as that, otherwise we will say lots of garbage)}
%%%
We will be interested in the idempotent elements of $\hat \calG$.
For two elements  $p, q \in \hat \calG$,
we say that $q$ \textit{resolves} $p$, if $p q = q$.
We also say equivalently $p$ is resolved by $q$. 
It is clear that the binary relation
\textit{resolves} is antisymmetric and transitive and,
when restricted to idempotents, reflexive.
Furthermore, it is easy to see that the binary 
relation \textit{resolves} on $\hat \calG$ has the following properties:

\begin{enumerate}
\item The idempotent $0 = \calK$ resolves everything and $1 = u_\emptyset = 
U_\emptyset + \calK = K_0 + \calK$ is resolved by everything.
\item If $a b = 0$ and $c$ resolves both $a$ and $b$, then $c = 0$;
\item If $a$ resolves $b$, then $c$ resolves  $a$ iff $c$ resolves $a b$.
\end{enumerate}

In the algebra $\bbF^r$ ($r \ge 0$), 
the idempotents are 0-1 tuples in $\bbF^r$, and for idempotents
$q = (q_1, \ldots, q_r)$ and $p = (p_1, \ldots, p_r)$,
$q$ resolves $p$ iff $q_i=1$ implies $p_i=1$.

Let $S$ be a finite subset of $\posints$ with $|S|=k$, and set $r = r_{k}$
as above.
By Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)},
$\hat \calG(S) \cong \bbF^r$ as algebras,
so $\hat \calG(S)$ has a (uniquely determined idempotent) basis $\calP_S = \{ p_1^S, \ldots, p_r^S \}$
such that $(p_i^S)^2 = p_i^S$ and $p_i^S p_j^S = 0$ for $i \ne j$.
These correspond to the canonical basis $\{e_i\}_{1 \le i \le r}$ of $\bbF^r$
under this isomorphism.
%Namely, it corresponds to the canonical basis of $\bbF^r$ under this isomorphism.
For $i \ne j$, we have $\langle p_i^S, p_j^S \rangle = f(p_i^S p_j^S) = 0$.
Furthermore, for all $1 \le i \le r$,
%$f(p_i^S) = f((p_i^S)^2) = \langle p_i^S, p_i^S \rangle \ne 0$,
\begin{equation}\label{eq:nonzero-idempotent}
f(p_i^S) = f((p_i^S)^2) = \langle p_i^S, p_i^S \rangle \ne 0,
\end{equation}
%which is obvious under the isomorphism.
otherwise $\hat \calG(S)$ contains a nonzero element orthogonal to $\hat \calG(S)$
with respect to the bilinear form $\langle \cdot, \cdot \rangle$
restricted to $\hat \calG(S) \times \hat \calG(S)$, 
contradicting Lemma~\ref{lem:empty-annihilator-for-hat-calG(subseteq)(S)}.
We will call the elements $p_i^S \in \calP_S$ basic idempotents. %(of/in $\hat \calG(S)$).

%{\color{red} From now on, when talking about label sets (such as $S, T, U$ (not a unit this time)),
%we will always assume that they are finite subsets of $\posints$ but frequently omit it.}
%
%%% this was said in beginning of sec 5: JYC added that.

We denote by $\calP_{T, p}$ the set of all idempotents in $\calP_T$
that resolve a given element $p \in \hat \calG$.
If $p \in \calP_S$ and $S \subset T$ and $|T| = |S| + 1$,
then the number of elements in $\calP_{T, p}$
will be called the degree of $p \in \calP_S$, and denoted by $\deg(p)$.
Obviously, this value is independent of
which $(|S| + 1)$-element superset $T$ of $S$ we take.

For any $q \in \hat \calG(T)$, we have $q u_{T \setminus S} = q$. (Here by definition, $u_{T \setminus S} = U_{T \setminus S} + \calK \in \hat \calG(T \setminus S) \subseteq \hat \calG(T) \subseteq \hat \calG$.) 
%(JYC: added with brackets around)
It follows that for any $S \subseteq T$ and $p \in \hat \calG$,
we have  $q$ resolves $p$ iff $q$ resolves $p u_{T \setminus S}$,
since $q p = q u_{T \setminus S} p = q p u_{T \setminus S}$.
It is also important to point out that
an element in $\hat \calG(S)$ is an idempotent in $\hat \calG(S)$
iff it is an idempotent in $\hat \calG$.

%{\color{red} (propose the following change)
%
%Since $\hat \calG(S) \cong \bbF^r$, where $r = r_{|S|} \ge 0$, (by Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)} but already mentioned before)
%the unit $u_S$ of the algebra $\hat \calG(S)$
%corresponds to the all one tuple $(1, \ldots, 1) \in \bbF^r$, where $r = r_{|S|}$,
%(when $r = r_{|S|} = 0$, it is the empty tuple),
%which is the sum of the canonical basis elements of $\bbF^r$.
%Therefore in $\hat \calG(S)$ we have
%\begin{equation}\label{eqn:uS-decomposition-in-idempotent-basis}
%u_S = \sum_{p \in \calP_S} p
%\end{equation}
%
%In fact, a more general statement is true.
%}

\begin{claim}\label{clm:idempotent-is-sum-of-its-resolving-basic-idempotents}
Let $x$ be any idempotent element of $\hat \calG(S)$.
Then $x$ is the sum of exactly those idempotents in $\calP_S$ that resolve it,
\[
x = \sum_{p \in \calP_{S, x}} p.
\]
\end{claim}
\begin{proof}
Let $k = |S|$, and $r = r_{k}$.  By the isomorphism  $\hat \calG(S) \cong \bbF^{r}$, %{\color{red} (JYC: removed $_{|S|}$)}
every 0-1 tuple $x = (x_1, \ldots, x_r) \in \bbF^r$
is the sum $\sum_{i=1}^r  x_i e_i$.
\end{proof}
%Viewed under the isomorphism  $\hat \calG(S) \cong \bbF^r$
%this is obvious: every 0-1 tuple $x = (x_1, \ldots, x_r) \in \bbF^r$
%is the sum $\sum  x_i e_i$.
%$\sum_{i: x_i =1} e_i$.
%\end{proof}
%Since $\calP_S$ is a basis, we can write $x$
%uniquely as a linear combination of $\calP_S$,
%\[
%x = \sum_{p \in \calP_S} c_p p
%\]
%with some scalars $c_x$.
%Since $x$ is an idempotent:
%\[
%x = x^2 = \sum_{p, p' \in \calP_S} c_p c_{p'} p p' = 
%\sum_{p \in \calP_S} c_p^2 p,
%\]
%which shows that $c_p^2 = c_p$ for every $p$,
%and so $c_p \in \{ 0, 1 \}$. 
%It follows that $x$ is the sum of some subset $X \subseteq \calP_S$. 
%It is clear that $x p = p$ for $p \in X$
%and $x p = 0 \ne p$ for $p \in \calP_S \setminus X$, so $X = \calP_{S, x}$,
%exactly those elements of $\calP_S$ that resolve $x$.
%\end{proof}

%As a special case, we see that
In particular
\begin{equation}\label{eqn:uS-decomposition-in-idempotent-basis}
u_S = \sum_{p \in \calP_S} p,
\end{equation}
since  $u_S \in \hat \calG(S)$ corresponds
to the all-1 tuple in $\bbF^r$.
%since every $p \in  \calP_S$ resolves $u_S$.
%{\color{red} (However, it is also clear since $\hat \calG(S) \cong \bbF^r$ where $r = r_{|S|}$ by construction.)}

\begin{claim}\label{clm:subset-inclusion-and-uniqueness-of-resolving-basic-idempotents}
Let $S \subseteq T$ be two finite sets.
Then every $q \in \calP_T$ resolves exactly one element of $\calP_S$.
\end{claim}
\begin{proof}
Let $k' = |T|$ and $r' = r_{k'}$.
Consider the idempotents $pu_{T \setminus S}$
(which could be 0) under the isomorphism $\hat \calG(T) \cong \bbF^{r'}$,
where $p \in \calP_S$.
We can write the 0-1 tuple corresponding to $pu_{T \setminus S}$
in $\bbF^{r'}$ as the sum of those canonical basis $0$-$1$ vectors.
Recall that for any $q \in \calP_T$,
$q$ resolves $p$
iff $q$  resolves $pu_{T \setminus S}$.
Note that $pu_{T \setminus S}$ must have disjoint positions with entry 1 
for distinct $p \in \calP_S$, and the sum $\sum_{p \in \calP_S} 
pu_{T \setminus S} = u_S u_{T \setminus S} = u_T$ is the all-1 
tuple in $\bbF^{r'}$. 
Thus each $q \in \calP_T$ resolves exactly one $p \in \calP_S$.
\end{proof}

%For every $p \in \calP_S$, $p u_{T \setminus S} \in \hat \calG(T)$ is
%a product of two idempotents, therefore also an idempotent.
%As an idempotent in $\hat \calG(T)$ we can write it as
%\[
%p u_{T \setminus S} = \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p u_{T \setminus S}}} q.
%\]
%Now by (\ref{eqn:uS-decomposition-in-idempotent-basis}) we have
%\[
%u_T = u_S u_{T \setminus S} = \sum_{p \in \calP_S} p u_{T \setminus S} = \sum_{p \in \calP_S} \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p u_{T \setminus S}}} q = \sum_{p \in \calP_S} \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p}} q
%\]
%and also
%\[
%u_T = \sum_{q \in \calP_T} q.
%\]
%Furthermore, for distinct $p, p' \in \calP_S$, we have $p p' = 0$,
%so they cannot be resolved by the same $q \in \calP_T$,
%for otherwise $q = p q = p p' q = 0$ which is false.
%So by the uniqueness of the expansion of $u_T$
%in the basis $\calP_T$ we get that
%\[
%\calP_T = \bigsqcup_{p \in \calP_S} \calP_{T, p} 
%\]
%as a disjoint union.
%Therefore every $q \in \calP_T$ resolves exactly one $p \in \calP_S$.
%\end{proof}
%Under the isomorphism $\hat \calG(T) \cong \bbF^{r_{|T|}}$,
%this proof is also transparent.
%Recall that $q \in \calP_T$ resolves $p \in \calP_S$
%iff $q$  resolves $pu_{T \setminus S}$, which is also an idempotent
%(although possibly 0).
%Then we can write the 0-1 tuple corresponding to $pu_{T \setminus S}$
%in $\bbF^{r_{|T|}}$ as the sum of those canonical basis 0-1 vectors.
%Note that $pu_{T \setminus S}$ must have disjoint positions with entry 1
%for distinct $p \in \calP_S$, and the sum $\sum_{p \in \calP_S}
%pu_{T \setminus S} = u_S u_{T \setminus S} = u_T$ is the all-1
%tuple in $\bbF^{r_{|T|}}$.

\begin{claim}\label{clm:projection-removal-inside-f}
Let $T$ and $U$ be finite sets, and let $S = T \cap U$.
If $x \in \hat \calG(T)$ and $y \in \hat \calG(U)$, then
\[
f(x y) = f(\hat \pi_S(x) y).
\]
\end{claim}
\begin{proof}
%For every $T$-labeled graph $G_1$ and $U$-labeled graph $G_2$,
%the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic,
%because only the labeled vertices in $S$ are identified in $G_1 G_2$,
%as well as in $\pi_S(G_1) G_2$.
%Then we extend the equality from $\calPLG$ by linearity.
%{\color{red} (modified proof)}
%
For every $T$-labeled graph $G_1$ and $U$-labeled graph $G_2$,
the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic as unlabeled graphs.
Hence $f(G_1 G_2) = f(\pi_S(G_1) G_2)$ as $f$ ignores labels.
Then we extend the equality from $\calPLG$ by linearity to $\calG$
and after that proceed to the quotient $\hat \calG = \calG / \calK$
using the definition of $f$ on $\hat \calG$.
%, because only the labeled vertices in $S$ are identified in $G_1 G_2$,
%as well as in $\pi_S(G_1) G_2$.
\end{proof}

%\sout{We have remarked earlier} 
We remarked in~(\ref{eq:nonzero-idempotent})  that $f(p) \ne 0$ for any $p \in \calP_S$.
\begin{claim}\label{clm:projection-formula}
Let $S \subseteq T$ be two finite sets.
If $q \in \calP_T$ resolves $p \in \calP_S$, then
\[
\hat \pi_S(q) = \frac{f(q)}{f(p)} p.
\]
\end{claim}
\begin{proof}
Note that $q \in \hat \calG(T)$.
Since $S \subseteq T$, it follows that $\hat \pi_S(q) \in \hat \calG(S)$.
Because the only element from $\hat \calG(S)$ orthogonal to $\hat \calG(S)$
with respect to the dot product $\langle \cdot, \cdot \rangle$
restricted to $\hat \calG(S) \times \hat \calG(S)$ is $0$ (by Lemma~\ref{lem:empty-annihilator-for-hat-calG(subseteq)(S)}),
it suffices to show that both sides give
the same dot product with every basis element in $\cal P_S$.
%\sout{Since $q$ does not resolve any $p' \in \calP_S \setminus \{ p \}$, we have $p' q = 0$ for every such $p'$.}
For any $p' \in \calP_S \setminus \{ p \}$, we have $p' p = 0$ so $p' q = p' p q = 0$.
By Claim~\ref{clm:projection-removal-inside-f},
this implies that
\[
\langle p', \hat \pi_S(q) \rangle = f(p' \hat \pi_S(q)) = f(p' q) = 0 = \langle p', \frac{f(q)}{f(p)} p \rangle.
\]
Furthermore,
\[
\langle p, \hat \pi_S(q) \rangle = f(p \hat \pi_S(q)) = f(p q) = f(q) = \langle p, \frac{f(q)}{f(p)} p \rangle.
\]
This proves the claim.
\end{proof}

\begin{claim}\label{clm:swaps-within-f}
Let $T$ and $U$ be finite sets and let $S = T \cap U$.
Then for any $p \in \calP_S, q \in \calP_{T, p}$ and $r \in \hat \calG(U)$ we have
\[f(q r) = \frac{f(q)}{f(p)} f(rp).\]
%In other words,
%\[
%f(p) f(q r) = f(q) f(rp).
%\]
\end{claim}
\begin{proof}
By 
Claims~\ref{clm:projection-removal-inside-f}~and~\ref{clm:projection-formula},
\[
f(q r) = f(\hat \pi_S(q) r) = \frac{f(q)}{f(p)} f(rp).
\]
\end{proof}

\begin{claim}\label{clm:basic-idempotents-nonzero-product}
Let $T$ and $U$ be finite sets and let $S = T \cap U$.
If both $q \in \calP_T, r \in \calP_U$ resolve $p \in \calP_S$, then $q r \ne 0$.
\end{claim}
\begin{proof}
By Claim~\ref{clm:swaps-within-f},
\[
f(q r) = \frac{f(q)}{f(p)} f(r p) = \frac{f(q)}{f(p)} f(r) \ne 0.
\]
\end{proof}

\begin{claim}\label{clm:degree-monotonicity}
If $S \subseteq T$, and $q \in \calP_T$ resolves $p \in \calP_S$, then $\deg(q) \ge \deg(p)$.
\end{claim}
\begin{proof}
It suffices to show this in the case when $|T| = |S| + 1$.
Let $U \subset \posints$ be any $(|S| + 1)$-element superset of $S$ different from $T$;
suppose this is the disjoint union $U = S \sqcup \{ a \},\, a \notin T$. 
Let $Y$ be the set of elements in $\calP_U$ resolving $p u_{\{ a \}}$
(equivalently, resolving $p$, because
every $r \in \calP_U$ resolves $u_{\{ a \}}$ as $a \in U$).
Then $p u_{\{ a \}} = \sum_{r \in Y} r$
by Claim~\ref{clm:idempotent-is-sum-of-its-resolving-basic-idempotents}.
Here $|Y| = \deg(p)$.
Furthermore, we have
%\[
\begin{equation}\label{eqn:qr-summing-to-qu_(a)}
\sum_{r \in Y} q r = q \sum_{r \in Y} r = q p u_{\{ a \}} = q u_{\{ a \}}.
\end{equation}
%]
Each term $q r$ on the left hand side is nonzero
by Claim~\ref{clm:basic-idempotents-nonzero-product},
and since the terms are all idempotent,
each of them is a sum of one or more elements of $\calP_{T \cup U}$.
Furthermore, if $r, r' \in Y$ ($r \ne r'$),
then we have the orthogonality relation
\[
(q r) (q r') = q (r r')  = 0,
\]
so the sets of basic idempotents of $\calP_{T \cup U}$
in the expansion of each term are pairwise disjoint.
Therefore the expansion $\sum_{r \in Y} q r$
in $\calP_{T \cup U}$ contains at least $|Y| = \deg(p)$ terms.
On the right hand side of~(\ref{eqn:qr-summing-to-qu_(a)}), for any $z \in \calP_{T \cup U}$,
$z$ resolves $q$ iff $z$ resolves $q u_{\{ a \}}$ since $a \in U$.
Thus the number of terms in the expansion of $q u_{\{ a \}}$
in the basis $\calP_{T \cup U}$ is precisely $\deg(q)$ by definition.
Thus, $\deg(q) \ge |Y| = \deg(p)$.
The claim is proved.
\end{proof}

\subsection{Bounding the expansion}\label{subsec:Bounding-expansion}

At this point, we finally assume that all the conditions of
Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened}
are satisfied, i.e.,
$f(K_0) = 1$ and there is an integer $q \ge 0$ such that for 
every $k \ge 0$ there exists $n = n_k \ge 2$ satisfying
$r_{k, n} = \symrank T(f, k, n) \le \min(n - 1, q^k)$.
In particular $r_{0, n} \le q^0 = 1$ for $n = n_0 \ge 2$.
Clearly, $r_{0, n} \ne 0$ since $f(K_0) = 1$ so $r_{0, n} = 1$.
By Proposition~\ref{prop:graph-paramater-multiplicativity-criterion}, $f$ is multiplicative.

Next, from $f(K_0) = 1$,
we have $U_\emptyset = K_0 \notin \calK$
so that $u_\emptyset = U_\emptyset + \calK$ is a nonzero identity
in $\hat \calG(\emptyset) = \hat \calG[0] \ne 0$.
As $u_\emptyset$ is the sum of all basic idempotents in $\calG(\emptyset)$
we infer that $\calP_\emptyset \ne 0$.
Hence there is at least one basic idempotent.

%\sout{If for any $S$, a basic idempotent $p \in \calP_S$ has degree $D$,
%then by Claim~\ref{clm:degree-monotonicity}
%for any superset $T$ with $|T| = |S| + 1$, 
%there are $D$ basic idempotents resolving $p$ with degree $\ge D$.
%This can be iterated.}
 
If for any finite $S \subseteq \posints$,
a basic idempotent $p \in \calP_S$ has degree $D \ge 0$,
then for any superset $T \subseteq \posints$ of $S$ with $|T| = |S| + 1$, 
there are $D$ basic idempotents resolving $p$.
Let $S \subseteq T$, $t = |T \setminus S|$,
and $T \setminus S = \{u_1, u_2, \ldots, u_t\}$.
For each $1 \le i \le t$, we can pick $D$ basic idempotents
$q^{u_i}_j \in \calP_{S \cup \{u_i\}}$ resolving $p$, where $1 \le j \le D$.
For any mapping $\phi \colon \{1, \ldots, t\} \rightarrow \{1, \ldots, D\}$,
we can form the product $q_\phi = \prod_{i = 1}^t  q^{u_i}_{\phi(i)}$.
If $t = 0$, we assume $q_\phi = p$.
These are clearly idempotents resolving $p$.
If $\phi \ne \phi'$ then for some $i$, 
we have the orthogonality relation $q^{u_i}_{\phi(i)} q^{u_i}_{\phi'(i)} = 0$.
Thus $q_\phi q_{\phi'} = 0$. 
Also by applying Claim~\ref{clm:swaps-within-f} $t$ times,
\begin{equation}\label{f(q-phi)-factored-into-product-and-nonzero-1stpass}
f(q_\phi) = f(q_\phi p) = f(\prod_{i = 1}^t q^{u_i}_{\phi(i)} p ) = (\prod_{i = 1}^t \frac{f(q^{u_i}_{\phi(v)})}{f(p)}) f(p) \ne 0,
\end{equation}
and so $q_\phi \ne 0$.
Thus the set $\{q_\phi \mid \phi \colon \{1, \ldots, t\} \rightarrow \{1, \ldots, D\} \}$ is linearly independent. 
This implies that the dimension of $\hat \calG(T)$ over $\bbF$
is at least $D^{t} = D^{|T| - |S|}$.
But by Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)}
and the hypothesis of Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened}
we also have the upper bound $q^{|T|}$.
If $D > q$, this leads to a contradiction if $|T|$ is large.
It follows that $D \le q$,
i.e., the degrees of basic idempotents for any $S$
and any $p \in \calP_S$ are bounded by $q$.
Let $D \ge 0$ denote the maximum degree
over all such $S$ and $p \in \calP_S$,
and suppose it is attained at some particular $S$ and $p \in \calP_S$.
We now fix this $S$ and $p$.
Note that for the existence of $D$
we also use the existence of a basic idempotent.

For $u \in \posints \setminus S$, let $q_1^u, \ldots, q_D^u$
denote the elements of $\calP_{S \cup \{ u \}}$ resolving $p$.
Note that for $u, v \in \posints \setminus S$,
there is a natural isomorphism between $\hat \calG(S \cup \{ u \})$ and $\hat \calG(S \cup \{ v \})$
(induced by the map that fixes $S$ pointwise and maps $u$ to $v$),
and we may choose the indexing so that
$q_i^u$ corresponds to $q_i^v$ under this isomorphism.

%{\color{red} (say that we use the previous reasoning)}

Now for any finite set $T \supseteq S$
all basic idempotents in $\calP_T$ that resolve $p$ can be described.
%\sout{These are indeed the $q_\phi$'s we have already defined.}
To describe these,
 let $V = T \setminus S$, and for every map $\phi \colon V \to \{ 1, \ldots, D \}$, we 
%\sout{have} {\color{red} define as before}
define as before
\begin{equation}\label{eqn:q-phi-factored-into-product}
q_\phi = \prod_{v \in V} q_{\phi(v)}^v.
\end{equation}

We have shown that these are linearly independent.

\begin{claim}\label{clm:calP_(T,p)-resolved-by-q_phi}
\[
\calP_{T, p} = \{ q_\phi \colon \phi \in \{ 1, \ldots, D \}^V \}.
\]
\end{claim}
\begin{proof}
We prove this by induction on the cardinality of $V = T \setminus S$.
For $|V| = 0, 1$ the assertion is trivial.
Suppose that $|V| > 1$.
Pick any $u \in V$,  let $U = S \cup \{ u \}$
and $W = T \setminus \{ u \}$; thus $U \cap W = S$.
By the induction hypothesis, the basic idempotents in $\calP_W$ resolving $p$
are elements of the form $q_\psi$,
%for $\psi \in \{1, \ldots, D \}^{V \setminus \{ u \}}$.
for $\psi \in \{1, \ldots, D \}^{W}$.

Let $r$ be one of these.
By Claim~\ref{clm:basic-idempotents-nonzero-product},
$r q_i^u \ne 0$ for any $1 \le i \le D$, and clearly resolves $r$.
We can write $r q_i^u$ as a sum of basic idempotents in $\calP_T$
resolving it,
and it is easy to see that these also resolve $r$ (as 
\emph{resolve} is transitive).
For each  $r q_i^u$ the sum is nonempty as $r q_i^u \ne 0$.
Furthermore, the sets of basic idempotents occurring
in the expressions for $r q_i^u$ and $r q_j^u$ ($i \ne j$) are disjoint;
this follows from item 2 stated at the beginning of this subsection,
and $q_i^u q_j^u =0$.
%But $r$ has degree $D$,
%%% JYC
%%% this originally in my mind was justified by claim 5.22 
%%% (the last claim of sec 5.4.)  but you want NOT to use it, and netherless
%%% keep it there.
%%% anyway, i wrote an alternative  justification
%%%
If the sum  for any $r q_i^u$ has more than one basic idempotent,
then $r$ would have degree $>D$, violating the maximality of $D$.
%%% as r would have >D many basic idempotents in $\calP_T$ resolving it.
So each $r q_i^u$ must be a basic idempotent in $\calP_T$ itself.

Each $r \in \calP_{W}$ resolves $p$ iff $r$ resolves $p u_{W}$.
Hence $p u_{W} = \sum_{r \in \calP_{W, p}} r$.
Also $p u_{\{ u \}} = \sum_{i = 1}^D q_i^u$.
Therefore we have
\[
p u_{T} = p u_{W} p u_{\{ u \}} = \sum_{r \in \calP_{W, p}, 1 \le i \le D} r q_i^u
\]
i.e., the basic idempotents $r q_i^u$ ($r \in \calP_{W, p},\, 1 \le i \le D)$
form the set of basic idempotents in $\calP_{T}$ resolving $p u_{T}$,
which is equivalent to resolving $p$.
It follows that these are all the elements of $\calP_{T, p}$.
This proves the claim.
\end{proof}

It is immediate from the definition that
an idempotent $q_\phi$ resolves $q_i^v u_V$ (equivalently $q_i^v$) iff $\phi(v) = i$.
Hence it also follows that
%\begin{equation}\label{eqn:q-i-v-times-u-v-factored-into-product}
\[
q_i^v u_V= \sum_{\phi \colon \phi(v) = i} q_\phi.
\]
%\end{equation}
By the same reason, it also follows that for $u, v \in V$, $u \ne v$,
and any $1 \le i, j \le D$, 
\begin{equation}\label{eqn:q-i-v-times-u-v-factored-into-product-pairs}
q_i^u q_j^v u_V= \sum_{\substack{\phi \colon \phi(u) = i \\ 
\quad \phi(v) = j}} q_\phi.
\end{equation}

\subsection{Constructing the target graph}

Now we can define $H$ as follows.
Let $S$ and $p$ be fixed as above. 
For any $u \in \posints \setminus S$, let $\{q_1^u, \ldots, q_D^u\}$ 
%and
%for any $T \supseteq S$, 
%$q_\phi$ is 
be defined as in subsection~\ref{subsec:Bounding-expansion}.
%%% JYC i added this T \supseteq S.  without T there is no \phi

Let $H$ be the looped complete graph on $V(H) = \{ 1, \ldots, D \}$.
We have to define the node weights and edge weights.
For every $i \in V(H)$, let
\[
\alpha_i = \frac{f(q_i^u)}{f(p)}
\]
be the weight of node $i$~\footnote{For $\bbF = \bbR$,
if we require the positive semidefiniteness
of the connection matrices $M(f, k)$ for $k \ge 0$,
then since $p$ and $q_i^u$ are basic idempotents,
$f(p) = f(p^2) > 0$ and similarly $f(q_i^u) > 0$.
Thus $\alpha_i > 0$, and so we recover the positive vertex weight case; 
see~\cite{Freedman-Lovasz-Schrijver-2007}.}. 
This definition does not depend on the choice of $u$,
because if $v \in \posints \setminus S$
and $v \ne u$, then the isomorphism
from $\hat \calG(S \cup \{ u \})$ to $\hat \calG(S \cup \{ v \})$ 
(induced by the map that fixes $S$ and maps $u$ to $v$),
will send $q_i^u$ to $q_i^v$.

%{\color{red} (original incorrect)}
%{\color{blue}
%
%Let $u, v \in \posints \setminus S,\, u \ne v$, and let $W = S \cup \{ u, v \}$.
%Let $K_{u v}$ denote the graph on $W$ which has only one edge connecting $u$ and $v$,
%and let $k_{u v}$ denote the corresponding element of $\hat \calG(W)$.
%We can express $p k_{u v}$ as a linear combination
%of the basis elements from $\calP_{W}$.
%Note that $r \in \calP_{W}$ resolves $p$ iff it resolves $p u_{\{ u, v \}}$,
%thus $p u_{\{ u, v \}} = \sum_{r \in \calP_{W, p}} r$.
%So if $r' \in \calP_{W} \setminus \calP_{W, p}$,
%we have $r' p = r' u_{\{u,v\}} p =0$.
%Thus $r' p k_{u v} = 0$. It follows that $p k_{u v}$ is a linear 
%combination of the basis elements from the subset $\calP_{W, p}$.
%We write this unique expression
%}
%
%{\color{red} (correct argument)}

Let $u, v \in \posints \setminus S,\, u \ne v$, and let $W = S \cup \{ u, v \}$.
Let $K_{u v}$ denote the graph on the vertices $u$ and $v$
that are correspondingly labeled $u$ and $v$,
and has only one edge connecting $u$ and $v$.
Let $k_{u v} = K_{u v} + \calK$ denote the corresponding element of $\hat \calG(\{ u, v \})$.
We can express $p k_{u v}$ as a linear combination
of the basic idempotents from $\calP_W$.
Note that $r \in \calP_{W}$ resolves $p$ iff $r$ resolves $p u_{\{ u,v \}}$,
thus $p u_{\{ u, v \}} = \sum_{r \in \calP_{W, p}} r$.
So if $r' \in \calP_W \setminus \calP_{W, p}$, we have $r' p = r' u_{\{ u, v \}} p =0$.
Thus $r' p k_{u v} = 0$. It follows that $p k_{u v}$ is a linear 
combination of the basic idempotents from the subset $\calP_{W, p}$.
We write this unique expression
\[
p k_{u v} = \sum_{i, j = 1}^D \beta_{i j} q_i^u q_j^v.
\]
This defines (by the uniqueness) the weight $\beta_{i j}$ of the edge $i j$.
Note that $\beta_{i j} = \beta_{j i}$ for all $i, j$, since $p k_{u v} = p k_{v u}$.

We prove that this weighted graph $H$ gives the desired homomorphism function.

\begin{claim}\label{clm:f-equals-hom(,H)}
For every finite graph $G$, $f(G) = \hom(G, H)$.
\end{claim}
\begin{proof}
%{\color{red} (original incorrect)}
%{\color{blue}
%
%Let $V$ be a finite subset of $\posints$ disjoint from $S$ of cardinality $|V(G)|$.
%We label $V(G)$ by $V$ thus making $G$ a $V$-labeled graph.
%Since $f$ ignores labels, we may identify $V$ and $V(G)$, and assume $V(G) = V$.
%By (\ref{eqn:q-i-v-times-u-v-factored-into-product-pairs}),
%we have for each pair $u, v$ of distinct elements of $V(G)$,
%\[
%p k_{u v} u_V = \sum_{i, j \in V(H)} \beta_{i j} q_i^u q_j^v u_V = \sum_{i, j \in V(H)} \beta_{i, j} \sum_{\substack{\phi \colon \phi(u) = i \\
%\quad \phi(v) = j}} q_\phi = \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi.
%\]
%Here the last equality follows from the fact that
%\[
%\{ \phi : V \rightarrow V(H) \} = \bigcup_{i,j \in V(H)} \{ \phi \in V(H)^V : \phi(u) = i, \phi(v) = j \}
%\]
%is a partition.
%Let $g$ be the corresponding element of $G$ in $\hat \calG(V)$.
%Clearly $g = \prod_{u v \in E(G)} k_{u v}$.
%Also note that $g u_V = g$ so $g = g u_V^{|E(G)|}$.
%Also, $p$ is an idempotent so $p = p^{|E(G)| + 1}$.
%Then
%\[
%p g = p^{|E(G)| + 1} g u_V^{|E(G)|} = p \prod_{u v \in E(G)} p k_{u v} u_V = p \prod_{u v \in E(G)} ( \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi ) 
%\]
%Note that when we expand the product of sum
%as a sum of products, for any two edges $u v \in E(G)$ and $u' v' \in E(G)$,
%if the mappings $\phi$ and $\phi' \in V(H)^V$ (in the respective sums)
%disagree on any vertex of $V = V(G)$, the product $q_\phi q_{\phi'} =0$.
%This implies that in the sum of products expression
%we only sum over all $\phi \in V(H)^V$ (and not over $|E(G)|$-tuples of these).
%Also $q_\phi$ resolves $p$, so $q_\phi p = q_\phi$.
%This implies that
%\[
%p g = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) q_\phi.
%\]
%Note that $p \in \hat \calG(S),\, g \in \hat \calG(V)$ and $S \cap V = \emptyset$,
%and $p$ and $g$ have representatives in $\calG(S)$
%and $\calG(V)$ that are (linear sums of) labeled graphs with disjoint vertex sets.
%We conclude that  $f(p) f(g) = f(p q)$, and so by
%(\ref{f(q-phi)-factored-into-product-and-nonzero-1stpass})
%and (\ref{eqn:q-phi-factored-into-product}),
%\[
%\begin{split}
%f(p) f(g) &= f(p g) = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) f(q_\phi) \\
%&= \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) ( \prod_{v \in V(G)} \alpha_{\phi(v)}) f(p),
%\end{split}
%\]
%The factor $f(p) \ne 0$ can be canceled from both sides, completing the proof.
%}
%
%{\color{red} (correct proof)}
%
Let $V$ be a finite subset of $\posints$ disjoint from $S$ of cardinality $|V(G)|$.
We label $V(G)$ by $V$ thus making $G$ a $V$-labeled graph, so now $G \in \calG(V)$.
Since $f$ ignores labels, we may identify $V$ and $V(G)$, and assume $V(G) = V$.
Now we take $T = S \sqcup V$,
thus $V = T \setminus S$. This defines $q_\phi$
as in subsection~\ref{subsec:Bounding-expansion}.
 %To define the set of mappings $\phi$ we take $T = S \sqcup V$,
%thus $V = T \setminus S$.
By (\ref{eqn:q-i-v-times-u-v-factored-into-product-pairs}),
we have for each pair $u, v$ of distinct elements of $V(G)$,
\[
p k_{u v} u_V = \sum_{i, j \in V(H)} \beta_{i j} q_i^u q_j^v u_V = \sum_{i, j \in V(H)} \beta_{i, j} \sum_{\substack{\phi \colon \phi(u) = i \\
\quad \phi(v) = j}} q_\phi = \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi.
\]
Here to define the set of mappings $\phi$ we take $T = S \sqcup V$,
thus $V = T \setminus S$.
Then the last equality follows from the fact that
\[
\{ \phi : V \rightarrow V(H) \} = \bigsqcup_{i,j \in V(H)} \{ \phi \in V(H)^V : \phi(u) = i, \phi(v) = j \}
\]
is a partition.
Let $g = G + \calK$ be the corresponding element of $G$ in $\hat \calG(V)$.
Clearly $G = (\prod_{u v \in E(G)} K_{u, v}) U_V$ so $g = (\prod_{u v \in E(G)} k_{u v}) u_V$.
(When $E(G) = \emptyset$, we view it as $G = U_V$ so $g = u_V$.)
We have $f(G) = f(g)$ by the definition of $f$ on $\hat \calG$.
Also note that $g u_V = g$ so $g = g u_V^{|E(G)|}$.
Also, $p$ is an idempotent so $p = p^{|E(G)| + 1}$.
Then
\[
p g = p^{|E(G)| + 1} g u_V^{|E(G)|} = p \big( \prod_{u v \in E(G)} p k_{u v} u_V \big) u_V = p \big( \prod_{u v \in E(G)} ( \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi ) \big) u_V.
\]
(When $E(G) = \emptyset$, this is simply $p g = p u_V$.)
Note that when we expand the product of sum
as a sum of products, for any two edges $uv \in E(G)$ and $u'v' \in E(G)$,
if the mappings $\phi$ and $\phi' \in V(H)^V$ (in the respective sums)
disagree on any vertex of $V = V(G)$, the product $q_\phi q_{\phi'} =0$.
This implies that in the sum of products expression
we only sum over all $\phi \in V(H)^V$ (and not over the $|E(G)|$-tuples of these).
Also $q_\phi$ resolves $p$, so $p q_\phi = q_\phi$.
Moreover, each $q_\phi \in \hat \calG(S \cup V)$ so $q_\phi u_V = q_\phi$.
This implies that
\[
p g = \big( \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) q_\phi \big) u_V = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) q_\phi.
\]
(When $E(G) = \emptyset$, we view it as $p g = p u_V = \sum_{\phi \colon V \to V(H)} q_\phi = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) q_\phi$ 
%{\color{red} (need the entire formula)}
which is true by Claims~\ref{clm:idempotent-is-sum-of-its-resolving-basic-idempotents} and~\ref{clm:calP_(T,p)-resolved-by-q_phi} with $T = S \cup V$
and the fact that an element $h \in \hat \calG(S \cup V)$ resolves $p$ iff $h$ resolves $p u_V$.)
Note that $p \in \hat \calG(S)$
and has a representative in $\calG(S)$ as a 
linear combination of labeled graphs from $\calPLG(S)$,
$g \in \hat \calG(V)$ has the representative $G \in \calPLG(V) \subseteq \calG(V)$,
 and $S \cap V = \emptyset$.
Hence $f(p) f(g) = f(p g)$,  as $f$ is multiplicative, $f$ ignores labels and 
also by the definition of $f$ on $\hat \calG$.
Therefore by 
(\ref{f(q-phi)-factored-into-product-and-nonzero-1stpass})
and (\ref{eqn:q-phi-factored-into-product}),
\[
\begin{split}
f(p) f(G) &= f(p) f(g) = f(p g) = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) f(q_\phi) \\
&= \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) ( \prod_{v \in V(G)} \alpha_{\phi(v)}) f(p),
\end{split}
\]
Since $f(p) \ne 0$, we can cancel it on both sides,
and complete the proof.
%The factor $f(p) \ne 0$ can be canceled from both sides, completing the proof.

\begin{remark}
Note that if $D = 0$, then from the proof we get that $H$ is the empty graph,
so $f(G) = 0$ unless $G = K_0$ (the empty graph) and $f(K_0) = 1$.
After that, we trivially get $\hat \calG(T) = 0$ for any $T \ne \emptyset$
and $\hat \calG(\emptyset) \cong \bbF$ as algebras.
However, $p \in \calP_S$ so it follows that $S = \emptyset$.
Therefore by the previous isomorphism $\calP_\emptyset = \{ p \}$
so $p$ is the only basic idempotent in $\hat \calG(\emptyset)$ and so in the entire $\hat \calG$.
\end{remark} 
\end{proof}



==> pm-rk-con-ten-GH-article-(cpc-submission)/one-lemma-preliminary.tex <==
%%% omitted
\begin{lemma}\label{lem:tensor-powers-pairwise-implies-linear-independence-long}
Let $r \ge 0$, and
let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ be $r$ nonzero
\emph{pairwise} linearly independent vectors. Then for any nonnegative integer $n \ge r-1$, the rank-$1$ symmetric tensors
\[
\bfx_1^{\otimes n}, \ldots, \bfx_r^{\otimes n} \in \Sym^n(\bbF^\calI)
\]
are linearly independent.
\end{lemma}
%% omitted
\begin{proof}
The case $r=0$ is vacuously true.
It is also trivially true for $r = 1$, 
since $\bfx_1^{\otimes n}$ is nonzero.
%%% JYC what does that sentence mean, after the sentence before it?
%%% including $\bfx_1^{\otimes 0}$ which is the scalar $1$.
Assume $r \ge 2$. %Let 
%$U = \Span \{\bfx_1,  \ldots, \bfx_r \}$.
By pairwise linear independence, for every $1 \le i, j \le r$, $i \ne j$, 
from Lemma~\ref{lem:linear-independence-and-dual-vectors-long}
there exists $h_{i j}$ such that $\bfx_i(h_{i j}) = 1$, $\bfx_j(h_{i j}) = 0$. 
Suppose $\sum_{i = 1}^r \lambda_i \bfx_i^{\otimes n} = 0$ 
where $\lambda_i \in \bbF,\, 1 \le i \le r$. 
Applying $\bigotimes_{1 \le j \le r,\, j \ne i} h_{i j}$,
we get $\lambda_i \bfx_i^{\otimes (n - (r-1))} = 0$ for
$1 \le i \le r$, and thus $\lambda_i =0$ since $n \ge r-1$
and therefore $\bfx_i^{\otimes (n - (r-1))}$ is nonzero. 
Hence $\bfx_1^{\otimes n}, \ldots, \bfx_r^{\otimes n}$ are linearly independent.
\end{proof}

\begin{remark}
For $r \ge 2$,
the nonzero hypothesis is subsumed by
%already implied by
pairwise linear independence.
\end{remark}



==> pm-rk-con-ten-GH-article-(cpc-submission)/our-preamble.tex <==
%\documentclass[11pt,twoside]{article}
\usepackage{amsmath, amsfonts, amssymb, amsthm, amscd, graphicx, 
%hyperref, 
enumerate, footmisc, mathtools, xcolor}
\setcounter{MaxMatrixCols}{30}
\setcounter{tocdepth}{10}
\providecommand{\U}[1]{\protect\rule{.1in}{.1in}}
\setlength{\topmargin}{-1.0in}
\setlength{\textheight}{9.25in}
\setlength{\oddsidemargin}{0.0in}
\setlength{\evensidemargin}{0.0in}
\setlength{\textwidth}{6.5in}
\def\labelenumi{\arabic{enumi}.}
\def\theenumi{\arabic{enumi}}
\def\labelenumii{(\alph{enumii})}
\def\theenumii{\alph{enumii}}
\def\p@enumii{\theenumi.}
\def\labelenumiii{\arabic{enumiii}.}
\def\theenumiii{\arabic{enumiii}}
\def\p@enumiii{(\theenumi)(\theenumii)}
\def\labelenumiv{\arabic{enumiv}.}
\def\theenumiv{\arabic{enumiv}}
\def\p@enumiv{\p@enumiii.\theenumiii}
\pagestyle{plain}
%\parindent=0pt
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}{Remark}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{axiom}{Axiom}

\newenvironment{lcases}
  {\left\lbrace\begin{aligned}}
  {\end{aligned}\right.}
\newcommand{\bbF}{\mathbb F}
\newcommand{\bbN}{\mathbb N}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbC}{\mathbb C}
\newcommand{\bbH}{\mathbb H}
\newcommand{\pmatch}{\operatorname{pm}}
\newcommand{\edgecol}{\operatorname{ec}}
\newcommand{\vdccover}{\operatorname{vdcc}}
\newcommand{\wmatch}{\operatorname{wm}}
\newcommand{\Char}{\operatorname{char}}
\newcommand{\Mod}{\operatorname{mod}}
%\newcommand{\rank}{\operatorname{rk}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\symrank}{\operatorname{rk_\mathsf S}}
\newcommand{\matrank}{\operatorname{rank}}
\newcommand{\im}{\operatorname{im}}
%\newcommand{\Holant}{\operatorname{Holant}}
%\newcommand{\trans}[4]{\ensuremath{\left[ \begin{smallmatrix} #1 & #2 \\ #3 & #4 \end{smallmatrix} \right]}}
\newcommand{\Span}{\operatorname{span}}
%\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\diag}{\operatorname{diag}}
%\newcommand{\dom}{\operatorname{dom}}
\newcommand{\Aut}{\operatorname{Aut}}

\newcommand{\calPLG}{\mathcal{PLG}}
\newcommand{\calG}{\mathcal G}
\newcommand{\calK}{\mathcal K}
\newcommand{\calP}{\mathcal P}
\newcommand{\bfx}{\mathbf x}
\newcommand{\bfy}{\mathbf y}
\newcommand{\bfz}{\mathbf z}
\newcommand{\sfS}{\mathsf S}
\newcommand{\sfT}{\mathsf T}
\newcommand{\calM}{\mathcal M}
\newcommand{\bfu}{\mathbf u}
\newcommand{\bfv}{\mathbf v}
\newcommand{\bff}{\mathbf f}
\newcommand{\textbfit}[1]{\textbf{\textit{#1}}}
\newcommand{\calI}{\mathcal I}
\newcommand{\calJ}{\mathcal J}
\newcommand{\calA}{\mathcal A}
\newcommand{\calT}{\mathcal T}

%%%\newcommand*{\mainflag}{}

%%%
\usepackage{fullpage}
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{mathrsfs}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\numberwithin{equation}{section}

==> pm-rk-con-ten-GH-article-(cpc-submission)/preliminary-short.tex <==
\section{Some Basic Concepts}\label{sec:Preliminary-short}

In this paper $\bbF$ denotes an arbitrary field, also
viewed as a one-dimensional vector space over $\bbF$. 
The  set $\bbF^\calI$ consists of tuples indexed by  $\calI$.
We let $\posints$ denote the set of positive integers.
For any integer $k \ge 0$, let $[k] = \{ 1, \ldots, k \}$. 
In particular, $[0] = \emptyset$.
For finite $\calI = [n]$ we write $\bbF^n$. By operations on components
$\bbF^\calI$ is an algebra (vector space and a ring).
%For convenience, we assume
By convention $\bbF^0 = \bbF^{\emptyset} = \{\emptyset\}$,
and $0^0 = 1$ in $\bbZ$, $\bbF$, etc.
We use $\bigsqcup$ to denote disjoint union.
In subsection~\ref{Multilinear-algebra-short}
we briefly state some concepts and results.
%Some more details are given in Section~\ref{sec:Preliminary-continued}.
A more detailed account is given in Section~\ref{sec:Preliminary-continued} as an appendix.

\subsection{Multilinear algebra}\label{Multilinear-algebra-short}

We assume that the reader is familiar with tensors.
A main feature in this paper is that we deal with
infinite dimensional spaces and their duals;  and this infinite dimensionality
causes some  technical complications.
% is a
%technical point that causes some complications.
E.g., 
multilinear functions on $\prod_{i = 1}^n V_i$ can be naturally identified 
with the dual space $(\bigotimes_{i = 1}^n V_i)^*$ of 
linear functions on $\bigotimes_{i = 1}^n V_i$.
Moreover, $\bigotimes_{i = 1}^n V_i^*$ canonically embeds into 
$(\bigotimes_{i = 1}^n V_i)^*$ via  
$(\otimes_{i = 1}^n f_i) (\otimes_{i = 1}^n v_i)
=
\prod_{i = 1}^n f_i(v_i)$. 
A special case is that $(V^*)^{\otimes n}$ embeds into $(V^{\otimes n})^*$.
If all $V_i$'s are finite 
dimensional then this embedding is an isomorphism. 
However, if $V_i$
are infinite dimensional, this embedding is \emph{not} surjective.
To see this, consider $V^{\otimes 2}$ where $V$ is the linear span of
%$\{e_i \mid 1 \le i < \omega\}$, ($\omega$ is the first countable ordinal).
$\{e_i \mid i \in {\posints}\}$, where $e_i$ is 
%an infinite dimensional
the $0$-$1$ vector indexed by ${\posints}$ with a single $1$ at the $i$th position.
Let $f \in (V^{\otimes 2})^*$ be such that
$f(e_i \otimes e_j) = \delta_{ij}$, which is $1$ if $i=j$ and $0$ otherwise.
Then 
there is no tensor  $T \in  (V^*)^{\otimes 2}$
that embeds as $f$.
Indeed, any $T \in  (V^*)^{\otimes 2}$ is, by definition, a \emph{finite} sum
$T = \sum_{1 \le k <n} c_k f_k \otimes g_k$. If $T$ were to embed as $f$,
then consider the $n\times n$ matrix where
the
$(i,j)$ entry is $f(e_i \otimes e_j)$, which is the identity 
matrix $I_n$ of rank $n$. 
%representing $f$ on the span of $\{e_i \mid 1 \le i \le n\}$.
However $T(e_i \otimes e_j) =
  \sum_{1 \le k <n} c_k f_k(e_i) \cdot g_k(e_j)$, and
so the matrix for the embedded $T$ has rank $< n$,
being a sum of $n-1$ matrices of rank $\le 1$.
%resulting in a matrix of rank 
%less than $n$.

%Any $A \in \bigotimes_{j = 1}^n V_j$ can be expressed as
%a finite sum
%\[
%A = \sum_{i = 1}^r \bfv_{i 1} \otimes \cdots \otimes \bfv_{i n},
%\quad \bfv_{i j}\in V_j.
%\]
%The least $r \ge 0$ for which $A$ has such an expression
%is called the
%rank of $A$,  denoted by $\rank(A)$.
%$A=0$ iff $\rank(A)=0$.
%If $r = \rank(A) > 0$ then in any such expression of $A$ of $r$ terms
%all vectors
% $\bfv_{i j} \ne 0$.
%
%Similarly, for symmetric tensor
For any symmetric tensor
  $A \in \Sym^n(V)$ we define the symmetric rank of  $A$
to be the  least $r \ge 0$ for which $A$ can be expressed as
\[
A = \sum_{i = 1}^r \lambda_i \bfv_i^{\otimes n},
\quad \lambda_i \in \bbF, \bfv_i \in V,
\]
and we denote it by $\symrank(A)$.
If there is no such decomposition we define $\symrank(A) = \infty$. 
If $\symrank(A) < \infty$ then in any such expression of $A$
as a sum of $\symrank(A)$ terms
all $\lambda_i \ne 0$, all $\bfv_i \ne 0$ and are
pairwise linearly independent.
%Adapting the proof of Lemma 4.2 in~\cite{Comon-Golub-Lim-Mourrain-2008}
In subsection~\ref{sec:fin-sym-ten-rank} we show that if $\bbF$ is infinite,
then $\symrank(A) < \infty$ for all $A \in \Sym^n(V)$.
%
%The rank of a  multilinear  function is just an
%extension of the tensor
%rank from $\bigotimes_{i = 1}^n V_i^*$
% to $(\bigotimes_{i = 1}^n V_i)^*$.
%Similarly 
%The symmetric rank is the  extension 
%from $\Sym^n(V^*)$ to $\Sym((V^{\otimes n})^*)$.
%%Clearly for all symmetric $A$,
%% \in \Sym^n(V)$, 
%$\rank(A) \le \symrank(A)$.
%
%\begin{lemma}\label{lem:nonsym-leq-sym-rk}
%%For all $A \in \Sym^n(V)$, $\rank(A) \le \symrank(A)$.
%\end{lemma}
%
%{\color{red} (need to mention that proofs of the below lemmas are also in Appendix?)}
%
%\sout{We state some facts below; proofs can be 
%found in the Appendix (Section~\ref{sec:Preliminary-continued}).}
We prove all needed
 technical multilinear algebra statements in the Appendix (Section~\ref{sec:Preliminary-continued}). 

%\begin{lemma}\label{lem:rk-1-dec-uniqueness}
%Let $a \in \bbF \setminus \{0\}$ and $0 \ne \bfx_i \in \bbF^\calI$ for $1 \le i \le n$. 
%If $a \otimes_{i=1}^{n} \bfx_i = b \otimes_{i=1}^{n} \bfy_i$, where $b \in \bbF$ and $\bfy_i \in \bbF^\calI,\, 1 \le i \le n$, 
%then $\bfy_i \not = 0$,
%and $\bfx_i = \lambda_i \bfy_i$  for
 %some $\lambda_i \in \bbF  \setminus \{0\}$ ($1 \le i \le n$).
%\end{lemma}
%%%%% above not used. so commented out.

%\begin{lemma}\label{lem:linear-independence-and-nonzero-minor}
%The vectors $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ are linearly independent iff in the $r \times \calI$ 
%matrix formed by $\bfx_1, \ldots, \bfx_r$ as rows 
%there exists a nonzero $r \times r$ minor.
%\end{lemma}
%
%For $\bfx = (x_i)_{i \in \calI} \in \bbF^\calI$
%and  $h = (h_i)_{i \in \calI}  \in \bigoplus_\calI \bbF$ 
%(in a direct sum, only finitely many $h_i$ are zero),
%we denote their dot product
% by $\bfx(h) = \sum_{i \in \calI} x_i h_i \in \bbF$. {\color{red} Here we view $\bbF^\calI$ as the dual space of $\bigoplus_\calI \bbF$. (JYC: added)} 
%(In general the dot product for $\bfx, \bfy  \in \bbF^\calI$
%is not defined.)
%
%\begin{lemma}\label{lem:linear-independence-and-dual-vectors}
%Let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ be linearly independent. Then there exist $h_1, \ldots, h_r \in \bigoplus_{\calI} \bbF$ dual
%to $\bfx_1, \ldots, \bfx_r$, i.e., $\bfx_i(h_j) = \delta_{i j},\, 1 \le i, j 
%\le  r$.
%\end{lemma}
%
%\begin{lemma}\label{lem:quotient-space-dimension}
%Let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$. Consider the linear map $\Phi \colon \bigoplus_\calI \bbF \to \bbF^r,\, h \mapsto ( \bfx_1(h), \ldots, \bfx_r(h) )$. Then $\dim (\bigoplus_\calI \bbF / \ker \Phi) = \dim \Span \{ \bfx_i \}_{i = 1}^r$.
%\end{lemma}
%
%\begin{lemma}\label{lem:tensor-powers-linear-independence-symmetric-rank-and-uniqueness}
%Let $r \ge 0$, and
%let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ be $r$ linearly independent vectors and $a_1, \ldots, a_r \in \bbF \setminus \{0\}$. Then for any integer $n \ge 2$, the symmetric tensor
%\begin{equation}\label{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-decomposition}
%A = \sum_{i = 1}^r a_i \bfx_i^{\otimes n} \in \Sym^n(\bbF^\calI)
%\end{equation}
%has $\symrank(A) = r$. For $n \ge 3$, any expression of $A$ as $\sum_{i = 1}^r b_i \bfy_i^{\otimes n}$ is a permutation of the sum in (\ref{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-decomposition}).
%\end{lemma}
%
%\begin{lemma}\label{lem:tensor-powers-pairwise-implies-linear-independence}
%Let $r \ge 0$, and
%let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ be $r$ nonzero
%\emph{pairwise} linearly independent vectors. Then for any nonnegative integer $n \ge r-1$, the rank-$1$ symmetric tensors
%\[
%\bfx_1^{\otimes n}, \ldots, \bfx_r^{\otimes n} \in \Sym^n(\bbF^\calI)
%\]
%are linearly independent.
%\end{lemma}

\subsection{Weighted graph homomorphisms}

We recap the notion of weighted graph homomorphisms \cite{Freedman-Lovasz-Schrijver-2007}, but state it for an arbitrary field $\bbF$.

An ($\bbF$-)\textit{weighted graph} $H$ is a graph with a weight $\alpha_H(i) \in \bbF \setminus \{0\}$ associated with each node $i$ and a weight $\beta_H(i, j) \in \bbF$ associated with each edge $ij$. For undirected GH,
% graphs $G$,
we assume $\beta_H(i, j)= \beta_H(j, i)$.

Let $G$ be an unweighted graph (with possible multiple edges, but no loops) and $H$ a weighted graph (with possible loops, but no multiple edges). 
A map $\phi \colon V(G) \to V(H)$ is a homomorphism if
every edge of $G$
goes to an edge or loop of $H$.
In this paper, it is convenient to assume that 
$H$ is a complete graph with a loop at all nodes by adding
all missing edges and loops with weight $0$. Then the weighted graph $H$ is described by an integer $q = |V(H)| \ge 0$ ($H$ can be the empty graph), a nowhere zero vector $a = (\alpha_1, \ldots, \alpha_q) \in \bbF^q$ and a symmetric matrix $B = (\beta_{i j}) \in \bbF^{q \times q}$.
In this setting every map  $\phi \colon V(G) \to V(H)$ is a homomorphism.
 %To every homomorphism $\phi$
 We assign the weights
\begin{equation}\label{eqn:hom-phi-def}
\alpha_\phi = \prod_{u \in V(G)} \alpha_H(\phi(u)),
\quad \quad \quad
\hom_\phi(G, H) = \prod_{u v \in E(G)} \beta_H(\phi(u), \phi(v)),
\end{equation}
and define
\begin{equation}\label{eqn:hom-def}
\hom(G, H) = \sum_{\phi \colon V(G) \to V(H)}
\alpha_\phi \hom_\phi(G, H).
%\hom(G, H) = \sum_{\small \substack{\phi \colon V(G) \to V(H) \\ \text{homomorhpism}}} \alpha_\phi \hom_\phi(G, H). %\tiny
\end{equation}
When $G$ is the empty graph, i.e., $V(G) = \emptyset$, the only
map $\phi \colon \emptyset \to V(H)$ is the empty map $\phi = \emptyset$;
in that case we have the empty products
$\alpha_\emptyset = 1$, $\hom_\emptyset = 1$, and $\hom(G, H) = 1$.

If all node-weights and edge-weights in $H$ are $1$, then this is the number of homomorphisms from $G$ into $H$.
% (with no weights).
Without loss of generality we require 
all vertex weights $\alpha_H(i) \ne 0$ since any vertex $i$ with
 $\alpha_H(i) = 0$ 
can be deleted together with all incident edges $ij$ and loops at $i$.
%such a vertex $i$ and all incident edges $ij$  irrelevant as they only
%contribute zero to $\hom(G, H)$.)
%
%
%{\color{red} (and loop at $i$ to together with the edes $ij$?)}

%For the purpose of this paper, it will be convenient to assume that $H$ is a complete graph with a loop at all nodes by adding
%all missing edges and loops with weight $0$. Then the weighted graph $H$ is completely described by a nonnegative integer $q = |V(H)|$ ($H$ could be the empty graph), a nowhere zero vector $a = (\alpha_1, \ldots, \alpha_q) \in \bbF^q$ and a symmetric matrix $B = (\beta_{i j}) \in \bbF^{q \times q}$. 

Note that when $H$ is the empty graph, then
$\hom(G, H) = 0$ if $G$ is not the empty graph 
(because there is no map $\phi \colon V(G) \to V(H)$ in this case),
and $\hom(G, H) = 1$ if  $G$ is the empty graph
(because there is  precisely one 
 empty map $\phi = \emptyset$ in this case.)
The function $f_H = \hom(\cdot, H)$ is
a graph parameter, a concept to be formally defined  shortly.

%\begin{remark}\label{rem:GH-0-weights}
%Allowing vertex weights $\alpha_H(i)$ to be $0$ makes
%such a vertex $i$ and all incident edges $ij$  irrelevant as they only 
%contribute in zero terms in the sum $\hom(G, H)$.
%% in (\ref{eqn:hom-def}).
%\end{remark}



==> pm-rk-con-ten-GH-article-(cpc-submission)/preliminary.tex <==
%\newpage
%\section*{Appendix}

\section{Appendix}\label{sec:Preliminary-continued}
%: Some Basic Concepts and Results}\label{sec:Preliminary-continued}
%\section{More on Tensors}\label{sec:Preliminary-continued}
%Preliminary}

%We recap some preliminaries and give some proofs. 
%(There is some overlap with Section~\ref{sec:Preliminary-short}.)
%In this paper $\bbF$ is assumed to be an arbitrary field. 
%The  set $\bbF^\calI$ consists of tuples indexed by  $\calI$.
%For integer $k \ge 0$, let $[k] = \{ 1, \ldots, k \}$. 
%In particular, $[0] = \emptyset$.
%For finite $\calI = [n]$ we write $\bbF^n$. By operations on components
%$\bbF^\calI$ is an algebra (vector space and a ring).
%For convenience, we assume $\bbF^0 = \bbF^{\emptyset} = \{\emptyset\}$,
%and $0^0 = 1$ in $\bbZ$, $\bbF$, etc.


\subsection{Multilinear algebra}

We prove some statements we need about tensors. We assume that the reader is familiar with the definition of a multilinear function, 
tensor product, and dual space. It is good to start
with coordinate-free definitions because it allows a succinct notation.
But we will mostly use coordinates. 
The results are concrete, and they can be understood without too much
formalism.

Unless stated otherwise,
we do not impose a particular order
on the rows and columns
  of  matrices, or coordinates of  tensors.
The vector spaces may be infinite dimensional; and this infinite dimensionality is a
main technical point that causes some complications.

The tensor product of vector spaces $V_1, \ldots, V_n$ over $\bbF$ is denoted by $V_1 \otimes \cdots \otimes V_n$ or $\bigotimes_{i = 1}^n V_i$.
Elements of $\bigotimes_{i = 1}^n V_i$ are called order-$n$ tensors.
%Elements of this product are called order-$n$ tensors. 
When $V_i = V$ for $1 \le i \le n$, 
we denote the tensor product by $V^{\otimes n}$.
(By convention $V^{\otimes 0} = \bbF$, and $v^{\otimes 0} = 1 \in \bbF$.)
%and call it the $n$-th tensor power of $V$. 
%%% this term is not used.
%We can define a group action by
Define a group action by
 $S_n$ 
on $V^{\otimes n}$ induced by
$\sigma(\otimes_{i = 1}^n v_i) = \otimes_{i = 1}^n v_{\sigma(i)}$.
%$\sigma(\bfx_1 \otimes \cdots \otimes \bfx_n) 
%= \bfx_{\sigma(1)} \otimes \cdots \otimes \bfx_{\sigma(n)}$.
Recall that $V^{\otimes n}$ consists of finite linear combinations of
such terms. 
We call a tensor $A \in V^{\otimes n}$ symmetric 
if $\sigma(A) = A$ for all $\sigma \in S_n$,
and denote by $\Sym^n(V)$ the set of symmetric tensors in $V^{\otimes n}$.
%Note that because 
As $\bbF$ may have finite characteristic $p$,
the usual symmetrizing operator from $V^{\otimes n}$ to $\Sym^n(V)$,
which requires division by $n!$, 
is in general not defined.

Multilinear functions on $\prod_{i = 1}^n V_i$ can be naturally identified 
with the dual space $(\bigotimes_{i = 1}^n V_i)^*$ of 
linear functions on $\bigotimes_{i = 1}^n V_i$,
induced by  $f \mapsto f'$, satisfying $f'(\otimes_{i = 1}^n v_i) 
= f(v_1, \ldots, v_n)$.
Moreover, $\bigotimes_{i = 1}^n V_i^*$ canonically embeds into 
$(\bigotimes_{i = 1}^n V_i)^*$ via  
$(\otimes_{i = 1}^n f_i) (\otimes_{i = 1}^n v_i)
=
\prod_{i = 1}^n f_i(v_i)$. 
A special case is that $(V^*)^{\otimes n}$ embeds into $(V^{\otimes n})^*$.
If all $V_i$'s are finite 
dimensional then this embedding is an isomorphism. 
However, if $V_i$
are infinite dimensional, this embedding is \emph{not} surjective.
This was illustrated in subsection~\ref{Multilinear-algebra-short}.
\begin{comment} % alrady in sec 2.1
To see this, consider $V^{\otimes 2}$ where $V$ is the linear span of
%$\{e_i \mid 1 \le i < \omega\}$, ($\omega$ is the first countable ordinal).
$\{e_i \mid i \in {\bbN}\}$.
Let $f \in (V^{\otimes 2})^*$ be such that
$f(e_i \otimes e_j) = \delta_{ij}$, which is 1 if $i=j$ and 0 otherwise.
Then
there is no tensor  $T \in  (V^*)^{\otimes 2}$
that embeds as $f$.
Indeed, any $T \in  (V^*)^{\otimes 2}$ is, by definition, a \emph{finite} sum
$T = \sum_{1 \le k <n} c_k f_k \otimes g_k$. If $T$ were to embed as $f$,
then consider the $n\times n$ matrix where
the
$(i,j)$ entry is $f(e_i \otimes e_j)$, which is the identity
matrix $I_n$ of rank $n$.
%representing $f$ on the span of $\{e_i \mid 1 \le i \le n\}$.
However $T(e_i \otimes e_j) =
  \sum_{1 \le k <n} c_k f_k(e_i) \cdot g_k(e_j)$, and
so the matrix for the embedded $T$ has rank $< n$,
being a sum of $n-1$ matrices of rank $\le 1$.
\end{comment}

Let  $A_i \colon V_i \to U_i$ 
($1 \le i \le n$) be linear maps  of vector spaces.
 They induce a homomorphism  $(\bigotimes_{i = 1}^n U_i)^* \to 
(\bigotimes_{i = 1}^n V_i)^*$ via $f \mapsto g$,
satisfying $g(\otimes_{i = 1}^n v_i) =
 f( \otimes_{i = 1}^n A_i v_i)$.

If $V_i$ are vector subspaces of $U_i$,  then $\bigotimes_{i=1}^n V_i$
canonically embeds in $\bigotimes_{i=1}^n U_i$.
In particular, if $V \subseteq U$, then $V^{\otimes n}$ and $\Sym^n(V)$
canonically embed in $U^{\otimes n}$ and $\Sym^n(U)$ respectively.
Under this embedding $\Sym^n(V) = \Sym^n(U) \cap V^{\otimes n}$.
%
We will also denote the space of symmetric 
$n$-fold multilinear functions on $V$ by $\Sym((V^{\otimes n})^*)$, 
i.e., the functions from $(V^{\otimes n})^*$ that are symmetric.
We have $(V^*)^{\otimes n} \cap \Sym((V^{\otimes n})^*) = \Sym^n (V^*)$.

In this paper, we are interested in vector spaces of the form
 $V = \bigoplus_{i \in {\calI}} \bbF_i$, 
or just $\bigoplus_{{\calI}} \bbF$,
where $\calI$ is an (index) set and each $\bbF_i,\, i \in {\calI}$, is a copy of $\bbF$ indexed by $i$.
In this case $V$ has a basis $\{e_i \mid  i \in {\calI}\}$,
and a vector $v \in V$ has finitely many nonzeros in this basis.
Note that for  infinite $\calI$ this is a proper subset of $\bbF^\calI$,
and in particular $\{e_i \mid  i \in {\calI}\}$
is \emph{not} a basis~\footnote{Of course every vector space 
has a basis; however this requires Zorn's Lemma so 
the proof is nonconstructive. In this paper our results are
constructive usually working with an explicitly given basis.} for  $\bbF^\calI$.
%Every vector space $V$ can be written in this form because
%a basis always exists; however this requires Zorn's Lemma so 
%the proof is nonconstructive. In particular
%$\{e_i \mid  i \in {\calI}\}$ 
%is \emph{not} a basis for  $\bbF^\calI$, for infinite $\calI$. 
 %However, in this paper our results are
%constructive, usually working with an explicitly given basis.
For $V = \bigoplus_{{\calI}} \bbF$, the dual
space $V^*$ can be 
identified with $\bbF^\calI$ via $f \mapsto (f(e_i))_{i \in {\calI}}$.
For  $V = \bigoplus_{{\calI}} \bbF$,
we have $V^{\otimes n} = \bigoplus_{{\calI}^n} \bbF$,
and $(V^{\otimes n})^*$ can be identified with
$\bbF^{\calI^n}$, the $n$-dimensional arrays.
%We use $\Sym(\bbF^{{\calI}^n}) = \Sym((V^{\otimes n})^*)$
%to denote symmetric arrays. 
%{\color{red} Instead of this sentence it's more correct to say the 
%following: Then 
We can view $\Sym(\bbF^{\calI^n}) = \Sym((V^{\otimes n})^*)$ as 
symmetric arrays, i.e., arrays in $\bbF^{\calI^n}$ that are 
invariant under permutations from $S_n$,
 with respect to the 
basis $\{e_i \mid  i \in {\calI}\}$ of $V = \bigoplus_{i \in \calI} \bbF_i$.


%$V = \bigoplus_{i \in \calI} \bbF$.

%We have $(V^*)^{\otimes n} \cap
% \Sym((V^{\otimes n})^*) = \Sym^n (V^*)$. {\color{red} We don't need this sentence here. It's been moved upwards.}
%{\color{red} (define a symmetric array, i.e., invariant under permutations from $S_n$.)}
 
Any $A \in \bigotimes_{j = 1}^n V_j$, where $n \ge 1$, can be expressed as
a finite sum
\[
A = \sum_{i = 1}^r \bfv_{i 1} \otimes \cdots \otimes \bfv_{i n},
\quad \bfv_{i j}\in V_j.
\]
The least $r \ge 0$ for which $A$ has such an expression
is called the
rank of $A$,  denoted by $\rank(A)$.
$A=0$ iff $\rank(A)=0$.
If $r = \rank(A) > 0$ then in any such expression of $A$ of $r$ terms
all vectors
 $\bfv_{i j} \ne 0$.
When $n = 0$, $\bigotimes_{j = 1}^n V_j$ is $\bbF$,
and we define $\rank(A) = 1$ for $A \ne 0$ and $\rank(A) = 0$ for $A = 0$.

Similarly, for $A \in \Sym^n(V)$ we define the symmetric rank of $A$
to be the  least $r \ge 0$ for which $A$ can be expressed as
\[
A = \sum_{i = 1}^r \lambda_i \bfv_i^{\otimes n},
\quad \lambda_i \in \bbF, \bfv_i \in V,
\]
and is denoted by $\symrank(A)$.
If there is no such decomposition we define $\symrank(A) = \infty$. 
If $\symrank(A) < \infty$ then in any such expression of $A$
as a sum of $\symrank(A)$ terms
all $\lambda_i \ne 0$, all $\bfv_i \ne 0$ and are
pairwise linearly independent.
%Adapting the proof of Lemma 4.2 in~\cite{Comon-Golub-Lim-Mourrain-2008}
%(see Section~\ref{sec:fin-sym-ten-rank}),
We show in Lemma~\ref{lm:finite-symmetric-tensor-rank} that
  for infinite $\bbF$,
$\symrank(A) < \infty$ for all $A \in \Sym^n(V)$.

We also need to refer to the rank of functions
in $(\bigotimes_{i = 1}^n V_i)^*$. As mentioned before 
$\bigotimes_{i = 1}^n V_i^*$ is embedded as a subspace 
of $(\bigotimes_{i = 1}^n V_i)^*$.
For a function $F \in (\bigotimes_{i = 1}^n V_i)^*$, where $n \ge 1$,
we define the rank of the function $F$ to be $\infty$ if $F \notin \bigotimes_{i = 1}^n V_i^*$,
and if $F \in \bigotimes_{i = 1}^n V_i^*$,
the rank of $F$ is the least $r$ for which $F$ can be written as
\[
F = \sum_{i = 1}^r \bff_{i 1} \otimes \cdots \otimes \bff_{i n},
\quad \quad \bff_{i j} \in V_j^*.
\]
When $n = 0$, $(\bigotimes_{j = 1}^n V_j)^*$ is $(\bbF)^* \cong \bbF$,
% ($\bbF^*$ seems ambiguous, use $(\bbF)^*$?),
and we define $\rank(F) = 1$ for $F \ne 0$ and $\rank(F) = 0$ for $F = 0$.
The symmetric rank  $\symrank(F)$ of $F \in \Sym((V^{\otimes n})^*)$
% =
%\Sym(\bbF^{{\calI}^n})$
  is similarly defined. 
%{\color{red}(remove ${\color{red} =  \Sym(\bbF^{{\calI}^n})}$)}
It is $\infty$ if $F \not \in \Sym^n(V^*)$.
For $F \in \Sym^n(V^*)$, we define  $\symrank(F)$  to be the least $r$ 
such that
% $F$ is expressible as
\[
F = \sum_{i = 1}^r \lambda_i \bff_i^{\otimes n},
\quad \quad \lambda_i \in \bbF, \quad \bff_i \in V^*,
\]
if such an expression exists; $\symrank(F) = \infty$ otherwise.
By the same Lemma~\ref{lm:finite-symmetric-tensor-rank}
for infinite $\bbF$, we have
$\symrank(F) < \infty$ for all $F \in \Sym^n(V^*)$.
%{\color{red} Also we need to define the symmetric rank for $n = 0$ analogously to the nonsymmetric case but this time for functions.}

Basically, the rank of a  multilinear  function is just an
extension of the tensor
rank from $\bigotimes_{i = 1}^n V_i^*$
 to $(\bigotimes_{i = 1}^n V_i)^*$.
Similarly the symmetric rank is the  extension 
from $\Sym^n(V^*)$ to $\Sym((V^{\otimes n})^*)$.
Clearly for all symmetric $A$,
% \in \Sym^n(V)$, 
$\rank(A) \le \symrank(A)$.
Both $\rank$ and  $\symrank$ are unchanged when moving from 
 $\bigotimes V_i$ to $\bigotimes U_i$,
if $V_i \subseteq U_i$. 

%\begin{lemma}\label{lem:nonsym-leq-sym-rk}
%%For all $A \in \Sym^n(V)$, $\rank(A) \le \symrank(A)$.
%\end{lemma}

%The following Lemmas~\ref{lem:linear-independence-and-nonzero-minor-long}-\ref{lem:tensor-powers-pairwise-implies-linear-independence-long} are
%restatements of Lemmas~\ref{lem:linear-independence-and-nonzero-minor}-\ref{lem:tensor-powers-pairwise-implies-linear-independence},
%respectively, but with proofs included. %or Corollaries

%\begin{lemma}\label{lem:rk-1-dec-uniqueness-long}
%Let $a \in \bbF \setminus \{0\}$ and $0 \ne \bfx_i \in \bbF^\calI$ for $1 \le i \le n$. 
%If $a \otimes_{i=1}^{n} \bfx_i = b \otimes_{i=1}^{n} \bfy_i$, where $b \in \bbF$ and $\bfy_i \in \bbF^\calI,\, 1 \le i \le n$, 
%then $\bfy_i \not = 0$,
%and $\bfx_i = \lambda_i \bfy_i$  for
 %some $\lambda_i \in \bbF  \setminus \{0\}$ ($1 \le i \le n$).
%\end{lemma}
%\begin{proof}
%We can fix $j_1, \ldots, j_n \in \calI$ such that $(\bfx_i)_{j_i} \ne 0, \, 1 \le i \le n$. Restricting both sides of the equality to $(j_1, \ldots, j_{i - 1}, j_{i + 1}, \ldots, j_n)$ except the $i$-th component, we get
%$\bfx_i = \lambda_i \bfy_i$ for some  $\lambda_i \in \bbF$.
%Then clearly $\lambda_i \not = 0$ and $\bfy_i \not = 0$.
%\end{proof}
%%%%% above not used. so commented out.

%{\color{red} (JYC: no need to say we prove some facts below, let's not insert text)}

\begin{lemma}\label{lem:linear-independence-and-nonzero-minor-long}
The vectors $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ are linearly independent iff in the $r \times \calI$ 
matrix formed by $\bfx_1, \ldots, \bfx_r$ as rows 
there exists a nonzero $r \times r$ minor.
\end{lemma}
\begin{proof}
$\Leftarrow$ is obvious, so let us prove $\Rightarrow$.
Let $R \subseteq [r]$ be a maximal subset satisfying the property that
for some finite subset $C \subseteq \calI$ the
set of vectors $\{\bfx_i\mid_{C} \: : \, i \in R\}$ is linearly independent,
where $\bfx_i\mid_{C}$ is the restriction of $\bfx_i$ to $C$.
Suppose linear independence is achieved by $C$ for $R$.
Then
it also holds for any $C' \supseteq C$. 

If  $R \not = [r]$,  let $j \in [r] \setminus R$,
and consider $R^+ = R \cup \{j\}$. 
$\{\bfx_i\mid_{C}  \: : \, i \in R^+\}$ is linearly dependent.
Hence a unique linear combination holds for some $c_i \in \bbF$ ($i \in R$),
\begin{equation}\label{eqn:onC-lin-dep}
\bfx_j\mid_{C} \, = \sum_{i\in R} c_i \bfx_i\mid_{C}.
\end{equation}
For any $k \not \in C$,
$\{\bfx_i\mid_{C\cup\{k\}}  \: : \, i \in R^+\}$ is
also linearly dependent, and 
we have $\bfx_j\mid_{C\cup\{k\}}
= \sum_{i\in R} c'_i \bfx_i\mid_{C\cup\{k\}}$ for some $c'_i \in \bbF$.
Compared to (\ref{eqn:onC-lin-dep}), $c'_i = c_i$ for all $i \in R$.
Hence $\bfx_j \, = \sum_{i\in R} c_i \bfx_i$, a contradiction
to $\{\bfx_1, \ldots, \bfx_r\}$ being linearly independent.
So $R = [r]$.  There exists a nonzero $r \times r$ minor
in the $R \times C$ submatrix.
\end{proof}

For $\bfx = (x_i)_{i \in \calI} \in \bbF^\calI$
and  $h = (h_i)_{i \in \calI}  \in \bigoplus_\calI \bbF$ 
(in a direct sum, only finitely many $h_i$ are zero),
%(thus all but finitely many $h_i$ are zero),
we denote their dot product
 by $\bfx(h) = \sum_{i \in \calI} x_i h_i \in \bbF$. 
 Here we view $\bbF^\calI$ as the dual space of $\bigoplus_\calI \bbF$. 
(In general the dot product of the pair  $\bfx, \bfy  \in \bbF^\calI$
is not defined.)

\begin{lemma}\label{lem:linear-independence-and-dual-vectors-long}
Let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ be linearly independent. Then there exist $h_1, \ldots, h_r \in \bigoplus_{\calI} \bbF$ dual
to $\bfx_1, \ldots, \bfx_r$, i.e., $\bfx_i(h_j) = \delta_{i j},\, 1 \le i, j 
\le  r$.
\end{lemma}
\begin{proof}
By Lemma~\ref{lem:linear-independence-and-nonzero-minor-long}, there exist $r$ 
%pairwise
distinct indices $k_j \in \calI,\, 1 \le j \le r$ such that the matrix $A = (a_{i j})_{i, j = 1}^r = ((\bfx_i)_{k_j})_{i, j = 1}^r$ is invertible,
and let $B = (b_{i j}) = A^{-1}$.
%_{i, j = 1}^r$.
%Let $B = (b_{i j})_{i, j = 1}^r$ be its inverse. 
Taking $h_i = \sum_{j = 1}^r b_{j i} e_{k_j} \in \bigoplus_\calI \bbF,\, 1 \le i \le r$, we see that the 
equality 
$AB = I_r$ directly translates into the desired result.
\end{proof}

\begin{lemma}\label{lem:quotient-space-dimension-long}
Let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$. Consider the linear map $\Phi \colon \bigoplus_\calI \bbF \to \bbF^r,\, h \mapsto ( \bfx_1(h), \ldots, \bfx_r(h) )$. Then $\dim (\bigoplus_\calI \bbF / \ker \Phi) = \dim \Span \{ \bfx_i \}_{i = 1}^r$.
\end{lemma}
\begin{proof}
By the First Isomorphism Theorem for vector spaces $\bigoplus_I \bbF / \ker \Phi \cong \im \Phi$.
So it suffices to prove $\dim \im \Phi = \dim \Span \{ \bfx_i \}_{i = 1}^r$. 
Clearly it suffices to prove the case when
$\bfx_1, \ldots, \bfx_r$ are linearly independent, and that follows
directly from Lemma~\ref{lem:linear-independence-and-dual-vectors-long}.
\end{proof}

%\begin{lemma}\label{lem:tensor-product-linear-implies-linear-independence-long}
%Suppose $S$ is a (possibly infinite) set
%of  linearly independent elements from $\bbF^\calI$.
%Then the set $\{\bfy_1 \otimes \cdots \otimes \bfy_n
%\mid \bfy_i \in S,  1 \le i \le n \}$ 
%is also linearly independent.
%\end{lemma}
%\begin{proof}
%Let $S = \{\bfx_{j} \mid  j \in \calJ\}$, and
%suppose  $\sum a_{j_1 \ldots j_n} \bfx_{j_1} \otimes \cdots \otimes \bfx_{j_n}
 %= 0$ over finitely many tuples $(j_1, \ldots, j_n)$ 
%where each $j_i \in \calJ$. Let
%$\calI$ be the \emph{finite} set of indices $j \in \calJ$
%for which  $\bfx_{j}$ appears in this sum. 
%By Lemma~\ref{lem:linear-independence-and-dual-vectors-long}, 
 %there are dual vectors
 %$\{h_{j} \mid j \in \calI\}$,  
 %i.e.,
 %$\bfx_{i}(h_{j}) = \delta_{i j}$ for $i, j \in \calI$. 
%Applying  $h_{j_1} \otimes \cdots \otimes h_{j_n}$ to the sum,
 %only one term indexed by $(j_1, \ldots, j_n)$ remains, and
%we obtain $a_{j_1 \ldots j_n} = 0$.
%\end{proof}
%In this proof we define  $\calI$, and use it instead of $\calJ$,
%because the latter may be infinite.
%
%\begin{corollary}
%\label{cor:tensor-powers-linear-implies-linear-independence-long}
%Let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ be $r$ linearly independent vectors. Then for any integer $n \ge 1$, the rank-$1$ symmetric tensors
%\(
%\bfx_1^{\otimes n}, \ldots, \bfx_r^{\otimes n} \in \Sym^n(\bbF^\calI)
%\)
%are linearly independent.
%\end{corollary}

\begin{lemma}\label{lem:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-long}
Let $r \ge 0$, and
let $\bfx_1, \ldots, \bfx_r \in \bbF^\calI$ be $r$ linearly independent vectors and $a_1, \ldots, a_r \in \bbF \setminus \{0\}$. Then for any integer $n \ge 2$, the symmetric tensor
\begin{equation}\label{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-decomposition-long}
A = \sum_{i = 1}^r a_i \bfx_i^{\otimes n} \in \Sym^n(\bbF^\calI)
\end{equation}
has $\symrank(A) = r$. For $n \ge 3$, any expression of $A$ as $\sum_{i = 1}^r b_i \bfy_i^{\otimes n}$ is a permutation of the sum in (\ref{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-decomposition-long}).
\end{lemma}
\begin{proof}
When $r = 0$, the statement is trivially true so we assume $r \ge 1$.
Let $n \ge 2$ and $\symrank(A) = s$. Clearly $s \le r$. By being
of symmetric rank $s$, there
exist $\bfy_1, \ldots, \bfy_s \in \bbF^\calI$
 and $b_1, \ldots, b_s \in \bbF \setminus \{0\}$ such that
\begin{equation}\label{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-lemma-two-sided-decomposition-long}
\sum_{i = 1}^r a_i \bfx_i^{\otimes n} = A = \sum_{j = 1}^s b_j \bfy_j^{\otimes n}.
\end{equation}
By Lemma~\ref{lem:linear-independence-and-dual-vectors-long},
there exist $h_1, \ldots, h_r$ dual to
$\bfx_1, \ldots, \bfx_r$.
For any $1 \le i \le r$,
applying $h_i^{\otimes (n-1)}$ to the sum, 
we get $a_i \bfx_i$ as a linear combination
of $\bfy_1, \ldots, \bfy_s$. 
Hence $s \ge r$ as $\bfx_1, \ldots, \bfx_r$ are linearly independent.
So $s = r$,
and $\bfy_1, \ldots, \bfy_s$ are linearly independent.

Next, let $n \ge 3$ and consider 
(\ref{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-lemma-two-sided-decomposition-long}) again, where $s = r$.
Since $\symrank(A) = r$, all $b_j \ne 0$.
Applying $h_i$, we get
\begin{equation}\label{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-lemma-expression-of-ai-xi-to-(n-1)-alt-long}
a_i \bfx_i^{\otimes (n - 1)}  = B = \sum_{j = 1}^r  b_j \bfy_j(h_i) \bfy_j^{\otimes (n - 1)}.
\end{equation}
From the LHS, $\symrank(B) = 1$.
 By what has just been proved,
 $\symrank(B)$ is the number of 
terms with nonzero coefficients on the RHS. %We are given $b_j \not = 0$.
Hence for any $i$, there is  exactly one $j$ such that
 $\bfy_j(h_i) \not = 0$.
Applying  $h_i^{\otimes (n-2)}$ to 
(\ref{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-lemma-expression-of-ai-xi-to-(n-1)-alt-long}), we get
$a_i \bfx_i =  b'_j \bfy_j$,
where $ b'_j = b_j (\bfy_j(h_i))^{n-1} \not = 0$.
Since $\bfx_1, \ldots, \bfx_r$ are linearly independent, the map
$i \mapsto j$ is a permutation.
%{\color{red} Since the terms in
%(\ref{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-lemma-two-sided-decomposition-long}) are linearly independent by Corollary~\ref{cor:tensor-powers-linear-implies-linear-independence-long},
%the expression is the same up to a permutation.}
%
%{\color{red} (better explanation)}
%
From $a_i \bfx_i =  b'_j \bfy_j$
we get $a_i = b'_j \bfy_j(h_i) = b_j (\bfy_j(h_i))^n$.
%Then $\bfy_j = a_i / b'_j \bfx_i = b_j (\bfy_j(h_i))^n / (b_j (\bfy_j(h_i))^{n-1}) \bfx_i = \bfy_j(h_i) \bfx_i$.
It follows that $\bfy_j = (a_i/b'_j)  \bfx_i = \bfy_j(h_i) \bfx_i$.
Therefore $b_j \bfy_j^{\otimes n} = b_j (\bfy_j(h_i))^n \bfx_i^{\otimes n} = a_i \bfx_i^{\otimes n}$.
%Here $i, j$ are any such that $i \mapsto j$.
Thus the expressions on LHS and RHS of~(\ref{eqn:tensor-powers-linear-independence-symmetric-rank-and-uniqueness-lemma-two-sided-decomposition-long})
are the same up to a permutation of the terms.
\end{proof}

\input{one-lemma-preliminary}

\input{finite-symmetric-tensor-rank}

\subsection{Subalgebras of \texorpdfstring{$\bbF^m$}{F\textasciicircum{m}}}\label{subsec:bbF^m-subalgebras}

%{\color{red} text repeated as in section 5, need to say it again?}
%
%It is easy to classify all subalgebras of $\bbF^m$ for $m \ge 0$.
%Recall that we allow zero algebras %(i.e., $\bbF^0 = \{ \emptyset \}$, where $0 = 1 = \emptyset$)
%and require any subalgebra of an algebra to share the multiplicative identity {\color{red} with the larger algebra (added)}.
%
%{\color{red} (maybe just say the following or rephrase it as in the previous section instead of the above)}
%
We give a proof of Lemma~\ref{lem:F^m-subalgebras},
restated below.

\begin{lemma}\label{lem:F^m-subalgebras-long}
All subalgebras of $\bbF^m$, where $m \ge 0$, are of the following form:
For some partition $[m] = \bigsqcup_{i = 1}^s \calI_i$,
where $s \ge 0$, and $\calI_i \ne \emptyset$ for $i \in [s]$, 
the subalgebra has equal values on each $I_i$,
\[
\bbF^{(\calI_1, \ldots, \calI_s)} = \{ (c_1, \ldots, c_m) \in \bbF^m \mid \forall i \in [s], \ \forall j, j' \in \calI_i, \ c_j = c_{j'} \}.
\]
\end{lemma}
\begin{proof}
When $m = 0$, the statements is obvious.
Let $m \ge 1$ and $S \subseteq \bbF^m$ be a subalgebra of $\bbF^m$.
In particular, the multiplicative identity
is the $m$-tuple $(1, \dots, 1) \in S$.
We call $i, j \in [m]$ equivalent if $x_i = x_j$ for any $x = (x_1, \ldots, x_m) \in S$.
This is clearly an equivalence relation so
it partitions $[m]$ into (nonempty) equivalence classes $\calI_1, \ldots, \calI_s$
so that $[m] = \bigsqcup_{i = 1}^s \calI_i$.
As $[m] \ne \emptyset$ we have $s \ge 1$. %$m \ge 1$
We claim that $S = \bbF^{(\calI_1, \ldots, \calI_s)}$.
Clearly, $S \subseteq \bbF^{(\calI_1, \ldots, \calI_s)}$.
We prove the reverse inclusion.
For $s = 1$ this is clearly true
since the $m$-tuple $(1, \ldots, 1) \in S$
and $S$ is closed under scalar multiplication.

Now we let $s \ge 2$. By renaming  and omitting repeated coordinates
it is sufficient to prove the case when $m=s$ and  $\calI_i = \{i\}$.
Let $S' = \{(c_2, \ldots, c_s) \mid \exists c_1 \in \bbF,
(c_1, c_2, \ldots, c_s) \in S\}$ be the projection of $S$ to $\bbF^{s-1}$.
Clearly $S'$ is a subalgebra of $\bbF^{s-1}$, and 
by induction $S' = \bbF^{s-1}$.
Thus for some $b_1, \ldots, b_{s-1} \in \bbF$,
all  $s-1$ row vectors of the following $(s-1)\times s$
matrix $B$ belong to $S$, 
\begin{equation}\label{eqn:listing-elements-in-S'}
B = \left[
\begin{array}{ccccc}
b_1 & 1  &  0 & \ldots  & 0 \\
b_2 & 0  &  1 & \ldots  & 0 \\
\vdots & \vdots & \vdots & \ddots & \vdots \\
b_{s-1} &  0  &  0 & \ldots  & 1
\end{array}
\right].
\end{equation}
If all $b_i =0$, we let $v = (1, 1, \ldots, 1) \in S$.
Otherwise we may assume $b_1 \not =  0$.
By the definition of $I_1$ and $I_2$ and by the
closure of $S$ under scalar product and possibly adding $(1, 1, \ldots, 1)$,
for some $c_1 \not =  1$ and for some $c_3, \ldots, c_s \in \bbF$,
 we have $v' = (c_1, 1,  c_3, \ldots, c_s) \in S$.
Then multiplying $v'$ with the first row in (\ref{eqn:listing-elements-in-S'})
we get $v = (b_1c_1, 1, 0, \ldots, 0) \in S$.
Here $b_1c_1 \ne b_1$.
In either case, we obtain a matrix $A$ of rank $s$ by appending $v$  as
the last row to $B$.
Thus for all row
vectors $d \in \bbF^s$ the linear
system $x A = d$ has a solution $x \in \bbF^s$.
This shows that $d \in S$.
\end{proof}





%\begin{proof}
%When $m = 0$, the statements is obvious.
%Let $m \ge 1$ and $S \subseteq \bbF^m$ be a subalgebra of $\bbF^m$.
%In particular, the multiplicative identity
%is the $m$-tuple $(1, \dots, 1) \in S$.
%We call $i, j \in [m]$ equivalent if $x_i = x_j$ for any $x = (x_1, \ldots, x_m) \in S$.
%This is clearly an equivalence relation so
%it partitions $[m]$ into (nonempty) equivalence classes $\calI_1, \ldots, \calI_s$
%so that $[m] = \bigsqcup_{i = 1}^s \calI_i$.
%As $[m] \ne \emptyset$ we have $s \ge 1$. %$m \ge 1$
%We claim that $S = \bbF^{(\calI_1, \ldots, \calI_s)}$.
%Clearly, $S \subseteq \bbF^{(\calI_1, \ldots, \calI_s)}$.
%We prove the reverse inclusion.
%For  $s = 1$ this is clearly true
%since the $m$-tuple $(1, \ldots, 1) \in S$ 
%and $S$ is closed under scalar multiplication.
%
%Now we let $s \ge 2$. By renaming coordinates
%we may assume $i \in \calI_i$ for $i \in [s]$.
%By the definition of $\calI_1, \ldots, \calI_s$,
%for any $1 \le i < j \le s$,
%we can fix $c_{i j} = (c_{i j 1}, \ldots, c_{i j m}) \in S$
%so that $c_{i j i} \ne c_{i j j}$.
%% for any $k \ne \calI_i$ and $\ell \in \calI_j$
%%(so that $c_{i j | \calI_i} = const \ne c_{i j | \calI_j} = const$).
%For any nonnegative tuple $\bar h = (h_{i j})_{1 \le i < j \le s}$,
%consider the 
%element $p_{\bar h} = \prod_{1 \le i < j \le s} c_{i j}^{h_{i j}}$. 
%%\in S$.
%Since $S$ is a subalgebra, $p_{\bar h} \in S$.
%% it closed under multiplication
%%Note that $p_{\bar h} \in S$ is true because $S$, as a subalgebra, is
%%closed under multiplication and each $c_{i j} = (c_{i j k})_{k = 1}^m \in S$ when not all $h_{i j} = 0$,
%%and also because $p_{\bar h} = 1_m \in S$ when all $h_{i j} = 0$.
%For each $1 \le i < j \le s$, let $D_{i j}$
%be the set of distinct elements in $\{ c_{i j k} \mid k \in [m]\}$
 %(removing all repetitions)
%and let $d_{i j} = |D_{i j}|$ be its cardinality.
%Then $2 \le d_{i j} \le m$.
%We impose a linear order on each $D_{i j}$ and also regard it as a tuple.
%Let $H = \{\bar h = (h_{i j})_{1 \le i < j \le s} \mid 0 \le h_{i j} < d_{i j},\, 1 \le i < j \le s\}$.
%%(Note that $H \ne \emptyset$.)
%Consider the  matrix $A = (A_{k \bar h})_{k \in [m], \bar h \in H}$
%having rows indexed by $[m]$ and columns indexed by $H$,
%with entries $A_{k \bar h} = \prod_{1 \le i < j \le s} c_{i j k}^{h_{i j}}$
%where $k \in [m]$ and $\bar h = (h_{i j})_{1 \le i < j \le s} \in H$.
%Note that the first $s$ rows of $A$
 %are pairwise distinct; the other $m-s$ rows are repeated rows according to
%the equivalence relation.
%
%For each $1 \le i < j \le s$, let $B^{(i j)} = (\lambda^t)_{\lambda \in D_{i j}, 0 \le t \le d_{i j} - 1}$
%be the square Vandermonde matrix having rows indexed by $\lambda \in D_{i j}$
%and columns indexed by $0 \le t \le d_{i j} - 1$.
%Since all elements of $D_{i j}$ are distinct,
%the Vandermonde matrix $B^{(i j)}$ is nondegenerate for $1 \le i < j \le s$.
%Therefore the Kronecker product $B = \bigotimes_{1 \le i < j < s} B^{(i j)}$
%is a nondegenerate square matrix of order $\prod_{1 \le i < j \le s} d_{i j}$.
%%,
%%which is an $\prod_{1 \le i < j \le s} D_{i j}$ by $\prod_{1 \le i < j \le s} d_{i j}$ square matrix is nondegenerate.
%
%It is easy to see that for every $k \in [m]$, row $k$ of $A$ %, i.e., $A_{k, \cdot} = (\prod_{1 \le i < j \le s} c_{i j k}^{h_{i j}})_{\bar h \in H}$
%is precisely the row of $B$ indexed by
%the tuple $(c_{i j k})_{1 \le i < j \le s}$.
%Here $c_{i j k} \in D_{i j}$ for $1 \le i < j \le s$ 
%so the tuple 
%$(c_{i j k})_{1 \le i < j \le s} \in \prod_{1 \le i < j \le s} D_{i j}$ as a direct
%product set, for $k \in [m]$.
%In particular the first $s$ rows of $A$ correspond
%to distinct rows of $B$.
%Since $B$ is nondegenerate,  it follows that $\rank(A) = s$.
%%Note that if $k, \ell \in [m]$ are in the same $I_i$,
%%where $i \in [s]$, %$k, \ell \in [m]$ and 
%%then the rows $k$ and $\ell$ of $A$ are the 
%%same and correspond to the same row of $B$,
%%and if $k, \ell \in [m]$ are in different $I_i$'s, %$k, \ell \in [m]$, $k < \ell$,
%%then the rows $k$ and $\ell$ of $A$ correspond to different rows of $B$.
%%This way distinct rows of $A$ correspond to distinct rows of $B$.
%%Since $A$ has precisely $s$ pairwise distinct rows (up to repetitions),
%%and $B$ is nondegenerate, it follows that $\rank(A) = s$.
%
%We show that $\im A = \{ A x \mid x \in \bbF^m \} 
%= \bbF^{(\calI_1, \ldots, \calI_s)}$, with the latter 
%thought of as a column space.
%Obviously, $\im A \subseteq \bbF^{(\calI_1, \ldots, \calI_s)}$
%as for any $i \in [s]$, rows $k, \ell \in I_i$ of $A$ are the same.
%Since $\rank(A) = s$, we have $\dim \im A = s$ but clearly $\dim \bbF^{(\calI_1, \ldots, \calI_s)} = s$
%and so $\im A = \bbF^{(\calI_1, \ldots, \calI_s)}$.
%From this, it follows that for any
%column vector $a = (a_k)_{k \in [m]} \in \bbF^{(\calI_1, \ldots, \calI_s)}$
%we have $a = \sum_{\bar h \in H} x_{\bar h} p_{\bar h}$ 
%for some $x_{\bar h} \in \bbF$.
%But each $p_{\bar h} \in S$, which as a subalgebra is certainly
 %a vector subspace,
 %so $a \in S$. 
%This implies $\bbF^{(\calI_1, \ldots, \calI_s)} \subseteq S$ and we are done.
%%\end{proof}


==> pm-rk-con-ten-GH-article-(cpc-submission)/ttttttttttt <==
\section{Proof of Main Theorem}\label{sec:proof-of-main-results}

For now, we do not make any assumptions on the graph parameter $f$;
we will introduce more assumptions as needed to prove the desired statements.
When we speak of submonoids, subrings and subalgebras we require
that the multiplicative identity coincide with that of the larger structure.
When a subset with the induced operations forms a monoid, ring or algebra
we will simply say that it is respectively
a monoid, ring or algebra in the larger structure. 
We \emph{allow} zero algebras and rings, in which $0 = 1$. 
Statements about such structures can be easily checked. 
%For convenience, we will assume that the product of "zero" elements in a multiplicative structure,
%be it a monoid, ring or algebra is its (multiplicative) identity.
A function of arity zero is a scalar.
We identify a (labeled) graph with its (labeled) graph isomorphism class.

\subsection{The monoid and algebra of graphs}\label{subsec:monoid-and-algebra-of-graphs}

For every finite set $S \subseteq \posints$, we denote
by $U_S$ the graph with $|S|$ nodes labeled by $S$ and no edges. 
Note that $U_\emptyset = K_0$ is the empty graph.

We put all $k$-labeled graphs into a single structure as follows.
By a \textit{partially labeled graph} we mean a finite graph
in which some of the nodes are labeled by distinct positive integers.
(All label sets are finite.)
Two partially labeled graphs are \textit{isomorphic}
if there is an isomorphism between them preserving all labels.
For two partially labeled graphs $G_1$ and $G_2$,
let $G_1 G_2$ denote the partially labeled graph
obtained by taking the disjoint union of $G_1$ and $G_2$,
and identifying the nodes with the same label;
the union of the label sets become the labels of $G_1 G_2$.
This way we obtain a commutative monoid $\calPLG$
with the empty graph $U_\emptyset$ being the identity~\footnote{In \cite{Freedman-Lovasz-Schrijver-2007},
the word semigroup instead of monoid is used.
A monoid is a semigroup with identity,
and all semigroups in~\cite{Freedman-Lovasz-Schrijver-2007}
have or assume to have identity.
Thus, our use of the term monoid is consistent with that of~\cite{Freedman-Lovasz-Schrijver-2007}.}.
For every finite set $S \subseteq \posints$,
we call a partially labeled graph $S$\textit{-labeled},
if its labels form the set $S$.
We call a partially labeled graph ${\subseteq} S$\textit{-labeled},
if its labels form a subset of $S$.
%So every $S$-labeled graph is automatically an ${\subseteq} S$-labeled graph.
We define $\calPLG(S)$, respectively  $\calPLG_\subseteq(S)$,
  to be the subset of $\calPLG$
consisting of all isomorphism classes of $S$-labeled,
respectively ${\subseteq} S$-labeled, graphs.
Clearly $\calPLG(S) \subseteq \calPLG_\subseteq(S)$.
%Next, we define $\calPLG_\subseteq(S)$ to be the subset of $\calPLG$
%consisting of all isomorphism classes of ${\subseteq} S$-labeled graphs.
Then both $\calPLG(S)$ and $\calPLG_\subseteq(S)$ are commutative monoids in $\calPLG$.
$\calPLG_\subseteq(S)$ is a submonoid of $\calPLG$
with the same identity $U_\emptyset$,
while  $\calPLG(S)$ is a submonoid of $\calPLG$ iff $S = \emptyset$,
as the identity in $\calPLG(S)$ is $U_S$.

%Given a monoid $M$, we call a map $g \colon M \to \bbF$ a \textit{(monoid) character}
%if $g$ is a monoid homomorphism, where $\bbF$ is viewed as a monoid under multiplication.
%That is, $g$ is a character iff $g(e) = 1$ where $e$ is the identity in $M$
%and $g(a b) = g(a) g(b)$ for all $a, b \in M$.
%Note that we allow $g$ to take zero values.
%Let $\bbF M$ be the monoid algebra of $M$ over $\bbF$,
%which consists of formal finite linear combinations of $M$.
%Extending $g$ by linearity we can assume that
%$g \colon \bbF M \to \bbF$ is an algebra homomorphism.
%Clearly, this correspondence is a bijection between the characters from $M$ to $\bbF$
%and the algebra homomorphisms from $\bbF M$ to $\bbF$,
%so we can implicitly identify one with another.

%%{\color{red} (added the definitions of quantum graphs)
%

Let $\mathcal G$ denote the
 monoid algebra $\bbF \calPLG$ consisting of all finite formal
linear combinations of $\calPLG$ with coefficients from $\bbF$; they are
called (partially labeled, $\bbF$-)\textit{quantum graphs}.
Restricting the labels to precisely $S$ or to subsets of $S$, 
we have $\bbF \calPLG(S)$ or $\bbF \calPLG_\subseteq(S)$,
respectively the  $S$-labeled or  $\subseteq S$-labeled 
\textit{quantum graphs},
respectively denoted  by  $\calG(S)$ or $\calG_\subseteq(S)$.
$\calG(S)$ is  
an algebra inside $\calG$ with $U_S$ being the multiplicative identity,
and $\calG_\subseteq(S)$ is a subalgebra of $\calG$.
%with $U_\emptyset$ being the identity in both.
The empty sum is the additive identity in all.

%
%A (partially labeled, $\bbF$-)\textit{quantum graph} is a finite formal 
%linear combination of finite   with coefficients from $\bbF$.
%linear combination)
%An $S$-labeled  ($\bbF$-)\textit{quantum graph} is a finite formal 
%linear combination (with coefficients from $\bbF$)
%of finite  $S$-labeled graphs. 
%The notion of a $\subseteq S$-labeled ($\bbF$-)\textit{quantum graph} is 
%defined analogously.
%%When the label sets of the constituent graphs 
%%(with nonzero coefficients) are precisely
%%$S$ ($\subseteq S$)-labeled graphs,
%%we call such a quantum graph an $S$ ($\subseteq S$)-labeled \textit{quantum graph}.
%%%((alternative phrasing) An $S$ ($\subseteq S$)-labeled \textit{quantum graph} is a finite formal linear 
%%%combination of finite  $S$ ($\subseteq S$)-labeled) graphs.)
%%%If the coefficients come from $\bbF$ we call these objects
%%%(partially, $S$ or $\subseteq S$-labeled) $\bbF$-quantum graphs, respectively.
%%%}
%
%Let $\mathcal G$ denote the monoid algebra $\bbF \calPLG$,
%i.e., the (infinite dimensional) vector space of
%finite formal $\bbF$-linear combinations of elements of $\calPLG$,
%or, {\color{red}(need to have a specifier) partially labeled} $\bbF$-quantum graphs. 
%Restricting the label set,
%for every finite set $S \subseteq \posints$,
%we have the monoid algebra $\calG(S) = \bbF \calPLG(S)$.
%This is an algebra inside $\calG$ with $U_S$ being the identity. 
%We also have the monoid algebra $\calG_\subseteq(S) = \bbF \calPLG_\subseteq(S)$.
%This $\calG_\subseteq(S)$ is a subalgebra of $\calG$,
%%with $U_\emptyset$ being the identity in both. 

%Let us consider the case
%when $f = \hom(\cdot, H)$ for some weighted graph $H$.
%For every map $\Phi \colon \posints \to V(H)$,
%and every partially labeled graph $G$ with the label set $S$,
%we define $\hom_\Phi(G, H) = \hom_{\Phi|_S}(G, H)$,
%(see Equation (\ref{eqn:partial-hom-dec})).
%Equation (\ref{eqn:partial-hom-mult}) implies that the function $\hom_\Phi(\cdot, H)$ is a 
%character of the monoid $\calPLG(S)$ and formula (\ref{eqn:full-hom-dec}) gives 
%an expression of $f$ as a linear combination of these 
%characters (from $\calPLG(S)$ to $\bbF$).
%{\color{red} (the actual labels make no difference, that's why the transition $[k] \to S$ is fine)}

Because many definitions, notations and statements
for $\calPLG(S), \calG(S)$ and $\calPLG_\subseteq(S), \calG_\subseteq(S)$ appear similar, 
we will often commingle them to minimize repetitions,
e.g., we use $\calG_{(\subseteq)}(S)$ to denote
either $\calG(S)$ or $\calG_\subseteq(S)$ (and the statements are asserted for both).

We can extend $f$ to a linear map on $\calG$, and
define an $n$-fold multilinear form,  where $n \ge 1$,
\[
\langle x_1, \ldots, x_n \rangle_{(n)} = f(x_1 \cdots x_n),~~~~~~\mbox{for}~~
x_1, \ldots, x_n \in  \calG.
\]
%for every $n \ge 1$ and $x_1, \ldots, x_n \in \calG$.
%for $x_1, \ldots, x_n \in \calG$.  
It is symmetric because $\calG$ is commutative.
Note that if we restrict each argument to $\calG[k]$
and then write it with respect to the basis $\calPLG[k]$ of $\calG[k]$,
we get precisely the connection tensor (array) $T(f, k, n)$.

Let
\[
\calK = \{ x \in \calG \colon f(x y) = \langle x, y \rangle = 0 \ \forall y \in \calG \}
\]
be the annihilator of $\calG$.
Clearly, $\calK$ is an ideal in $\calG$,
so we can form the quotient algebra $\hat \calG = \calG / \calK$
which is commutative as well.
We denote its identity by $u_\emptyset = U_\emptyset + \calK$.
More generally, we denote $u_S = U_S + \calK$
 for any finite subset $S \subseteq \posints$.
%Furthermore, 
If $x \in \calK$, then $f(x) = f(x U_\emptyset) = 0$
and so $f$ can also be considered as a linear map on $\hat \calG$.
For a partially labeled graph $G$ we 
denote by $\hat G = G + \calK$ the corresponding element of $\hat \calG$.
More generally, we write $\hat x = x + \calK$ for any $x \in \calG$. 
Since $\calK$ is an ideal in $\calG$, the form
$\langle \cdot, \ldots, \cdot \rangle_{(n)}$ on $\calG$ induces
an $n$-fold multilinear form on $\hat \calG$,  where $n \ge 1$, 
%\[
\begin{equation}\label{eqn:f-on-hat-calG}
\langle x_1, \ldots, x_n \rangle_{(n)} = f(x_1 \cdots x_n),~~~~~~\mbox{for}~~
x_1, \ldots, x_n \in \hat \calG.
\end{equation}
%\]
%for every $n \ge 1$ and $x_1, \ldots, x_n \in \hat \calG$.
%for $x_1, \ldots, x_n \in \hat \calG$.

%{\color{red} (remove)
%
%If $S, T \subseteq \posints$ are finite subsets,
%then $\calPLG_{(\subseteq)}(S) \, \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$
%so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$. 
%%Going to the quotients, we conclude that $\hat \calG_{(\subseteq)}(S) \, \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cap T)$.
%}

We can also define
\[
\hat \calG_{(\subseteq)}(S) = (\calG_{(\subseteq)}(S) + \calK) / \calK = \{ x + \calK \mid x \in \calG_{(\subseteq)}(S) + \calK \}
= \{ x + \calK \mid x \in \calG_{(\subseteq)}(S)\}.
\]
%Then
%\[
%\hat \calG_{(\subseteq)}(S) = \{ x + \calK \mid x \in \calG_{(\subseteq)}(S)\}.
%\]
It is easy to see that $\hat \calG_\subseteq(S)$ is a subalgebra of $\hat \calG$
with the same identity $u_\emptyset = U_\emptyset + \calK$,
and $\hat \calG(S)$ is an algebra inside $\hat \calG$
with the identity $u_S = U_S + \calK$~\footnote{In contrast to \cite{Freedman-Lovasz-Schrijver-2007}
we cannot normalize $f$ to make all elements $u_S$, for finite $S \subseteq \posints$,
the same in the quotient algebra $\hat \calG$.
In our more general setting, it is possible $f(K_1) = 0$,
in which case the normalization step from \cite{Freedman-Lovasz-Schrijver-2007} fails.}.
%\sout{$\calK$ is also an ideal in $\calG_{(\subseteq)}(S) + \calK$ and therefore $(\calG_{(\subseteq)}(S) + \calK) / \calK$ is an algebra (a subalgebra, resp.) in $\calG / \calK$.}

%{\color{red} (added here)

If $S, T \subseteq \posints$ are finite subsets,
then $\calPLG_{(\subseteq)}(S) \, \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$
so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$
and so, going to the quotitents, we have $\hat \calG_{(\subseteq)}(S) \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cup T)$.
Also note that for a finite $S \subseteq \posints$,
we have $\calPLG(S) \subseteq \calPLG_\subseteq(S)$
so by linearity $\calG(S) \subseteq \calG_\subseteq(S)$
and then by going to the quotients we obtain $\hat \calG(S) \subseteq \hat \calG_\subseteq(S)$.
%}

Since
% $\calK$ is an ideal in $\calG$,
%we also have that 
$\calG_{(\subseteq)}(S) \cap \calK$ is an ideal in $\calG_{(\subseteq)}(S)$,
 we can also form 
another quotient algebra 
\[
\tilde \calG_{(\subseteq)}(S) = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK).
\] 
%%%
%
%{\color{red} (say it here instead)
%If $S, T \subseteq \posints$ are finite subsets, then $\calPLG_{(\subseteq)}(S) \, \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$ so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$
%and so, going to the quotitents, we have $\hat \calG_{(\subseteq)}(S) \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cup T)$.
%Also note that for a finite $S \subseteq \posints$, we have $\calPLG(S) \subseteq \calPLG_\subseteq(S)$ so by linearity $\calG(S) \subseteq \calG_\subseteq(S)$
%and then by going to the quotients we obtain $\hat \calG(S) \subseteq \hat \calG_\subseteq(S)$.}
%
%%%
%The following lemma provides us with canonical isomorphisms. {\color{red} (change the sentence)}
We have the following
 canonical isomorphisms between $\tilde \calG_{(\subseteq)}(S)$
 and $\hat \calG_{(\subseteq)}(S)$.
\begin{lemma}\label{lem:calG(subseteq)(S)/calK(subseteq)S-canonical-isomorphism}
Let $S \subseteq \posints$ be finite. Then $\tilde \calG_{(\subseteq)}(S) \cong \hat \calG_{(\subseteq)}(S)$ as algebras via $x + \calG_{(\subseteq)}(S) \cap \calK \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$.
\end{lemma}
\begin{proof}
It follows from
the 
%standard 
Second Isomorphism Theorem for algebraic structures
(see~\cite{Cohn-book} p. 8).
%(e.g., see page 8 of~\cite{Cohn-book}).
%, or \cite{Jacobson-book}). 
%
%We repeat the standard proof of the Second Isomorphism Theorem for algebraic structures.
%
%Obviously, the map $\calG_{(\subseteq)}(S) \mapsto (\calG_{(\subseteq)}(S) + \calK) / \calK,\, x \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$ is a surjective algrebra homormophism with the kernel equal to $\calG_{(\subseteq)}(S) \cap \calK$ which is an ideal in $\calG_{(\subseteq)}(S)$. Then this map factors through $\calG_{(\subseteq)}(S) / \calK_S$ resulting in an algebra isomorphism between $\tilde \calG_{\subseteq}(S) = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK)$ and $\hat \calG_{(\subseteq)}(S) = \calG_{(\subseteq)}(S) / \calK$ given by $x + \calK_S \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$.
\end{proof}

We say that elements $x, y \in \calG \,(\text{or } \hat \calG)$
are orthogonal (with respect to $f$),
if $f(x y) = 0$ and denote it by $x \perp y$.
For a subset $A \subseteq \calG \,(\text{or } \hat \calG)$, 
denote by $A^\perp = \{ x \in \calG \,(\text{or } \hat \calG) \mid x \perp y, \, \forall y \in A \}$
those in $\calG \,(\text{or } \hat \calG)$ orthogonal to all elements in $A$.
Next, we say that subsets $A, B \subseteq \calG \,(\text{or } \hat \calG)$
are orthogonal (with respect to $f$),
if $x \perp y$ for all $x \in A$ and $y \in B$.
Similarly, we can talk about an element of $\calG \,(\text{or } \hat \calG)$
being orthogonal to a subset of $\calG \,(\text{or } \hat \calG)$ and vice versa.
Note that the notion of orthogonality is symmetric
since all the multiplication operations considered are commutative.
From the definition, we have $\calK = \calG^\perp$.
Next, denote (commingling the notations $\calK_S$ and $\calK_{\subseteq S}$)
\[
\calK_{(\subseteq) S} = \{ x \in \calG_{(\subseteq)} (S) \mid x \perp y, \ \forall y \in \calG_{(\subseteq)}(S) \} = \calG_{(\subseteq)}(S) \cap (\calG_{(\subseteq)}(S))^\perp.
\]
Clearly, $\calK_{(\subseteq) S}$ is an ideal in $\calG_{(\subseteq)}(S)$,
so we can form yet another quotient algebra $\calG_{(\subseteq)}(S) / \calK_{(\subseteq) S}$. 

Next, we define an orthogonal projection
from $\hat \calG$ to the subalgebra $\hat \calG_\subseteq(S)$.
We will show how to do it in a series of lemmas.
Let $S \subseteq \posints$ be finite.
For every partial labeled graph $G$,
let $G_S$ denote the ${\subseteq} S$-labeled graph obtained by deleting
the labels not in $S$ from the vertices of $G$ (unlabeling such vertices).
Extending this map by linearity,
we get a linear map $\pi_S \colon \calG \to \calG_\subseteq(S)$.
Note that $(\pi_S)_{| \calG_\subseteq(S)} = \id_{|\calG_\subseteq(S)}$.
In particular, $\pi_S \colon \calG \to \calG_\subseteq(S)$ is surjective.

\begin{lemma}\label{lem:projection}
Let $S \subseteq \posints$ be finite.
If $x \in \calG$ and $y \in \calG_\subseteq(S)$, then
\[
f(x y) = f(\pi_S(x) y).
\]
\end{lemma}
\begin{proof}
For every $G_1 \in \calPLG$ and $G_2 \in \calPLG_\subseteq(S)$,
the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic as unlabeled graphs.
Hence $f(G_1 G_2) = f(\pi_S(G_1) G_2)$ as $f$ ignores labels.
The lemma follows by linearity.
\end{proof}

\begin{corollary}\label{cor:projection-part-orthogonality}
Let $S \subseteq \posints$ be finite.
If $x \in \calG$, then $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
\end{corollary}
\begin{proof}
Fix any $y \in \calG_\subseteq(S)$. By Lemma~\ref{lem:projection},
$f(x y) = f(\pi_S(x) y)$ so $f((x - \pi_S(x)) y) = 0$.
Thus $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
\end{proof}

So for any $x \in \calG$, we can write $x = \pi_S(x) + (x - \pi_S(x))$
where $\pi_S(x) \in \calG_\subseteq(S)$, and $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
%by Corollary~\ref{cor:projection-part-orthogonality}.
This gives a decomposition $\calG = \calG_\subseteq(S) + (\calG_\subseteq(S))^\perp$.
%To get a similar decomposition into a direct sum,
To get a direct sum decomposition,
% make such a decomposition into a direct sum,
we need to pass to the quotient algebra.
But to do so properly we need some lemmas.
%first  it correctly we first need to prove some statements.

\begin{lemma}\label{lem:calKS}
Let $S \subseteq \posints$ be finite.
Then $\calK_S = \calG(S) \cap \calK$.
\end{lemma}
\begin{proof}
Clearly,
$\calG(S) \cap \calK = \calG(S) \cap \calG^\perp \subseteq
 \calG(S) \cap (\calG(S))^\perp = \calK_S$,
% $\calK_S = \calG(S) \cap (\calG(S))^\perp \supseteq \calG(S) \cap \calG^\perp = \calG(S) \cap \calK$,
so we only need to prove the reverse inclusion. 
Let $x \in \calK_S = \calG(S) \cap (\calG(S))^\perp$.
Take any $y \in \calG$. Then
\[
f(x y) \stackrel{(1)}{=} f(x \pi_S(y)) \stackrel{(2)}{=} f(x U_S \pi_S(y)) \stackrel{(3)}{=} 0.
\]
Here step $(1)$ uses Lemma~\ref{lem:projection} 
as $x \in \calG(S) \subseteq \calG_{\subseteq}(S)$;
$(2)$ is true because $x = x U_S$ for $x \in \calG(S)$;
$(3)$ is true as $\pi_S(y) \in \calG_\subseteq(S)$
so $U_S \pi_S(y) \in \calG(S)$, and as $x \in (\calG(S))^\perp$.
Then $x \in \calK$ so $x \in \calG(S) \cap \calK$,
implying $\calK_S \subseteq \calG(S) \cap \calK$.
\end{proof}

\begin{lemma}\label{lem:calKsubseteqS}
Let $S \subseteq \posints$ be finite.
Then $\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap \calK$.
\end{lemma}
\begin{proof}
Clearly,
$\calG_\subseteq(S) \cap \calK = \calG_\subseteq(S) \cap \calG^\perp
\subseteq  \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp = 
\calK_{{\subseteq}S}$,
% $\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp \supseteq \calG_\subseteq(S) \cap \calG^\perp = \calG_\subseteq(S) \cap \calK$,
so we only need to prove the reverse inclusion. 
Let $x \in \calK_{{\subseteq}S} = \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp$.
Take any $y \in \calG$. Then
\[
f(x y) \stackrel{(1)}{=} f(x \pi_S(y)) \stackrel{(2)}{=} 0.
\]
Here step $(1)$ uses Lemma~\ref{lem:projection};
$(2)$ is true as $\pi_S(y) \in \calG_\subseteq(S)$
and $x \in (\calG_\subseteq(S))^\perp$.
Then $x \in \calK$ so $x \in \calG_\subseteq(S) \cap \calK$,
implying $\calK_{\subseteq S} \subseteq \calG_\subseteq(S) \cap \cal K$.
\end{proof}

It follows from Lemmas~\ref{lem:calKS}~and~\ref{lem:calKsubseteqS} that
$\calG_{(\subseteq)}(S) / \calK_{(\subseteq) S} = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK) = \tilde \calG_{(\subseteq)}(S)$
so the (canonical) isomorphism of algebras from
Lemma~\ref{lem:calG(subseteq)(S)/calK(subseteq)S-canonical-isomorphism} takes the following form:
\begin{equation}\label{eqn:calG(subseteq)(S)-canonical-isomorphisms-new}
\tilde \calG_{(\subseteq)}(S) \cong \hat \calG_{(\subseteq)}(S),\quad x + \calK_{(\subseteq) S} \mapsto x + \calK,\quad x \in \calG_{(\subseteq)}(S).
\end{equation}

\begin{lemma}\label{lem:projection-and-preimage-of-calK-ideals}
Let $S \subseteq \posints$ be finite.
For the linear map $\pi_S \colon \calG \to \calG_\subseteq(S)$
we have $\pi_S(\calK) = \calK_{{\subseteq}S}$.
\end{lemma}
\begin{proof}
Because $(\pi_S)_{| \calG_\subseteq(S)} = \id_{|\calG_\subseteq(S)}$ and by Lemma~\ref{lem:calKsubseteqS}
$\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap \calK$,
we infer that $\pi_S(\calK) \supseteq \calK_{{\subseteq}S}$.
For the reverse inclusion, let $x \in \calK$.
Fix any $y \in \calG_\subseteq(S)$.
Then by Lemma~\ref{lem:projection}, $f(\pi_S(x) y) = f(x y) = 0$,
the last equality is true because $x \in \calK$.
Hence $\pi_S(x) \in \calK_{{\subseteq}S}$
so that $\pi_S(\calK) \subseteq \calK_{{\subseteq}S}$.
\end{proof}

For the linear map $\pi_S \colon \calG \to \calG_\subseteq(S) \subseteq \calG$
by Lemmas~\ref{lem:projection-and-preimage-of-calK-ideals} and~\ref{lem:calKsubseteqS},
$\pi_S(\calK) = \calK_{{\subseteq}S} = \calG_{\subseteq}(S) \cap \calK$,
so that we have the well-defined linear map (which we denote by $\hat \pi_S$)
\begin{equation}\label{eqn:quotient-projection}
\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S),\quad \hat \pi_S(x + \calK) = \pi_S(x) + \calK,\quad x \in \calG.
\end{equation}
 
It is easy to see that $(\hat \pi_S)_{| \hat \calG_\subseteq(S)} = \id_{|\hat \calG_\subseteq(S)}$.
In particular, $\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$ is surjective.
 
\begin{lemma}\label{lem:quotion-decomposition-through-projeciton}
Let $S \subseteq \posints$ be finite. Then $\hat \calG = \hat \calG_\subseteq(S) \oplus (\hat \calG_\subseteq(S))^\perp$ via $x = \hat \pi_S(x) + (x - \hat \pi_S(x)),\, x \in \hat \calG$.
\end{lemma}
\begin{proof}
%First, let $x \in \hat \calG$. Write $x = y + \calK$ where $y \in \calG$. Then $\hat \pi_S(x) = \pi_S(y) + \calK$ and $\pi_S(y) \in \calG_\subseteq(S)$ so $\hat \pi_S(x) \in \hat \calG_\subseteq(S)$.
%Also $x - \hat \pi_S(x) = y - \pi_S(y) + \calK$. By Corollary~\ref{cor:projection-part-orthogonality}, $y - \pi_S(y) \in (\calG_\subseteq(S))^\perp$ so that $x - \hat \pi_S(x) \in (\hat \calG_\subseteq(S))^\perp$.
%
%So we only need to show that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0 (= \calK)$. Let $z$ belong to this intersection.
%Write $z = t + \calK = t' + \calK$ where $t \in \calG_\subseteq(S)$
%and $t' \in (\calG_\subseteq(S))^\perp$. Then $t-t' \in  \calK$,
%and so $t \in (\calG_\subseteq(S))^\perp$.
%Thus $t \in \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp
%= \calK_{{\subseteq}S} \subseteq \calK$, the last inclusion holds by Lemma~\ref{lem:calKsubseteqS}. 
%Therefore $z = t + \calK = \calK$, implying that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0$.

%%%corrected proof
First, let $x \in \hat \calG$. Write $x = y + \calK$ where $y \in \calG$.
Then $\hat \pi_S(x) = \pi_S(y) + \calK$ and $\pi_S(y) \in \calG_\subseteq(S)$.
We have $x - \hat \pi_S(x) = y - \pi_S(y) + \calK$.
By Corollary~\ref{cor:projection-part-orthogonality}, $y - \pi_S(y) \in (\calG_\subseteq(S))^\perp$
so that $x - \hat \pi_S(x) \in (\hat \calG_\subseteq(S))^\perp$,
since the bilinear form on $\calG$ extends to $\hat \calG$ in~(\ref{eqn:f-on-hat-calG}).

So we only need to show that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0 (= \{\calK\})$.
Let $z$ belong to this intersection.
Write $z = t + \calK = t' + \calK$ where $t \in \calG_\subseteq(S)$
and $t' \in (\calG_\subseteq(S))^\perp$.
Then clearly $t - t' \in  \calK \subseteq (\calG_{\subseteq}(S))^\perp$,
%%% i removed ( and ) in \calG_{(\subseteq)}(S)
and so $t = (t - t') + t' \in (\calG_\subseteq(S))^\perp$.
Thus $t \in \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp = \calK_{{\subseteq}S} \subseteq \calK$,
the last inclusion holds by Lemma~\ref{lem:calKsubseteqS}. 
Therefore $z = t + \calK = \calK$,
implying that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0$.
\end{proof}

Thus Lemma~\ref{lem:quotion-decomposition-through-projeciton} allows us
to rightfully call $\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$
an orthogonal projection of $\hat \calG$ to $\hat \calG_\subseteq(S)$.

If $S, T \subseteq \posints$ are finite subsets,
then $\pi_S(\calPLG_{(\subseteq)}(T)) = \calPLG_{(\subseteq)}(S \cap T)$,
where the projection is surjective because
the restriction $(\pi_S)_{| \calPLG_{(\subseteq)}(S \cap T)} = \id_{|\calPLG_{(\subseteq)}(S \cap T)}$.
So by linearity we get $\pi_S(\calG_{(\subseteq)}(T)) = \calG_{(\subseteq)}(S \cap T)$.
Going to the quotients, we conclude that $\hat \pi_S(\hat \calG_{(\subseteq)}(T)) = \hat \calG_{(\subseteq)}(S \cap T)$.

\begin{lemma}\label{lem:orthogonal-complement-equivalence-for-calG(subseteq)(S)}
Let $n \ge 2$ and $S \subseteq \posints$ be finite.
Then for any $x \in \calG_{(\subseteq)}(S)$, we have $x \in \calK_{(\subseteq) S}$
iff $f(x x_1 \cdots x_{n - 1}) = 0$ for all $x_1, \ldots, x_{n - 1} \in \calG_{(\subseteq)}(S)$.
\end{lemma}
\begin{proof}
%For $\Rightarrow$, it suffices to note that $\calG_{(\subseteq)}(S)$ is 
%closed under multiplication (in $\calG$). To prove $\Leftarrow$, note that $n - 2 \ge 0$ and for any $y \in \calG_{(\subseteq)}(S)$, we have $f(x y) = f(x y U_0^{n - 2}) = 0$ so $x \in \calK_{(\subseteq) S}$.

%%%corrected proof
For $\Rightarrow$, it suffices to note that $\calG_{(\subseteq)}(S)$
is closed under multiplication (in $\calG$).
To prove $\Leftarrow$, note that $n - 2 \ge 0$ and for any $y \in \calG_{(\subseteq)}(S)$,
we have $f(x y) = f(x y U^{n - 2}) = 0$,
where $U = U_\emptyset$ in the $\calG_\subseteq(S)$ case and
$U = U_S$ in the $\calG(S)$ case,
so $x \in \calK_{(\subseteq) S}$.
\end{proof}

\begin{lemma}\label{lem:empty-annihilator-for-hat-calG(subseteq)(S)}
Let $S \subseteq \posints$ be finite.
Then the annihilator of $\hat \calG_{(\subseteq)}(S)$ in $\hat \calG_{(\subseteq)}(S)$ is zero, i.e.,
if $x \in \hat \calG_{(\subseteq)}(S)$ and $f(x y) = 0$
for every $y \in \hat \calG_{(\subseteq)}(S)$, then $x$
is
the zero element of $\hat \calG_{(\subseteq)}(S)$, namely $\calK$.
%for every $y \in \hat \calG_{(\subseteq)}(S)$, then $x = \calK$.
\end{lemma}
\begin{proof}
%%% corrected proof
Let $x \in \hat \calG_{(\subseteq)}(S)$ be
an element satisfying the hypothesis of the lemma.
Write $x = h_1 + \calK$ where $h_1 \in \calG_{(\subseteq)}(S)$.
By hypothesis, for every 
$y \in \hat \calG_{(\subseteq)}(S)$ we have $f(x y) = 0$.
Let $h_2 \in \calG_{(\subseteq)}(S)$
and put $y = h_2 + \calK \in \hat \calG_{(\subseteq)}(S)$.
Then $x y = h_1 h_2 + \calK$.
By the definition of $f$ on $\hat \calG$, $f(h_1 h_2) = f(x y) = 0$. 
Hence $h_1 \in \calK_{(\subseteq) S} \subseteq \calK$
where the last inclusion is true by Lemmas~\ref{lem:calKS} and~\ref{lem:calKsubseteqS}.
This implies that $x$ is the  zero element of $\hat \calG_{(\subseteq)}(S)$,
which is $\calK$.
\end{proof}

\begin{lemma}\label{lem:calK[k]-T(f,k,n)-xi(h)-criterion}
Let $k, r \ge 0$ and $n \ge \max(2, r)$.
Suppose the connection tensor $T(f, k, n)$ can be expressed as
\[
T(f, k, n) = \sum_{i = 1}^r a_i \bfx_i^{\otimes n},
\]
where $a_i \ne 0$ and $\bfx_i
\in \bbF^{\calPLG[k]}$ are nonzero and \emph{pairwise} linearly independent for $1 \le i \le r$.
Then for any $h \in \calG[k]$, we have $h \in \calK_{[k]}$ iff $\bfx_i(h) = 0, \, 1 \le i \le r$.
\end{lemma}
\begin{proof}
The lemma is clearly true for $r=0$. Let $r \ge 1$.
By Lemma~\ref{lem:orthogonal-complement-equivalence-for-calG(subseteq)(S)},
$h \in \calK_{[k]}$ iff $f(h h_1 \cdots h_{n - 1}) = 0$ for all $h_1, \ldots, h_{n - 1} \in \calG[k]$.
In terms of $T(f, k, n)$, this is equivalent to $(T(f, k, n))(h, \cdot, \ldots, \cdot) = 0$
which is the same as
\[
\sum_{i = 1}^r a_i \, \bfx_i(h) \, \bfx_i^{\otimes (n - 1)} = 0.
\]
Now if $\bfx_i(h) = 0, \, 1 \le i \le r$, then this equality clearly holds.
Conversely, if this equality holds, then by Lemma~\ref{lem:tensor-powers-pairwise-implies-linear-independence},
$a_i \bfx_i(h) = 0$ but $a_i \ne 0$ so $\bfx_i(h) = 0, \,  1 \le i \le r$.
\end{proof}

We will also need the following lemma 
that classifies all subalgebras of $\bbF^m$ for $m \ge 0$.
A proof is given in
 subsection~\ref{subsec:bbF^m-subalgebras} of the Appendix. 
%(or the Appendix (Section~\ref{sec:Preliminary-continued}).)
Recall that we allow zero algebras %(i.e., $\bbF^0 = \{ \emptyset \}$, where $0 = 1 = \emptyset$)
and require any subalgebra of an algebra to share the multiplicative identity.
%{\color{red} with the larger algebra (added)}.

\begin{lemma}\label{lem:F^m-subalgebras}
All subalgebras of $\bbF^m$, where $m \ge 0$, are of the following form:
For some partition $[m] = \bigsqcup_{i = 1}^s \calI_s$,
where $s \ge 0$, and $\calI_i \ne \emptyset$ for $i \in [s]$, 
the subalgebra has equal values on each $I_i$,
\[
\bbF^{(\calI_1, \ldots, \calI_s)} = \{ (c_1, \ldots, c_m) \in \bbF^m \mid \forall i \in [s], \ \forall j, j' \in \calI_i, \ c_j = c_{j'} \}.
\]
\end{lemma}

\subsection{Building an algebra isomorphism~\label{sec:build-alg-isom}}

In this part of the proof regarding $f$ we assume that for every $k \ge 0$
there exists $n = n_k \ge 2$ such that $\symrank T(f, k, n) \le n - 1$.
We will pick an arbitrary such $n$ and call it $n_k$,
and then write $r_k = \symrank T(f, k, n_k)$. 
(Note that this is weaker than the
uniform exponential bounded in $k$ for $\symrank T(f, k, n)$
in Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse},
nor do we require $f(K_0) = 1$ here.)
% to be (uniformly) exponentially bounded in $k$ or $f(K_0) = 1$,
%as the conditions in Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse} would require.)
% {\color{red} (require / do / just remove)}.)
%The results of this part will be valid without these assumptions.

Then, for $n = n_k$, we can write,
\begin{equation}\label{eqn:T(f,k,n)-gen-dec}
T(f, k, n) = \sum_{i = 1}^{r_{k}} a_{k, n, i} \bfx_{k, n, i}^{\otimes n}.
\end{equation}
Then $a_{k, n, i} \ne 0$ and $0 \ne\bfx_{k, n, i} \in \bbF^{\calPLG[k]}$ 
are pairwise linearly independent for $1 \le i \le r_{k}$.

Define the linear map
\begin{equation}\label{eqn:Phi-map}
\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}},\quad \Phi_{k, n}(h) = ( \bfx_{k, n, i}(h) )_{i= 1, \ldots, r_{k}}, \quad h \in \calG[k].
\end{equation}
We show that $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$
is a surjective algebra homomorphism.
% (algebra epimorphism).
Clearly, as $n \ge 2$, 
%{\color{red} (check the commas)}
\[
h_1 \cdot h_2 \cdot h_3 \cdots h_n = (h_1 h_2) \cdot U_k \cdot h_3 \cdots h_n
\]
so
\[
f(h_1 \cdot h_2 \cdot h_3 \cdots h_n) = f((h_1 h_2) \cdot U_k \cdot h_3 \cdots h_n)
\]
for all $h_1, \ldots, h_n \in \calG[k]$.
(When $n = 2$ this is $f(h_1 h_2) = f((h_1 h_2) U_k)$.)
Therefore
\[
(T(f, k, n))(h_1, h_2, \cdot, \ldots, \cdot) =  (T(f, k, n))(h_1 h_2, U_k, \cdot, \ldots, \cdot)
\]
for all $h_1, h_2 \in \calG[k]$.
In terms of the decomposition in (\ref{eqn:T(f,k,n)-gen-dec}),
this is equivalent to 
\[
\sum_{i = 1}^{r_{k}} \, a_{k, n, i} \, \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) \, \bfx_{k, n, i}^{\otimes (n - 2)} = \sum_{i = 1}^{r_{k}} a_{k, n, i} \, \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k) \, \bfx_{k, n, i}^{\otimes (n - 2)}.
\]
It follows that
\[
\sum_{i = 1}^{r_{k}} a_{k, n, i} \, \left( \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) - \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k) \right) \, \bfx_{k, i}^{\otimes (n - 2)} = 0
\]
for any $h_1, h_2 \in \calG[k]$.
The condition $r_{k} \le n - 1$ allows
us to apply Lemma~\ref{lem:tensor-powers-pairwise-implies-linear-independence}.
Since $a_{k, n, i} \ne 0$ for $1 \le i \le r_{k}$,
we obtain that
\begin{equation}\label{eqn:char-prop-unsimp}
\bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) = \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k), \quad h_1, h_2 \in \calG[k], \quad 1 \le i \le r_{k}.
\end{equation}
Let $1 \le i \le r_{k}$.
Since $\bfx_{k, n, i} \ne 0$, there exists $h \in \calG[k]$ such that $\bfx_{k, n, i}(h) \ne 0$.
Substituting $h_1 = h_2 = h$ into (\ref{eqn:char-prop-unsimp}),
we infer that $\bfx_{k, n, i}(U_k) \ne 0, \, 1 \le i \le r_{k}$.

Therefore we can assume
in (\ref{eqn:T(f,k,n)-gen-dec})
 that each $\bfx_{k, n, i}$ is normalized so that $\bfx_{k, n, i}(U_k) = 1$ ($1 \le i \le r_{k}$).
Combined with this, condition (\ref{eqn:char-prop-unsimp}) becomes for $1 \le i \le r_{k}$,
\begin{equation}\label{eqn:char-prop-simp-full}
\begin{lcases}
\bfx_{k, n, i}(h_1 h_2) &= \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2), \quad h_1, h_2 \in \calG[k]; \\
\bfx_{k, n, i}(U_k) &= 1;
\end{lcases}
\end{equation}
so the linear functions $\bfx_{k, n, i} \colon \calG[k] \to \bbF, \, 1 \le i \le r_{k}$
are algebra homomophisms. %(equivalently, characters from $\calPLG[k]$ to $\bbF$).
Then we have
\begin{gather*}
\Phi_{k, n}(g h) = ( \bfx_{k, n, 1}(g h), \ldots, \bfx_{k, n, r_k}(g h) ) = ( \bfx_{k, n, 1}(g) \, \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(g) \, \bfx_{k, n, r_k}(h)) \\
= ( \bfx_{k, n, 1}(g), \ldots, \bfx_{k, n, r_k}(g) ) \cdot ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ) = \Phi_{k, n}(g) \Phi_{k, n}(h). 
\end{gather*}
So we have
\begin{gather*}
\Phi_{k, n}(g h) = \Phi_{k, n}(g) \Phi_{k, n}(h), \quad g, h \in \calG[k], \\
\Phi_{k, n}(U_k) = ( \bfx_{k, n, 1}(U_k) \ldots, \bfx_{k, n, r_k}(U_k) ) = \underbrace{(1, \ldots, 1)}_{r_{k} \text{ times}} \in \bbF^{r_{k}},
\end{gather*}
and therefore $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$ is an algebra homomorphism.
We now prove its surjectivity.
Clearly, $\im(\Phi_{k, n})$ is a subalgebra of $\bbF^{r_{k}}$.
By Lemma~\ref{lem:F^m-subalgebras},
we may assume that $\im(\Phi_{k, n})$
has the form $\bbF^{(\calI_1, \ldots, \calI_s)}$ for some partition
$\{I_1, \ldots, \calI_s\}$ of $[r_{k}]$.
The pairwise linear independence of $\bfx_{k, n, i}$
for $1 \le i \le r_{k}$ implies that for any $1 \le i_1 < i_2 \le r_{k}$,
we have $\bfx_{i_1} \ne \bfx_{i_2}$,
so there exists $h \in \calG[k]$ such that $\bfx_{k, n, i_1}(h) \ne \bfx_{k, n, i_2}(h)$.
Since each $\calI_i \ne \emptyset$,
it follows that $|\calI_i| = 1$ for $1 \le i \le s$.
Hence $\im(\Phi_{k, n}) = \bbF^{(\{ 1 \}, \ldots, \{ r_k \})} = \bbF^{r_{k}}$.
We have shown that $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$ is surjective.

Next, by $r_{k} \le n - 1$ and $n \ge 2$, 
clearly $n \ge \max(2, r_{k})$, 
so Lemma~\ref{lem:calK[k]-T(f,k,n)-xi(h)-criterion} applies. So we have
\[
\ker \Phi_{k, n} = \{ h \in \calG[k] \mid \bfx_{k, n, i}(h) = 0,\,
1 \le i \le r_{k}  \} = \calK_{[k]},
\]
where the first equality is by the definition of $\Phi_{k, n}$,
and the second equality is by Lemma~\ref{lem:calK[k]-T(f,k,n)-xi(h)-criterion}.
Note that by Lemma~\ref{lem:calKS}, we have $\calK_{[k]} =
\calG[k] \cap \calK$.
%
%Therefore
Then $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_k}$
factors through $\calG[k] / \ker \Phi_{k, n} = \calG[k] / \calK_{[k]} = \tilde \calG[k]$,
inducing an algebra isomomorphism
\[
\tilde \Phi_{k, n} \colon \tilde \calG[k] \to \bbF^{r_{k}}, \quad \tilde \Phi_{k, n}(h + \calK_{[k]}) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \calG[k].
\]
It follows that $\dim \tilde \calG[k] = \dim \bbF^{r_{k}} = r_{k}$.
In particular, $\tilde \calG[k]$ is a finite dimensional algebra.
Applying Lemma~\ref{lem:quotient-space-dimension},
we get $\dim \tilde \calG[k] = \dim \Span \{ \bfx_{k, n, i} \}_{i = 1}^{r_{k}}$.
Then $\dim \Span \{ \bfx_{k, n, i} \}_{i = 1}^{r_{k}} = r_{k}$
implying that $\bfx_{k, n, i}$,  $1 \le i \le r_{k}$, are linearly independent.
(Note that we started off only assuming they are nonzero and pairwise linearly independent.)
%
We formalize some of the results obtained above.
\begin{lemma}\label{lem:Phi(k)-tilde-calG[k]-isomorphism}
Assume for every $k \ge 0$ there exists $n = n_k \ge 2$ 
such that $r_{k} = \symrank T(f, k, n_k) \le n_k - 1$.
Then the constructed map
\[
\tilde \Phi_{k, n} \colon \tilde \calG[k] \to \bbF^{r_{k}}, \quad \tilde \Phi_k(h + \calK_{[k]}) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \tilde \calG[k].
\]
is an algebra isomorphism and $\dim \tilde \calG[k] = r_{k}$.
\end{lemma}

Composing $\tilde \Phi_k \colon \tilde \calG[k] \to \bbF^{r_{k}}$
with the canonical algebra isomorphism between $\tilde \calG[k]$ and $\hat \calG[k]$
given in (\ref{eqn:calG(subseteq)(S)-canonical-isomorphisms-new}),
we have an algebra isomorphism $\hat \Phi_k \colon \hat \calG[k] \to \bbF^{r_{k}}$.
In particular, $\dim \hat \calG[k] = \dim \tilde \calG[k] = r_{k}$.
\begin{corollary}\label{cor:Phi(k)-hat-calG[k]-isomorphism}
With the same assumption as in Lemma~\ref{lem:Phi(k)-tilde-calG[k]-isomorphism},
for any $k \ge 0$, the  map
%constructed map
\[
\hat \Phi_{k, n} \colon \hat \calG[k] \to \bbF^{r_{k}}, \quad \hat \Phi_{k, n}(h + \calK) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \hat \calG[k].
\]
is an algebra isomorphism and  $\dim \hat \calG[k] = r_{k}$.
\end{corollary}

Note that if $S \subseteq \posints$ is finite and $|S| = k$,
there are natural isomoprphisms between $\tilde \calG(S)$ and $\tilde \calG[k]$
and also between $\hat \calG(S)$ and $\hat \calG[k]$,
both resulting from any bijective map between $S$ and $[k]$.
As a result, we conclude the following.
\begin{corollary}\label{cor:dimension-of-tilde-hat-calG(S)}
%Let $S \subseteq \posints$ be finite, $k = |S|$ and suppose there exists
%some $n \ge 2$ so that $\symrank(T(f, k, n))  \le n - 1$. 
%Let $n = n_k$ be any such choice, and let
%$r_k = \symrank(T(f, k, n_k))$.
%Then  $\tilde \calG(S) \cong \hat \calG(S) \cong \bbF^{r_{k}}$ and $\dim \tilde \calG(S) = \dim \hat \calG(S) = r_{k}$. In particular,
%the value $r_k$ is independent of any particular choice of $n_k$.
%
%%corrected
%{\color{red} corrected statement}
For any $k \ge 0$ and finite $S \subseteq \posints$ with $|S| = k$,
suppose there exists some $n \ge 2$ so that $\symrank(T(f, k, n)) \le n - 1$. 
Let $n = n_k$ be any such choice where $k \ge 0$, and let $r_k = \symrank(T(f, k, n_k))$.
Then $\tilde \calG(S) \cong \hat \calG(S) \cong \bbF^{r_{k}}$
and $\dim \tilde \calG(S) = \dim \hat \calG(S) = r_{k}$.
In particular, the value $r_k$ is independent of any particular choice of $n_k$.
\end{corollary}

\subsection{One $n$ implies for all $n$~\label{sec:one-implies-all}}

Let $n_k$ retain the same meaning
as in Lemma~\ref{lem:Phi(k)-tilde-calG[k]-isomorphism},
and let $r = r_k =  \symrank(T(f, k, n_k))$.
For any $h \in \calG[k]$, clearly
$h = h U_k^{n_k - 1}$ so $f(h) = f(h U_k^{n_k - 1})$.
As $\bfx_{k, n_k, i}(U_k) = 1, \, 1 \le i \le r$,
%Therefore
\[
\begin{split}
f(h) &= f(h U_k^{n_k - 1}) = (T(f, k, n_k))(h, U_k, \ldots, U_k) = \sum_{i = 1}^r a_{k, n_k, i} (\bfx_{k, n_k, i}(U_k))^{n_k - 1} \bfx_{k, n_k, i}(h) \\
&= \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h)
\end{split}
\]
for any $h \in \calG[k]$.
Hence $f_{|\calG[k]} = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}$, i.e.,
$f_{|\calG[k]}$ is a linear combination of $r$ algebra 
homomorphisms $\bfx_{k, n_k, i} \colon \calG[k] \to \bbF$, for $1 \le i \le r$.
In particular, applying to the product $h_1 \cdots h_n$,
for any $n \ge 0$ and  any  $h_1, \ldots, h_n \in \calG[k]$,
(note that this $n$ is arbitrary, not only for  those $n$ satisfying
the requirements for the choice of $n_k$)
\[
f(h_1 \cdots h_n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h_1 \cdots h_n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h_1) \cdots  \bfx_{k, n_k, i}(h_n).
\]
(When $n = 0$, we view it as $f(U_k) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(U_k) = \sum_{i = 1}^r a_{k, n_k, i}$.)
Hence
\begin{equation}\label{eqn:T(f,k,n)-char-dec}
T(f, k, n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}^{\otimes n}
\end{equation}
for all $n \ge 0$.
(When $n = 0$, 
%we continue the previous consideration for this case,
%so 
(\ref{eqn:T(f,k,n)-char-dec}) is still valid as
$T(f, k, 0) = f(U_k) = \sum_{i = 1}^r a_{k, n_k, i} = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}^{\otimes 0}$
where the last equality is true as $\bfx_{k, n_k, i}^{\otimes 0} = 1$.)
% by convention,
%and therefore in this case (\ref{eqn:T(f,k,n)-char-dec}) is still correct.)}

As shown before, $\bfx_{k, n_k, i}$ where $1 \le i \le r$ are linearly independent.
Then by Lemma~\ref{lem:tensor-powers-linear-independence-symmetric-rank-and-uniqueness} 
applied to (\ref{eqn:T(f,k,n)-char-dec}),
we get $\symrank(T(f, k, n)) = r$ for all $n \ge 2$;
and the decomposition (\ref{eqn:T(f,k,n)-char-dec})
is actually unique up to a permutation for $n \ge 3$. 

\begin{theorem}\label{thm:T(f,k,n)-rk-unif-dec-uniq}
Let $k \ge 0$.
Assume that for some $n = n_k \ge 2$, $\symrank T(f, k, n) = r \le n - 1$.
Then the following hold:
\begin{enumerate}
\item $\symrank T(f, k, n) = r$ for every $n \ge 2$.
\item There exist $r$ linearly independent algebra homomophisms $\bfx_i \colon \calG[k] \to \bbF$,
and $a_1, \ldots, a_r \in \bbF \setminus \{ 0 \}$ such that $f_{|\calG[k]} = \sum_{i = 1}^r a_i \bfx_i$;
also for every $n \ge 0$,
\begin{equation}\label{eqn:T(f,k,n)-unif-dec}
T(f, k, n) = \sum_{i = 1}^r a_i \bfx_i^{\otimes n}.
\end{equation}
Moreover, for any $n \ge 3$, any expression of $T(f, k, n)$ as $\sum_{i = 1}^r b_i \bfy_i^{\otimes n}$,
where $\bfy_i \colon \calG[k] \to \bbF$ are linear maps,
is a permutation of the sum in (\ref{eqn:T(f,k,n)-unif-dec}).
\end{enumerate}
\end{theorem}

%The reader may agree that
%something very nontrivial has happened.
We remark that this proves a nontrivial statement:
The existence of some $n_k$ has produced
a uniform expression for the tensors $T(f, k, n)$
all the way down to $n = 0$.

\subsection{Putting things together}

Having developed the theory in a more general setting,
we can now follow the proof in~\cite{Freedman-Lovasz-Schrijver-2007} closely.
We will be interested in the idempotent elements of $\hat \calG$.
For two elements  $p, q \in \hat \calG$,
we say that $q$ resolves $p$, if $p q = q$.
We also say equivalently $p$ is resolved by $q$. 
It is clear that the binary relation
\textit{resolves} is antisymmetric and transitive and,
when restricted to idempotents, reflexive.
Furthermore, it is easy to see that the binary 
relation \textit{resolves} on $\hat \calG$ has the following properties:

\begin{enumerate}
\item The idempotent $0 = \calK$ resolves everything and $1 = u_\emptyset = 
U_\emptyset + \calK = K_0 + \calK$ is resolved by everything.
\item If $a b = 0$ and $c$ resolves both $a$ and $b$, then $c = 0$;
\item If $a$ resolves $b$, then $c$ resolves  $a$ iff $c$ resolves $a b$.
\end{enumerate}

In the algebra $\bbF^r$ ($r \ge 0$), 
the idempotents are 0-1 tuples in $\bbF^r$, and for idempotents
$q = (q_1, \ldots, q_r)$ and $p = (p_1, \ldots, p_r)$,
$q$ resolves $p$ iff $q_i=1$ implies $p_i=1$.

Let $S$ be a finite subset of $\posints$ with $|S|=k$, and set $r = r_{k}$
as above.
By Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)},
$\hat \calG(S) \cong \bbF^r$ as algebras,
so $\hat \calG(S)$ has a (uniquely determined idempotent) basis $\calP_S = \{ p_1^S, \ldots, p_r^S \}$
such that $(p_i^S)^2 = p_i^S$ and $p_i^S p_j^S = 0$ for $i \ne j$.
These correspond to the canonical basis $\{e_i\}_{1 \le i \le r}$ of $\bbF^r$
under this isomorphism.
%Namely, it corresponds to the canonical basis of $\bbF^r$ under this isomorphism.
For $i \ne j$, we have $\langle p_i^S, p_j^S \rangle = f(p_i^S p_j^S) = 0$.
Furthermore, for all $1 \le i \le r$, $f(p_i^S) = f((p_i^S)^2) = \langle p_i^S, p_i^S \rangle \ne 0$,
%which is obvious under the isomorphism.
otherwise $\hat \calG(S)$ contains a nonzero element orthogonal to $\hat \calG(S)$
with respect to the bilinear form $\langle \cdot, \cdot \rangle$
restricted to $\hat \calG(S) \times \hat \calG(S)$, 
contradicting Lemma~\ref{lem:empty-annihilator-for-hat-calG(subseteq)(S)}.
We will call the elements $p_i^S \in \calP_S$ basic idempotents. %(of/in $\hat \calG(S)$).

%{\color{red} From now on, when talking about label sets (such as $S, T, U$ (not a unit this time)),
%we will always assume that they are finite subsets of $\posints$ but frequently omit it.}
%
%%% this was said in beginning of sec 5: JYC added that.

We denote by $\calP_{T, p}$ the set of all idempotents in $\calP_T$
that resolve a given element $p \in \hat \calG$.
If $p \in \calP_S$ and $S \subset T$ and $|T| = |S| + 1$,
then the number of elements in $\calP_{T, p}$
will be called the degree of $p \in \calP_S$, and denoted by $\deg(p)$.
Obviously, this value is independent of
which $(|S| + 1)$-element superset $T$ of $S$ we take.

For any $q \in \hat \calG(T)$, we have $q u_{T \setminus S} = q$.
It follows that for any $S \subseteq T$ and $p \in \hat \calG$,
we have  $q$ resolves $p$ iff $q$ resolves $p u_{T \setminus S}$,
since $q p = q u_{T \setminus S} p = q p u_{T \setminus S}$.
It is also important to point out that
an element in $\hat \calG(S)$ is an idempotent in $\hat \calG(S)$
iff it is an idempotent in $\hat \calG$.

%{\color{red} (propose the following change)
%
%Since $\hat \calG(S) \cong \bbF^r$, where $r = r_{|S|} \ge 0$, (by Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)} but already mentioned before)
%the unit $u_S$ of the algebra $\hat \calG(S)$
%corresponds to the all one tuple $(1, \ldots, 1) \in \bbF^r$, where $r = r_{|S|}$,
%(when $r = r_{|S|} = 0$, it is the empty tuple),
%which is the sum of the canonical basis elements of $\bbF^r$.
%Therefore in $\hat \calG(S)$ we have
%\begin{equation}\label{eqn:uS-decomposition-in-idempotent-basis}
%u_S = \sum_{p \in \calP_S} p
%\end{equation}
%
%In fact, a more general statement is true.
%}

\begin{claim}\label{clm:idempotent-is-sum-of-its-resolving-basic-idempotents}
Let $x$ be any idempotent element of $\hat \calG(S)$.
Then $x$ is the sum of exactly those idempotents in $\calP_S$ that resolve it,
\[
x = \sum_{p \in \calP_{S, x}} p.
\]
\end{claim}
\begin{proof}
By the isomorphism  $\hat \calG(S) \cong \bbF^r$,
every 0-1 tuple $x = (x_1, \ldots, x_r) \in \bbF^r$
is the sum $\sum  x_i e_i$.
\end{proof}
%Viewed under the isomorphism  $\hat \calG(S) \cong \bbF^r$
%this is obvious: every 0-1 tuple $x = (x_1, \ldots, x_r) \in \bbF^r$
%is the sum $\sum  x_i e_i$.
%$\sum_{i: x_i =1} e_i$.
%\end{proof}
%Since $\calP_S$ is a basis, we can write $x$
%uniquely as a linear combination of $\calP_S$,
%\[
%x = \sum_{p \in \calP_S} c_p p
%\]
%with some scalars $c_x$.
%Since $x$ is an idempotent:
%\[
%x = x^2 = \sum_{p, p' \in \calP_S} c_p c_{p'} p p' = 
%\sum_{p \in \calP_S} c_p^2 p,
%\]
%which shows that $c_p^2 = c_p$ for every $p$,
%and so $c_p \in \{ 0, 1 \}$. 
%It follows that $x$ is the sum of some subset $X \subseteq \calP_S$. 
%It is clear that $x p = p$ for $p \in X$
%and $x p = 0 \ne p$ for $p \in \calP_S \setminus X$, so $X = \calP_{S, x}$,
%exactly those elements of $\calP_S$ that resolve $x$.
%\end{proof}

%As a special case, we see that
In particular
\begin{equation}\label{eqn:uS-decomposition-in-idempotent-basis}
u_S = \sum_{p \in \calP_S} p,
\end{equation}
since  $u_S \in \hat \calG(S)$ corresponds
to the all-1 tuple in $\bbF^r$.
%since every $p \in  \calP_S$ resolves $u_S$.
%{\color{red} (However, it is also clear since $\hat \calG(S) \cong \bbF^r$ where $r = r_{|S|}$ by construction.)}

\begin{claim}\label{clm:subset-inclusion-and-uniqueness-of-resolving-basic-idempotents}
Let $S \subseteq T$ be two finite sets.
Then every $q \in \calP_T$ resolves exactly one element of $\calP_S$.
\end{claim}
\begin{proof}
Consider the idempotents $pu_{T \setminus S}$
(which could be 0) under the isomorphism $\hat \calG(T) \cong \bbF^{r_{|T|}}$,
where $p \in \calP_S$.
We can write the 0-1 tuple corresponding to $pu_{T \setminus S}$
in $\bbF^{r_{|T|}}$ as the sum of those canonical basis 0-1 vectors.
Recall that for any $q \in \calP_T$,
$q$ resolves $p$
iff $q$  resolves $pu_{T \setminus S}$.
Note that $pu_{T \setminus S}$ must have disjoint positions with entry 1 
for distinct $p \in \calP_S$, and the sum $\sum_{p \in \calP_S} 
pu_{T \setminus S} = u_S u_{T \setminus S} = u_T$ is the all-1 
tuple in $\bbF^{r_{|T|}}$. 
Thus each $q \in \calP_T$ resolves exactly one $p \in \calP_S$.
\end{proof}

%For every $p \in \calP_S$, $p u_{T \setminus S} \in \hat \calG(T)$ is
%a product of two idempotents, therefore also an idempotent.
%As an idempotent in $\hat \calG(T)$ we can write it as
%\[
%p u_{T \setminus S} = \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p u_{T \setminus S}}} q.
%\]
%Now by (\ref{eqn:uS-decomposition-in-idempotent-basis}) we have
%\[
%u_T = u_S u_{T \setminus S} = \sum_{p \in \calP_S} p u_{T \setminus S} = \sum_{p \in \calP_S} \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p u_{T \setminus S}}} q = \sum_{p \in \calP_S} \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p}} q
%\]
%and also
%\[
%u_T = \sum_{q \in \calP_T} q.
%\]
%Furthermore, for distinct $p, p' \in \calP_S$, we have $p p' = 0$,
%so they cannot be resolved by the same $q \in \calP_T$,
%for otherwise $q = p q = p p' q = 0$ which is false.
%So by the uniqueness of the expansion of $u_T$
%in the basis $\calP_T$ we get that
%\[
%\calP_T = \bigsqcup_{p \in \calP_S} \calP_{T, p} 
%\]
%as a disjoint union.
%Therefore every $q \in \calP_T$ resolves exactly one $p \in \calP_S$.
%\end{proof}
%Under the isomorphism $\hat \calG(T) \cong \bbF^{r_{|T|}}$,
%this proof is also transparent.
%Recall that $q \in \calP_T$ resolves $p \in \calP_S$
%iff $q$  resolves $pu_{T \setminus S}$, which is also an idempotent
%(although possibly 0).
%Then we can write the 0-1 tuple corresponding to $pu_{T \setminus S}$
%in $\bbF^{r_{|T|}}$ as the sum of those canonical basis 0-1 vectors.
%Note that $pu_{T \setminus S}$ must have disjoint positions with entry 1
%for distinct $p \in \calP_S$, and the sum $\sum_{p \in \calP_S}
%pu_{T \setminus S} = u_S u_{T \setminus S} = u_T$ is the all-1
%tuple in $\bbF^{r_{|T|}}$.

\begin{claim}\label{clm:projection-removal-inside-f}
Let $T$ and $U$ be finite sets, and let $S = T \cap U$.
If $x \in \hat \calG(T)$ and $y \in \hat \calG(U)$, then
\[
f(x y) = f(\hat \pi_S(x) y).
\]
\end{claim}
\begin{proof}
%For every $T$-labeled graph $G_1$ and $U$-labeled graph $G_2$,
%the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic,
%because only the labeled vertices in $S$ are identified in $G_1 G_2$,
%as well as in $\pi_S(G_1) G_2$.
%Then we extend the equality from $\calPLG$ by linearity.
%{\color{red} (modified proof)}
%
For every $T$-labeled graph $G_1$ and $U$-labeled graph $G_2$,
the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic,
because only the labeled vertices in $S$ are identified in $G_1 G_2$,
as well as in $\pi_S(G_1) G_2$.
Then we extend the equality from $\calPLG$ by linearity to $\calG$
and after that proceed to the quotient $\hat \calG = \calG / \calK$
using the definition of $f$ on $\hat \calG$.
\end{proof}

We have remarked earlier that $f(p) \ne 0$ for any $p \in \calP_S$.
\begin{claim}\label{clm:projection-formula}
Let $S \subseteq T$ be two finite sets.
If $q \in \calP_T$ resolves $p \in \calP_S$, then
\[
\hat \pi_S(q) = \frac{f(q)}{f(p)} p.
\]
\end{claim}
\begin{proof}
Note that $q \in \hat \calG(T)$.
Since $S \subseteq T$, it follows that $\hat \pi_S(q) \in \hat \calG(S)$.
Because the only element from $\hat \calG(S)$ orthogonal to $\hat \calG(S)$
with respect to the dot product $\langle \cdot, \cdot \rangle$
restricted to $\hat \calG(S) \times \hat \calG(S)$ is $0$ (by Lemma~\ref{lem:empty-annihilator-for-hat-calG(subseteq)(S)}),
it suffices to show that both sides give
the same dot product with every basis element in $\cal P_S$.
%\sout{Since $q$ does not resolve any $p' \in \calP_S \setminus \{ p \}$, we have $p' q = 0$ for every such $p'$.}
For any $p' \in \calP_S \setminus \{ p \}$, we have $p' p = 0$ so $p' q = p' p q = 0$.
By Claim~\ref{clm:projection-removal-inside-f},
this implies that
\[
\langle p', \hat \pi_S(q) \rangle = f(p' \hat \pi_S(q)) = f(p' q) = 0 = \langle p', \frac{f(q)}{f(p)} p \rangle.
\]
Furthermore,
\[
\langle p, \hat \pi_S(q) \rangle = f(p \hat \pi_S(q)) = f(p q) = f(q) = \langle p, \frac{f(q)}{f(p)} p \rangle.
\]
This proves the claim.
\end{proof}

\begin{claim}\label{clm:swaps-within-f}
Let $T$ and $U$ be finite sets and let $S = T \cap U$.
Then for any $p \in \calP_S, q \in \calP_{T, p}$ and $r \in \hat \calG(U)$ we have
\[f(q r) = \frac{f(q)}{f(p)} f(rp).\]
In other words,
\[
f(p) f(q r) = f(q) f(rp).
\]
\end{claim}
\begin{proof}
By 
Claims~\ref{clm:projection-removal-inside-f}~and~\ref{clm:projection-formula},
\[
f(q r) = f(\hat \pi_S(q) r) = \frac{f(q)}{f(p)} f(rp).
\]
\end{proof}

\begin{claim}\label{clm:basic-idempotents-nonzero-product}
Let $T$ and $U$ be finite sets and let $S = T \cap U$.
If both $q \in \calP_T, r \in \calP_U$ resolve $p \in \calP_S$, then $q r \ne 0$.
\end{claim}
\begin{proof}
By Claim~\ref{clm:swaps-within-f},
\[
f(q r) = \frac{f(q)}{f(p)} f(r p) = \frac{f(q)}{f(p)} f(r) \ne 0.
\]
\end{proof}

\begin{claim}\label{clm:degree-monotonicity}
If $S \subseteq T$, and $q \in \calP_T$ resolves $p \in \calP_S$, then $\deg(q) \ge \deg(p)$.
\end{claim}
\begin{proof}
It suffices to show this in the case when $|T| = |S| + 1$.
Let $U \subset \posints$ be any $(|S| + 1)$-element superset of $S$ different from $T$;
suppose this is the disjoint union $U = S \sqcup \{ a \},\, a \notin T$. 
Let $Y$ be the set of elements in $\calP_U$ resolving $p u_{\{ a \}}$
(equivalently, resolving $p$, because
every $r \in \calP_U$ resolves $u_{\{ a \}}$ as $a \in U$).
Then $p u_{\{ a \}} = \sum_{r \in Y} r$
by Claim~\ref{clm:idempotent-is-sum-of-its-resolving-basic-idempotents}.
Here $|Y| = \deg(p)$.
Furthermore, we have
%\[
\begin{equation}\label{eqn:qr-summing-to-qu_(a)}
\sum_{r \in Y} q r = q \sum_{r \in Y} r = q p u_{\{ a \}} = q u_{\{ a \}}.
\end{equation}
%]
Each term $q r$ on the left hand side is nonzero
by Claim~\ref{clm:basic-idempotents-nonzero-product},
and since the terms are all idempotent,
each of them is a sum of one or more elements of $\calP_{T \cup U}$.
Furthermore, if $r, r' \in Y$ ($r \ne r'$),
then we have the orthogonality relation
\[
(q r) (q r') = q (r r')  = 0,
\]
so the sets of basic idempotents of $\calP_{T \cup U}$
in the expansion of each term are pairwise disjoint.
Therefore the expansion $\sum_{r \in Y} q r$
in $\calP_{T \cup U}$ contains at least $|Y| = \deg(p)$ terms.
On the right hand side of~(\ref{eqn:qr-summing-to-qu_(a)}), for any $z \in \calP_{T \cup U}$,
$z$ resolves $q$ iff $z$ resolves $q u_{\{ a \}}$ since $a \in U$.
Thus the number of terms in the expansion of $q u_{\{ a \}}$
in the basis $\calP_{T \cup U}$ is precisely $\deg(q)$ by definition.
Thus, $\deg(q) \ge |Y| = \deg(p)$.
The claim is proved.
\end{proof}

\subsection{Bounding the expansion}\label{subsec:Bounding-expansion}

At this point, we finally assume that all the conditions of
Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened}
are satisfied, i.e.,
$f(K_0) = 1$ and there is an integer $q \ge 0$ such that for 
every $k \ge 0$ there exists $n = n_k \ge 2$ satisfying
$r_{k, n} = \symrank(T(f, k, n)) \le \min(n - 1, q^k)$.
In particular $r_{0, n} \le q^0 = 1$ for $n = n_0 \ge 2$.
Clearly, $r_{0, n} \ne 0$ since $f(K_0) = 1$ so $r_{0, n} = 1$.
By Proposition~\ref{prop:graph-paramater-multiplicativity-criterion}, $f$ is multiplicative.

Next, from $f(K_0) = 1$,
we have $U_\emptyset = K_0 \notin \calK$
so that $u_\emptyset = U_\emptyset + \calK$ is a nonzero identity
in $\hat \calG(\emptyset) = \hat \calG[0] \ne 0$.
As $u_\emptyset$ is the sum of all basic idempotents in $\calG(\emptyset)$
we infer that $\calP_\emptyset \ne 0$.
Hence there is at least one basic idempotent.

%\sout{If for any $S$, a basic idempotent $p \in \calP_S$ has degree $D$,
%then by Claim~\ref{clm:degree-monotonicity}
%for any superset $T$ with $|T| = |S| + 1$, 
%there are $D$ basic idempotents resolving $p$ with degree $\ge D$.
%This can be iterated.}
 
If for any finite $S \subseteq \posints$,
a basic idempotent $p \in \calP_S$ has degree $D \ge 0$,
then for any superset $T \subseteq \posints$ of $S$ with $|T| = |S| + 1$, 
there are $D$ basic idempotents resolving $p$.
Let $S \subseteq T$, $t = |T \setminus S|$,
and $T \setminus S = \{u_1, u_2, \ldots, u_t\}$.
For each $1 \le i \le t$, we can pick $D$ basic idempotents
$q^{u_i}_j \in \calP_{S \cup \{u_i\}}$ resolving $p$, where $1 \le j \le D$.
For any mapping $\phi \colon \{1, \ldots, t\} \rightarrow \{1, \ldots, D\}$,
we can form the product $q_\phi = \prod_{i = 1}^t  q^{u_i}_{\phi(i)}$.
If $t = 0$, we assume $q_\phi = p$.
These are clearly idempotents resolving $p$.
If $\phi \ne \phi'$ then for some $i$, 
we have the orthogonality relation $q^{u_i}_{\phi(i)} q^{u_i}_{\phi'(i)} = 0$.
Thus $q_\phi q_{\phi'} = 0$. 
Also by applying Claim~\ref{clm:swaps-within-f} $t$ times,
\begin{equation}\label{f(q-phi)-factored-into-product-and-nonzero-1stpass}
f(q_\phi) = f(q_\phi p) = f(\prod_{i = 1}^t q^{u_i}_{\phi(i)} p ) = (\prod_{i = 1}^t \frac{f(q^{u_i}_{\phi(v)})}{f(p)}) f(p) \ne 0,
\end{equation}
and so $q_\phi \ne 0$.
Thus the set $\{q_\phi \mid \phi \colon \{1, \ldots, t\} \rightarrow \{1, \ldots, D\} \}$ is linearly independent. 
This implies that the dimension of $\hat \calG(T)$ over $\bbF$
is at least $D^{t} = D^{|T| - |S|}$.
But by Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)}
we also have the upper bound $q^{|T|}$.
If $D > q$, this leads to a contradiction if $|T|$ is large.
It follows that $D \le q$,
i.e., the degrees of basic idempotents for any $S$
and any $p \in \calP_S$ are bounded by $q$.
Let $D \ge 0$ denote the maximum degree
over all such $S$ and $p \in \calP_S$,
and suppose it is attained at some particular $S$ and $p \in \calP_S$.
We now fix this $S$ and $p$.
Note that for the existence of $D$
we also use the existence of a basic idempotent.

For $u \in \posints \setminus S$, let $q_1^u, \ldots, q_D^u$
denote the elements of $\calP_{S \cup \{ u \}}$ resolving $p$.
Note that for $u, v \in \posints \setminus S$,
there is a natural isomorphism between $\hat \calG(S \cup \{ u \})$ and $\hat \calG(S \cup \{ v \})$
(induced by the map that fixes $S$ pointwise and maps $u$ to $v$),
and we may choose the indexing so that
$q_i^u$ corresponds to $q_i^v$ under this isomorphism.

%{\color{red} (say that we use the previous reasoning)}

Now for any finite set $T \supseteq S$
all basic idempotents in $\calP_T$ that resolve $p$ can be described.
%\sout{These are indeed the $q_\phi$'s we have already defined.}
To describe these,
 let $V = T \setminus S$, and for every map $\phi \colon V \to \{ 1, \ldots, D \}$, we 
%\sout{have} {\color{red} define as before}
define as before
\begin{equation}\label{eqn:q-phi-factored-into-product}
q_\phi = \prod_{v \in V} q_{\phi(v)}^v.
\end{equation}

We have shown that these are linearly independent.

\begin{claim}\label{clm:calP_(T,p)-resolved-by-q_phi}
\[
\calP_{T, p} = \{ q_\phi \colon \phi \in \{ 1, \ldots, D \}^V \}.
\]
\end{claim}
\begin{proof}
We prove this by induction on the cardinality of $V = T \setminus S$.
For $|V| = 0, 1$ the assertion is trivial.
Suppose that $|V| > 1$.
Pick any $u \in V$,  let $U = S \cup \{ u \}$
and $W = T \setminus \{ u \}$; thus $U \cap W = S$.
By the induction hypothesis, the basic idempotents in $\calP_W$ resolving $p$
are elements of the form $q_\psi$,
%for $\psi \in \{1, \ldots, D \}^{V \setminus \{ u \}}$.
for $\psi \in \{1, \ldots, D \}^{W}$.

Let $r$ be one of these.
By Claim~\ref{clm:basic-idempotents-nonzero-product},
$r q_i^u \ne 0$ for any $1 \le i \le D$, and clearly resolves $r$.
We can write $r q_i^u$ as a sum of basic idempotents in $\calP_T$
resolving it,
and it is easy to see that these also resolve $r$ (as 
\emph{resolve} is transitive).
For each  $r q_i^u$ the sum is nonempty as $r q_i^u \ne 0$.
Furthermore, the sets of basic idempotents occurring
in the expressions for $r q_i^u$ and $r q_j^u$ ($i \ne j$) are disjoint;
this follows from item 2 stated at the beginning of this subsection,
and $q_i^u q_j^u =0$.
%But $r$ has degree $D$,
%%% JYC
%%% this originally in my mind was justified by claim 5.22 
%%% (the last claim of sec 5.4.)  but you want NOT to use it, and netherless
%%% keep it there.
%%% anyway, i wrote an alternative  justification
%%%
If the sum  for any $r q_i^u$ has more than one basic idempotent,
then $r$ would have degree $>D$, violating the maximality of $D$.
%%% as r would have >D many basic idempotents in $\calP_T$ resolving it.
So each $r q_i^u$ must be a basic idempotent in $\calP_T$ itself.

Each $r \in \calP_{W}$ resolves $p$ iff $r$ resolves $p u_{W}$.
Hence $p u_{W} = \sum_{r \in \calP_{W, p}} r$.
Also $p u_{\{ u \}} = \sum_{i = 1}^D q_i^u$.
Therefore we have
\[
p u_{T} = p u_{W} p u_{\{ u \}} = \sum_{r \in \calP_{W, p}, 1 \le i \le D} r q_i^u
\]
i.e., the basic idempotents $r q_i^u$ ($r \in \calP_{W, p},\, 1 \le i \le D)$
form the set of basic idempotents in $\calP_{T}$ resolving $p u_{T}$,
which is equivalent to resolving $p$.
It follows that these are all the elements of $\calP_{T, p}$.
This proves the claim.
\end{proof}

It is immediate from the definition that
an idempotent $q_\phi$ resolves $q_i^v u_V$ (equivalently $q_i^v$) iff $\phi(v) = i$.
Hence it also follows that
%\begin{equation}\label{eqn:q-i-v-times-u-v-factored-into-product}
\[
q_i^v u_V= \sum_{\phi \colon \phi(v) = i} q_\phi.
\]
%\end{equation}
By the same reason, it also follows that for $u, v \in V$, $u \ne v$,
and any $1 \le i, j \le D$, 
\begin{equation}\label{eqn:q-i-v-times-u-v-factored-into-product-pairs}
q_i^u q_j^v u_V= \sum_{\substack{\phi \colon \phi(u) = i \\ 
\quad \phi(v) = j}} q_\phi.
\end{equation}

\subsection{Constructing the target graph}

Now we can define $H$ as follows.
Let $S$ and $p$ be fixed as above. 
For any $u \in \posints \setminus S$, let $\{q_1^u, \ldots, q_D^u\}$ and
for any $T \supseteq S$, 
$q_\phi$ is defined as in subsection~\ref{subsec:Bounding-expansion}.
%%% JYC i added this T \supseteq S.  without T there is no \phi

Let $H$ be the looped complete graph on $V(H) = \{ 1, \ldots, D \}$.
We have to define the node weights and edge weights.
For every $i \in V(H)$, let
\[
\alpha_i = \frac{f(q_i^u)}{f(p)}
\]
be the weight of node $i$~\footnote{For $\bbF = \bbR$,
if we require the positive semidefiniteness
of the connection matrices $M(f, k)$ for $k \ge 0$,
then since $p$ and $q_i^u$ are basic idempotents,
$f(p) = f(p^2) > 0$ and similarly $f(q_i^u) > 0$.
Thus $\alpha_i > 0$, and so we recover the positive vertex weight case; 
see~\cite{Freedman-Lovasz-Schrijver-2007}.}. 
This definition does not depend on the choice of $u$,
because if $v \in \posints \setminus S$
and $v \ne u$, then the isomorphism
from $\hat \calG(S \cup \{ u \})$ to $\hat \calG(S \cup \{ v \})$ 
(induced by the map that fixes $S$ and maps $u$ to $v$),
will send $q_i^u$ to $q_i^v$.

%{\color{red} (original incorrect)}
%{\color{blue}
%
%Let $u, v \in \posints \setminus S,\, u \ne v$, and let $W = S \cup \{ u, v \}$.
%Let $K_{u v}$ denote the graph on $W$ which has only one edge connecting $u$ and $v$,
%and let $k_{u v}$ denote the corresponding element of $\hat \calG(W)$.
%We can express $p k_{u v}$ as a linear combination
%of the basis elements from $\calP_{W}$.
%Note that $r \in \calP_{W}$ resolves $p$ iff it resolves $p u_{\{ u, v \}}$,
%thus $p u_{\{ u, v \}} = \sum_{r \in \calP_{W, p}} r$.
%So if $r' \in \calP_{W} \setminus \calP_{W, p}$,
%we have $r' p = r' u_{\{u,v\}} p =0$.
%Thus $r' p k_{u v} = 0$. It follows that $p k_{u v}$ is a linear 
%combination of the basis elements from the subset $\calP_{W, p}$.
%We write this unique expression
%}
%
%{\color{red} (correct argument)}

Let $u, v \in \posints \setminus S,\, u \ne v$, and let $W = S \cup \{ u, v \}$.
Let $K_{u v}$ denote the graph on the vertices $u$ and $v$
that are correspondingly labeled $u$ and $v$,
and has only one edge connecting $u$ and $v$.
Let $k_{u v} = K_{u v} + \calK$ denote the corresponding element of $\hat \calG(\{ u, v \})$.
We can express $p k_{u v}$ as a linear combination
of the basic idempotents from $\calP_W$.
Note that $r \in \calP_{W}$ resolves $p$ iff $r$ resolves $p u_{\{ u,v \}}$,
thus $p u_{\{ u, v \}} = \sum_{r \in \calP_{W, p}} r$.
So if $r' \in \calP_W \setminus \calP_{W, p}$, we have $r' p = r' u_{\{ u, v \}} p =0$.
Thus $r' p k_{u v} = 0$. It follows that $p k_{u v}$ is a linear 
combination of the basic idempotents from the subset $\calP_{W, p}$.
We write this unique expression
\[
p k_{u v} = \sum_{i, j = 1}^D \beta_{i j} q_i^u q_j^v.
\]
This defines (by the uniqueness) the weight $\beta_{i j}$ of the edge $i j$.
Note that $\beta_{i j} = \beta_{j i}$ for all $i, j$, since $p k_{u v} = p k_{v u}$.

We prove that this weighted graph $H$ gives the desired homomorphism function.

\begin{claim}\label{clm:f-equals-hom(,H)}
For every finite graph $G$, $f(G) = \hom(G, H)$.
\end{claim}
\begin{proof}
%{\color{red} (original incorrect)}
%{\color{blue}
%
%Let $V$ be a finite subset of $\posints$ disjoint from $S$ of cardinality $|V(G)|$.
%We label $V(G)$ by $V$ thus making $G$ a $V$-labeled graph.
%Since $f$ ignores labels, we may identify $V$ and $V(G)$, and assume $V(G) = V$.
%By (\ref{eqn:q-i-v-times-u-v-factored-into-product-pairs}),
%we have for each pair $u, v$ of distinct elements of $V(G)$,
%\[
%p k_{u v} u_V = \sum_{i, j \in V(H)} \beta_{i j} q_i^u q_j^v u_V = \sum_{i, j \in V(H)} \beta_{i, j} \sum_{\substack{\phi \colon \phi(u) = i \\
%\quad \phi(v) = j}} q_\phi = \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi.
%\]
%Here the last equality follows from the fact that
%\[
%\{ \phi : V \rightarrow V(H) \} = \bigcup_{i,j \in V(H)} \{ \phi \in V(H)^V : \phi(u) = i, \phi(v) = j \}
%\]
%is a partition.
%Let $g$ be the corresponding element of $G$ in $\hat \calG(V)$.
%Clearly $g = \prod_{u v \in E(G)} k_{u v}$.
%Also note that $g u_V = g$ so $g = g u_V^{|E(G)|}$.
%Also, $p$ is an idempotent so $p = p^{|E(G)| + 1}$.
%Then
%\[
%p g = p^{|E(G)| + 1} g u_V^{|E(G)|} = p \prod_{u v \in E(G)} p k_{u v} u_V = p \prod_{u v \in E(G)} ( \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi ) 
%\]
%Note that when we expand the product of sum
%as a sum of products, for any two edges $u v \in E(G)$ and $u' v' \in E(G)$,
%if the mappings $\phi$ and $\phi' \in V(H)^V$ (in the respective sums)
%disagree on any vertex of $V = V(G)$, the product $q_\phi q_{\phi'} =0$.
%This implies that in the sum of products expression
%we only sum over all $\phi \in V(H)^V$ (and not over $|E(G)|$-tuples of these).
%Also $q_\phi$ resolves $p$, so $q_\phi p = q_\phi$.
%This implies that
%\[
%p g = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) q_\phi.
%\]
%Note that $p \in \hat \calG(S),\, g \in \hat \calG(V)$ and $S \cap V = \emptyset$,
%and $p$ and $g$ have representatives in $\calG(S)$
%and $\calG(V)$ that are (linear sums of) labeled graphs with disjoint vertex sets.
%We conclude that  $f(p) f(g) = f(p q)$, and so by
%(\ref{f(q-phi)-factored-into-product-and-nonzero-1stpass})
%and (\ref{eqn:q-phi-factored-into-product}),
%\[
%\begin{split}
%f(p) f(g) &= f(p g) = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) f(q_\phi) \\
%&= \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) ( \prod_{v \in V(G)} \alpha_{\phi(v)}) f(p),
%\end{split}
%\]
%The factor $f(p) \ne 0$ can be canceled from both sides, completing the proof.
%}
%
%{\color{red} (correct proof)}
%
Let $V$ be a finite subset of $\posints$ disjoint from $S$ of cardinality $|V(G)|$.
We label $V(G)$ by $V$ thus making $G$ a $V$-labeled graph, so now $G \in \calG(V)$.
Since $f$ ignores labels, we may identify $V$ and $V(G)$, and assume $V(G) = V$.
By (\ref{eqn:q-i-v-times-u-v-factored-into-product-pairs}),
we have for each pair $u, v$ of distinct elements of $V(G)$,
\[
p k_{u v} u_V = \sum_{i, j \in V(H)} \beta_{i j} q_i^u q_j^v u_V = \sum_{i, j \in V(H)} \beta_{i, j} \sum_{\substack{\phi \colon \phi(u) = i \\
\quad \phi(v) = j}} q_\phi = \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi.
\]
Here the 
???MANY LINES MISSING
However, $p \in \calP_S$ so it follows that $S = \emptyset$.
Therefore by the previous isomorphism $\calP_\emptyset = \{ p \}$
so $p$ is the only basic idempotent in $\hat \calG(\emptyset)$ and so in the entire $\hat \calG$.)  
\end{proof}



==> ttttttttttt <==
\section{Proof of Main Theorem}\label{sec:proof-of-main-results}

For now, we do not make any assumptions on the graph parameter $f$;
we will introduce more assumptions as needed to prove the desired statements.
When we speak of submonoids, subrings and subalgebras we require
that the multiplicative identity coincide with that of the larger structure.
When a subset with the induced operations forms a monoid, ring or algebra
we will simply say that it is respectively
a monoid, ring or algebra in the larger structure. 
We \emph{allow} zero algebras and rings, in which $0 = 1$. 
Statements about such structures can be easily checked. 
%For convenience, we will assume that the product of "zero" elements in a multiplicative structure,
%be it a monoid, ring or algebra is its (multiplicative) identity.
A function of arity zero is a scalar.
We identify a (labeled) graph with its (labeled) graph isomorphism class.

\subsection{The monoid and algebra of graphs}\label{subsec:monoid-and-algebra-of-graphs}

For every finite set $S \subseteq \posints$, we denote
by $U_S$ the graph with $|S|$ nodes labeled by $S$ and no edges. 
Note that $U_\emptyset = K_0$ is the empty graph.

We put all $k$-labeled graphs into a single structure as follows.
By a \textit{partially labeled graph} we mean a finite graph
in which some of the nodes are labeled by distinct positive integers.
(All label sets are finite.)
Two partially labeled graphs are \textit{isomorphic}
if there is an isomorphism between them preserving all labels.
For two partially labeled graphs $G_1$ and $G_2$,
let $G_1 G_2$ denote the partially labeled graph
obtained by taking the disjoint union of $G_1$ and $G_2$,
and identifying the nodes with the same label;
the union of the label sets become the labels of $G_1 G_2$.
This way we obtain a commutative monoid $\calPLG$
with the empty graph $U_\emptyset$ being the identity~\footnote{In \cite{Freedman-Lovasz-Schrijver-2007},
the word semigroup instead of monoid is used.
A monoid is a semigroup with identity,
and all semigroups in~\cite{Freedman-Lovasz-Schrijver-2007}
have or assume to have identity.
Thus, our use of the term monoid is consistent with that of~\cite{Freedman-Lovasz-Schrijver-2007}.}.
For every finite set $S \subseteq \posints$,
we call a partially labeled graph $S$\textit{-labeled},
if its labels form the set $S$.
We call a partially labeled graph ${\subseteq} S$\textit{-labeled},
if its labels form a subset of $S$.
%So every $S$-labeled graph is automatically an ${\subseteq} S$-labeled graph.
We define $\calPLG(S)$, respectively  $\calPLG_\subseteq(S)$,
  to be the subset of $\calPLG$
consisting of all isomorphism classes of $S$-labeled,
respectively ${\subseteq} S$-labeled, graphs.
Clearly $\calPLG(S) \subseteq \calPLG_\subseteq(S)$.
%Next, we define $\calPLG_\subseteq(S)$ to be the subset of $\calPLG$
%consisting of all isomorphism classes of ${\subseteq} S$-labeled graphs.
Then both $\calPLG(S)$ and $\calPLG_\subseteq(S)$ are commutative monoids in $\calPLG$.
$\calPLG_\subseteq(S)$ is a submonoid of $\calPLG$
with the same identity $U_\emptyset$,
while  $\calPLG(S)$ is a submonoid of $\calPLG$ iff $S = \emptyset$,
as the identity in $\calPLG(S)$ is $U_S$.

%Given a monoid $M$, we call a map $g \colon M \to \bbF$ a \textit{(monoid) character}
%if $g$ is a monoid homomorphism, where $\bbF$ is viewed as a monoid under multiplication.
%That is, $g$ is a character iff $g(e) = 1$ where $e$ is the identity in $M$
%and $g(a b) = g(a) g(b)$ for all $a, b \in M$.
%Note that we allow $g$ to take zero values.
%Let $\bbF M$ be the monoid algebra of $M$ over $\bbF$,
%which consists of formal finite linear combinations of $M$.
%Extending $g$ by linearity we can assume that
%$g \colon \bbF M \to \bbF$ is an algebra homomorphism.
%Clearly, this correspondence is a bijection between the characters from $M$ to $\bbF$
%and the algebra homomorphisms from $\bbF M$ to $\bbF$,
%so we can implicitly identify one with another.

%%{\color{red} (added the definitions of quantum graphs)
%

Let $\mathcal G$ denote the
 monoid algebra $\bbF \calPLG$ consisting of all finite formal
linear combinations of $\calPLG$ with coefficients from $\bbF$; they are
called (partially labeled, $\bbF$-)\textit{quantum graphs}.
Restricting the labels to precisely $S$ or to subsets of $S$, 
we have $\bbF \calPLG(S)$ or $\bbF \calPLG_\subseteq(S)$,
respectively the  $S$-labeled or  $\subseteq S$-labeled 
\textit{quantum graphs},
respectively denoted  by  $\calG(S)$ or $\calG_\subseteq(S)$.
$\calG(S)$ is  
an algebra inside $\calG$ with $U_S$ being the multiplicative identity,
and $\calG_\subseteq(S)$ is a subalgebra of $\calG$.
%with $U_\emptyset$ being the identity in both.
The empty sum is the additive identity in all.

%
%A (partially labeled, $\bbF$-)\textit{quantum graph} is a finite formal 
%linear combination of finite   with coefficients from $\bbF$.
%linear combination)
%An $S$-labeled  ($\bbF$-)\textit{quantum graph} is a finite formal 
%linear combination (with coefficients from $\bbF$)
%of finite  $S$-labeled graphs. 
%The notion of a $\subseteq S$-labeled ($\bbF$-)\textit{quantum graph} is 
%defined analogously.
%%When the label sets of the constituent graphs 
%%(with nonzero coefficients) are precisely
%%$S$ ($\subseteq S$)-labeled graphs,
%%we call such a quantum graph an $S$ ($\subseteq S$)-labeled \textit{quantum graph}.
%%%((alternative phrasing) An $S$ ($\subseteq S$)-labeled \textit{quantum graph} is a finite formal linear 
%%%combination of finite  $S$ ($\subseteq S$)-labeled) graphs.)
%%%If the coefficients come from $\bbF$ we call these objects
%%%(partially, $S$ or $\subseteq S$-labeled) $\bbF$-quantum graphs, respectively.
%%%}
%
%Let $\mathcal G$ denote the monoid algebra $\bbF \calPLG$,
%i.e., the (infinite dimensional) vector space of
%finite formal $\bbF$-linear combinations of elements of $\calPLG$,
%or, {\color{red}(need to have a specifier) partially labeled} $\bbF$-quantum graphs. 
%Restricting the label set,
%for every finite set $S \subseteq \posints$,
%we have the monoid algebra $\calG(S) = \bbF \calPLG(S)$.
%This is an algebra inside $\calG$ with $U_S$ being the identity. 
%We also have the monoid algebra $\calG_\subseteq(S) = \bbF \calPLG_\subseteq(S)$.
%This $\calG_\subseteq(S)$ is a subalgebra of $\calG$,
%%with $U_\emptyset$ being the identity in both. 

%Let us consider the case
%when $f = \hom(\cdot, H)$ for some weighted graph $H$.
%For every map $\Phi \colon \posints \to V(H)$,
%and every partially labeled graph $G$ with the label set $S$,
%we define $\hom_\Phi(G, H) = \hom_{\Phi|_S}(G, H)$,
%(see Equation (\ref{eqn:partial-hom-dec})).
%Equation (\ref{eqn:partial-hom-mult}) implies that the function $\hom_\Phi(\cdot, H)$ is a 
%character of the monoid $\calPLG(S)$ and formula (\ref{eqn:full-hom-dec}) gives 
%an expression of $f$ as a linear combination of these 
%characters (from $\calPLG(S)$ to $\bbF$).
%{\color{red} (the actual labels make no difference, that's why the transition $[k] \to S$ is fine)}

Because many definitions, notations and statements
for $\calPLG(S), \calG(S)$ and $\calPLG_\subseteq(S), \calG_\subseteq(S)$ appear similar, 
we will often commingle them to minimize repetitions,
e.g., we use $\calG_{(\subseteq)}(S)$ to denote
either $\calG(S)$ or $\calG_\subseteq(S)$ (and the statements are asserted for both).

We can extend $f$ to a linear map on $\calG$, and
define an $n$-fold multilinear form,  where $n \ge 1$,
\[
\langle x_1, \ldots, x_n \rangle_{(n)} = f(x_1 \cdots x_n),~~~~~~\mbox{for}~~
x_1, \ldots, x_n \in  \calG.
\]
%for every $n \ge 1$ and $x_1, \ldots, x_n \in \calG$.
%for $x_1, \ldots, x_n \in \calG$.  
It is symmetric because $\calG$ is commutative.
Note that if we restrict each argument to $\calG[k]$
and then write it with respect to the basis $\calPLG[k]$ of $\calG[k]$,
we get precisely the connection tensor (array) $T(f, k, n)$.

Let
\[
\calK = \{ x \in \calG \colon f(x y) = \langle x, y \rangle = 0 \ \forall y \in \calG \}
\]
be the annihilator of $\calG$.
Clearly, $\calK$ is an ideal in $\calG$,
so we can form the quotient algebra $\hat \calG = \calG / \calK$
which is commutative as well.
We denote its identity by $u_\emptyset = U_\emptyset + \calK$.
More generally, we denote $u_S = U_S + \calK$
 for any finite subset $S \subseteq \posints$.
%Furthermore, 
If $x \in \calK$, then $f(x) = f(x U_\emptyset) = 0$
and so $f$ can also be considered as a linear map on $\hat \calG$.
For a partially labeled graph $G$ we 
denote by $\hat G = G + \calK$ the corresponding element of $\hat \calG$.
More generally, we write $\hat x = x + \calK$ for any $x \in \calG$. 
Since $\calK$ is an ideal in $\calG$, the form
$\langle \cdot, \ldots, \cdot \rangle_{(n)}$ on $\calG$ induces
an $n$-fold multilinear form on $\hat \calG$,  where $n \ge 1$, 
%\[
\begin{equation}\label{eqn:f-on-hat-calG}
\langle x_1, \ldots, x_n \rangle_{(n)} = f(x_1 \cdots x_n),~~~~~~\mbox{for}~~
x_1, \ldots, x_n \in \hat \calG.
\end{equation}
%\]
%for every $n \ge 1$ and $x_1, \ldots, x_n \in \hat \calG$.
%for $x_1, \ldots, x_n \in \hat \calG$.

%{\color{red} (remove)
%
%If $S, T \subseteq \posints$ are finite subsets,
%then $\calPLG_{(\subseteq)}(S) \, \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$
%so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$. 
%%Going to the quotients, we conclude that $\hat \calG_{(\subseteq)}(S) \, \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cap T)$.
%}

We can also define
\[
\hat \calG_{(\subseteq)}(S) = (\calG_{(\subseteq)}(S) + \calK) / \calK = \{ x + \calK \mid x \in \calG_{(\subseteq)}(S) + \calK \}
= \{ x + \calK \mid x \in \calG_{(\subseteq)}(S)\}.
\]
%Then
%\[
%\hat \calG_{(\subseteq)}(S) = \{ x + \calK \mid x \in \calG_{(\subseteq)}(S)\}.
%\]
It is easy to see that $\hat \calG_\subseteq(S)$ is a subalgebra of $\hat \calG$
with the same identity $u_\emptyset = U_\emptyset + \calK$,
and $\hat \calG(S)$ is an algebra inside $\hat \calG$
with the identity $u_S = U_S + \calK$~\footnote{In contrast to \cite{Freedman-Lovasz-Schrijver-2007}
we cannot normalize $f$ to make all elements $u_S$, for finite $S \subseteq \posints$,
the same in the quotient algebra $\hat \calG$.
In our more general setting, it is possible $f(K_1) = 0$,
in which case the normalization step from \cite{Freedman-Lovasz-Schrijver-2007} fails.}.
%\sout{$\calK$ is also an ideal in $\calG_{(\subseteq)}(S) + \calK$ and therefore $(\calG_{(\subseteq)}(S) + \calK) / \calK$ is an algebra (a subalgebra, resp.) in $\calG / \calK$.}

%{\color{red} (added here)

If $S, T \subseteq \posints$ are finite subsets,
then $\calPLG_{(\subseteq)}(S) \, \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$
so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$
and so, going to the quotitents, we have $\hat \calG_{(\subseteq)}(S) \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cup T)$.
Also note that for a finite $S \subseteq \posints$,
we have $\calPLG(S) \subseteq \calPLG_\subseteq(S)$
so by linearity $\calG(S) \subseteq \calG_\subseteq(S)$
and then by going to the quotients we obtain $\hat \calG(S) \subseteq \hat \calG_\subseteq(S)$.
%}

Since
% $\calK$ is an ideal in $\calG$,
%we also have that 
$\calG_{(\subseteq)}(S) \cap \calK$ is an ideal in $\calG_{(\subseteq)}(S)$,
 we can also form 
another quotient algebra 
\[
\tilde \calG_{(\subseteq)}(S) = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK).
\] 
%%%
%
%{\color{red} (say it here instead)
%If $S, T \subseteq \posints$ are finite subsets, then $\calPLG_{(\subseteq)}(S) \, \calPLG_{(\subseteq)}(T) \subseteq \calPLG_{(\subseteq)}(S \cup T)$ so by linearity we get $\calG_{(\subseteq)}(S) \, \calG_{(\subseteq)}(T) \subseteq \calG_{(\subseteq)}(S \cup T)$
%and so, going to the quotitents, we have $\hat \calG_{(\subseteq)}(S) \hat \calG_{(\subseteq)}(T) \subseteq \hat \calG_{(\subseteq)}(S \cup T)$.
%Also note that for a finite $S \subseteq \posints$, we have $\calPLG(S) \subseteq \calPLG_\subseteq(S)$ so by linearity $\calG(S) \subseteq \calG_\subseteq(S)$
%and then by going to the quotients we obtain $\hat \calG(S) \subseteq \hat \calG_\subseteq(S)$.}
%
%%%
%The following lemma provides us with canonical isomorphisms. {\color{red} (change the sentence)}
We have the following
 canonical isomorphisms between $\tilde \calG_{(\subseteq)}(S)$
 and $\hat \calG_{(\subseteq)}(S)$.
\begin{lemma}\label{lem:calG(subseteq)(S)/calK(subseteq)S-canonical-isomorphism}
Let $S \subseteq \posints$ be finite. Then $\tilde \calG_{(\subseteq)}(S) \cong \hat \calG_{(\subseteq)}(S)$ as algebras via $x + \calG_{(\subseteq)}(S) \cap \calK \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$.
\end{lemma}
\begin{proof}
It follows from
the 
%standard 
Second Isomorphism Theorem for algebraic structures
(see~\cite{Cohn-book} p. 8).
%(e.g., see page 8 of~\cite{Cohn-book}).
%, or \cite{Jacobson-book}). 
%
%We repeat the standard proof of the Second Isomorphism Theorem for algebraic structures.
%
%Obviously, the map $\calG_{(\subseteq)}(S) \mapsto (\calG_{(\subseteq)}(S) + \calK) / \calK,\, x \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$ is a surjective algrebra homormophism with the kernel equal to $\calG_{(\subseteq)}(S) \cap \calK$ which is an ideal in $\calG_{(\subseteq)}(S)$. Then this map factors through $\calG_{(\subseteq)}(S) / \calK_S$ resulting in an algebra isomorphism between $\tilde \calG_{\subseteq}(S) = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK)$ and $\hat \calG_{(\subseteq)}(S) = \calG_{(\subseteq)}(S) / \calK$ given by $x + \calK_S \mapsto x + \calK,\, x \in \calG_{(\subseteq)}(S)$.
\end{proof}

We say that elements $x, y \in \calG \,(\text{or } \hat \calG)$
are orthogonal (with respect to $f$),
if $f(x y) = 0$ and denote it by $x \perp y$.
For a subset $A \subseteq \calG \,(\text{or } \hat \calG)$, 
denote by $A^\perp = \{ x \in \calG \,(\text{or } \hat \calG) \mid x \perp y, \, \forall y \in A \}$
those in $\calG \,(\text{or } \hat \calG)$ orthogonal to all elements in $A$.
Next, we say that subsets $A, B \subseteq \calG \,(\text{or } \hat \calG)$
are orthogonal (with respect to $f$),
if $x \perp y$ for all $x \in A$ and $y \in B$.
Similarly, we can talk about an element of $\calG \,(\text{or } \hat \calG)$
being orthogonal to a subset of $\calG \,(\text{or } \hat \calG)$ and vice versa.
Note that the notion of orthogonality is symmetric
since all the multiplication operations considered are commutative.
From the definition, we have $\calK = \calG^\perp$.
Next, denote (commingling the notations $\calK_S$ and $\calK_{\subseteq S}$)
\[
\calK_{(\subseteq) S} = \{ x \in \calG_{(\subseteq)} (S) \mid x \perp y, \ \forall y \in \calG_{(\subseteq)}(S) \} = \calG_{(\subseteq)}(S) \cap (\calG_{(\subseteq)}(S))^\perp.
\]
Clearly, $\calK_{(\subseteq) S}$ is an ideal in $\calG_{(\subseteq)}(S)$,
so we can form yet another quotient algebra $\calG_{(\subseteq)}(S) / \calK_{(\subseteq) S}$. 

Next, we define an orthogonal projection
from $\hat \calG$ to the subalgebra $\hat \calG_\subseteq(S)$.
We will show how to do it in a series of lemmas.
Let $S \subseteq \posints$ be finite.
For every partial labeled graph $G$,
let $G_S$ denote the ${\subseteq} S$-labeled graph obtained by deleting
the labels not in $S$ from the vertices of $G$ (unlabeling such vertices).
Extending this map by linearity,
we get a linear map $\pi_S \colon \calG \to \calG_\subseteq(S)$.
Note that $(\pi_S)_{| \calG_\subseteq(S)} = \id_{|\calG_\subseteq(S)}$.
In particular, $\pi_S \colon \calG \to \calG_\subseteq(S)$ is surjective.

\begin{lemma}\label{lem:projection}
Let $S \subseteq \posints$ be finite.
If $x \in \calG$ and $y \in \calG_\subseteq(S)$, then
\[
f(x y) = f(\pi_S(x) y).
\]
\end{lemma}
\begin{proof}
For every $G_1 \in \calPLG$ and $G_2 \in \calPLG_\subseteq(S)$,
the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic as unlabeled graphs.
Hence $f(G_1 G_2) = f(\pi_S(G_1) G_2)$ as $f$ ignores labels.
The lemma follows by linearity.
\end{proof}

\begin{corollary}\label{cor:projection-part-orthogonality}
Let $S \subseteq \posints$ be finite.
If $x \in \calG$, then $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
\end{corollary}
\begin{proof}
Fix any $y \in \calG_\subseteq(S)$. By Lemma~\ref{lem:projection},
$f(x y) = f(\pi_S(x) y)$ so $f((x - \pi_S(x)) y) = 0$.
Thus $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
\end{proof}

So for any $x \in \calG$, we can write $x = \pi_S(x) + (x - \pi_S(x))$
where $\pi_S(x) \in \calG_\subseteq(S)$, and $x - \pi_S(x) \in (\calG_\subseteq(S))^\perp$.
%by Corollary~\ref{cor:projection-part-orthogonality}.
This gives a decomposition $\calG = \calG_\subseteq(S) + (\calG_\subseteq(S))^\perp$.
%To get a similar decomposition into a direct sum,
To get a direct sum decomposition,
% make such a decomposition into a direct sum,
we need to pass to the quotient algebra.
But to do so properly we need some lemmas.
%first  it correctly we first need to prove some statements.

\begin{lemma}\label{lem:calKS}
Let $S \subseteq \posints$ be finite.
Then $\calK_S = \calG(S) \cap \calK$.
\end{lemma}
\begin{proof}
Clearly,
$\calG(S) \cap \calK = \calG(S) \cap \calG^\perp \subseteq
 \calG(S) \cap (\calG(S))^\perp = \calK_S$,
% $\calK_S = \calG(S) \cap (\calG(S))^\perp \supseteq \calG(S) \cap \calG^\perp = \calG(S) \cap \calK$,
so we only need to prove the reverse inclusion. 
Let $x \in \calK_S = \calG(S) \cap (\calG(S))^\perp$.
Take any $y \in \calG$. Then
\[
f(x y) \stackrel{(1)}{=} f(x \pi_S(y)) \stackrel{(2)}{=} f(x U_S \pi_S(y)) \stackrel{(3)}{=} 0.
\]
Here step $(1)$ uses Lemma~\ref{lem:projection} 
as $x \in \calG(S) \subseteq \calG_{\subseteq}(S)$;
$(2)$ is true because $x = x U_S$ for $x \in \calG(S)$;
$(3)$ is true as $\pi_S(y) \in \calG_\subseteq(S)$
so $U_S \pi_S(y) \in \calG(S)$, and as $x \in (\calG(S))^\perp$.
Then $x \in \calK$ so $x \in \calG(S) \cap \calK$,
implying $\calK_S \subseteq \calG(S) \cap \calK$.
\end{proof}

\begin{lemma}\label{lem:calKsubseteqS}
Let $S \subseteq \posints$ be finite.
Then $\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap \calK$.
\end{lemma}
\begin{proof}
Clearly,
$\calG_\subseteq(S) \cap \calK = \calG_\subseteq(S) \cap \calG^\perp
\subseteq  \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp = 
\calK_{{\subseteq}S}$,
% $\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp \supseteq \calG_\subseteq(S) \cap \calG^\perp = \calG_\subseteq(S) \cap \calK$,
so we only need to prove the reverse inclusion. 
Let $x \in \calK_{{\subseteq}S} = \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp$.
Take any $y \in \calG$. Then
\[
f(x y) \stackrel{(1)}{=} f(x \pi_S(y)) \stackrel{(2)}{=} 0.
\]
Here step $(1)$ uses Lemma~\ref{lem:projection};
$(2)$ is true as $\pi_S(y) \in \calG_\subseteq(S)$
and $x \in (\calG_\subseteq(S))^\perp$.
Then $x \in \calK$ so $x \in \calG_\subseteq(S) \cap \calK$,
implying $\calK_{\subseteq S} \subseteq \calG_\subseteq(S) \cap \cal K$.
\end{proof}

It follows from Lemmas~\ref{lem:calKS}~and~\ref{lem:calKsubseteqS} that
$\calG_{(\subseteq)}(S) / \calK_{(\subseteq) S} = \calG_{(\subseteq)}(S) / (\calG_{(\subseteq)}(S) \cap \calK) = \tilde \calG_{(\subseteq)}(S)$
so the (canonical) isomorphism of algebras from
Lemma~\ref{lem:calG(subseteq)(S)/calK(subseteq)S-canonical-isomorphism} takes the following form:
\begin{equation}\label{eqn:calG(subseteq)(S)-canonical-isomorphisms-new}
\tilde \calG_{(\subseteq)}(S) \cong \hat \calG_{(\subseteq)}(S),\quad x + \calK_{(\subseteq) S} \mapsto x + \calK,\quad x \in \calG_{(\subseteq)}(S).
\end{equation}

\begin{lemma}\label{lem:projection-and-preimage-of-calK-ideals}
Let $S \subseteq \posints$ be finite.
For the linear map $\pi_S \colon \calG \to \calG_\subseteq(S)$
we have $\pi_S(\calK) = \calK_{{\subseteq}S}$.
\end{lemma}
\begin{proof}
Because $(\pi_S)_{| \calG_\subseteq(S)} = \id_{|\calG_\subseteq(S)}$ and by Lemma~\ref{lem:calKsubseteqS}
$\calK_{{\subseteq}S} = \calG_\subseteq(S) \cap \calK$,
we infer that $\pi_S(\calK) \supseteq \calK_{{\subseteq}S}$.
For the reverse inclusion, let $x \in \calK$.
Fix any $y \in \calG_\subseteq(S)$.
Then by Lemma~\ref{lem:projection}, $f(\pi_S(x) y) = f(x y) = 0$,
the last equality is true because $x \in \calK$.
Hence $\pi_S(x) \in \calK_{{\subseteq}S}$
so that $\pi_S(\calK) \subseteq \calK_{{\subseteq}S}$.
\end{proof}

For the linear map $\pi_S \colon \calG \to \calG_\subseteq(S) \subseteq \calG$
by Lemmas~\ref{lem:projection-and-preimage-of-calK-ideals} and~\ref{lem:calKsubseteqS},
$\pi_S(\calK) = \calK_{{\subseteq}S} = \calG_{\subseteq}(S) \cap \calK$,
so that we have the well-defined linear map (which we denote by $\hat \pi_S$)
\begin{equation}\label{eqn:quotient-projection}
\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S),\quad \hat \pi_S(x + \calK) = \pi_S(x) + \calK,\quad x \in \calG.
\end{equation}
 
It is easy to see that $(\hat \pi_S)_{| \hat \calG_\subseteq(S)} = \id_{|\hat \calG_\subseteq(S)}$.
In particular, $\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$ is surjective.
 
\begin{lemma}\label{lem:quotion-decomposition-through-projeciton}
Let $S \subseteq \posints$ be finite. Then $\hat \calG = \hat \calG_\subseteq(S) \oplus (\hat \calG_\subseteq(S))^\perp$ via $x = \hat \pi_S(x) + (x - \hat \pi_S(x)),\, x \in \hat \calG$.
\end{lemma}
\begin{proof}
%First, let $x \in \hat \calG$. Write $x = y + \calK$ where $y \in \calG$. Then $\hat \pi_S(x) = \pi_S(y) + \calK$ and $\pi_S(y) \in \calG_\subseteq(S)$ so $\hat \pi_S(x) \in \hat \calG_\subseteq(S)$.
%Also $x - \hat \pi_S(x) = y - \pi_S(y) + \calK$. By Corollary~\ref{cor:projection-part-orthogonality}, $y - \pi_S(y) \in (\calG_\subseteq(S))^\perp$ so that $x - \hat \pi_S(x) \in (\hat \calG_\subseteq(S))^\perp$.
%
%So we only need to show that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0 (= \calK)$. Let $z$ belong to this intersection.
%Write $z = t + \calK = t' + \calK$ where $t \in \calG_\subseteq(S)$
%and $t' \in (\calG_\subseteq(S))^\perp$. Then $t-t' \in  \calK$,
%and so $t \in (\calG_\subseteq(S))^\perp$.
%Thus $t \in \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp
%= \calK_{{\subseteq}S} \subseteq \calK$, the last inclusion holds by Lemma~\ref{lem:calKsubseteqS}. 
%Therefore $z = t + \calK = \calK$, implying that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0$.

%%%corrected proof
First, let $x \in \hat \calG$. Write $x = y + \calK$ where $y \in \calG$.
Then $\hat \pi_S(x) = \pi_S(y) + \calK$ and $\pi_S(y) \in \calG_\subseteq(S)$.
We have $x - \hat \pi_S(x) = y - \pi_S(y) + \calK$.
By Corollary~\ref{cor:projection-part-orthogonality}, $y - \pi_S(y) \in (\calG_\subseteq(S))^\perp$
so that $x - \hat \pi_S(x) \in (\hat \calG_\subseteq(S))^\perp$,
since the bilinear form on $\calG$ extends to $\hat \calG$ in~(\ref{eqn:f-on-hat-calG}).

So we only need to show that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0 (= \{\calK\})$.
Let $z$ belong to this intersection.
Write $z = t + \calK = t' + \calK$ where $t \in \calG_\subseteq(S)$
and $t' \in (\calG_\subseteq(S))^\perp$.
Then clearly $t - t' \in  \calK \subseteq (\calG_{\subseteq}(S))^\perp$,
%%% i removed ( and ) in \calG_{(\subseteq)}(S)
and so $t = (t - t') + t' \in (\calG_\subseteq(S))^\perp$.
Thus $t \in \calG_\subseteq(S) \cap (\calG_\subseteq(S))^\perp = \calK_{{\subseteq}S} \subseteq \calK$,
the last inclusion holds by Lemma~\ref{lem:calKsubseteqS}. 
Therefore $z = t + \calK = \calK$,
implying that $\hat \calG_\subseteq(S) \cap (\hat \calG_\subseteq(S))^\perp = 0$.
\end{proof}

Thus Lemma~\ref{lem:quotion-decomposition-through-projeciton} allows us
to rightfully call $\hat \pi_S \colon \hat \calG \to \hat \calG_\subseteq(S)$
an orthogonal projection of $\hat \calG$ to $\hat \calG_\subseteq(S)$.

If $S, T \subseteq \posints$ are finite subsets,
then $\pi_S(\calPLG_{(\subseteq)}(T)) = \calPLG_{(\subseteq)}(S \cap T)$,
where the projection is surjective because
the restriction $(\pi_S)_{| \calPLG_{(\subseteq)}(S \cap T)} = \id_{|\calPLG_{(\subseteq)}(S \cap T)}$.
So by linearity we get $\pi_S(\calG_{(\subseteq)}(T)) = \calG_{(\subseteq)}(S \cap T)$.
Going to the quotients, we conclude that $\hat \pi_S(\hat \calG_{(\subseteq)}(T)) = \hat \calG_{(\subseteq)}(S \cap T)$.

\begin{lemma}\label{lem:orthogonal-complement-equivalence-for-calG(subseteq)(S)}
Let $n \ge 2$ and $S \subseteq \posints$ be finite.
Then for any $x \in \calG_{(\subseteq)}(S)$, we have $x \in \calK_{(\subseteq) S}$
iff $f(x x_1 \cdots x_{n - 1}) = 0$ for all $x_1, \ldots, x_{n - 1} \in \calG_{(\subseteq)}(S)$.
\end{lemma}
\begin{proof}
%For $\Rightarrow$, it suffices to note that $\calG_{(\subseteq)}(S)$ is 
%closed under multiplication (in $\calG$). To prove $\Leftarrow$, note that $n - 2 \ge 0$ and for any $y \in \calG_{(\subseteq)}(S)$, we have $f(x y) = f(x y U_0^{n - 2}) = 0$ so $x \in \calK_{(\subseteq) S}$.

%%%corrected proof
For $\Rightarrow$, it suffices to note that $\calG_{(\subseteq)}(S)$
is closed under multiplication (in $\calG$).
To prove $\Leftarrow$, note that $n - 2 \ge 0$ and for any $y \in \calG_{(\subseteq)}(S)$,
we have $f(x y) = f(x y U^{n - 2}) = 0$,
where $U = U_\emptyset$ in the $\calG_\subseteq(S)$ case and
$U = U_S$ in the $\calG(S)$ case,
so $x \in \calK_{(\subseteq) S}$.
\end{proof}

\begin{lemma}\label{lem:empty-annihilator-for-hat-calG(subseteq)(S)}
Let $S \subseteq \posints$ be finite.
Then the annihilator of $\hat \calG_{(\subseteq)}(S)$ in $\hat \calG_{(\subseteq)}(S)$ is zero, i.e.,
if $x \in \hat \calG_{(\subseteq)}(S)$ and $f(x y) = 0$
for every $y \in \hat \calG_{(\subseteq)}(S)$, then $x$
is
the zero element of $\hat \calG_{(\subseteq)}(S)$, namely $\calK$.
%for every $y \in \hat \calG_{(\subseteq)}(S)$, then $x = \calK$.
\end{lemma}
\begin{proof}
%%% corrected proof
Let $x \in \hat \calG_{(\subseteq)}(S)$ be
an element satisfying the hypothesis of the lemma.
Write $x = h_1 + \calK$ where $h_1 \in \calG_{(\subseteq)}(S)$.
By hypothesis, for every 
$y \in \hat \calG_{(\subseteq)}(S)$ we have $f(x y) = 0$.
Let $h_2 \in \calG_{(\subseteq)}(S)$
and put $y = h_2 + \calK \in \hat \calG_{(\subseteq)}(S)$.
Then $x y = h_1 h_2 + \calK$.
By the definition of $f$ on $\hat \calG$, $f(h_1 h_2) = f(x y) = 0$. 
Hence $h_1 \in \calK_{(\subseteq) S} \subseteq \calK$
where the last inclusion is true by Lemmas~\ref{lem:calKS} and~\ref{lem:calKsubseteqS}.
This implies that $x$ is the  zero element of $\hat \calG_{(\subseteq)}(S)$,
which is $\calK$.
\end{proof}

\begin{lemma}\label{lem:calK[k]-T(f,k,n)-xi(h)-criterion}
Let $k, r \ge 0$ and $n \ge \max(2, r)$.
Suppose the connection tensor $T(f, k, n)$ can be expressed as
\[
T(f, k, n) = \sum_{i = 1}^r a_i \bfx_i^{\otimes n},
\]
where $a_i \ne 0$ and $\bfx_i
\in \bbF^{\calPLG[k]}$ are nonzero and \emph{pairwise} linearly independent for $1 \le i \le r$.
Then for any $h \in \calG[k]$, we have $h \in \calK_{[k]}$ iff $\bfx_i(h) = 0, \, 1 \le i \le r$.
\end{lemma}
\begin{proof}
The lemma is clearly true for $r=0$. Let $r \ge 1$.
By Lemma~\ref{lem:orthogonal-complement-equivalence-for-calG(subseteq)(S)},
$h \in \calK_{[k]}$ iff $f(h h_1 \cdots h_{n - 1}) = 0$ for all $h_1, \ldots, h_{n - 1} \in \calG[k]$.
In terms of $T(f, k, n)$, this is equivalent to $(T(f, k, n))(h, \cdot, \ldots, \cdot) = 0$
which is the same as
\[
\sum_{i = 1}^r a_i \, \bfx_i(h) \, \bfx_i^{\otimes (n - 1)} = 0.
\]
Now if $\bfx_i(h) = 0, \, 1 \le i \le r$, then this equality clearly holds.
Conversely, if this equality holds, then by Lemma~\ref{lem:tensor-powers-pairwise-implies-linear-independence},
$a_i \bfx_i(h) = 0$ but $a_i \ne 0$ so $\bfx_i(h) = 0, \,  1 \le i \le r$.
\end{proof}

We will also need the following lemma 
that classifies all subalgebras of $\bbF^m$ for $m \ge 0$.
A proof is given in
 subsection~\ref{subsec:bbF^m-subalgebras} of the Appendix. 
%(or the Appendix (Section~\ref{sec:Preliminary-continued}).)
Recall that we allow zero algebras %(i.e., $\bbF^0 = \{ \emptyset \}$, where $0 = 1 = \emptyset$)
and require any subalgebra of an algebra to share the multiplicative identity.
%{\color{red} with the larger algebra (added)}.

\begin{lemma}\label{lem:F^m-subalgebras}
All subalgebras of $\bbF^m$, where $m \ge 0$, are of the following form:
For some partition $[m] = \bigsqcup_{i = 1}^s \calI_s$,
where $s \ge 0$, and $\calI_i \ne \emptyset$ for $i \in [s]$, 
the subalgebra has equal values on each $I_i$,
\[
\bbF^{(\calI_1, \ldots, \calI_s)} = \{ (c_1, \ldots, c_m) \in \bbF^m \mid \forall i \in [s], \ \forall j, j' \in \calI_i, \ c_j = c_{j'} \}.
\]
\end{lemma}

\subsection{Building an algebra isomorphism~\label{sec:build-alg-isom}}

In this part of the proof regarding $f$ we assume that for every $k \ge 0$
there exists $n = n_k \ge 2$ such that $\symrank T(f, k, n) \le n - 1$.
We will pick an arbitrary such $n$ and call it $n_k$,
and then write $r_k = \symrank T(f, k, n_k)$. 
(Note that this is weaker than the
uniform exponential bounded in $k$ for $\symrank T(f, k, n)$
in Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse},
nor do we require $f(K_0) = 1$ here.)
% to be (uniformly) exponentially bounded in $k$ or $f(K_0) = 1$,
%as the conditions in Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse} would require.)
% {\color{red} (require / do / just remove)}.)
%The results of this part will be valid without these assumptions.

Then, for $n = n_k$, we can write,
\begin{equation}\label{eqn:T(f,k,n)-gen-dec}
T(f, k, n) = \sum_{i = 1}^{r_{k}} a_{k, n, i} \bfx_{k, n, i}^{\otimes n}.
\end{equation}
Then $a_{k, n, i} \ne 0$ and $0 \ne\bfx_{k, n, i} \in \bbF^{\calPLG[k]}$ 
are pairwise linearly independent for $1 \le i \le r_{k}$.

Define the linear map
\begin{equation}\label{eqn:Phi-map}
\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}},\quad \Phi_{k, n}(h) = ( \bfx_{k, n, i}(h) )_{i= 1, \ldots, r_{k}}, \quad h \in \calG[k].
\end{equation}
We show that $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$
is a surjective algebra homomorphism.
% (algebra epimorphism).
Clearly, as $n \ge 2$, 
%{\color{red} (check the commas)}
\[
h_1 \cdot h_2 \cdot h_3 \cdots h_n = (h_1 h_2) \cdot U_k \cdot h_3 \cdots h_n
\]
so
\[
f(h_1 \cdot h_2 \cdot h_3 \cdots h_n) = f((h_1 h_2) \cdot U_k \cdot h_3 \cdots h_n)
\]
for all $h_1, \ldots, h_n \in \calG[k]$.
(When $n = 2$ this is $f(h_1 h_2) = f((h_1 h_2) U_k)$.)
Therefore
\[
(T(f, k, n))(h_1, h_2, \cdot, \ldots, \cdot) =  (T(f, k, n))(h_1 h_2, U_k, \cdot, \ldots, \cdot)
\]
for all $h_1, h_2 \in \calG[k]$.
In terms of the decomposition in (\ref{eqn:T(f,k,n)-gen-dec}),
this is equivalent to 
\[
\sum_{i = 1}^{r_{k}} \, a_{k, n, i} \, \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) \, \bfx_{k, n, i}^{\otimes (n - 2)} = \sum_{i = 1}^{r_{k}} a_{k, n, i} \, \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k) \, \bfx_{k, n, i}^{\otimes (n - 2)}.
\]
It follows that
\[
\sum_{i = 1}^{r_{k}} a_{k, n, i} \, \left( \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) - \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k) \right) \, \bfx_{k, i}^{\otimes (n - 2)} = 0
\]
for any $h_1, h_2 \in \calG[k]$.
The condition $r_{k} \le n - 1$ allows
us to apply Lemma~\ref{lem:tensor-powers-pairwise-implies-linear-independence}.
Since $a_{k, n, i} \ne 0$ for $1 \le i \le r_{k}$,
we obtain that
\begin{equation}\label{eqn:char-prop-unsimp}
\bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2) = \bfx_{k, n, i}(h_1 h_2) \, \bfx_{k, n, i}(U_k), \quad h_1, h_2 \in \calG[k], \quad 1 \le i \le r_{k}.
\end{equation}
Let $1 \le i \le r_{k}$.
Since $\bfx_{k, n, i} \ne 0$, there exists $h \in \calG[k]$ such that $\bfx_{k, n, i}(h) \ne 0$.
Substituting $h_1 = h_2 = h$ into (\ref{eqn:char-prop-unsimp}),
we infer that $\bfx_{k, n, i}(U_k) \ne 0, \, 1 \le i \le r_{k}$.

Therefore we can assume
in (\ref{eqn:T(f,k,n)-gen-dec})
 that each $\bfx_{k, n, i}$ is normalized so that $\bfx_{k, n, i}(U_k) = 1$ ($1 \le i \le r_{k}$).
Combined with this, condition (\ref{eqn:char-prop-unsimp}) becomes for $1 \le i \le r_{k}$,
\begin{equation}\label{eqn:char-prop-simp-full}
\begin{lcases}
\bfx_{k, n, i}(h_1 h_2) &= \bfx_{k, n, i}(h_1) \, \bfx_{k, n, i}(h_2), \quad h_1, h_2 \in \calG[k]; \\
\bfx_{k, n, i}(U_k) &= 1;
\end{lcases}
\end{equation}
so the linear functions $\bfx_{k, n, i} \colon \calG[k] \to \bbF, \, 1 \le i \le r_{k}$
are algebra homomophisms. %(equivalently, characters from $\calPLG[k]$ to $\bbF$).
Then we have
\begin{gather*}
\Phi_{k, n}(g h) = ( \bfx_{k, n, 1}(g h), \ldots, \bfx_{k, n, r_k}(g h) ) = ( \bfx_{k, n, 1}(g) \, \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(g) \, \bfx_{k, n, r_k}(h)) \\
= ( \bfx_{k, n, 1}(g), \ldots, \bfx_{k, n, r_k}(g) ) \cdot ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ) = \Phi_{k, n}(g) \Phi_{k, n}(h). 
\end{gather*}
So we have
\begin{gather*}
\Phi_{k, n}(g h) = \Phi_{k, n}(g) \Phi_{k, n}(h), \quad g, h \in \calG[k], \\
\Phi_{k, n}(U_k) = ( \bfx_{k, n, 1}(U_k) \ldots, \bfx_{k, n, r_k}(U_k) ) = \underbrace{(1, \ldots, 1)}_{r_{k} \text{ times}} \in \bbF^{r_{k}},
\end{gather*}
and therefore $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$ is an algebra homomorphism.
We now prove its surjectivity.
Clearly, $\im(\Phi_{k, n})$ is a subalgebra of $\bbF^{r_{k}}$.
By Lemma~\ref{lem:F^m-subalgebras},
we may assume that $\im(\Phi_{k, n})$
has the form $\bbF^{(\calI_1, \ldots, \calI_s)}$ for some partition
$\{I_1, \ldots, \calI_s\}$ of $[r_{k}]$.
The pairwise linear independence of $\bfx_{k, n, i}$
for $1 \le i \le r_{k}$ implies that for any $1 \le i_1 < i_2 \le r_{k}$,
we have $\bfx_{i_1} \ne \bfx_{i_2}$,
so there exists $h \in \calG[k]$ such that $\bfx_{k, n, i_1}(h) \ne \bfx_{k, n, i_2}(h)$.
Since each $\calI_i \ne \emptyset$,
it follows that $|\calI_i| = 1$ for $1 \le i \le s$.
Hence $\im(\Phi_{k, n}) = \bbF^{(\{ 1 \}, \ldots, \{ r_k \})} = \bbF^{r_{k}}$.
We have shown that $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_{k}}$ is surjective.

Next, by $r_{k} \le n - 1$ and $n \ge 2$, 
clearly $n \ge \max(2, r_{k})$, 
so Lemma~\ref{lem:calK[k]-T(f,k,n)-xi(h)-criterion} applies. So we have
\[
\ker \Phi_{k, n} = \{ h \in \calG[k] \mid \bfx_{k, n, i}(h) = 0,\,
1 \le i \le r_{k}  \} = \calK_{[k]},
\]
where the first equality is by the definition of $\Phi_{k, n}$,
and the second equality is by Lemma~\ref{lem:calK[k]-T(f,k,n)-xi(h)-criterion}.
Note that by Lemma~\ref{lem:calKS}, we have $\calK_{[k]} =
\calG[k] \cap \calK$.
%
%Therefore
Then $\Phi_{k, n} \colon \calG[k] \to \bbF^{r_k}$
factors through $\calG[k] / \ker \Phi_{k, n} = \calG[k] / \calK_{[k]} = \tilde \calG[k]$,
inducing an algebra isomomorphism
\[
\tilde \Phi_{k, n} \colon \tilde \calG[k] \to \bbF^{r_{k}}, \quad \tilde \Phi_{k, n}(h + \calK_{[k]}) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \calG[k].
\]
It follows that $\dim \tilde \calG[k] = \dim \bbF^{r_{k}} = r_{k}$.
In particular, $\tilde \calG[k]$ is a finite dimensional algebra.
Applying Lemma~\ref{lem:quotient-space-dimension},
we get $\dim \tilde \calG[k] = \dim \Span \{ \bfx_{k, n, i} \}_{i = 1}^{r_{k}}$.
Then $\dim \Span \{ \bfx_{k, n, i} \}_{i = 1}^{r_{k}} = r_{k}$
implying that $\bfx_{k, n, i}$,  $1 \le i \le r_{k}$, are linearly independent.
(Note that we started off only assuming they are nonzero and pairwise linearly independent.)
%
We formalize some of the results obtained above.
\begin{lemma}\label{lem:Phi(k)-tilde-calG[k]-isomorphism}
Assume for every $k \ge 0$ there exists $n = n_k \ge 2$ 
such that $r_{k} = \symrank T(f, k, n_k) \le n_k - 1$.
Then the constructed map
\[
\tilde \Phi_{k, n} \colon \tilde \calG[k] \to \bbF^{r_{k}}, \quad \tilde \Phi_k(h + \calK_{[k]}) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \tilde \calG[k].
\]
is an algebra isomorphism and $\dim \tilde \calG[k] = r_{k}$.
\end{lemma}

Composing $\tilde \Phi_k \colon \tilde \calG[k] \to \bbF^{r_{k}}$
with the canonical algebra isomorphism between $\tilde \calG[k]$ and $\hat \calG[k]$
given in (\ref{eqn:calG(subseteq)(S)-canonical-isomorphisms-new}),
we have an algebra isomorphism $\hat \Phi_k \colon \hat \calG[k] \to \bbF^{r_{k}}$.
In particular, $\dim \hat \calG[k] = \dim \tilde \calG[k] = r_{k}$.
\begin{corollary}\label{cor:Phi(k)-hat-calG[k]-isomorphism}
With the same assumption as in Lemma~\ref{lem:Phi(k)-tilde-calG[k]-isomorphism},
for any $k \ge 0$, the  map
%constructed map
\[
\hat \Phi_{k, n} \colon \hat \calG[k] \to \bbF^{r_{k}}, \quad \hat \Phi_{k, n}(h + \calK) = ( \bfx_{k, n, 1}(h), \ldots, \bfx_{k, n, r_k}(h) ),\quad h \in \hat \calG[k].
\]
is an algebra isomorphism and  $\dim \hat \calG[k] = r_{k}$.
\end{corollary}

Note that if $S \subseteq \posints$ is finite and $|S| = k$,
there are natural isomoprphisms between $\tilde \calG(S)$ and $\tilde \calG[k]$
and also between $\hat \calG(S)$ and $\hat \calG[k]$,
both resulting from any bijective map between $S$ and $[k]$.
As a result, we conclude the following.
\begin{corollary}\label{cor:dimension-of-tilde-hat-calG(S)}
%Let $S \subseteq \posints$ be finite, $k = |S|$ and suppose there exists
%some $n \ge 2$ so that $\symrank(T(f, k, n))  \le n - 1$. 
%Let $n = n_k$ be any such choice, and let
%$r_k = \symrank(T(f, k, n_k))$.
%Then  $\tilde \calG(S) \cong \hat \calG(S) \cong \bbF^{r_{k}}$ and $\dim \tilde \calG(S) = \dim \hat \calG(S) = r_{k}$. In particular,
%the value $r_k$ is independent of any particular choice of $n_k$.
%
%%corrected
%{\color{red} corrected statement}
For any $k \ge 0$ and finite $S \subseteq \posints$ with $|S| = k$,
suppose there exists some $n \ge 2$ so that $\symrank(T(f, k, n)) \le n - 1$. 
Let $n = n_k$ be any such choice where $k \ge 0$, and let $r_k = \symrank(T(f, k, n_k))$.
Then $\tilde \calG(S) \cong \hat \calG(S) \cong \bbF^{r_{k}}$
and $\dim \tilde \calG(S) = \dim \hat \calG(S) = r_{k}$.
In particular, the value $r_k$ is independent of any particular choice of $n_k$.
\end{corollary}

\subsection{One $n$ implies for all $n$~\label{sec:one-implies-all}}

Let $n_k$ retain the same meaning
as in Lemma~\ref{lem:Phi(k)-tilde-calG[k]-isomorphism},
and let $r = r_k =  \symrank(T(f, k, n_k))$.
For any $h \in \calG[k]$, clearly
$h = h U_k^{n_k - 1}$ so $f(h) = f(h U_k^{n_k - 1})$.
As $\bfx_{k, n_k, i}(U_k) = 1, \, 1 \le i \le r$,
%Therefore
\[
\begin{split}
f(h) &= f(h U_k^{n_k - 1}) = (T(f, k, n_k))(h, U_k, \ldots, U_k) = \sum_{i = 1}^r a_{k, n_k, i} (\bfx_{k, n_k, i}(U_k))^{n_k - 1} \bfx_{k, n_k, i}(h) \\
&= \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h)
\end{split}
\]
for any $h \in \calG[k]$.
Hence $f_{|\calG[k]} = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}$, i.e.,
$f_{|\calG[k]}$ is a linear combination of $r$ algebra 
homomorphisms $\bfx_{k, n_k, i} \colon \calG[k] \to \bbF$, for $1 \le i \le r$.
In particular, applying to the product $h_1 \cdots h_n$,
for any $n \ge 0$ and  any  $h_1, \ldots, h_n \in \calG[k]$,
(note that this $n$ is arbitrary, not only for  those $n$ satisfying
the requirements for the choice of $n_k$)
\[
f(h_1 \cdots h_n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h_1 \cdots h_n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(h_1) \cdots  \bfx_{k, n_k, i}(h_n).
\]
(When $n = 0$, we view it as $f(U_k) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}(U_k) = \sum_{i = 1}^r a_{k, n_k, i}$.)
Hence
\begin{equation}\label{eqn:T(f,k,n)-char-dec}
T(f, k, n) = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}^{\otimes n}
\end{equation}
for all $n \ge 0$.
(When $n = 0$, 
%we continue the previous consideration for this case,
%so 
(\ref{eqn:T(f,k,n)-char-dec}) is still valid as
$T(f, k, 0) = f(U_k) = \sum_{i = 1}^r a_{k, n_k, i} = \sum_{i = 1}^r a_{k, n_k, i} \bfx_{k, n_k, i}^{\otimes 0}$
where the last equality is true as $\bfx_{k, n_k, i}^{\otimes 0} = 1$.)
% by convention,
%and therefore in this case (\ref{eqn:T(f,k,n)-char-dec}) is still correct.)}

As shown before, $\bfx_{k, n_k, i}$ where $1 \le i \le r$ are linearly independent.
Then by Lemma~\ref{lem:tensor-powers-linear-independence-symmetric-rank-and-uniqueness} 
applied to (\ref{eqn:T(f,k,n)-char-dec}),
we get $\symrank(T(f, k, n)) = r$ for all $n \ge 2$;
and the decomposition (\ref{eqn:T(f,k,n)-char-dec})
is actually unique up to a permutation for $n \ge 3$. 

\begin{theorem}\label{thm:T(f,k,n)-rk-unif-dec-uniq}
Let $k \ge 0$.
Assume that for some $n = n_k \ge 2$, $\symrank T(f, k, n) = r \le n - 1$.
Then the following hold:
\begin{enumerate}
\item $\symrank T(f, k, n) = r$ for every $n \ge 2$.
\item There exist $r$ linearly independent algebra homomophisms $\bfx_i \colon \calG[k] \to \bbF$,
and $a_1, \ldots, a_r \in \bbF \setminus \{ 0 \}$ such that $f_{|\calG[k]} = \sum_{i = 1}^r a_i \bfx_i$;
also for every $n \ge 0$,
\begin{equation}\label{eqn:T(f,k,n)-unif-dec}
T(f, k, n) = \sum_{i = 1}^r a_i \bfx_i^{\otimes n}.
\end{equation}
Moreover, for any $n \ge 3$, any expression of $T(f, k, n)$ as $\sum_{i = 1}^r b_i \bfy_i^{\otimes n}$,
where $\bfy_i \colon \calG[k] \to \bbF$ are linear maps,
is a permutation of the sum in (\ref{eqn:T(f,k,n)-unif-dec}).
\end{enumerate}
\end{theorem}

%The reader may agree that
%something very nontrivial has happened.
We remark that this proves a nontrivial statement:
The existence of some $n_k$ has produced
a uniform expression for the tensors $T(f, k, n)$
all the way down to $n = 0$.

\subsection{Putting things together}

Having developed the theory in a more general setting,
we can now follow the proof in~\cite{Freedman-Lovasz-Schrijver-2007} closely.
We will be interested in the idempotent elements of $\hat \calG$.
For two elements  $p, q \in \hat \calG$,
we say that $q$ resolves $p$, if $p q = q$.
We also say equivalently $p$ is resolved by $q$. 
It is clear that the binary relation
\textit{resolves} is antisymmetric and transitive and,
when restricted to idempotents, reflexive.
Furthermore, it is easy to see that the binary 
relation \textit{resolves} on $\hat \calG$ has the following properties:

\begin{enumerate}
\item The idempotent $0 = \calK$ resolves everything and $1 = u_\emptyset = 
U_\emptyset + \calK = K_0 + \calK$ is resolved by everything.
\item If $a b = 0$ and $c$ resolves both $a$ and $b$, then $c = 0$;
\item If $a$ resolves $b$, then $c$ resolves  $a$ iff $c$ resolves $a b$.
\end{enumerate}

In the algebra $\bbF^r$ ($r \ge 0$), 
the idempotents are 0-1 tuples in $\bbF^r$, and for idempotents
$q = (q_1, \ldots, q_r)$ and $p = (p_1, \ldots, p_r)$,
$q$ resolves $p$ iff $q_i=1$ implies $p_i=1$.

Let $S$ be a finite subset of $\posints$ with $|S|=k$, and set $r = r_{k}$
as above.
By Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)},
$\hat \calG(S) \cong \bbF^r$ as algebras,
so $\hat \calG(S)$ has a (uniquely determined idempotent) basis $\calP_S = \{ p_1^S, \ldots, p_r^S \}$
such that $(p_i^S)^2 = p_i^S$ and $p_i^S p_j^S = 0$ for $i \ne j$.
These correspond to the canonical basis $\{e_i\}_{1 \le i \le r}$ of $\bbF^r$
under this isomorphism.
%Namely, it corresponds to the canonical basis of $\bbF^r$ under this isomorphism.
For $i \ne j$, we have $\langle p_i^S, p_j^S \rangle = f(p_i^S p_j^S) = 0$.
Furthermore, for all $1 \le i \le r$, $f(p_i^S) = f((p_i^S)^2) = \langle p_i^S, p_i^S \rangle \ne 0$,
%which is obvious under the isomorphism.
otherwise $\hat \calG(S)$ contains a nonzero element orthogonal to $\hat \calG(S)$
with respect to the bilinear form $\langle \cdot, \cdot \rangle$
restricted to $\hat \calG(S) \times \hat \calG(S)$, 
contradicting Lemma~\ref{lem:empty-annihilator-for-hat-calG(subseteq)(S)}.
We will call the elements $p_i^S \in \calP_S$ basic idempotents. %(of/in $\hat \calG(S)$).

%{\color{red} From now on, when talking about label sets (such as $S, T, U$ (not a unit this time)),
%we will always assume that they are finite subsets of $\posints$ but frequently omit it.}
%
%%% this was said in beginning of sec 5: JYC added that.

We denote by $\calP_{T, p}$ the set of all idempotents in $\calP_T$
that resolve a given element $p \in \hat \calG$.
If $p \in \calP_S$ and $S \subset T$ and $|T| = |S| + 1$,
then the number of elements in $\calP_{T, p}$
will be called the degree of $p \in \calP_S$, and denoted by $\deg(p)$.
Obviously, this value is independent of
which $(|S| + 1)$-element superset $T$ of $S$ we take.

For any $q \in \hat \calG(T)$, we have $q u_{T \setminus S} = q$.
It follows that for any $S \subseteq T$ and $p \in \hat \calG$,
we have  $q$ resolves $p$ iff $q$ resolves $p u_{T \setminus S}$,
since $q p = q u_{T \setminus S} p = q p u_{T \setminus S}$.
It is also important to point out that
an element in $\hat \calG(S)$ is an idempotent in $\hat \calG(S)$
iff it is an idempotent in $\hat \calG$.

%{\color{red} (propose the following change)
%
%Since $\hat \calG(S) \cong \bbF^r$, where $r = r_{|S|} \ge 0$, (by Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)} but already mentioned before)
%the unit $u_S$ of the algebra $\hat \calG(S)$
%corresponds to the all one tuple $(1, \ldots, 1) \in \bbF^r$, where $r = r_{|S|}$,
%(when $r = r_{|S|} = 0$, it is the empty tuple),
%which is the sum of the canonical basis elements of $\bbF^r$.
%Therefore in $\hat \calG(S)$ we have
%\begin{equation}\label{eqn:uS-decomposition-in-idempotent-basis}
%u_S = \sum_{p \in \calP_S} p
%\end{equation}
%
%In fact, a more general statement is true.
%}

\begin{claim}\label{clm:idempotent-is-sum-of-its-resolving-basic-idempotents}
Let $x$ be any idempotent element of $\hat \calG(S)$.
Then $x$ is the sum of exactly those idempotents in $\calP_S$ that resolve it,
\[
x = \sum_{p \in \calP_{S, x}} p.
\]
\end{claim}
\begin{proof}
By the isomorphism  $\hat \calG(S) \cong \bbF^r$,
every 0-1 tuple $x = (x_1, \ldots, x_r) \in \bbF^r$
is the sum $\sum  x_i e_i$.
\end{proof}
%Viewed under the isomorphism  $\hat \calG(S) \cong \bbF^r$
%this is obvious: every 0-1 tuple $x = (x_1, \ldots, x_r) \in \bbF^r$
%is the sum $\sum  x_i e_i$.
%$\sum_{i: x_i =1} e_i$.
%\end{proof}
%Since $\calP_S$ is a basis, we can write $x$
%uniquely as a linear combination of $\calP_S$,
%\[
%x = \sum_{p \in \calP_S} c_p p
%\]
%with some scalars $c_x$.
%Since $x$ is an idempotent:
%\[
%x = x^2 = \sum_{p, p' \in \calP_S} c_p c_{p'} p p' = 
%\sum_{p \in \calP_S} c_p^2 p,
%\]
%which shows that $c_p^2 = c_p$ for every $p$,
%and so $c_p \in \{ 0, 1 \}$. 
%It follows that $x$ is the sum of some subset $X \subseteq \calP_S$. 
%It is clear that $x p = p$ for $p \in X$
%and $x p = 0 \ne p$ for $p \in \calP_S \setminus X$, so $X = \calP_{S, x}$,
%exactly those elements of $\calP_S$ that resolve $x$.
%\end{proof}

%As a special case, we see that
In particular
\begin{equation}\label{eqn:uS-decomposition-in-idempotent-basis}
u_S = \sum_{p \in \calP_S} p,
\end{equation}
since  $u_S \in \hat \calG(S)$ corresponds
to the all-1 tuple in $\bbF^r$.
%since every $p \in  \calP_S$ resolves $u_S$.
%{\color{red} (However, it is also clear since $\hat \calG(S) \cong \bbF^r$ where $r = r_{|S|}$ by construction.)}

\begin{claim}\label{clm:subset-inclusion-and-uniqueness-of-resolving-basic-idempotents}
Let $S \subseteq T$ be two finite sets.
Then every $q \in \calP_T$ resolves exactly one element of $\calP_S$.
\end{claim}
\begin{proof}
Consider the idempotents $pu_{T \setminus S}$
(which could be 0) under the isomorphism $\hat \calG(T) \cong \bbF^{r_{|T|}}$,
where $p \in \calP_S$.
We can write the 0-1 tuple corresponding to $pu_{T \setminus S}$
in $\bbF^{r_{|T|}}$ as the sum of those canonical basis 0-1 vectors.
Recall that for any $q \in \calP_T$,
$q$ resolves $p$
iff $q$  resolves $pu_{T \setminus S}$.
Note that $pu_{T \setminus S}$ must have disjoint positions with entry 1 
for distinct $p \in \calP_S$, and the sum $\sum_{p \in \calP_S} 
pu_{T \setminus S} = u_S u_{T \setminus S} = u_T$ is the all-1 
tuple in $\bbF^{r_{|T|}}$. 
Thus each $q \in \calP_T$ resolves exactly one $p \in \calP_S$.
\end{proof}

%For every $p \in \calP_S$, $p u_{T \setminus S} \in \hat \calG(T)$ is
%a product of two idempotents, therefore also an idempotent.
%As an idempotent in $\hat \calG(T)$ we can write it as
%\[
%p u_{T \setminus S} = \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p u_{T \setminus S}}} q.
%\]
%Now by (\ref{eqn:uS-decomposition-in-idempotent-basis}) we have
%\[
%u_T = u_S u_{T \setminus S} = \sum_{p \in \calP_S} p u_{T \setminus S} = \sum_{p \in \calP_S} \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p u_{T \setminus S}}} q = \sum_{p \in \calP_S} \sum_{\substack{q \in \calP_T \\ q \text{ resolves } p}} q
%\]
%and also
%\[
%u_T = \sum_{q \in \calP_T} q.
%\]
%Furthermore, for distinct $p, p' \in \calP_S$, we have $p p' = 0$,
%so they cannot be resolved by the same $q \in \calP_T$,
%for otherwise $q = p q = p p' q = 0$ which is false.
%So by the uniqueness of the expansion of $u_T$
%in the basis $\calP_T$ we get that
%\[
%\calP_T = \bigsqcup_{p \in \calP_S} \calP_{T, p} 
%\]
%as a disjoint union.
%Therefore every $q \in \calP_T$ resolves exactly one $p \in \calP_S$.
%\end{proof}
%Under the isomorphism $\hat \calG(T) \cong \bbF^{r_{|T|}}$,
%this proof is also transparent.
%Recall that $q \in \calP_T$ resolves $p \in \calP_S$
%iff $q$  resolves $pu_{T \setminus S}$, which is also an idempotent
%(although possibly 0).
%Then we can write the 0-1 tuple corresponding to $pu_{T \setminus S}$
%in $\bbF^{r_{|T|}}$ as the sum of those canonical basis 0-1 vectors.
%Note that $pu_{T \setminus S}$ must have disjoint positions with entry 1
%for distinct $p \in \calP_S$, and the sum $\sum_{p \in \calP_S}
%pu_{T \setminus S} = u_S u_{T \setminus S} = u_T$ is the all-1
%tuple in $\bbF^{r_{|T|}}$.

\begin{claim}\label{clm:projection-removal-inside-f}
Let $T$ and $U$ be finite sets, and let $S = T \cap U$.
If $x \in \hat \calG(T)$ and $y \in \hat \calG(U)$, then
\[
f(x y) = f(\hat \pi_S(x) y).
\]
\end{claim}
\begin{proof}
%For every $T$-labeled graph $G_1$ and $U$-labeled graph $G_2$,
%the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic,
%because only the labeled vertices in $S$ are identified in $G_1 G_2$,
%as well as in $\pi_S(G_1) G_2$.
%Then we extend the equality from $\calPLG$ by linearity.
%{\color{red} (modified proof)}
%
For every $T$-labeled graph $G_1$ and $U$-labeled graph $G_2$,
the graphs $G_1 G_2$ and $\pi_S(G_1) G_2$ are isomorphic,
because only the labeled vertices in $S$ are identified in $G_1 G_2$,
as well as in $\pi_S(G_1) G_2$.
Then we extend the equality from $\calPLG$ by linearity to $\calG$
and after that proceed to the quotient $\hat \calG = \calG / \calK$
using the definition of $f$ on $\hat \calG$.
\end{proof}

We have remarked earlier that $f(p) \ne 0$ for any $p \in \calP_S$.
\begin{claim}\label{clm:projection-formula}
Let $S \subseteq T$ be two finite sets.
If $q \in \calP_T$ resolves $p \in \calP_S$, then
\[
\hat \pi_S(q) = \frac{f(q)}{f(p)} p.
\]
\end{claim}
\begin{proof}
Note that $q \in \hat \calG(T)$.
Since $S \subseteq T$, it follows that $\hat \pi_S(q) \in \hat \calG(S)$.
Because the only element from $\hat \calG(S)$ orthogonal to $\hat \calG(S)$
with respect to the dot product $\langle \cdot, \cdot \rangle$
restricted to $\hat \calG(S) \times \hat \calG(S)$ is $0$ (by Lemma~\ref{lem:empty-annihilator-for-hat-calG(subseteq)(S)}),
it suffices to show that both sides give
the same dot product with every basis element in $\cal P_S$.
%\sout{Since $q$ does not resolve any $p' \in \calP_S \setminus \{ p \}$, we have $p' q = 0$ for every such $p'$.}
For any $p' \in \calP_S \setminus \{ p \}$, we have $p' p = 0$ so $p' q = p' p q = 0$.
By Claim~\ref{clm:projection-removal-inside-f},
this implies that
\[
\langle p', \hat \pi_S(q) \rangle = f(p' \hat \pi_S(q)) = f(p' q) = 0 = \langle p', \frac{f(q)}{f(p)} p \rangle.
\]
Furthermore,
\[
\langle p, \hat \pi_S(q) \rangle = f(p \hat \pi_S(q)) = f(p q) = f(q) = \langle p, \frac{f(q)}{f(p)} p \rangle.
\]
This proves the claim.
\end{proof}

\begin{claim}\label{clm:swaps-within-f}
Let $T$ and $U$ be finite sets and let $S = T \cap U$.
Then for any $p \in \calP_S, q \in \calP_{T, p}$ and $r \in \hat \calG(U)$ we have
\[f(q r) = \frac{f(q)}{f(p)} f(rp).\]
In other words,
\[
f(p) f(q r) = f(q) f(rp).
\]
\end{claim}
\begin{proof}
By 
Claims~\ref{clm:projection-removal-inside-f}~and~\ref{clm:projection-formula},
\[
f(q r) = f(\hat \pi_S(q) r) = \frac{f(q)}{f(p)} f(rp).
\]
\end{proof}

\begin{claim}\label{clm:basic-idempotents-nonzero-product}
Let $T$ and $U$ be finite sets and let $S = T \cap U$.
If both $q \in \calP_T, r \in \calP_U$ resolve $p \in \calP_S$, then $q r \ne 0$.
\end{claim}
\begin{proof}
By Claim~\ref{clm:swaps-within-f},
\[
f(q r) = \frac{f(q)}{f(p)} f(r p) = \frac{f(q)}{f(p)} f(r) \ne 0.
\]
\end{proof}

\begin{claim}\label{clm:degree-monotonicity}
If $S \subseteq T$, and $q \in \calP_T$ resolves $p \in \calP_S$, then $\deg(q) \ge \deg(p)$.
\end{claim}
\begin{proof}
It suffices to show this in the case when $|T| = |S| + 1$.
Let $U \subset \posints$ be any $(|S| + 1)$-element superset of $S$ different from $T$;
suppose this is the disjoint union $U = S \sqcup \{ a \},\, a \notin T$. 
Let $Y$ be the set of elements in $\calP_U$ resolving $p u_{\{ a \}}$
(equivalently, resolving $p$, because
every $r \in \calP_U$ resolves $u_{\{ a \}}$ as $a \in U$).
Then $p u_{\{ a \}} = \sum_{r \in Y} r$
by Claim~\ref{clm:idempotent-is-sum-of-its-resolving-basic-idempotents}.
Here $|Y| = \deg(p)$.
Furthermore, we have
%\[
\begin{equation}\label{eqn:qr-summing-to-qu_(a)}
\sum_{r \in Y} q r = q \sum_{r \in Y} r = q p u_{\{ a \}} = q u_{\{ a \}}.
\end{equation}
%]
Each term $q r$ on the left hand side is nonzero
by Claim~\ref{clm:basic-idempotents-nonzero-product},
and since the terms are all idempotent,
each of them is a sum of one or more elements of $\calP_{T \cup U}$.
Furthermore, if $r, r' \in Y$ ($r \ne r'$),
then we have the orthogonality relation
\[
(q r) (q r') = q (r r')  = 0,
\]
so the sets of basic idempotents of $\calP_{T \cup U}$
in the expansion of each term are pairwise disjoint.
Therefore the expansion $\sum_{r \in Y} q r$
in $\calP_{T \cup U}$ contains at least $|Y| = \deg(p)$ terms.
On the right hand side of~(\ref{eqn:qr-summing-to-qu_(a)}), for any $z \in \calP_{T \cup U}$,
$z$ resolves $q$ iff $z$ resolves $q u_{\{ a \}}$ since $a \in U$.
Thus the number of terms in the expansion of $q u_{\{ a \}}$
in the basis $\calP_{T \cup U}$ is precisely $\deg(q)$ by definition.
Thus, $\deg(q) \ge |Y| = \deg(p)$.
The claim is proved.
\end{proof}

\subsection{Bounding the expansion}\label{subsec:Bounding-expansion}

At this point, we finally assume that all the conditions of
Theorem~\ref{thm:uniform-exponential-rank-boundedness-converse-strengthened}
are satisfied, i.e.,
$f(K_0) = 1$ and there is an integer $q \ge 0$ such that for 
every $k \ge 0$ there exists $n = n_k \ge 2$ satisfying
$r_{k, n} = \symrank(T(f, k, n)) \le \min(n - 1, q^k)$.
In particular $r_{0, n} \le q^0 = 1$ for $n = n_0 \ge 2$.
Clearly, $r_{0, n} \ne 0$ since $f(K_0) = 1$ so $r_{0, n} = 1$.
By Proposition~\ref{prop:graph-paramater-multiplicativity-criterion}, $f$ is multiplicative.

Next, from $f(K_0) = 1$,
we have $U_\emptyset = K_0 \notin \calK$
so that $u_\emptyset = U_\emptyset + \calK$ is a nonzero identity
in $\hat \calG(\emptyset) = \hat \calG[0] \ne 0$.
As $u_\emptyset$ is the sum of all basic idempotents in $\calG(\emptyset)$
we infer that $\calP_\emptyset \ne 0$.
Hence there is at least one basic idempotent.

%\sout{If for any $S$, a basic idempotent $p \in \calP_S$ has degree $D$,
%then by Claim~\ref{clm:degree-monotonicity}
%for any superset $T$ with $|T| = |S| + 1$, 
%there are $D$ basic idempotents resolving $p$ with degree $\ge D$.
%This can be iterated.}
 
If for any finite $S \subseteq \posints$,
a basic idempotent $p \in \calP_S$ has degree $D \ge 0$,
then for any superset $T \subseteq \posints$ of $S$ with $|T| = |S| + 1$, 
there are $D$ basic idempotents resolving $p$.
Let $S \subseteq T$, $t = |T \setminus S|$,
and $T \setminus S = \{u_1, u_2, \ldots, u_t\}$.
For each $1 \le i \le t$, we can pick $D$ basic idempotents
$q^{u_i}_j \in \calP_{S \cup \{u_i\}}$ resolving $p$, where $1 \le j \le D$.
For any mapping $\phi \colon \{1, \ldots, t\} \rightarrow \{1, \ldots, D\}$,
we can form the product $q_\phi = \prod_{i = 1}^t  q^{u_i}_{\phi(i)}$.
If $t = 0$, we assume $q_\phi = p$.
These are clearly idempotents resolving $p$.
If $\phi \ne \phi'$ then for some $i$, 
we have the orthogonality relation $q^{u_i}_{\phi(i)} q^{u_i}_{\phi'(i)} = 0$.
Thus $q_\phi q_{\phi'} = 0$. 
Also by applying Claim~\ref{clm:swaps-within-f} $t$ times,
\begin{equation}\label{f(q-phi)-factored-into-product-and-nonzero-1stpass}
f(q_\phi) = f(q_\phi p) = f(\prod_{i = 1}^t q^{u_i}_{\phi(i)} p ) = (\prod_{i = 1}^t \frac{f(q^{u_i}_{\phi(v)})}{f(p)}) f(p) \ne 0,
\end{equation}
and so $q_\phi \ne 0$.
Thus the set $\{q_\phi \mid \phi \colon \{1, \ldots, t\} \rightarrow \{1, \ldots, D\} \}$ is linearly independent. 
This implies that the dimension of $\hat \calG(T)$ over $\bbF$
is at least $D^{t} = D^{|T| - |S|}$.
But by Corollary~\ref{cor:dimension-of-tilde-hat-calG(S)}
we also have the upper bound $q^{|T|}$.
If $D > q$, this leads to a contradiction if $|T|$ is large.
It follows that $D \le q$,
i.e., the degrees of basic idempotents for any $S$
and any $p \in \calP_S$ are bounded by $q$.
Let $D \ge 0$ denote the maximum degree
over all such $S$ and $p \in \calP_S$,
and suppose it is attained at some particular $S$ and $p \in \calP_S$.
We now fix this $S$ and $p$.
Note that for the existence of $D$
we also use the existence of a basic idempotent.

For $u \in \posints \setminus S$, let $q_1^u, \ldots, q_D^u$
denote the elements of $\calP_{S \cup \{ u \}}$ resolving $p$.
Note that for $u, v \in \posints \setminus S$,
there is a natural isomorphism between $\hat \calG(S \cup \{ u \})$ and $\hat \calG(S \cup \{ v \})$
(induced by the map that fixes $S$ pointwise and maps $u$ to $v$),
and we may choose the indexing so that
$q_i^u$ corresponds to $q_i^v$ under this isomorphism.

%{\color{red} (say that we use the previous reasoning)}

Now for any finite set $T \supseteq S$
all basic idempotents in $\calP_T$ that resolve $p$ can be described.
%\sout{These are indeed the $q_\phi$'s we have already defined.}
To describe these,
 let $V = T \setminus S$, and for every map $\phi \colon V \to \{ 1, \ldots, D \}$, we 
%\sout{have} {\color{red} define as before}
define as before
\begin{equation}\label{eqn:q-phi-factored-into-product}
q_\phi = \prod_{v \in V} q_{\phi(v)}^v.
\end{equation}

We have shown that these are linearly independent.

\begin{claim}\label{clm:calP_(T,p)-resolved-by-q_phi}
\[
\calP_{T, p} = \{ q_\phi \colon \phi \in \{ 1, \ldots, D \}^V \}.
\]
\end{claim}
\begin{proof}
We prove this by induction on the cardinality of $V = T \setminus S$.
For $|V| = 0, 1$ the assertion is trivial.
Suppose that $|V| > 1$.
Pick any $u \in V$,  let $U = S \cup \{ u \}$
and $W = T \setminus \{ u \}$; thus $U \cap W = S$.
By the induction hypothesis, the basic idempotents in $\calP_W$ resolving $p$
are elements of the form $q_\psi$,
%for $\psi \in \{1, \ldots, D \}^{V \setminus \{ u \}}$.
for $\psi \in \{1, \ldots, D \}^{W}$.

Let $r$ be one of these.
By Claim~\ref{clm:basic-idempotents-nonzero-product},
$r q_i^u \ne 0$ for any $1 \le i \le D$, and clearly resolves $r$.
We can write $r q_i^u$ as a sum of basic idempotents in $\calP_T$
resolving it,
and it is easy to see that these also resolve $r$ (as 
\emph{resolve} is transitive).
For each  $r q_i^u$ the sum is nonempty as $r q_i^u \ne 0$.
Furthermore, the sets of basic idempotents occurring
in the expressions for $r q_i^u$ and $r q_j^u$ ($i \ne j$) are disjoint;
this follows from item 2 stated at the beginning of this subsection,
and $q_i^u q_j^u =0$.
%But $r$ has degree $D$,
%%% JYC
%%% this originally in my mind was justified by claim 5.22 
%%% (the last claim of sec 5.4.)  but you want NOT to use it, and netherless
%%% keep it there.
%%% anyway, i wrote an alternative  justification
%%%
If the sum  for any $r q_i^u$ has more than one basic idempotent,
then $r$ would have degree $>D$, violating the maximality of $D$.
%%% as r would have >D many basic idempotents in $\calP_T$ resolving it.
So each $r q_i^u$ must be a basic idempotent in $\calP_T$ itself.

Each $r \in \calP_{W}$ resolves $p$ iff $r$ resolves $p u_{W}$.
Hence $p u_{W} = \sum_{r \in \calP_{W, p}} r$.
Also $p u_{\{ u \}} = \sum_{i = 1}^D q_i^u$.
Therefore we have
\[
p u_{T} = p u_{W} p u_{\{ u \}} = \sum_{r \in \calP_{W, p}, 1 \le i \le D} r q_i^u
\]
i.e., the basic idempotents $r q_i^u$ ($r \in \calP_{W, p},\, 1 \le i \le D)$
form the set of basic idempotents in $\calP_{T}$ resolving $p u_{T}$,
which is equivalent to resolving $p$.
It follows that these are all the elements of $\calP_{T, p}$.
This proves the claim.
\end{proof}

It is immediate from the definition that
an idempotent $q_\phi$ resolves $q_i^v u_V$ (equivalently $q_i^v$) iff $\phi(v) = i$.
Hence it also follows that
%\begin{equation}\label{eqn:q-i-v-times-u-v-factored-into-product}
\[
q_i^v u_V= \sum_{\phi \colon \phi(v) = i} q_\phi.
\]
%\end{equation}
By the same reason, it also follows that for $u, v \in V$, $u \ne v$,
and any $1 \le i, j \le D$, 
\begin{equation}\label{eqn:q-i-v-times-u-v-factored-into-product-pairs}
q_i^u q_j^v u_V= \sum_{\substack{\phi \colon \phi(u) = i \\ 
\quad \phi(v) = j}} q_\phi.
\end{equation}

\subsection{Constructing the target graph}

Now we can define $H$ as follows.
Let $S$ and $p$ be fixed as above. 
For any $u \in \posints \setminus S$, let $\{q_1^u, \ldots, q_D^u\}$ and
for any $T \supseteq S$, 
$q_\phi$ is defined as in subsection~\ref{subsec:Bounding-expansion}.
%%% JYC i added this T \supseteq S.  without T there is no \phi

Let $H$ be the looped complete graph on $V(H) = \{ 1, \ldots, D \}$.
We have to define the node weights and edge weights.
For every $i \in V(H)$, let
\[
\alpha_i = \frac{f(q_i^u)}{f(p)}
\]
be the weight of node $i$~\footnote{For $\bbF = \bbR$,
if we require the positive semidefiniteness
of the connection matrices $M(f, k)$ for $k \ge 0$,
then since $p$ and $q_i^u$ are basic idempotents,
$f(p) = f(p^2) > 0$ and similarly $f(q_i^u) > 0$.
Thus $\alpha_i > 0$, and so we recover the positive vertex weight case; 
see~\cite{Freedman-Lovasz-Schrijver-2007}.}. 
This definition does not depend on the choice of $u$,
because if $v \in \posints \setminus S$
and $v \ne u$, then the isomorphism
from $\hat \calG(S \cup \{ u \})$ to $\hat \calG(S \cup \{ v \})$ 
(induced by the map that fixes $S$ and maps $u$ to $v$),
will send $q_i^u$ to $q_i^v$.

%{\color{red} (original incorrect)}
%{\color{blue}
%
%Let $u, v \in \posints \setminus S,\, u \ne v$, and let $W = S \cup \{ u, v \}$.
%Let $K_{u v}$ denote the graph on $W$ which has only one edge connecting $u$ and $v$,
%and let $k_{u v}$ denote the corresponding element of $\hat \calG(W)$.
%We can express $p k_{u v}$ as a linear combination
%of the basis elements from $\calP_{W}$.
%Note that $r \in \calP_{W}$ resolves $p$ iff it resolves $p u_{\{ u, v \}}$,
%thus $p u_{\{ u, v \}} = \sum_{r \in \calP_{W, p}} r$.
%So if $r' \in \calP_{W} \setminus \calP_{W, p}$,
%we have $r' p = r' u_{\{u,v\}} p =0$.
%Thus $r' p k_{u v} = 0$. It follows that $p k_{u v}$ is a linear 
%combination of the basis elements from the subset $\calP_{W, p}$.
%We write this unique expression
%}
%
%{\color{red} (correct argument)}

Let $u, v \in \posints \setminus S,\, u \ne v$, and let $W = S \cup \{ u, v \}$.
Let $K_{u v}$ denote the graph on the vertices $u$ and $v$
that are correspondingly labeled $u$ and $v$,
and has only one edge connecting $u$ and $v$.
Let $k_{u v} = K_{u v} + \calK$ denote the corresponding element of $\hat \calG(\{ u, v \})$.
We can express $p k_{u v}$ as a linear combination
of the basic idempotents from $\calP_W$.
Note that $r \in \calP_{W}$ resolves $p$ iff $r$ resolves $p u_{\{ u,v \}}$,
thus $p u_{\{ u, v \}} = \sum_{r \in \calP_{W, p}} r$.
So if $r' \in \calP_W \setminus \calP_{W, p}$, we have $r' p = r' u_{\{ u, v \}} p =0$.
Thus $r' p k_{u v} = 0$. It follows that $p k_{u v}$ is a linear 
combination of the basic idempotents from the subset $\calP_{W, p}$.
We write this unique expression
\[
p k_{u v} = \sum_{i, j = 1}^D \beta_{i j} q_i^u q_j^v.
\]
This defines (by the uniqueness) the weight $\beta_{i j}$ of the edge $i j$.
Note that $\beta_{i j} = \beta_{j i}$ for all $i, j$, since $p k_{u v} = p k_{v u}$.

We prove that this weighted graph $H$ gives the desired homomorphism function.

\begin{claim}\label{clm:f-equals-hom(,H)}
For every finite graph $G$, $f(G) = \hom(G, H)$.
\end{claim}
\begin{proof}
%{\color{red} (original incorrect)}
%{\color{blue}
%
%Let $V$ be a finite subset of $\posints$ disjoint from $S$ of cardinality $|V(G)|$.
%We label $V(G)$ by $V$ thus making $G$ a $V$-labeled graph.
%Since $f$ ignores labels, we may identify $V$ and $V(G)$, and assume $V(G) = V$.
%By (\ref{eqn:q-i-v-times-u-v-factored-into-product-pairs}),
%we have for each pair $u, v$ of distinct elements of $V(G)$,
%\[
%p k_{u v} u_V = \sum_{i, j \in V(H)} \beta_{i j} q_i^u q_j^v u_V = \sum_{i, j \in V(H)} \beta_{i, j} \sum_{\substack{\phi \colon \phi(u) = i \\
%\quad \phi(v) = j}} q_\phi = \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi.
%\]
%Here the last equality follows from the fact that
%\[
%\{ \phi : V \rightarrow V(H) \} = \bigcup_{i,j \in V(H)} \{ \phi \in V(H)^V : \phi(u) = i, \phi(v) = j \}
%\]
%is a partition.
%Let $g$ be the corresponding element of $G$ in $\hat \calG(V)$.
%Clearly $g = \prod_{u v \in E(G)} k_{u v}$.
%Also note that $g u_V = g$ so $g = g u_V^{|E(G)|}$.
%Also, $p$ is an idempotent so $p = p^{|E(G)| + 1}$.
%Then
%\[
%p g = p^{|E(G)| + 1} g u_V^{|E(G)|} = p \prod_{u v \in E(G)} p k_{u v} u_V = p \prod_{u v \in E(G)} ( \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi ) 
%\]
%Note that when we expand the product of sum
%as a sum of products, for any two edges $u v \in E(G)$ and $u' v' \in E(G)$,
%if the mappings $\phi$ and $\phi' \in V(H)^V$ (in the respective sums)
%disagree on any vertex of $V = V(G)$, the product $q_\phi q_{\phi'} =0$.
%This implies that in the sum of products expression
%we only sum over all $\phi \in V(H)^V$ (and not over $|E(G)|$-tuples of these).
%Also $q_\phi$ resolves $p$, so $q_\phi p = q_\phi$.
%This implies that
%\[
%p g = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) q_\phi.
%\]
%Note that $p \in \hat \calG(S),\, g \in \hat \calG(V)$ and $S \cap V = \emptyset$,
%and $p$ and $g$ have representatives in $\calG(S)$
%and $\calG(V)$ that are (linear sums of) labeled graphs with disjoint vertex sets.
%We conclude that  $f(p) f(g) = f(p q)$, and so by
%(\ref{f(q-phi)-factored-into-product-and-nonzero-1stpass})
%and (\ref{eqn:q-phi-factored-into-product}),
%\[
%\begin{split}
%f(p) f(g) &= f(p g) = \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) f(q_\phi) \\
%&= \sum_{\phi \colon V \to V(H)} ( \prod_{u v \in E(G)} \beta_{\phi(u), \phi(v)} ) ( \prod_{v \in V(G)} \alpha_{\phi(v)}) f(p),
%\end{split}
%\]
%The factor $f(p) \ne 0$ can be canceled from both sides, completing the proof.
%}
%
%{\color{red} (correct proof)}
%
Let $V$ be a finite subset of $\posints$ disjoint from $S$ of cardinality $|V(G)|$.
We label $V(G)$ by $V$ thus making $G$ a $V$-labeled graph, so now $G \in \calG(V)$.
Since $f$ ignores labels, we may identify $V$ and $V(G)$, and assume $V(G) = V$.
By (\ref{eqn:q-i-v-times-u-v-factored-into-product-pairs}),
we have for each pair $u, v$ of distinct elements of $V(G)$,
\[
p k_{u v} u_V = \sum_{i, j \in V(H)} \beta_{i j} q_i^u q_j^v u_V = \sum_{i, j \in V(H)} \beta_{i, j} \sum_{\substack{\phi \colon \phi(u) = i \\
\quad \phi(v) = j}} q_\phi = \sum_{\phi \in V(H)^V} \beta_{\phi(u), \phi(v)} q_\phi.
\]
Here the 
???MANY LINES MISSING
However, $p \in \calP_S$ so it follows that $S = \emptyset$.
Therefore by the previous isomorphism $\calP_\emptyset = \{ p \}$
so $p$ is the only basic idempotent in $\hat \calG(\emptyset)$ and so in the entire $\hat \calG$.)  
\end{proof}


